Leveraging Probabilistic Circuits for Nonparametric Multi-Output Regression

Inspired by recent advances in the field of expert-based approximations of Gaussian processes (GPs), we present an expert-based approach to large-scale multi-output regression using single-output GP experts. Employing a deeply structured mixture of single-output GPs encoded via a probabilistic circuit allows us to capture correlations between multiple output dimensions accurately. By recursively partitioning the covariate space and the output space, posterior inference in our model reduces to inference on single-output GP experts, which only need to be conditioned on a small subset of the observations. We show that inference can be performed exactly and efficiently in our model, that it can capture correlations between output dimensions and, hence, often outperforms approaches that do not incorporate inter-output correlations, as demonstrated on several data sets in terms of the negative log predictive density.

==> pgflibrarypgfplots.colorbrewer.code.tex <==
\usetikzlibrary{colorbrewer}
\pgfplotscreateplotcyclelist{YlGn-3}{%
  YlGn-3-1\\%
  YlGn-3-2\\%
  YlGn-3-3\\%
}
\pgfplotscreateplotcyclelist{YlGn-4}{%
  YlGn-4-1\\%
  YlGn-4-2\\%
  YlGn-4-3\\%
  YlGn-4-4\\%
}
\pgfplotscreateplotcyclelist{YlGn-5}{%
  YlGn-5-1\\%
  YlGn-5-2\\%
  YlGn-5-3\\%
  YlGn-5-4\\%
  YlGn-5-5\\%
}
\pgfplotscreateplotcyclelist{YlGn-6}{%
  YlGn-6-1\\%
  YlGn-6-2\\%
  YlGn-6-3\\%
  YlGn-6-4\\%
  YlGn-6-5\\%
  YlGn-6-6\\%
}
\pgfplotscreateplotcyclelist{YlGn-7}{%
  YlGn-7-1\\%
  YlGn-7-2\\%
  YlGn-7-3\\%
  YlGn-7-4\\%
  YlGn-7-5\\%
  YlGn-7-6\\%
  YlGn-7-7\\%
}
\pgfplotscreateplotcyclelist{YlGn-8}{%
  YlGn-8-1\\%
  YlGn-8-2\\%
  YlGn-8-3\\%
  YlGn-8-4\\%
  YlGn-8-5\\%
  YlGn-8-6\\%
  YlGn-8-7\\%
  YlGn-8-8\\%
}
\pgfplotscreateplotcyclelist{YlGn-9}{%
  YlGn-9-1\\%
  YlGn-9-2\\%
  YlGn-9-3\\%
  YlGn-9-4\\%
  YlGn-9-5\\%
  YlGn-9-6\\%
  YlGn-9-7\\%
  YlGn-9-8\\%
  YlGn-9-9\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-3}{%
  YlGnBu-3-1\\%
  YlGnBu-3-2\\%
  YlGnBu-3-3\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-4}{%
  YlGnBu-4-1\\%
  YlGnBu-4-2\\%
  YlGnBu-4-3\\%
  YlGnBu-4-4\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-5}{%
  YlGnBu-5-1\\%
  YlGnBu-5-2\\%
  YlGnBu-5-3\\%
  YlGnBu-5-4\\%
  YlGnBu-5-5\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-6}{%
  YlGnBu-6-1\\%
  YlGnBu-6-2\\%
  YlGnBu-6-3\\%
  YlGnBu-6-4\\%
  YlGnBu-6-5\\%
  YlGnBu-6-6\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-7}{%
  YlGnBu-7-1\\%
  YlGnBu-7-2\\%
  YlGnBu-7-3\\%
  YlGnBu-7-4\\%
  YlGnBu-7-5\\%
  YlGnBu-7-6\\%
  YlGnBu-7-7\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-8}{%
  YlGnBu-8-1\\%
  YlGnBu-8-2\\%
  YlGnBu-8-3\\%
  YlGnBu-8-4\\%
  YlGnBu-8-5\\%
  YlGnBu-8-6\\%
  YlGnBu-8-7\\%
  YlGnBu-8-8\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-9}{%
  YlGnBu-9-1\\%
  YlGnBu-9-2\\%
  YlGnBu-9-3\\%
  YlGnBu-9-4\\%
  YlGnBu-9-5\\%
  YlGnBu-9-6\\%
  YlGnBu-9-7\\%
  YlGnBu-9-8\\%
  YlGnBu-9-9\\%
}
\pgfplotscreateplotcyclelist{GnBu-3}{%
  GnBu-3-1\\%
  GnBu-3-2\\%
  GnBu-3-3\\%
}
\pgfplotscreateplotcyclelist{GnBu-4}{%
  GnBu-4-1\\%
  GnBu-4-2\\%
  GnBu-4-3\\%
  GnBu-4-4\\%
}
\pgfplotscreateplotcyclelist{GnBu-5}{%
  GnBu-5-1\\%
  GnBu-5-2\\%
  GnBu-5-3\\%
  GnBu-5-4\\%
  GnBu-5-5\\%
}
\pgfplotscreateplotcyclelist{GnBu-6}{%
  GnBu-6-1\\%
  GnBu-6-2\\%
  GnBu-6-3\\%
  GnBu-6-4\\%
  GnBu-6-5\\%
  GnBu-6-6\\%
}
\pgfplotscreateplotcyclelist{GnBu-7}{%
  GnBu-7-1\\%
  GnBu-7-2\\%
  GnBu-7-3\\%
  GnBu-7-4\\%
  GnBu-7-5\\%
  GnBu-7-6\\%
  GnBu-7-7\\%
}
\pgfplotscreateplotcyclelist{GnBu-8}{%
  GnBu-8-1\\%
  GnBu-8-2\\%
  GnBu-8-3\\%
  GnBu-8-4\\%
  GnBu-8-5\\%
  GnBu-8-6\\%
  GnBu-8-7\\%
  GnBu-8-8\\%
}
\pgfplotscreateplotcyclelist{GnBu-9}{%
  GnBu-9-1\\%
  GnBu-9-2\\%
  GnBu-9-3\\%
  GnBu-9-4\\%
  GnBu-9-5\\%
  GnBu-9-6\\%
  GnBu-9-7\\%
  GnBu-9-8\\%
  GnBu-9-9\\%
}
\pgfplotscreateplotcyclelist{BuGn-3}{%
  BuGn-3-1\\%
  BuGn-3-2\\%
  BuGn-3-3\\%
}
\pgfplotscreateplotcyclelist{BuGn-4}{%
  BuGn-4-1\\%
  BuGn-4-2\\%
  BuGn-4-3\\%
  BuGn-4-4\\%
}
\pgfplotscreateplotcyclelist{BuGn-5}{%
  BuGn-5-1\\%
  BuGn-5-2\\%
  BuGn-5-3\\%
  BuGn-5-4\\%
  BuGn-5-5\\%
}
\pgfplotscreateplotcyclelist{BuGn-6}{%
  BuGn-6-1\\%
  BuGn-6-2\\%
  BuGn-6-3\\%
  BuGn-6-4\\%
  BuGn-6-5\\%
  BuGn-6-6\\%
}
\pgfplotscreateplotcyclelist{BuGn-7}{%
  BuGn-7-1\\%
  BuGn-7-2\\%
  BuGn-7-3\\%
  BuGn-7-4\\%
  BuGn-7-5\\%
  BuGn-7-6\\%
  BuGn-7-7\\%
}
\pgfplotscreateplotcyclelist{BuGn-8}{%
  BuGn-8-1\\%
  BuGn-8-2\\%
  BuGn-8-3\\%
  BuGn-8-4\\%
  BuGn-8-5\\%
  BuGn-8-6\\%
  BuGn-8-7\\%
  BuGn-8-8\\%
}
\pgfplotscreateplotcyclelist{BuGn-9}{%
  BuGn-9-1\\%
  BuGn-9-2\\%
  BuGn-9-3\\%
  BuGn-9-4\\%
  BuGn-9-5\\%
  BuGn-9-6\\%
  BuGn-9-7\\%
  BuGn-9-8\\%
  BuGn-9-9\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-3}{%
  PuBuGn-3-1\\%
  PuBuGn-3-2\\%
  PuBuGn-3-3\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-4}{%
  PuBuGn-4-1\\%
  PuBuGn-4-2\\%
  PuBuGn-4-3\\%
  PuBuGn-4-4\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-5}{%
  PuBuGn-5-1\\%
  PuBuGn-5-2\\%
  PuBuGn-5-3\\%
  PuBuGn-5-4\\%
  PuBuGn-5-5\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-6}{%
  PuBuGn-6-1\\%
  PuBuGn-6-2\\%
  PuBuGn-6-3\\%
  PuBuGn-6-4\\%
  PuBuGn-6-5\\%
  PuBuGn-6-6\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-7}{%
  PuBuGn-7-1\\%
  PuBuGn-7-2\\%
  PuBuGn-7-3\\%
  PuBuGn-7-4\\%
  PuBuGn-7-5\\%
  PuBuGn-7-6\\%
  PuBuGn-7-7\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-8}{%
  PuBuGn-8-1\\%
  PuBuGn-8-2\\%
  PuBuGn-8-3\\%
  PuBuGn-8-4\\%
  PuBuGn-8-5\\%
  PuBuGn-8-6\\%
  PuBuGn-8-7\\%
  PuBuGn-8-8\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-9}{%
  PuBuGn-9-1\\%
  PuBuGn-9-2\\%
  PuBuGn-9-3\\%
  PuBuGn-9-4\\%
  PuBuGn-9-5\\%
  PuBuGn-9-6\\%
  PuBuGn-9-7\\%
  PuBuGn-9-8\\%
  PuBuGn-9-9\\%
}
\pgfplotscreateplotcyclelist{PuBu-3}{%
  PuBu-3-1\\%
  PuBu-3-2\\%
  PuBu-3-3\\%
}
\pgfplotscreateplotcyclelist{PuBu-4}{%
  PuBu-4-1\\%
  PuBu-4-2\\%
  PuBu-4-3\\%
  PuBu-4-4\\%
}
\pgfplotscreateplotcyclelist{PuBu-5}{%
  PuBu-5-1\\%
  PuBu-5-2\\%
  PuBu-5-3\\%
  PuBu-5-4\\%
  PuBu-5-5\\%
}
\pgfplotscreateplotcyclelist{PuBu-6}{%
  PuBu-6-1\\%
  PuBu-6-2\\%
  PuBu-6-3\\%
  PuBu-6-4\\%
  PuBu-6-5\\%
  PuBu-6-6\\%
}
\pgfplotscreateplotcyclelist{PuBu-7}{%
  PuBu-7-1\\%
  PuBu-7-2\\%
  PuBu-7-3\\%
  PuBu-7-4\\%
  PuBu-7-5\\%
  PuBu-7-6\\%
  PuBu-7-7\\%
}
\pgfplotscreateplotcyclelist{PuBu-8}{%
  PuBu-8-1\\%
  PuBu-8-2\\%
  PuBu-8-3\\%
  PuBu-8-4\\%
  PuBu-8-5\\%
  PuBu-8-6\\%
  PuBu-8-7\\%
  PuBu-8-8\\%
}
\pgfplotscreateplotcyclelist{PuBu-9}{%
  PuBu-9-1\\%
  PuBu-9-2\\%
  PuBu-9-3\\%
  PuBu-9-4\\%
  PuBu-9-5\\%
  PuBu-9-6\\%
  PuBu-9-7\\%
  PuBu-9-8\\%
  PuBu-9-9\\%
}
\pgfplotscreateplotcyclelist{BuPu-3}{%
  BuPu-3-1\\%
  BuPu-3-2\\%
  BuPu-3-3\\%
}
\pgfplotscreateplotcyclelist{BuPu-4}{%
  BuPu-4-1\\%
  BuPu-4-2\\%
  BuPu-4-3\\%
  BuPu-4-4\\%
}
\pgfplotscreateplotcyclelist{BuPu-5}{%
  BuPu-5-1\\%
  BuPu-5-2\\%
  BuPu-5-3\\%
  BuPu-5-4\\%
  BuPu-5-5\\%
}
\pgfplotscreateplotcyclelist{BuPu-6}{%
  BuPu-6-1\\%
  BuPu-6-2\\%
  BuPu-6-3\\%
  BuPu-6-4\\%
  BuPu-6-5\\%
  BuPu-6-6\\%
}
\pgfplotscreateplotcyclelist{BuPu-7}{%
  BuPu-7-1\\%
  BuPu-7-2\\%
  BuPu-7-3\\%
  BuPu-7-4\\%
  BuPu-7-5\\%
  BuPu-7-6\\%
  BuPu-7-7\\%
}
\pgfplotscreateplotcyclelist{BuPu-8}{%
  BuPu-8-1\\%
  BuPu-8-2\\%
  BuPu-8-3\\%
  BuPu-8-4\\%
  BuPu-8-5\\%
  BuPu-8-6\\%
  BuPu-8-7\\%
  BuPu-8-8\\%
}
\pgfplotscreateplotcyclelist{BuPu-9}{%
  BuPu-9-1\\%
  BuPu-9-2\\%
  BuPu-9-3\\%
  BuPu-9-4\\%
  BuPu-9-5\\%
  BuPu-9-6\\%
  BuPu-9-7\\%
  BuPu-9-8\\%
  BuPu-9-9\\%
}
\pgfplotscreateplotcyclelist{RdPu-3}{%
  RdPu-3-1\\%
  RdPu-3-2\\%
  RdPu-3-3\\%
}
\pgfplotscreateplotcyclelist{RdPu-4}{%
  RdPu-4-1\\%
  RdPu-4-2\\%
  RdPu-4-3\\%
  RdPu-4-4\\%
}
\pgfplotscreateplotcyclelist{RdPu-5}{%
  RdPu-5-1\\%
  RdPu-5-2\\%
  RdPu-5-3\\%
  RdPu-5-4\\%
  RdPu-5-5\\%
}
\pgfplotscreateplotcyclelist{RdPu-6}{%
  RdPu-6-1\\%
  RdPu-6-2\\%
  RdPu-6-3\\%
  RdPu-6-4\\%
  RdPu-6-5\\%
  RdPu-6-6\\%
}
\pgfplotscreateplotcyclelist{RdPu-7}{%
  RdPu-7-1\\%
  RdPu-7-2\\%
  RdPu-7-3\\%
  RdPu-7-4\\%
  RdPu-7-5\\%
  RdPu-7-6\\%
  RdPu-7-7\\%
}
\pgfplotscreateplotcyclelist{RdPu-8}{%
  RdPu-8-1\\%
  RdPu-8-2\\%
  RdPu-8-3\\%
  RdPu-8-4\\%
  RdPu-8-5\\%
  RdPu-8-6\\%
  RdPu-8-7\\%
  RdPu-8-8\\%
}
\pgfplotscreateplotcyclelist{RdPu-9}{%
  RdPu-9-1\\%
  RdPu-9-2\\%
  RdPu-9-3\\%
  RdPu-9-4\\%
  RdPu-9-5\\%
  RdPu-9-6\\%
  RdPu-9-7\\%
  RdPu-9-8\\%
  RdPu-9-9\\%
}
\pgfplotscreateplotcyclelist{PuRd-3}{%
  PuRd-3-1\\%
  PuRd-3-2\\%
  PuRd-3-3\\%
}
\pgfplotscreateplotcyclelist{PuRd-4}{%
  PuRd-4-1\\%
  PuRd-4-2\\%
  PuRd-4-3\\%
  PuRd-4-4\\%
}
\pgfplotscreateplotcyclelist{PuRd-5}{%
  PuRd-5-1\\%
  PuRd-5-2\\%
  PuRd-5-3\\%
  PuRd-5-4\\%
  PuRd-5-5\\%
}
\pgfplotscreateplotcyclelist{PuRd-6}{%
  PuRd-6-1\\%
  PuRd-6-2\\%
  PuRd-6-3\\%
  PuRd-6-4\\%
  PuRd-6-5\\%
  PuRd-6-6\\%
}
\pgfplotscreateplotcyclelist{PuRd-7}{%
  PuRd-7-1\\%
  PuRd-7-2\\%
  PuRd-7-3\\%
  PuRd-7-4\\%
  PuRd-7-5\\%
  PuRd-7-6\\%
  PuRd-7-7\\%
}
\pgfplotscreateplotcyclelist{PuRd-8}{%
  PuRd-8-1\\%
  PuRd-8-2\\%
  PuRd-8-3\\%
  PuRd-8-4\\%
  PuRd-8-5\\%
  PuRd-8-6\\%
  PuRd-8-7\\%
  PuRd-8-8\\%
}
\pgfplotscreateplotcyclelist{PuRd-9}{%
  PuRd-9-1\\%
  PuRd-9-2\\%
  PuRd-9-3\\%
  PuRd-9-4\\%
  PuRd-9-5\\%
  PuRd-9-6\\%
  PuRd-9-7\\%
  PuRd-9-8\\%
  PuRd-9-9\\%
}
\pgfplotscreateplotcyclelist{OrRd-3}{%
  OrRd-3-1\\%
  OrRd-3-2\\%
  OrRd-3-3\\%
}
\pgfplotscreateplotcyclelist{OrRd-4}{%
  OrRd-4-1\\%
  OrRd-4-2\\%
  OrRd-4-3\\%
  OrRd-4-4\\%
}
\pgfplotscreateplotcyclelist{OrRd-5}{%
  OrRd-5-1\\%
  OrRd-5-2\\%
  OrRd-5-3\\%
  OrRd-5-4\\%
  OrRd-5-5\\%
}
\pgfplotscreateplotcyclelist{OrRd-6}{%
  OrRd-6-1\\%
  OrRd-6-2\\%
  OrRd-6-3\\%
  OrRd-6-4\\%
  OrRd-6-5\\%
  OrRd-6-6\\%
}
\pgfplotscreateplotcyclelist{OrRd-7}{%
  OrRd-7-1\\%
  OrRd-7-2\\%
  OrRd-7-3\\%
  OrRd-7-4\\%
  OrRd-7-5\\%
  OrRd-7-6\\%
  OrRd-7-7\\%
}
\pgfplotscreateplotcyclelist{OrRd-8}{%
  OrRd-8-1\\%
  OrRd-8-2\\%
  OrRd-8-3\\%
  OrRd-8-4\\%
  OrRd-8-5\\%
  OrRd-8-6\\%
  OrRd-8-7\\%
  OrRd-8-8\\%
}
\pgfplotscreateplotcyclelist{OrRd-9}{%
  OrRd-9-1\\%
  OrRd-9-2\\%
  OrRd-9-3\\%
  OrRd-9-4\\%
  OrRd-9-5\\%
  OrRd-9-6\\%
  OrRd-9-7\\%
  OrRd-9-8\\%
  OrRd-9-9\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-3}{%
  YlOrRd-3-1\\%
  YlOrRd-3-2\\%
  YlOrRd-3-3\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-4}{%
  YlOrRd-4-1\\%
  YlOrRd-4-2\\%
  YlOrRd-4-3\\%
  YlOrRd-4-4\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-5}{%
  YlOrRd-5-1\\%
  YlOrRd-5-2\\%
  YlOrRd-5-3\\%
  YlOrRd-5-4\\%
  YlOrRd-5-5\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-6}{%
  YlOrRd-6-1\\%
  YlOrRd-6-2\\%
  YlOrRd-6-3\\%
  YlOrRd-6-4\\%
  YlOrRd-6-5\\%
  YlOrRd-6-6\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-7}{%
  YlOrRd-7-1\\%
  YlOrRd-7-2\\%
  YlOrRd-7-3\\%
  YlOrRd-7-4\\%
  YlOrRd-7-5\\%
  YlOrRd-7-6\\%
  YlOrRd-7-7\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-8}{%
  YlOrRd-8-1\\%
  YlOrRd-8-2\\%
  YlOrRd-8-3\\%
  YlOrRd-8-4\\%
  YlOrRd-8-5\\%
  YlOrRd-8-6\\%
  YlOrRd-8-7\\%
  YlOrRd-8-8\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-9}{%
  YlOrRd-9-1\\%
  YlOrRd-9-2\\%
  YlOrRd-9-3\\%
  YlOrRd-9-4\\%
  YlOrRd-9-5\\%
  YlOrRd-9-6\\%
  YlOrRd-9-7\\%
  YlOrRd-9-8\\%
  YlOrRd-9-9\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-3}{%
  YlOrBr-3-1\\%
  YlOrBr-3-2\\%
  YlOrBr-3-3\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-4}{%
  YlOrBr-4-1\\%
  YlOrBr-4-2\\%
  YlOrBr-4-3\\%
  YlOrBr-4-4\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-5}{%
  YlOrBr-5-1\\%
  YlOrBr-5-2\\%
  YlOrBr-5-3\\%
  YlOrBr-5-4\\%
  YlOrBr-5-5\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-6}{%
  YlOrBr-6-1\\%
  YlOrBr-6-2\\%
  YlOrBr-6-3\\%
  YlOrBr-6-4\\%
  YlOrBr-6-5\\%
  YlOrBr-6-6\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-7}{%
  YlOrBr-7-1\\%
  YlOrBr-7-2\\%
  YlOrBr-7-3\\%
  YlOrBr-7-4\\%
  YlOrBr-7-5\\%
  YlOrBr-7-6\\%
  YlOrBr-7-7\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-8}{%
  YlOrBr-8-1\\%
  YlOrBr-8-2\\%
  YlOrBr-8-3\\%
  YlOrBr-8-4\\%
  YlOrBr-8-5\\%
  YlOrBr-8-6\\%
  YlOrBr-8-7\\%
  YlOrBr-8-8\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-9}{%
  YlOrBr-9-1\\%
  YlOrBr-9-2\\%
  YlOrBr-9-3\\%
  YlOrBr-9-4\\%
  YlOrBr-9-5\\%
  YlOrBr-9-6\\%
  YlOrBr-9-7\\%
  YlOrBr-9-8\\%
  YlOrBr-9-9\\%
}
\pgfplotscreateplotcyclelist{Purples-3}{%
  Purples-3-1\\%
  Purples-3-2\\%
  Purples-3-3\\%
}
\pgfplotscreateplotcyclelist{Purples-4}{%
  Purples-4-1\\%
  Purples-4-2\\%
  Purples-4-3\\%
  Purples-4-4\\%
}
\pgfplotscreateplotcyclelist{Purples-5}{%
  Purples-5-1\\%
  Purples-5-2\\%
  Purples-5-3\\%
  Purples-5-4\\%
  Purples-5-5\\%
}
\pgfplotscreateplotcyclelist{Purples-6}{%
  Purples-6-1\\%
  Purples-6-2\\%
  Purples-6-3\\%
  Purples-6-4\\%
  Purples-6-5\\%
  Purples-6-6\\%
}
\pgfplotscreateplotcyclelist{Purples-7}{%
  Purples-7-1\\%
  Purples-7-2\\%
  Purples-7-3\\%
  Purples-7-4\\%
  Purples-7-5\\%
  Purples-7-6\\%
  Purples-7-7\\%
}
\pgfplotscreateplotcyclelist{Purples-8}{%
  Purples-8-1\\%
  Purples-8-2\\%
  Purples-8-3\\%
  Purples-8-4\\%
  Purples-8-5\\%
  Purples-8-6\\%
  Purples-8-7\\%
  Purples-8-8\\%
}
\pgfplotscreateplotcyclelist{Purples-9}{%
  Purples-9-1\\%
  Purples-9-2\\%
  Purples-9-3\\%
  Purples-9-4\\%
  Purples-9-5\\%
  Purples-9-6\\%
  Purples-9-7\\%
  Purples-9-8\\%
  Purples-9-9\\%
}
\pgfplotscreateplotcyclelist{Blues-3}{%
  Blues-3-1\\%
  Blues-3-2\\%
  Blues-3-3\\%
}
\pgfplotscreateplotcyclelist{Blues-4}{%
  Blues-4-1\\%
  Blues-4-2\\%
  Blues-4-3\\%
  Blues-4-4\\%
}
\pgfplotscreateplotcyclelist{Blues-5}{%
  Blues-5-1\\%
  Blues-5-2\\%
  Blues-5-3\\%
  Blues-5-4\\%
  Blues-5-5\\%
}
\pgfplotscreateplotcyclelist{Blues-6}{%
  Blues-6-1\\%
  Blues-6-2\\%
  Blues-6-3\\%
  Blues-6-4\\%
  Blues-6-5\\%
  Blues-6-6\\%
}
\pgfplotscreateplotcyclelist{Blues-7}{%
  Blues-7-1\\%
  Blues-7-2\\%
  Blues-7-3\\%
  Blues-7-4\\%
  Blues-7-5\\%
  Blues-7-6\\%
  Blues-7-7\\%
}
\pgfplotscreateplotcyclelist{Blues-8}{%
  Blues-8-1\\%
  Blues-8-2\\%
  Blues-8-3\\%
  Blues-8-4\\%
  Blues-8-5\\%
  Blues-8-6\\%
  Blues-8-7\\%
  Blues-8-8\\%
}
\pgfplotscreateplotcyclelist{Blues-9}{%
  Blues-9-1\\%
  Blues-9-2\\%
  Blues-9-3\\%
  Blues-9-4\\%
  Blues-9-5\\%
  Blues-9-6\\%
  Blues-9-7\\%
  Blues-9-8\\%
  Blues-9-9\\%
}
\pgfplotscreateplotcyclelist{Greens-3}{%
  Greens-3-1\\%
  Greens-3-2\\%
  Greens-3-3\\%
}
\pgfplotscreateplotcyclelist{Greens-4}{%
  Greens-4-1\\%
  Greens-4-2\\%
  Greens-4-3\\%
  Greens-4-4\\%
}
\pgfplotscreateplotcyclelist{Greens-5}{%
  Greens-5-1\\%
  Greens-5-2\\%
  Greens-5-3\\%
  Greens-5-4\\%
  Greens-5-5\\%
}
\pgfplotscreateplotcyclelist{Greens-6}{%
  Greens-6-1\\%
  Greens-6-2\\%
  Greens-6-3\\%
  Greens-6-4\\%
  Greens-6-5\\%
  Greens-6-6\\%
}
\pgfplotscreateplotcyclelist{Greens-7}{%
  Greens-7-1\\%
  Greens-7-2\\%
  Greens-7-3\\%
  Greens-7-4\\%
  Greens-7-5\\%
  Greens-7-6\\%
  Greens-7-7\\%
}
\pgfplotscreateplotcyclelist{Greens-8}{%
  Greens-8-1\\%
  Greens-8-2\\%
  Greens-8-3\\%
  Greens-8-4\\%
  Greens-8-5\\%
  Greens-8-6\\%
  Greens-8-7\\%
  Greens-8-8\\%
}
\pgfplotscreateplotcyclelist{Greens-9}{%
  Greens-9-1\\%
  Greens-9-2\\%
  Greens-9-3\\%
  Greens-9-4\\%
  Greens-9-5\\%
  Greens-9-6\\%
  Greens-9-7\\%
  Greens-9-8\\%
  Greens-9-9\\%
}
\pgfplotscreateplotcyclelist{Oranges-3}{%
  Oranges-3-1\\%
  Oranges-3-2\\%
  Oranges-3-3\\%
}
\pgfplotscreateplotcyclelist{Oranges-4}{%
  Oranges-4-1\\%
  Oranges-4-2\\%
  Oranges-4-3\\%
  Oranges-4-4\\%
}
\pgfplotscreateplotcyclelist{Oranges-5}{%
  Oranges-5-1\\%
  Oranges-5-2\\%
  Oranges-5-3\\%
  Oranges-5-4\\%
  Oranges-5-5\\%
}
\pgfplotscreateplotcyclelist{Oranges-6}{%
  Oranges-6-1\\%
  Oranges-6-2\\%
  Oranges-6-3\\%
  Oranges-6-4\\%
  Oranges-6-5\\%
  Oranges-6-6\\%
}
\pgfplotscreateplotcyclelist{Oranges-7}{%
  Oranges-7-1\\%
  Oranges-7-2\\%
  Oranges-7-3\\%
  Oranges-7-4\\%
  Oranges-7-5\\%
  Oranges-7-6\\%
  Oranges-7-7\\%
}
\pgfplotscreateplotcyclelist{Oranges-8}{%
  Oranges-8-1\\%
  Oranges-8-2\\%
  Oranges-8-3\\%
  Oranges-8-4\\%
  Oranges-8-5\\%
  Oranges-8-6\\%
  Oranges-8-7\\%
  Oranges-8-8\\%
}
\pgfplotscreateplotcyclelist{Oranges-9}{%
  Oranges-9-1\\%
  Oranges-9-2\\%
  Oranges-9-3\\%
  Oranges-9-4\\%
  Oranges-9-5\\%
  Oranges-9-6\\%
  Oranges-9-7\\%
  Oranges-9-8\\%
  Oranges-9-9\\%
}
\pgfplotscreateplotcyclelist{Reds-3}{%
  Reds-3-1\\%
  Reds-3-2\\%
  Reds-3-3\\%
}
\pgfplotscreateplotcyclelist{Reds-4}{%
  Reds-4-1\\%
  Reds-4-2\\%
  Reds-4-3\\%
  Reds-4-4\\%
}
\pgfplotscreateplotcyclelist{Reds-5}{%
  Reds-5-1\\%
  Reds-5-2\\%
  Reds-5-3\\%
  Reds-5-4\\%
  Reds-5-5\\%
}
\pgfplotscreateplotcyclelist{Reds-6}{%
  Reds-6-1\\%
  Reds-6-2\\%
  Reds-6-3\\%
  Reds-6-4\\%
  Reds-6-5\\%
  Reds-6-6\\%
}
\pgfplotscreateplotcyclelist{Reds-7}{%
  Reds-7-1\\%
  Reds-7-2\\%
  Reds-7-3\\%
  Reds-7-4\\%
  Reds-7-5\\%
  Reds-7-6\\%
  Reds-7-7\\%
}
\pgfplotscreateplotcyclelist{Reds-8}{%
  Reds-8-1\\%
  Reds-8-2\\%
  Reds-8-3\\%
  Reds-8-4\\%
  Reds-8-5\\%
  Reds-8-6\\%
  Reds-8-7\\%
  Reds-8-8\\%
}
\pgfplotscreateplotcyclelist{Reds-9}{%
  Reds-9-1\\%
  Reds-9-2\\%
  Reds-9-3\\%
  Reds-9-4\\%
  Reds-9-5\\%
  Reds-9-6\\%
  Reds-9-7\\%
  Reds-9-8\\%
  Reds-9-9\\%
}
\pgfplotscreateplotcyclelist{Greys-3}{%
  Greys-3-1\\%
  Greys-3-2\\%
  Greys-3-3\\%
}
\pgfplotscreateplotcyclelist{Greys-4}{%
  Greys-4-1\\%
  Greys-4-2\\%
  Greys-4-3\\%
  Greys-4-4\\%
}
\pgfplotscreateplotcyclelist{Greys-5}{%
  Greys-5-1\\%
  Greys-5-2\\%
  Greys-5-3\\%
  Greys-5-4\\%
  Greys-5-5\\%
}
\pgfplotscreateplotcyclelist{Greys-6}{%
  Greys-6-1\\%
  Greys-6-2\\%
  Greys-6-3\\%
  Greys-6-4\\%
  Greys-6-5\\%
  Greys-6-6\\%
}
\pgfplotscreateplotcyclelist{Greys-7}{%
  Greys-7-1\\%
  Greys-7-2\\%
  Greys-7-3\\%
  Greys-7-4\\%
  Greys-7-5\\%
  Greys-7-6\\%
  Greys-7-7\\%
}
\pgfplotscreateplotcyclelist{Greys-8}{%
  Greys-8-1\\%
  Greys-8-2\\%
  Greys-8-3\\%
  Greys-8-4\\%
  Greys-8-5\\%
  Greys-8-6\\%
  Greys-8-7\\%
  Greys-8-8\\%
}
\pgfplotscreateplotcyclelist{Greys-9}{%
  Greys-9-1\\%
  Greys-9-2\\%
  Greys-9-3\\%
  Greys-9-4\\%
  Greys-9-5\\%
  Greys-9-6\\%
  Greys-9-7\\%
  Greys-9-8\\%
  Greys-9-9\\%
}
\pgfplotscreateplotcyclelist{PuOr-3}{%
  PuOr-3-1\\%
  PuOr-3-2\\%
  PuOr-3-3\\%
}
\pgfplotscreateplotcyclelist{PuOr-4}{%
  PuOr-4-1\\%
  PuOr-4-2\\%
  PuOr-4-3\\%
  PuOr-4-4\\%
}
\pgfplotscreateplotcyclelist{PuOr-5}{%
  PuOr-5-1\\%
  PuOr-5-2\\%
  PuOr-5-3\\%
  PuOr-5-4\\%
  PuOr-5-5\\%
}
\pgfplotscreateplotcyclelist{PuOr-6}{%
  PuOr-6-1\\%
  PuOr-6-2\\%
  PuOr-6-3\\%
  PuOr-6-4\\%
  PuOr-6-5\\%
  PuOr-6-6\\%
}
\pgfplotscreateplotcyclelist{PuOr-7}{%
  PuOr-7-1\\%
  PuOr-7-2\\%
  PuOr-7-3\\%
  PuOr-7-4\\%
  PuOr-7-5\\%
  PuOr-7-6\\%
  PuOr-7-7\\%
}
\pgfplotscreateplotcyclelist{PuOr-8}{%
  PuOr-8-1\\%
  PuOr-8-2\\%
  PuOr-8-3\\%
  PuOr-8-4\\%
  PuOr-8-5\\%
  PuOr-8-6\\%
  PuOr-8-7\\%
  PuOr-8-8\\%
}
\pgfplotscreateplotcyclelist{PuOr-9}{%
  PuOr-9-1\\%
  PuOr-9-2\\%
  PuOr-9-3\\%
  PuOr-9-4\\%
  PuOr-9-5\\%
  PuOr-9-6\\%
  PuOr-9-7\\%
  PuOr-9-8\\%
  PuOr-9-9\\%
}
\pgfplotscreateplotcyclelist{PuOr-10}{%
  PuOr-10-1\\%
  PuOr-10-2\\%
  PuOr-10-3\\%
  PuOr-10-4\\%
  PuOr-10-5\\%
  PuOr-10-6\\%
  PuOr-10-7\\%
  PuOr-10-8\\%
  PuOr-10-9\\%
  PuOr-10-10\\%
}
\pgfplotscreateplotcyclelist{PuOr-11}{%
  PuOr-11-1\\%
  PuOr-11-2\\%
  PuOr-11-3\\%
  PuOr-11-4\\%
  PuOr-11-5\\%
  PuOr-11-6\\%
  PuOr-11-7\\%
  PuOr-11-8\\%
  PuOr-11-9\\%
  PuOr-11-10\\%
  PuOr-11-11\\%
}
\pgfplotscreateplotcyclelist{BrBG-3}{%
  BrBG-3-1\\%
  BrBG-3-2\\%
  BrBG-3-3\\%
}
\pgfplotscreateplotcyclelist{BrBG-4}{%
  BrBG-4-1\\%
  BrBG-4-2\\%
  BrBG-4-3\\%
  BrBG-4-4\\%
}
\pgfplotscreateplotcyclelist{BrBG-5}{%
  BrBG-5-1\\%
  BrBG-5-2\\%
  BrBG-5-3\\%
  BrBG-5-4\\%
  BrBG-5-5\\%
}
\pgfplotscreateplotcyclelist{BrBG-6}{%
  BrBG-6-1\\%
  BrBG-6-2\\%
  BrBG-6-3\\%
  BrBG-6-4\\%
  BrBG-6-5\\%
  BrBG-6-6\\%
}
\pgfplotscreateplotcyclelist{BrBG-7}{%
  BrBG-7-1\\%
  BrBG-7-2\\%
  BrBG-7-3\\%
  BrBG-7-4\\%
  BrBG-7-5\\%
  BrBG-7-6\\%
  BrBG-7-7\\%
}
\pgfplotscreateplotcyclelist{BrBG-8}{%
  BrBG-8-1\\%
  BrBG-8-2\\%
  BrBG-8-3\\%
  BrBG-8-4\\%
  BrBG-8-5\\%
  BrBG-8-6\\%
  BrBG-8-7\\%
  BrBG-8-8\\%
}
\pgfplotscreateplotcyclelist{BrBG-9}{%
  BrBG-9-1\\%
  BrBG-9-2\\%
  BrBG-9-3\\%
  BrBG-9-4\\%
  BrBG-9-5\\%
  BrBG-9-6\\%
  BrBG-9-7\\%
  BrBG-9-8\\%
  BrBG-9-9\\%
}
\pgfplotscreateplotcyclelist{BrBG-10}{%
  BrBG-10-1\\%
  BrBG-10-2\\%
  BrBG-10-3\\%
  BrBG-10-4\\%
  BrBG-10-5\\%
  BrBG-10-6\\%
  BrBG-10-7\\%
  BrBG-10-8\\%
  BrBG-10-9\\%
  BrBG-10-10\\%
}
\pgfplotscreateplotcyclelist{BrBG-11}{%
  BrBG-11-1\\%
  BrBG-11-2\\%
  BrBG-11-3\\%
  BrBG-11-4\\%
  BrBG-11-5\\%
  BrBG-11-6\\%
  BrBG-11-7\\%
  BrBG-11-8\\%
  BrBG-11-9\\%
  BrBG-11-10\\%
  BrBG-11-11\\%
}
\pgfplotscreateplotcyclelist{PRGn-3}{%
  PRGn-3-1\\%
  PRGn-3-2\\%
  PRGn-3-3\\%
}
\pgfplotscreateplotcyclelist{PRGn-4}{%
  PRGn-4-1\\%
  PRGn-4-2\\%
  PRGn-4-3\\%
  PRGn-4-4\\%
}
\pgfplotscreateplotcyclelist{PRGn-5}{%
  PRGn-5-1\\%
  PRGn-5-2\\%
  PRGn-5-3\\%
  PRGn-5-4\\%
  PRGn-5-5\\%
}
\pgfplotscreateplotcyclelist{PRGn-6}{%
  PRGn-6-1\\%
  PRGn-6-2\\%
  PRGn-6-3\\%
  PRGn-6-4\\%
  PRGn-6-5\\%
  PRGn-6-6\\%
}
\pgfplotscreateplotcyclelist{PRGn-7}{%
  PRGn-7-1\\%
  PRGn-7-2\\%
  PRGn-7-3\\%
  PRGn-7-4\\%
  PRGn-7-5\\%
  PRGn-7-6\\%
  PRGn-7-7\\%
}
\pgfplotscreateplotcyclelist{PRGn-8}{%
  PRGn-8-1\\%
  PRGn-8-2\\%
  PRGn-8-3\\%
  PRGn-8-4\\%
  PRGn-8-5\\%
  PRGn-8-6\\%
  PRGn-8-7\\%
  PRGn-8-8\\%
}
\pgfplotscreateplotcyclelist{PRGn-9}{%
  PRGn-9-1\\%
  PRGn-9-2\\%
  PRGn-9-3\\%
  PRGn-9-4\\%
  PRGn-9-5\\%
  PRGn-9-6\\%
  PRGn-9-7\\%
  PRGn-9-8\\%
  PRGn-9-9\\%
}
\pgfplotscreateplotcyclelist{PRGn-10}{%
  PRGn-10-1\\%
  PRGn-10-2\\%
  PRGn-10-3\\%
  PRGn-10-4\\%
  PRGn-10-5\\%
  PRGn-10-6\\%
  PRGn-10-7\\%
  PRGn-10-8\\%
  PRGn-10-9\\%
  PRGn-10-10\\%
}
\pgfplotscreateplotcyclelist{PRGn-11}{%
  PRGn-11-1\\%
  PRGn-11-2\\%
  PRGn-11-3\\%
  PRGn-11-4\\%
  PRGn-11-5\\%
  PRGn-11-6\\%
  PRGn-11-7\\%
  PRGn-11-8\\%
  PRGn-11-9\\%
  PRGn-11-10\\%
  PRGn-11-11\\%
}
\pgfplotscreateplotcyclelist{PiYG-3}{%
  PiYG-3-1\\%
  PiYG-3-2\\%
  PiYG-3-3\\%
}
\pgfplotscreateplotcyclelist{PiYG-4}{%
  PiYG-4-1\\%
  PiYG-4-2\\%
  PiYG-4-3\\%
  PiYG-4-4\\%
}
\pgfplotscreateplotcyclelist{PiYG-5}{%
  PiYG-5-1\\%
  PiYG-5-2\\%
  PiYG-5-3\\%
  PiYG-5-4\\%
  PiYG-5-5\\%
}
\pgfplotscreateplotcyclelist{PiYG-6}{%
  PiYG-6-1\\%
  PiYG-6-2\\%
  PiYG-6-3\\%
  PiYG-6-4\\%
  PiYG-6-5\\%
  PiYG-6-6\\%
}
\pgfplotscreateplotcyclelist{PiYG-7}{%
  PiYG-7-1\\%
  PiYG-7-2\\%
  PiYG-7-3\\%
  PiYG-7-4\\%
  PiYG-7-5\\%
  PiYG-7-6\\%
  PiYG-7-7\\%
}
\pgfplotscreateplotcyclelist{PiYG-8}{%
  PiYG-8-1\\%
  PiYG-8-2\\%
  PiYG-8-3\\%
  PiYG-8-4\\%
  PiYG-8-5\\%
  PiYG-8-6\\%
  PiYG-8-7\\%
  PiYG-8-8\\%
}
\pgfplotscreateplotcyclelist{PiYG-9}{%
  PiYG-9-1\\%
  PiYG-9-2\\%
  PiYG-9-3\\%
  PiYG-9-4\\%
  PiYG-9-5\\%
  PiYG-9-6\\%
  PiYG-9-7\\%
  PiYG-9-8\\%
  PiYG-9-9\\%
}
\pgfplotscreateplotcyclelist{PiYG-10}{%
  PiYG-10-1\\%
  PiYG-10-2\\%
  PiYG-10-3\\%
  PiYG-10-4\\%
  PiYG-10-5\\%
  PiYG-10-6\\%
  PiYG-10-7\\%
  PiYG-10-8\\%
  PiYG-10-9\\%
  PiYG-10-10\\%
}
\pgfplotscreateplotcyclelist{PiYG-11}{%
  PiYG-11-1\\%
  PiYG-11-2\\%
  PiYG-11-3\\%
  PiYG-11-4\\%
  PiYG-11-5\\%
  PiYG-11-6\\%
  PiYG-11-7\\%
  PiYG-11-8\\%
  PiYG-11-9\\%
  PiYG-11-10\\%
  PiYG-11-11\\%
}
\pgfplotscreateplotcyclelist{RdBu-3}{%
  RdBu-3-1\\%
  RdBu-3-2\\%
  RdBu-3-3\\%
}
\pgfplotscreateplotcyclelist{RdBu-4}{%
  RdBu-4-1\\%
  RdBu-4-2\\%
  RdBu-4-3\\%
  RdBu-4-4\\%
}
\pgfplotscreateplotcyclelist{RdBu-5}{%
  RdBu-5-1\\%
  RdBu-5-2\\%
  RdBu-5-3\\%
  RdBu-5-4\\%
  RdBu-5-5\\%
}
\pgfplotscreateplotcyclelist{RdBu-6}{%
  RdBu-6-1\\%
  RdBu-6-2\\%
  RdBu-6-3\\%
  RdBu-6-4\\%
  RdBu-6-5\\%
  RdBu-6-6\\%
}
\pgfplotscreateplotcyclelist{RdBu-7}{%
  RdBu-7-1\\%
  RdBu-7-2\\%
  RdBu-7-3\\%
  RdBu-7-4\\%
  RdBu-7-5\\%
  RdBu-7-6\\%
  RdBu-7-7\\%
}
\pgfplotscreateplotcyclelist{RdBu-8}{%
  RdBu-8-1\\%
  RdBu-8-2\\%
  RdBu-8-3\\%
  RdBu-8-4\\%
  RdBu-8-5\\%
  RdBu-8-6\\%
  RdBu-8-7\\%
  RdBu-8-8\\%
}
\pgfplotscreateplotcyclelist{RdBu-9}{%
  RdBu-9-1\\%
  RdBu-9-2\\%
  RdBu-9-3\\%
  RdBu-9-4\\%
  RdBu-9-5\\%
  RdBu-9-6\\%
  RdBu-9-7\\%
  RdBu-9-8\\%
  RdBu-9-9\\%
}
\pgfplotscreateplotcyclelist{RdBu-10}{%
  RdBu-10-1\\%
  RdBu-10-2\\%
  RdBu-10-3\\%
  RdBu-10-4\\%
  RdBu-10-5\\%
  RdBu-10-6\\%
  RdBu-10-7\\%
  RdBu-10-8\\%
  RdBu-10-9\\%
  RdBu-10-10\\%
}
\pgfplotscreateplotcyclelist{RdBu-11}{%
  RdBu-11-1\\%
  RdBu-11-2\\%
  RdBu-11-3\\%
  RdBu-11-4\\%
  RdBu-11-5\\%
  RdBu-11-6\\%
  RdBu-11-7\\%
  RdBu-11-8\\%
  RdBu-11-9\\%
  RdBu-11-10\\%
  RdBu-11-11\\%
}
\pgfplotscreateplotcyclelist{RdGy-3}{%
  RdGy-3-1\\%
  RdGy-3-2\\%
  RdGy-3-3\\%
}
\pgfplotscreateplotcyclelist{RdGy-4}{%
  RdGy-4-1\\%
  RdGy-4-2\\%
  RdGy-4-3\\%
  RdGy-4-4\\%
}
\pgfplotscreateplotcyclelist{RdGy-5}{%
  RdGy-5-1\\%
  RdGy-5-2\\%
  RdGy-5-3\\%
  RdGy-5-4\\%
  RdGy-5-5\\%
}
\pgfplotscreateplotcyclelist{RdGy-6}{%
  RdGy-6-1\\%
  RdGy-6-2\\%
  RdGy-6-3\\%
  RdGy-6-4\\%
  RdGy-6-5\\%
  RdGy-6-6\\%
}
\pgfplotscreateplotcyclelist{RdGy-7}{%
  RdGy-7-1\\%
  RdGy-7-2\\%
  RdGy-7-3\\%
  RdGy-7-4\\%
  RdGy-7-5\\%
  RdGy-7-6\\%
  RdGy-7-7\\%
}
\pgfplotscreateplotcyclelist{RdGy-8}{%
  RdGy-8-1\\%
  RdGy-8-2\\%
  RdGy-8-3\\%
  RdGy-8-4\\%
  RdGy-8-5\\%
  RdGy-8-6\\%
  RdGy-8-7\\%
  RdGy-8-8\\%
}
\pgfplotscreateplotcyclelist{RdGy-9}{%
  RdGy-9-1\\%
  RdGy-9-2\\%
  RdGy-9-3\\%
  RdGy-9-4\\%
  RdGy-9-5\\%
  RdGy-9-6\\%
  RdGy-9-7\\%
  RdGy-9-8\\%
  RdGy-9-9\\%
}
\pgfplotscreateplotcyclelist{RdGy-10}{%
  RdGy-10-1\\%
  RdGy-10-2\\%
  RdGy-10-3\\%
  RdGy-10-4\\%
  RdGy-10-5\\%
  RdGy-10-6\\%
  RdGy-10-7\\%
  RdGy-10-8\\%
  RdGy-10-9\\%
  RdGy-10-10\\%
}
\pgfplotscreateplotcyclelist{RdGy-11}{%
  RdGy-11-1\\%
  RdGy-11-2\\%
  RdGy-11-3\\%
  RdGy-11-4\\%
  RdGy-11-5\\%
  RdGy-11-6\\%
  RdGy-11-7\\%
  RdGy-11-8\\%
  RdGy-11-9\\%
  RdGy-11-10\\%
  RdGy-11-11\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-3}{%
  RdYlBu-3-1\\%
  RdYlBu-3-2\\%
  RdYlBu-3-3\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-4}{%
  RdYlBu-4-1\\%
  RdYlBu-4-2\\%
  RdYlBu-4-3\\%
  RdYlBu-4-4\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-5}{%
  RdYlBu-5-1\\%
  RdYlBu-5-2\\%
  RdYlBu-5-3\\%
  RdYlBu-5-4\\%
  RdYlBu-5-5\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-6}{%
  RdYlBu-6-1\\%
  RdYlBu-6-2\\%
  RdYlBu-6-3\\%
  RdYlBu-6-4\\%
  RdYlBu-6-5\\%
  RdYlBu-6-6\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-7}{%
  RdYlBu-7-1\\%
  RdYlBu-7-2\\%
  RdYlBu-7-3\\%
  RdYlBu-7-4\\%
  RdYlBu-7-5\\%
  RdYlBu-7-6\\%
  RdYlBu-7-7\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-8}{%
  RdYlBu-8-1\\%
  RdYlBu-8-2\\%
  RdYlBu-8-3\\%
  RdYlBu-8-4\\%
  RdYlBu-8-5\\%
  RdYlBu-8-6\\%
  RdYlBu-8-7\\%
  RdYlBu-8-8\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-9}{%
  RdYlBu-9-1\\%
  RdYlBu-9-2\\%
  RdYlBu-9-3\\%
  RdYlBu-9-4\\%
  RdYlBu-9-5\\%
  RdYlBu-9-6\\%
  RdYlBu-9-7\\%
  RdYlBu-9-8\\%
  RdYlBu-9-9\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-10}{%
  RdYlBu-10-1\\%
  RdYlBu-10-2\\%
  RdYlBu-10-3\\%
  RdYlBu-10-4\\%
  RdYlBu-10-5\\%
  RdYlBu-10-6\\%
  RdYlBu-10-7\\%
  RdYlBu-10-8\\%
  RdYlBu-10-9\\%
  RdYlBu-10-10\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-11}{%
  RdYlBu-11-1\\%
  RdYlBu-11-2\\%
  RdYlBu-11-3\\%
  RdYlBu-11-4\\%
  RdYlBu-11-5\\%
  RdYlBu-11-6\\%
  RdYlBu-11-7\\%
  RdYlBu-11-8\\%
  RdYlBu-11-9\\%
  RdYlBu-11-10\\%
  RdYlBu-11-11\\%
}
\pgfplotscreateplotcyclelist{Spectral-3}{%
  Spectral-3-1\\%
  Spectral-3-2\\%
  Spectral-3-3\\%
}
\pgfplotscreateplotcyclelist{Spectral-4}{%
  Spectral-4-1\\%
  Spectral-4-2\\%
  Spectral-4-3\\%
  Spectral-4-4\\%
}
\pgfplotscreateplotcyclelist{Spectral-5}{%
  Spectral-5-1\\%
  Spectral-5-2\\%
  Spectral-5-3\\%
  Spectral-5-4\\%
  Spectral-5-5\\%
}
\pgfplotscreateplotcyclelist{Spectral-6}{%
  Spectral-6-1\\%
  Spectral-6-2\\%
  Spectral-6-3\\%
  Spectral-6-4\\%
  Spectral-6-5\\%
  Spectral-6-6\\%
}
\pgfplotscreateplotcyclelist{Spectral-7}{%
  Spectral-7-1\\%
  Spectral-7-2\\%
  Spectral-7-3\\%
  Spectral-7-4\\%
  Spectral-7-5\\%
  Spectral-7-6\\%
  Spectral-7-7\\%
}
\pgfplotscreateplotcyclelist{Spectral-8}{%
  Spectral-8-1\\%
  Spectral-8-2\\%
  Spectral-8-3\\%
  Spectral-8-4\\%
  Spectral-8-5\\%
  Spectral-8-6\\%
  Spectral-8-7\\%
  Spectral-8-8\\%
}
\pgfplotscreateplotcyclelist{Spectral-9}{%
  Spectral-9-1\\%
  Spectral-9-2\\%
  Spectral-9-3\\%
  Spectral-9-4\\%
  Spectral-9-5\\%
  Spectral-9-6\\%
  Spectral-9-7\\%
  Spectral-9-8\\%
  Spectral-9-9\\%
}
\pgfplotscreateplotcyclelist{Spectral-10}{%
  Spectral-10-1\\%
  Spectral-10-2\\%
  Spectral-10-3\\%
  Spectral-10-4\\%
  Spectral-10-5\\%
  Spectral-10-6\\%
  Spectral-10-7\\%
  Spectral-10-8\\%
  Spectral-10-9\\%
  Spectral-10-10\\%
}
\pgfplotscreateplotcyclelist{Spectral-11}{%
  Spectral-11-1\\%
  Spectral-11-2\\%
  Spectral-11-3\\%
  Spectral-11-4\\%
  Spectral-11-5\\%
  Spectral-11-6\\%
  Spectral-11-7\\%
  Spectral-11-8\\%
  Spectral-11-9\\%
  Spectral-11-10\\%
  Spectral-11-11\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-3}{%
  RdYlGn-3-1\\%
  RdYlGn-3-2\\%
  RdYlGn-3-3\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-4}{%
  RdYlGn-4-1\\%
  RdYlGn-4-2\\%
  RdYlGn-4-3\\%
  RdYlGn-4-4\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-5}{%
  RdYlGn-5-1\\%
  RdYlGn-5-2\\%
  RdYlGn-5-3\\%
  RdYlGn-5-4\\%
  RdYlGn-5-5\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-6}{%
  RdYlGn-6-1\\%
  RdYlGn-6-2\\%
  RdYlGn-6-3\\%
  RdYlGn-6-4\\%
  RdYlGn-6-5\\%
  RdYlGn-6-6\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-7}{%
  RdYlGn-7-1\\%
  RdYlGn-7-2\\%
  RdYlGn-7-3\\%
  RdYlGn-7-4\\%
  RdYlGn-7-5\\%
  RdYlGn-7-6\\%
  RdYlGn-7-7\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-8}{%
  RdYlGn-8-1\\%
  RdYlGn-8-2\\%
  RdYlGn-8-3\\%
  RdYlGn-8-4\\%
  RdYlGn-8-5\\%
  RdYlGn-8-6\\%
  RdYlGn-8-7\\%
  RdYlGn-8-8\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-9}{%
  RdYlGn-9-1\\%
  RdYlGn-9-2\\%
  RdYlGn-9-3\\%
  RdYlGn-9-4\\%
  RdYlGn-9-5\\%
  RdYlGn-9-6\\%
  RdYlGn-9-7\\%
  RdYlGn-9-8\\%
  RdYlGn-9-9\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-10}{%
  RdYlGn-10-1\\%
  RdYlGn-10-2\\%
  RdYlGn-10-3\\%
  RdYlGn-10-4\\%
  RdYlGn-10-5\\%
  RdYlGn-10-6\\%
  RdYlGn-10-7\\%
  RdYlGn-10-8\\%
  RdYlGn-10-9\\%
  RdYlGn-10-10\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-11}{%
  RdYlGn-11-1\\%
  RdYlGn-11-2\\%
  RdYlGn-11-3\\%
  RdYlGn-11-4\\%
  RdYlGn-11-5\\%
  RdYlGn-11-6\\%
  RdYlGn-11-7\\%
  RdYlGn-11-8\\%
  RdYlGn-11-9\\%
  RdYlGn-11-10\\%
  RdYlGn-11-11\\%
}
\pgfplotscreateplotcyclelist{Set3-3}{%
  Set3-3-1\\%
  Set3-3-2\\%
  Set3-3-3\\%
}
\pgfplotscreateplotcyclelist{Set3-4}{%
  Set3-4-1\\%
  Set3-4-2\\%
  Set3-4-3\\%
  Set3-4-4\\%
}
\pgfplotscreateplotcyclelist{Set3-5}{%
  Set3-5-1\\%
  Set3-5-2\\%
  Set3-5-3\\%
  Set3-5-4\\%
  Set3-5-5\\%
}
\pgfplotscreateplotcyclelist{Set3-6}{%
  Set3-6-1\\%
  Set3-6-2\\%
  Set3-6-3\\%
  Set3-6-4\\%
  Set3-6-5\\%
  Set3-6-6\\%
}
\pgfplotscreateplotcyclelist{Set3-7}{%
  Set3-7-1\\%
  Set3-7-2\\%
  Set3-7-3\\%
  Set3-7-4\\%
  Set3-7-5\\%
  Set3-7-6\\%
  Set3-7-7\\%
}
\pgfplotscreateplotcyclelist{Set3-8}{%
  Set3-8-1\\%
  Set3-8-2\\%
  Set3-8-3\\%
  Set3-8-4\\%
  Set3-8-5\\%
  Set3-8-6\\%
  Set3-8-7\\%
  Set3-8-8\\%
}
\pgfplotscreateplotcyclelist{Set3-9}{%
  Set3-9-1\\%
  Set3-9-2\\%
  Set3-9-3\\%
  Set3-9-4\\%
  Set3-9-5\\%
  Set3-9-6\\%
  Set3-9-7\\%
  Set3-9-8\\%
  Set3-9-9\\%
}
\pgfplotscreateplotcyclelist{Set3-10}{%
  Set3-10-1\\%
  Set3-10-2\\%
  Set3-10-3\\%
  Set3-10-4\\%
  Set3-10-5\\%
  Set3-10-6\\%
  Set3-10-7\\%
  Set3-10-8\\%
  Set3-10-9\\%
  Set3-10-10\\%
}
\pgfplotscreateplotcyclelist{Set3-11}{%
  Set3-11-1\\%
  Set3-11-2\\%
  Set3-11-3\\%
  Set3-11-4\\%
  Set3-11-5\\%
  Set3-11-6\\%
  Set3-11-7\\%
  Set3-11-8\\%
  Set3-11-9\\%
  Set3-11-10\\%
  Set3-11-11\\%
}
\pgfplotscreateplotcyclelist{Set3-12}{%
  Set3-12-1\\%
  Set3-12-2\\%
  Set3-12-3\\%
  Set3-12-4\\%
  Set3-12-5\\%
  Set3-12-6\\%
  Set3-12-7\\%
  Set3-12-8\\%
  Set3-12-9\\%
  Set3-12-10\\%
  Set3-12-11\\%
  Set3-12-12\\%
}
\pgfplotscreateplotcyclelist{Pastel1-3}{%
  Pastel1-3-1\\%
  Pastel1-3-2\\%
  Pastel1-3-3\\%
}
\pgfplotscreateplotcyclelist{Pastel1-4}{%
  Pastel1-4-1\\%
  Pastel1-4-2\\%
  Pastel1-4-3\\%
  Pastel1-4-4\\%
}
\pgfplotscreateplotcyclelist{Pastel1-5}{%
  Pastel1-5-1\\%
  Pastel1-5-2\\%
  Pastel1-5-3\\%
  Pastel1-5-4\\%
  Pastel1-5-5\\%
}
\pgfplotscreateplotcyclelist{Pastel1-6}{%
  Pastel1-6-1\\%
  Pastel1-6-2\\%
  Pastel1-6-3\\%
  Pastel1-6-4\\%
  Pastel1-6-5\\%
  Pastel1-6-6\\%
}
\pgfplotscreateplotcyclelist{Pastel1-7}{%
  Pastel1-7-1\\%
  Pastel1-7-2\\%
  Pastel1-7-3\\%
  Pastel1-7-4\\%
  Pastel1-7-5\\%
  Pastel1-7-6\\%
  Pastel1-7-7\\%
}
\pgfplotscreateplotcyclelist{Pastel1-8}{%
  Pastel1-8-1\\%
  Pastel1-8-2\\%
  Pastel1-8-3\\%
  Pastel1-8-4\\%
  Pastel1-8-5\\%
  Pastel1-8-6\\%
  Pastel1-8-7\\%
  Pastel1-8-8\\%
}
\pgfplotscreateplotcyclelist{Pastel1-9}{%
  Pastel1-9-1\\%
  Pastel1-9-2\\%
  Pastel1-9-3\\%
  Pastel1-9-4\\%
  Pastel1-9-5\\%
  Pastel1-9-6\\%
  Pastel1-9-7\\%
  Pastel1-9-8\\%
  Pastel1-9-9\\%
}
\pgfplotscreateplotcyclelist{Set1-3}{%
  Set1-3-1\\%
  Set1-3-2\\%
  Set1-3-3\\%
}
\pgfplotscreateplotcyclelist{Set1-4}{%
  Set1-4-1\\%
  Set1-4-2\\%
  Set1-4-3\\%
  Set1-4-4\\%
}
\pgfplotscreateplotcyclelist{Set1-5}{%
  Set1-5-1\\%
  Set1-5-2\\%
  Set1-5-3\\%
  Set1-5-4\\%
  Set1-5-5\\%
}
\pgfplotscreateplotcyclelist{Set1-6}{%
  Set1-6-1\\%
  Set1-6-2\\%
  Set1-6-3\\%
  Set1-6-4\\%
  Set1-6-5\\%
  Set1-6-6\\%
}
\pgfplotscreateplotcyclelist{Set1-7}{%
  Set1-7-1\\%
  Set1-7-2\\%
  Set1-7-3\\%
  Set1-7-4\\%
  Set1-7-5\\%
  Set1-7-6\\%
  Set1-7-7\\%
}
\pgfplotscreateplotcyclelist{Set1-8}{%
  Set1-8-1\\%
  Set1-8-2\\%
  Set1-8-3\\%
  Set1-8-4\\%
  Set1-8-5\\%
  Set1-8-6\\%
  Set1-8-7\\%
  Set1-8-8\\%
}
\pgfplotscreateplotcyclelist{Set1-9}{%
  Set1-9-1\\%
  Set1-9-2\\%
  Set1-9-3\\%
  Set1-9-4\\%
  Set1-9-5\\%
  Set1-9-6\\%
  Set1-9-7\\%
  Set1-9-8\\%
  Set1-9-9\\%
}
\pgfplotscreateplotcyclelist{Pastel2-3}{%
  Pastel2-3-1\\%
  Pastel2-3-2\\%
  Pastel2-3-3\\%
}
\pgfplotscreateplotcyclelist{Pastel2-4}{%
  Pastel2-4-1\\%
  Pastel2-4-2\\%
  Pastel2-4-3\\%
  Pastel2-4-4\\%
}
\pgfplotscreateplotcyclelist{Pastel2-5}{%
  Pastel2-5-1\\%
  Pastel2-5-2\\%
  Pastel2-5-3\\%
  Pastel2-5-4\\%
  Pastel2-5-5\\%
}
\pgfplotscreateplotcyclelist{Pastel2-6}{%
  Pastel2-6-1\\%
  Pastel2-6-2\\%
  Pastel2-6-3\\%
  Pastel2-6-4\\%
  Pastel2-6-5\\%
  Pastel2-6-6\\%
}
\pgfplotscreateplotcyclelist{Pastel2-7}{%
  Pastel2-7-1\\%
  Pastel2-7-2\\%
  Pastel2-7-3\\%
  Pastel2-7-4\\%
  Pastel2-7-5\\%
  Pastel2-7-6\\%
  Pastel2-7-7\\%
}
\pgfplotscreateplotcyclelist{Pastel2-8}{%
  Pastel2-8-1\\%
  Pastel2-8-2\\%
  Pastel2-8-3\\%
  Pastel2-8-4\\%
  Pastel2-8-5\\%
  Pastel2-8-6\\%
  Pastel2-8-7\\%
  Pastel2-8-8\\%
}
\pgfplotscreateplotcyclelist{Set2-3}{%
  Set2-3-1\\%
  Set2-3-2\\%
  Set2-3-3\\%
}
\pgfplotscreateplotcyclelist{Set2-4}{%
  Set2-4-1\\%
  Set2-4-2\\%
  Set2-4-3\\%
  Set2-4-4\\%
}
\pgfplotscreateplotcyclelist{Set2-5}{%
  Set2-5-1\\%
  Set2-5-2\\%
  Set2-5-3\\%
  Set2-5-4\\%
  Set2-5-5\\%
}
\pgfplotscreateplotcyclelist{Set2-6}{%
  Set2-6-1\\%
  Set2-6-2\\%
  Set2-6-3\\%
  Set2-6-4\\%
  Set2-6-5\\%
  Set2-6-6\\%
}
\pgfplotscreateplotcyclelist{Set2-7}{%
  Set2-7-1\\%
  Set2-7-2\\%
  Set2-7-3\\%
  Set2-7-4\\%
  Set2-7-5\\%
  Set2-7-6\\%
  Set2-7-7\\%
}
\pgfplotscreateplotcyclelist{Set2-8}{%
  Set2-8-1\\%
  Set2-8-2\\%
  Set2-8-3\\%
  Set2-8-4\\%
  Set2-8-5\\%
  Set2-8-6\\%
  Set2-8-7\\%
  Set2-8-8\\%
}
\pgfplotscreateplotcyclelist{Dark2-3}{%
  Dark2-3-1\\%
  Dark2-3-2\\%
  Dark2-3-3\\%
}
\pgfplotscreateplotcyclelist{Dark2-4}{%
  Dark2-4-1\\%
  Dark2-4-2\\%
  Dark2-4-3\\%
  Dark2-4-4\\%
}
\pgfplotscreateplotcyclelist{Dark2-5}{%
  Dark2-5-1\\%
  Dark2-5-2\\%
  Dark2-5-3\\%
  Dark2-5-4\\%
  Dark2-5-5\\%
}
\pgfplotscreateplotcyclelist{Dark2-6}{%
  Dark2-6-1\\%
  Dark2-6-2\\%
  Dark2-6-3\\%
  Dark2-6-4\\%
  Dark2-6-5\\%
  Dark2-6-6\\%
}
\pgfplotscreateplotcyclelist{Dark2-7}{%
  Dark2-7-1\\%
  Dark2-7-2\\%
  Dark2-7-3\\%
  Dark2-7-4\\%
  Dark2-7-5\\%
  Dark2-7-6\\%
  Dark2-7-7\\%
}
\pgfplotscreateplotcyclelist{Dark2-8}{%
  Dark2-8-1\\%
  Dark2-8-2\\%
  Dark2-8-3\\%
  Dark2-8-4\\%
  Dark2-8-5\\%
  Dark2-8-6\\%
  Dark2-8-7\\%
  Dark2-8-8\\%
}
\pgfplotscreateplotcyclelist{Paired-3}{%
  Paired-3-1\\%
  Paired-3-2\\%
  Paired-3-3\\%
}
\pgfplotscreateplotcyclelist{Paired-4}{%
  Paired-4-1\\%
  Paired-4-2\\%
  Paired-4-3\\%
  Paired-4-4\\%
}
\pgfplotscreateplotcyclelist{Paired-5}{%
  Paired-5-1\\%
  Paired-5-2\\%
  Paired-5-3\\%
  Paired-5-4\\%
  Paired-5-5\\%
}
\pgfplotscreateplotcyclelist{Paired-6}{%
  Paired-6-1\\%
  Paired-6-2\\%
  Paired-6-3\\%
  Paired-6-4\\%
  Paired-6-5\\%
  Paired-6-6\\%
}
\pgfplotscreateplotcyclelist{Paired-7}{%
  Paired-7-1\\%
  Paired-7-2\\%
  Paired-7-3\\%
  Paired-7-4\\%
  Paired-7-5\\%
  Paired-7-6\\%
  Paired-7-7\\%
}
\pgfplotscreateplotcyclelist{Paired-8}{%
  Paired-8-1\\%
  Paired-8-2\\%
  Paired-8-3\\%
  Paired-8-4\\%
  Paired-8-5\\%
  Paired-8-6\\%
  Paired-8-7\\%
  Paired-8-8\\%
}
\pgfplotscreateplotcyclelist{Paired-9}{%
  Paired-9-1\\%
  Paired-9-2\\%
  Paired-9-3\\%
  Paired-9-4\\%
  Paired-9-5\\%
  Paired-9-6\\%
  Paired-9-7\\%
  Paired-9-8\\%
  Paired-9-9\\%
}
\pgfplotscreateplotcyclelist{Paired-10}{%
  Paired-10-1\\%
  Paired-10-2\\%
  Paired-10-3\\%
  Paired-10-4\\%
  Paired-10-5\\%
  Paired-10-6\\%
  Paired-10-7\\%
  Paired-10-8\\%
  Paired-10-9\\%
  Paired-10-10\\%
}
\pgfplotscreateplotcyclelist{Paired-11}{%
  Paired-11-1\\%
  Paired-11-2\\%
  Paired-11-3\\%
  Paired-11-4\\%
  Paired-11-5\\%
  Paired-11-6\\%
  Paired-11-7\\%
  Paired-11-8\\%
  Paired-11-9\\%
  Paired-11-10\\%
  Paired-11-11\\%
}
\pgfplotscreateplotcyclelist{Paired-12}{%
  Paired-12-1\\%
  Paired-12-2\\%
  Paired-12-3\\%
  Paired-12-4\\%
  Paired-12-5\\%
  Paired-12-6\\%
  Paired-12-7\\%
  Paired-12-8\\%
  Paired-12-9\\%
  Paired-12-10\\%
  Paired-12-11\\%
  Paired-12-12\\%
}
\pgfplotscreateplotcyclelist{Accent-3}{%
  Accent-3-1\\%
  Accent-3-2\\%
  Accent-3-3\\%
}
\pgfplotscreateplotcyclelist{Accent-4}{%
  Accent-4-1\\%
  Accent-4-2\\%
  Accent-4-3\\%
  Accent-4-4\\%
}
\pgfplotscreateplotcyclelist{Accent-5}{%
  Accent-5-1\\%
  Accent-5-2\\%
  Accent-5-3\\%
  Accent-5-4\\%
  Accent-5-5\\%
}
\pgfplotscreateplotcyclelist{Accent-6}{%
  Accent-6-1\\%
  Accent-6-2\\%
  Accent-6-3\\%
  Accent-6-4\\%
  Accent-6-5\\%
  Accent-6-6\\%
}
\pgfplotscreateplotcyclelist{Accent-7}{%
  Accent-7-1\\%
  Accent-7-2\\%
  Accent-7-3\\%
  Accent-7-4\\%
  Accent-7-5\\%
  Accent-7-6\\%
  Accent-7-7\\%
}
\pgfplotscreateplotcyclelist{Accent-8}{%
  Accent-8-1\\%
  Accent-8-2\\%
  Accent-8-3\\%
  Accent-8-4\\%
  Accent-8-5\\%
  Accent-8-6\\%
  Accent-8-7\\%
  Accent-8-8\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-3}{%
 YlGn-3-1!70!black, every mark/.append style={solid,fill=YlGn-3-1},mark=*\\%
 YlGn-3-2!70!black, every mark/.append style={solid,fill=YlGn-3-2},mark=square*\\%
 YlGn-3-3!70!black, every mark/.append style={solid,fill=YlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-4}{%
 YlGn-4-1!70!black, every mark/.append style={solid,fill=YlGn-4-1},mark=*\\%
 YlGn-4-2!70!black, every mark/.append style={solid,fill=YlGn-4-2},mark=square*\\%
 YlGn-4-3!70!black, every mark/.append style={solid,fill=YlGn-4-3},mark=triangle*\\%
 YlGn-4-4!70!black, every mark/.append style={solid,fill=YlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-5}{%
 YlGn-5-1!70!black, every mark/.append style={solid,fill=YlGn-5-1},mark=*\\%
 YlGn-5-2!70!black, every mark/.append style={solid,fill=YlGn-5-2},mark=square*\\%
 YlGn-5-3!70!black, every mark/.append style={solid,fill=YlGn-5-3},mark=triangle*\\%
 YlGn-5-4!70!black, every mark/.append style={solid,fill=YlGn-5-4},mark=diamond*\\%
 YlGn-5-5!70!black, every mark/.append style={solid,fill=YlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-6}{%
 YlGn-6-1!70!black, every mark/.append style={solid,fill=YlGn-6-1},mark=*\\%
 YlGn-6-2!70!black, every mark/.append style={solid,fill=YlGn-6-2},mark=square*\\%
 YlGn-6-3!70!black, every mark/.append style={solid,fill=YlGn-6-3},mark=triangle*\\%
 YlGn-6-4!70!black, every mark/.append style={solid,fill=YlGn-6-4},mark=diamond*\\%
 YlGn-6-5!70!black, every mark/.append style={solid,fill=YlGn-6-5},mark=pentagon*\\%
 YlGn-6-6!70!black, every mark/.append style={solid,fill=YlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-7}{%
 YlGn-7-1!70!black, every mark/.append style={solid,fill=YlGn-7-1},mark=*\\%
 YlGn-7-2!70!black, every mark/.append style={solid,fill=YlGn-7-2},mark=square*\\%
 YlGn-7-3!70!black, every mark/.append style={solid,fill=YlGn-7-3},mark=triangle*\\%
 YlGn-7-4!70!black, every mark/.append style={solid,fill=YlGn-7-4},mark=diamond*\\%
 YlGn-7-5!70!black, every mark/.append style={solid,fill=YlGn-7-5},mark=pentagon*\\%
 YlGn-7-6!70!black, every mark/.append style={solid,fill=YlGn-7-6},mark=x\\%
 YlGn-7-7!70!black, every mark/.append style={solid,fill=YlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-8}{%
 YlGn-8-1!70!black, every mark/.append style={solid,fill=YlGn-8-1},mark=*\\%
 YlGn-8-2!70!black, every mark/.append style={solid,fill=YlGn-8-2},mark=square*\\%
 YlGn-8-3!70!black, every mark/.append style={solid,fill=YlGn-8-3},mark=triangle*\\%
 YlGn-8-4!70!black, every mark/.append style={solid,fill=YlGn-8-4},mark=diamond*\\%
 YlGn-8-5!70!black, every mark/.append style={solid,fill=YlGn-8-5},mark=pentagon*\\%
 YlGn-8-6!70!black, every mark/.append style={solid,fill=YlGn-8-6},mark=x\\%
 YlGn-8-7!70!black, every mark/.append style={solid,fill=YlGn-8-7},mark=+\\%
 YlGn-8-8!70!black, every mark/.append style={solid,fill=YlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-9}{%
 YlGn-9-1!70!black, every mark/.append style={solid,fill=YlGn-9-1},mark=*\\%
 YlGn-9-2!70!black, every mark/.append style={solid,fill=YlGn-9-2},mark=square*\\%
 YlGn-9-3!70!black, every mark/.append style={solid,fill=YlGn-9-3},mark=triangle*\\%
 YlGn-9-4!70!black, every mark/.append style={solid,fill=YlGn-9-4},mark=diamond*\\%
 YlGn-9-5!70!black, every mark/.append style={solid,fill=YlGn-9-5},mark=pentagon*\\%
 YlGn-9-6!70!black, every mark/.append style={solid,fill=YlGn-9-6},mark=x\\%
 YlGn-9-7!70!black, every mark/.append style={solid,fill=YlGn-9-7},mark=+\\%
 YlGn-9-8!70!black, every mark/.append style={solid,fill=YlGn-9-8},mark=star\\%
 YlGn-9-9!70!black, every mark/.append style={solid,fill=YlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-3}{%
 YlGnBu-3-1!70!black, every mark/.append style={solid,fill=YlGnBu-3-1},mark=*\\%
 YlGnBu-3-2!70!black, every mark/.append style={solid,fill=YlGnBu-3-2},mark=square*\\%
 YlGnBu-3-3!70!black, every mark/.append style={solid,fill=YlGnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-4}{%
 YlGnBu-4-1!70!black, every mark/.append style={solid,fill=YlGnBu-4-1},mark=*\\%
 YlGnBu-4-2!70!black, every mark/.append style={solid,fill=YlGnBu-4-2},mark=square*\\%
 YlGnBu-4-3!70!black, every mark/.append style={solid,fill=YlGnBu-4-3},mark=triangle*\\%
 YlGnBu-4-4!70!black, every mark/.append style={solid,fill=YlGnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-5}{%
 YlGnBu-5-1!70!black, every mark/.append style={solid,fill=YlGnBu-5-1},mark=*\\%
 YlGnBu-5-2!70!black, every mark/.append style={solid,fill=YlGnBu-5-2},mark=square*\\%
 YlGnBu-5-3!70!black, every mark/.append style={solid,fill=YlGnBu-5-3},mark=triangle*\\%
 YlGnBu-5-4!70!black, every mark/.append style={solid,fill=YlGnBu-5-4},mark=diamond*\\%
 YlGnBu-5-5!70!black, every mark/.append style={solid,fill=YlGnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-6}{%
 YlGnBu-6-1!70!black, every mark/.append style={solid,fill=YlGnBu-6-1},mark=*\\%
 YlGnBu-6-2!70!black, every mark/.append style={solid,fill=YlGnBu-6-2},mark=square*\\%
 YlGnBu-6-3!70!black, every mark/.append style={solid,fill=YlGnBu-6-3},mark=triangle*\\%
 YlGnBu-6-4!70!black, every mark/.append style={solid,fill=YlGnBu-6-4},mark=diamond*\\%
 YlGnBu-6-5!70!black, every mark/.append style={solid,fill=YlGnBu-6-5},mark=pentagon*\\%
 YlGnBu-6-6!70!black, every mark/.append style={solid,fill=YlGnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-7}{%
 YlGnBu-7-1!70!black, every mark/.append style={solid,fill=YlGnBu-7-1},mark=*\\%
 YlGnBu-7-2!70!black, every mark/.append style={solid,fill=YlGnBu-7-2},mark=square*\\%
 YlGnBu-7-3!70!black, every mark/.append style={solid,fill=YlGnBu-7-3},mark=triangle*\\%
 YlGnBu-7-4!70!black, every mark/.append style={solid,fill=YlGnBu-7-4},mark=diamond*\\%
 YlGnBu-7-5!70!black, every mark/.append style={solid,fill=YlGnBu-7-5},mark=pentagon*\\%
 YlGnBu-7-6!70!black, every mark/.append style={solid,fill=YlGnBu-7-6},mark=x\\%
 YlGnBu-7-7!70!black, every mark/.append style={solid,fill=YlGnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-8}{%
 YlGnBu-8-1!70!black, every mark/.append style={solid,fill=YlGnBu-8-1},mark=*\\%
 YlGnBu-8-2!70!black, every mark/.append style={solid,fill=YlGnBu-8-2},mark=square*\\%
 YlGnBu-8-3!70!black, every mark/.append style={solid,fill=YlGnBu-8-3},mark=triangle*\\%
 YlGnBu-8-4!70!black, every mark/.append style={solid,fill=YlGnBu-8-4},mark=diamond*\\%
 YlGnBu-8-5!70!black, every mark/.append style={solid,fill=YlGnBu-8-5},mark=pentagon*\\%
 YlGnBu-8-6!70!black, every mark/.append style={solid,fill=YlGnBu-8-6},mark=x\\%
 YlGnBu-8-7!70!black, every mark/.append style={solid,fill=YlGnBu-8-7},mark=+\\%
 YlGnBu-8-8!70!black, every mark/.append style={solid,fill=YlGnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-9}{%
 YlGnBu-9-1!70!black, every mark/.append style={solid,fill=YlGnBu-9-1},mark=*\\%
 YlGnBu-9-2!70!black, every mark/.append style={solid,fill=YlGnBu-9-2},mark=square*\\%
 YlGnBu-9-3!70!black, every mark/.append style={solid,fill=YlGnBu-9-3},mark=triangle*\\%
 YlGnBu-9-4!70!black, every mark/.append style={solid,fill=YlGnBu-9-4},mark=diamond*\\%
 YlGnBu-9-5!70!black, every mark/.append style={solid,fill=YlGnBu-9-5},mark=pentagon*\\%
 YlGnBu-9-6!70!black, every mark/.append style={solid,fill=YlGnBu-9-6},mark=x\\%
 YlGnBu-9-7!70!black, every mark/.append style={solid,fill=YlGnBu-9-7},mark=+\\%
 YlGnBu-9-8!70!black, every mark/.append style={solid,fill=YlGnBu-9-8},mark=star\\%
 YlGnBu-9-9!70!black, every mark/.append style={solid,fill=YlGnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-3}{%
 GnBu-3-1!70!black, every mark/.append style={solid,fill=GnBu-3-1},mark=*\\%
 GnBu-3-2!70!black, every mark/.append style={solid,fill=GnBu-3-2},mark=square*\\%
 GnBu-3-3!70!black, every mark/.append style={solid,fill=GnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-4}{%
 GnBu-4-1!70!black, every mark/.append style={solid,fill=GnBu-4-1},mark=*\\%
 GnBu-4-2!70!black, every mark/.append style={solid,fill=GnBu-4-2},mark=square*\\%
 GnBu-4-3!70!black, every mark/.append style={solid,fill=GnBu-4-3},mark=triangle*\\%
 GnBu-4-4!70!black, every mark/.append style={solid,fill=GnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-5}{%
 GnBu-5-1!70!black, every mark/.append style={solid,fill=GnBu-5-1},mark=*\\%
 GnBu-5-2!70!black, every mark/.append style={solid,fill=GnBu-5-2},mark=square*\\%
 GnBu-5-3!70!black, every mark/.append style={solid,fill=GnBu-5-3},mark=triangle*\\%
 GnBu-5-4!70!black, every mark/.append style={solid,fill=GnBu-5-4},mark=diamond*\\%
 GnBu-5-5!70!black, every mark/.append style={solid,fill=GnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-6}{%
 GnBu-6-1!70!black, every mark/.append style={solid,fill=GnBu-6-1},mark=*\\%
 GnBu-6-2!70!black, every mark/.append style={solid,fill=GnBu-6-2},mark=square*\\%
 GnBu-6-3!70!black, every mark/.append style={solid,fill=GnBu-6-3},mark=triangle*\\%
 GnBu-6-4!70!black, every mark/.append style={solid,fill=GnBu-6-4},mark=diamond*\\%
 GnBu-6-5!70!black, every mark/.append style={solid,fill=GnBu-6-5},mark=pentagon*\\%
 GnBu-6-6!70!black, every mark/.append style={solid,fill=GnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-7}{%
 GnBu-7-1!70!black, every mark/.append style={solid,fill=GnBu-7-1},mark=*\\%
 GnBu-7-2!70!black, every mark/.append style={solid,fill=GnBu-7-2},mark=square*\\%
 GnBu-7-3!70!black, every mark/.append style={solid,fill=GnBu-7-3},mark=triangle*\\%
 GnBu-7-4!70!black, every mark/.append style={solid,fill=GnBu-7-4},mark=diamond*\\%
 GnBu-7-5!70!black, every mark/.append style={solid,fill=GnBu-7-5},mark=pentagon*\\%
 GnBu-7-6!70!black, every mark/.append style={solid,fill=GnBu-7-6},mark=x\\%
 GnBu-7-7!70!black, every mark/.append style={solid,fill=GnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-8}{%
 GnBu-8-1!70!black, every mark/.append style={solid,fill=GnBu-8-1},mark=*\\%
 GnBu-8-2!70!black, every mark/.append style={solid,fill=GnBu-8-2},mark=square*\\%
 GnBu-8-3!70!black, every mark/.append style={solid,fill=GnBu-8-3},mark=triangle*\\%
 GnBu-8-4!70!black, every mark/.append style={solid,fill=GnBu-8-4},mark=diamond*\\%
 GnBu-8-5!70!black, every mark/.append style={solid,fill=GnBu-8-5},mark=pentagon*\\%
 GnBu-8-6!70!black, every mark/.append style={solid,fill=GnBu-8-6},mark=x\\%
 GnBu-8-7!70!black, every mark/.append style={solid,fill=GnBu-8-7},mark=+\\%
 GnBu-8-8!70!black, every mark/.append style={solid,fill=GnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-9}{%
 GnBu-9-1!70!black, every mark/.append style={solid,fill=GnBu-9-1},mark=*\\%
 GnBu-9-2!70!black, every mark/.append style={solid,fill=GnBu-9-2},mark=square*\\%
 GnBu-9-3!70!black, every mark/.append style={solid,fill=GnBu-9-3},mark=triangle*\\%
 GnBu-9-4!70!black, every mark/.append style={solid,fill=GnBu-9-4},mark=diamond*\\%
 GnBu-9-5!70!black, every mark/.append style={solid,fill=GnBu-9-5},mark=pentagon*\\%
 GnBu-9-6!70!black, every mark/.append style={solid,fill=GnBu-9-6},mark=x\\%
 GnBu-9-7!70!black, every mark/.append style={solid,fill=GnBu-9-7},mark=+\\%
 GnBu-9-8!70!black, every mark/.append style={solid,fill=GnBu-9-8},mark=star\\%
 GnBu-9-9!70!black, every mark/.append style={solid,fill=GnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-3}{%
 BuGn-3-1!70!black, every mark/.append style={solid,fill=BuGn-3-1},mark=*\\%
 BuGn-3-2!70!black, every mark/.append style={solid,fill=BuGn-3-2},mark=square*\\%
 BuGn-3-3!70!black, every mark/.append style={solid,fill=BuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-4}{%
 BuGn-4-1!70!black, every mark/.append style={solid,fill=BuGn-4-1},mark=*\\%
 BuGn-4-2!70!black, every mark/.append style={solid,fill=BuGn-4-2},mark=square*\\%
 BuGn-4-3!70!black, every mark/.append style={solid,fill=BuGn-4-3},mark=triangle*\\%
 BuGn-4-4!70!black, every mark/.append style={solid,fill=BuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-5}{%
 BuGn-5-1!70!black, every mark/.append style={solid,fill=BuGn-5-1},mark=*\\%
 BuGn-5-2!70!black, every mark/.append style={solid,fill=BuGn-5-2},mark=square*\\%
 BuGn-5-3!70!black, every mark/.append style={solid,fill=BuGn-5-3},mark=triangle*\\%
 BuGn-5-4!70!black, every mark/.append style={solid,fill=BuGn-5-4},mark=diamond*\\%
 BuGn-5-5!70!black, every mark/.append style={solid,fill=BuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-6}{%
 BuGn-6-1!70!black, every mark/.append style={solid,fill=BuGn-6-1},mark=*\\%
 BuGn-6-2!70!black, every mark/.append style={solid,fill=BuGn-6-2},mark=square*\\%
 BuGn-6-3!70!black, every mark/.append style={solid,fill=BuGn-6-3},mark=triangle*\\%
 BuGn-6-4!70!black, every mark/.append style={solid,fill=BuGn-6-4},mark=diamond*\\%
 BuGn-6-5!70!black, every mark/.append style={solid,fill=BuGn-6-5},mark=pentagon*\\%
 BuGn-6-6!70!black, every mark/.append style={solid,fill=BuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-7}{%
 BuGn-7-1!70!black, every mark/.append style={solid,fill=BuGn-7-1},mark=*\\%
 BuGn-7-2!70!black, every mark/.append style={solid,fill=BuGn-7-2},mark=square*\\%
 BuGn-7-3!70!black, every mark/.append style={solid,fill=BuGn-7-3},mark=triangle*\\%
 BuGn-7-4!70!black, every mark/.append style={solid,fill=BuGn-7-4},mark=diamond*\\%
 BuGn-7-5!70!black, every mark/.append style={solid,fill=BuGn-7-5},mark=pentagon*\\%
 BuGn-7-6!70!black, every mark/.append style={solid,fill=BuGn-7-6},mark=x\\%
 BuGn-7-7!70!black, every mark/.append style={solid,fill=BuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-8}{%
 BuGn-8-1!70!black, every mark/.append style={solid,fill=BuGn-8-1},mark=*\\%
 BuGn-8-2!70!black, every mark/.append style={solid,fill=BuGn-8-2},mark=square*\\%
 BuGn-8-3!70!black, every mark/.append style={solid,fill=BuGn-8-3},mark=triangle*\\%
 BuGn-8-4!70!black, every mark/.append style={solid,fill=BuGn-8-4},mark=diamond*\\%
 BuGn-8-5!70!black, every mark/.append style={solid,fill=BuGn-8-5},mark=pentagon*\\%
 BuGn-8-6!70!black, every mark/.append style={solid,fill=BuGn-8-6},mark=x\\%
 BuGn-8-7!70!black, every mark/.append style={solid,fill=BuGn-8-7},mark=+\\%
 BuGn-8-8!70!black, every mark/.append style={solid,fill=BuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-9}{%
 BuGn-9-1!70!black, every mark/.append style={solid,fill=BuGn-9-1},mark=*\\%
 BuGn-9-2!70!black, every mark/.append style={solid,fill=BuGn-9-2},mark=square*\\%
 BuGn-9-3!70!black, every mark/.append style={solid,fill=BuGn-9-3},mark=triangle*\\%
 BuGn-9-4!70!black, every mark/.append style={solid,fill=BuGn-9-4},mark=diamond*\\%
 BuGn-9-5!70!black, every mark/.append style={solid,fill=BuGn-9-5},mark=pentagon*\\%
 BuGn-9-6!70!black, every mark/.append style={solid,fill=BuGn-9-6},mark=x\\%
 BuGn-9-7!70!black, every mark/.append style={solid,fill=BuGn-9-7},mark=+\\%
 BuGn-9-8!70!black, every mark/.append style={solid,fill=BuGn-9-8},mark=star\\%
 BuGn-9-9!70!black, every mark/.append style={solid,fill=BuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-3}{%
 PuBuGn-3-1!70!black, every mark/.append style={solid,fill=PuBuGn-3-1},mark=*\\%
 PuBuGn-3-2!70!black, every mark/.append style={solid,fill=PuBuGn-3-2},mark=square*\\%
 PuBuGn-3-3!70!black, every mark/.append style={solid,fill=PuBuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-4}{%
 PuBuGn-4-1!70!black, every mark/.append style={solid,fill=PuBuGn-4-1},mark=*\\%
 PuBuGn-4-2!70!black, every mark/.append style={solid,fill=PuBuGn-4-2},mark=square*\\%
 PuBuGn-4-3!70!black, every mark/.append style={solid,fill=PuBuGn-4-3},mark=triangle*\\%
 PuBuGn-4-4!70!black, every mark/.append style={solid,fill=PuBuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-5}{%
 PuBuGn-5-1!70!black, every mark/.append style={solid,fill=PuBuGn-5-1},mark=*\\%
 PuBuGn-5-2!70!black, every mark/.append style={solid,fill=PuBuGn-5-2},mark=square*\\%
 PuBuGn-5-3!70!black, every mark/.append style={solid,fill=PuBuGn-5-3},mark=triangle*\\%
 PuBuGn-5-4!70!black, every mark/.append style={solid,fill=PuBuGn-5-4},mark=diamond*\\%
 PuBuGn-5-5!70!black, every mark/.append style={solid,fill=PuBuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-6}{%
 PuBuGn-6-1!70!black, every mark/.append style={solid,fill=PuBuGn-6-1},mark=*\\%
 PuBuGn-6-2!70!black, every mark/.append style={solid,fill=PuBuGn-6-2},mark=square*\\%
 PuBuGn-6-3!70!black, every mark/.append style={solid,fill=PuBuGn-6-3},mark=triangle*\\%
 PuBuGn-6-4!70!black, every mark/.append style={solid,fill=PuBuGn-6-4},mark=diamond*\\%
 PuBuGn-6-5!70!black, every mark/.append style={solid,fill=PuBuGn-6-5},mark=pentagon*\\%
 PuBuGn-6-6!70!black, every mark/.append style={solid,fill=PuBuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-7}{%
 PuBuGn-7-1!70!black, every mark/.append style={solid,fill=PuBuGn-7-1},mark=*\\%
 PuBuGn-7-2!70!black, every mark/.append style={solid,fill=PuBuGn-7-2},mark=square*\\%
 PuBuGn-7-3!70!black, every mark/.append style={solid,fill=PuBuGn-7-3},mark=triangle*\\%
 PuBuGn-7-4!70!black, every mark/.append style={solid,fill=PuBuGn-7-4},mark=diamond*\\%
 PuBuGn-7-5!70!black, every mark/.append style={solid,fill=PuBuGn-7-5},mark=pentagon*\\%
 PuBuGn-7-6!70!black, every mark/.append style={solid,fill=PuBuGn-7-6},mark=x\\%
 PuBuGn-7-7!70!black, every mark/.append style={solid,fill=PuBuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-8}{%
 PuBuGn-8-1!70!black, every mark/.append style={solid,fill=PuBuGn-8-1},mark=*\\%
 PuBuGn-8-2!70!black, every mark/.append style={solid,fill=PuBuGn-8-2},mark=square*\\%
 PuBuGn-8-3!70!black, every mark/.append style={solid,fill=PuBuGn-8-3},mark=triangle*\\%
 PuBuGn-8-4!70!black, every mark/.append style={solid,fill=PuBuGn-8-4},mark=diamond*\\%
 PuBuGn-8-5!70!black, every mark/.append style={solid,fill=PuBuGn-8-5},mark=pentagon*\\%
 PuBuGn-8-6!70!black, every mark/.append style={solid,fill=PuBuGn-8-6},mark=x\\%
 PuBuGn-8-7!70!black, every mark/.append style={solid,fill=PuBuGn-8-7},mark=+\\%
 PuBuGn-8-8!70!black, every mark/.append style={solid,fill=PuBuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-9}{%
 PuBuGn-9-1!70!black, every mark/.append style={solid,fill=PuBuGn-9-1},mark=*\\%
 PuBuGn-9-2!70!black, every mark/.append style={solid,fill=PuBuGn-9-2},mark=square*\\%
 PuBuGn-9-3!70!black, every mark/.append style={solid,fill=PuBuGn-9-3},mark=triangle*\\%
 PuBuGn-9-4!70!black, every mark/.append style={solid,fill=PuBuGn-9-4},mark=diamond*\\%
 PuBuGn-9-5!70!black, every mark/.append style={solid,fill=PuBuGn-9-5},mark=pentagon*\\%
 PuBuGn-9-6!70!black, every mark/.append style={solid,fill=PuBuGn-9-6},mark=x\\%
 PuBuGn-9-7!70!black, every mark/.append style={solid,fill=PuBuGn-9-7},mark=+\\%
 PuBuGn-9-8!70!black, every mark/.append style={solid,fill=PuBuGn-9-8},mark=star\\%
 PuBuGn-9-9!70!black, every mark/.append style={solid,fill=PuBuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-3}{%
 PuBu-3-1!70!black, every mark/.append style={solid,fill=PuBu-3-1},mark=*\\%
 PuBu-3-2!70!black, every mark/.append style={solid,fill=PuBu-3-2},mark=square*\\%
 PuBu-3-3!70!black, every mark/.append style={solid,fill=PuBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-4}{%
 PuBu-4-1!70!black, every mark/.append style={solid,fill=PuBu-4-1},mark=*\\%
 PuBu-4-2!70!black, every mark/.append style={solid,fill=PuBu-4-2},mark=square*\\%
 PuBu-4-3!70!black, every mark/.append style={solid,fill=PuBu-4-3},mark=triangle*\\%
 PuBu-4-4!70!black, every mark/.append style={solid,fill=PuBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-5}{%
 PuBu-5-1!70!black, every mark/.append style={solid,fill=PuBu-5-1},mark=*\\%
 PuBu-5-2!70!black, every mark/.append style={solid,fill=PuBu-5-2},mark=square*\\%
 PuBu-5-3!70!black, every mark/.append style={solid,fill=PuBu-5-3},mark=triangle*\\%
 PuBu-5-4!70!black, every mark/.append style={solid,fill=PuBu-5-4},mark=diamond*\\%
 PuBu-5-5!70!black, every mark/.append style={solid,fill=PuBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-6}{%
 PuBu-6-1!70!black, every mark/.append style={solid,fill=PuBu-6-1},mark=*\\%
 PuBu-6-2!70!black, every mark/.append style={solid,fill=PuBu-6-2},mark=square*\\%
 PuBu-6-3!70!black, every mark/.append style={solid,fill=PuBu-6-3},mark=triangle*\\%
 PuBu-6-4!70!black, every mark/.append style={solid,fill=PuBu-6-4},mark=diamond*\\%
 PuBu-6-5!70!black, every mark/.append style={solid,fill=PuBu-6-5},mark=pentagon*\\%
 PuBu-6-6!70!black, every mark/.append style={solid,fill=PuBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-7}{%
 PuBu-7-1!70!black, every mark/.append style={solid,fill=PuBu-7-1},mark=*\\%
 PuBu-7-2!70!black, every mark/.append style={solid,fill=PuBu-7-2},mark=square*\\%
 PuBu-7-3!70!black, every mark/.append style={solid,fill=PuBu-7-3},mark=triangle*\\%
 PuBu-7-4!70!black, every mark/.append style={solid,fill=PuBu-7-4},mark=diamond*\\%
 PuBu-7-5!70!black, every mark/.append style={solid,fill=PuBu-7-5},mark=pentagon*\\%
 PuBu-7-6!70!black, every mark/.append style={solid,fill=PuBu-7-6},mark=x\\%
 PuBu-7-7!70!black, every mark/.append style={solid,fill=PuBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-8}{%
 PuBu-8-1!70!black, every mark/.append style={solid,fill=PuBu-8-1},mark=*\\%
 PuBu-8-2!70!black, every mark/.append style={solid,fill=PuBu-8-2},mark=square*\\%
 PuBu-8-3!70!black, every mark/.append style={solid,fill=PuBu-8-3},mark=triangle*\\%
 PuBu-8-4!70!black, every mark/.append style={solid,fill=PuBu-8-4},mark=diamond*\\%
 PuBu-8-5!70!black, every mark/.append style={solid,fill=PuBu-8-5},mark=pentagon*\\%
 PuBu-8-6!70!black, every mark/.append style={solid,fill=PuBu-8-6},mark=x\\%
 PuBu-8-7!70!black, every mark/.append style={solid,fill=PuBu-8-7},mark=+\\%
 PuBu-8-8!70!black, every mark/.append style={solid,fill=PuBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-9}{%
 PuBu-9-1!70!black, every mark/.append style={solid,fill=PuBu-9-1},mark=*\\%
 PuBu-9-2!70!black, every mark/.append style={solid,fill=PuBu-9-2},mark=square*\\%
 PuBu-9-3!70!black, every mark/.append style={solid,fill=PuBu-9-3},mark=triangle*\\%
 PuBu-9-4!70!black, every mark/.append style={solid,fill=PuBu-9-4},mark=diamond*\\%
 PuBu-9-5!70!black, every mark/.append style={solid,fill=PuBu-9-5},mark=pentagon*\\%
 PuBu-9-6!70!black, every mark/.append style={solid,fill=PuBu-9-6},mark=x\\%
 PuBu-9-7!70!black, every mark/.append style={solid,fill=PuBu-9-7},mark=+\\%
 PuBu-9-8!70!black, every mark/.append style={solid,fill=PuBu-9-8},mark=star\\%
 PuBu-9-9!70!black, every mark/.append style={solid,fill=PuBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-3}{%
 BuPu-3-1!70!black, every mark/.append style={solid,fill=BuPu-3-1},mark=*\\%
 BuPu-3-2!70!black, every mark/.append style={solid,fill=BuPu-3-2},mark=square*\\%
 BuPu-3-3!70!black, every mark/.append style={solid,fill=BuPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-4}{%
 BuPu-4-1!70!black, every mark/.append style={solid,fill=BuPu-4-1},mark=*\\%
 BuPu-4-2!70!black, every mark/.append style={solid,fill=BuPu-4-2},mark=square*\\%
 BuPu-4-3!70!black, every mark/.append style={solid,fill=BuPu-4-3},mark=triangle*\\%
 BuPu-4-4!70!black, every mark/.append style={solid,fill=BuPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-5}{%
 BuPu-5-1!70!black, every mark/.append style={solid,fill=BuPu-5-1},mark=*\\%
 BuPu-5-2!70!black, every mark/.append style={solid,fill=BuPu-5-2},mark=square*\\%
 BuPu-5-3!70!black, every mark/.append style={solid,fill=BuPu-5-3},mark=triangle*\\%
 BuPu-5-4!70!black, every mark/.append style={solid,fill=BuPu-5-4},mark=diamond*\\%
 BuPu-5-5!70!black, every mark/.append style={solid,fill=BuPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-6}{%
 BuPu-6-1!70!black, every mark/.append style={solid,fill=BuPu-6-1},mark=*\\%
 BuPu-6-2!70!black, every mark/.append style={solid,fill=BuPu-6-2},mark=square*\\%
 BuPu-6-3!70!black, every mark/.append style={solid,fill=BuPu-6-3},mark=triangle*\\%
 BuPu-6-4!70!black, every mark/.append style={solid,fill=BuPu-6-4},mark=diamond*\\%
 BuPu-6-5!70!black, every mark/.append style={solid,fill=BuPu-6-5},mark=pentagon*\\%
 BuPu-6-6!70!black, every mark/.append style={solid,fill=BuPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-7}{%
 BuPu-7-1!70!black, every mark/.append style={solid,fill=BuPu-7-1},mark=*\\%
 BuPu-7-2!70!black, every mark/.append style={solid,fill=BuPu-7-2},mark=square*\\%
 BuPu-7-3!70!black, every mark/.append style={solid,fill=BuPu-7-3},mark=triangle*\\%
 BuPu-7-4!70!black, every mark/.append style={solid,fill=BuPu-7-4},mark=diamond*\\%
 BuPu-7-5!70!black, every mark/.append style={solid,fill=BuPu-7-5},mark=pentagon*\\%
 BuPu-7-6!70!black, every mark/.append style={solid,fill=BuPu-7-6},mark=x\\%
 BuPu-7-7!70!black, every mark/.append style={solid,fill=BuPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-8}{%
 BuPu-8-1!70!black, every mark/.append style={solid,fill=BuPu-8-1},mark=*\\%
 BuPu-8-2!70!black, every mark/.append style={solid,fill=BuPu-8-2},mark=square*\\%
 BuPu-8-3!70!black, every mark/.append style={solid,fill=BuPu-8-3},mark=triangle*\\%
 BuPu-8-4!70!black, every mark/.append style={solid,fill=BuPu-8-4},mark=diamond*\\%
 BuPu-8-5!70!black, every mark/.append style={solid,fill=BuPu-8-5},mark=pentagon*\\%
 BuPu-8-6!70!black, every mark/.append style={solid,fill=BuPu-8-6},mark=x\\%
 BuPu-8-7!70!black, every mark/.append style={solid,fill=BuPu-8-7},mark=+\\%
 BuPu-8-8!70!black, every mark/.append style={solid,fill=BuPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-9}{%
 BuPu-9-1!70!black, every mark/.append style={solid,fill=BuPu-9-1},mark=*\\%
 BuPu-9-2!70!black, every mark/.append style={solid,fill=BuPu-9-2},mark=square*\\%
 BuPu-9-3!70!black, every mark/.append style={solid,fill=BuPu-9-3},mark=triangle*\\%
 BuPu-9-4!70!black, every mark/.append style={solid,fill=BuPu-9-4},mark=diamond*\\%
 BuPu-9-5!70!black, every mark/.append style={solid,fill=BuPu-9-5},mark=pentagon*\\%
 BuPu-9-6!70!black, every mark/.append style={solid,fill=BuPu-9-6},mark=x\\%
 BuPu-9-7!70!black, every mark/.append style={solid,fill=BuPu-9-7},mark=+\\%
 BuPu-9-8!70!black, every mark/.append style={solid,fill=BuPu-9-8},mark=star\\%
 BuPu-9-9!70!black, every mark/.append style={solid,fill=BuPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-3}{%
 RdPu-3-1!70!black, every mark/.append style={solid,fill=RdPu-3-1},mark=*\\%
 RdPu-3-2!70!black, every mark/.append style={solid,fill=RdPu-3-2},mark=square*\\%
 RdPu-3-3!70!black, every mark/.append style={solid,fill=RdPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-4}{%
 RdPu-4-1!70!black, every mark/.append style={solid,fill=RdPu-4-1},mark=*\\%
 RdPu-4-2!70!black, every mark/.append style={solid,fill=RdPu-4-2},mark=square*\\%
 RdPu-4-3!70!black, every mark/.append style={solid,fill=RdPu-4-3},mark=triangle*\\%
 RdPu-4-4!70!black, every mark/.append style={solid,fill=RdPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-5}{%
 RdPu-5-1!70!black, every mark/.append style={solid,fill=RdPu-5-1},mark=*\\%
 RdPu-5-2!70!black, every mark/.append style={solid,fill=RdPu-5-2},mark=square*\\%
 RdPu-5-3!70!black, every mark/.append style={solid,fill=RdPu-5-3},mark=triangle*\\%
 RdPu-5-4!70!black, every mark/.append style={solid,fill=RdPu-5-4},mark=diamond*\\%
 RdPu-5-5!70!black, every mark/.append style={solid,fill=RdPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-6}{%
 RdPu-6-1!70!black, every mark/.append style={solid,fill=RdPu-6-1},mark=*\\%
 RdPu-6-2!70!black, every mark/.append style={solid,fill=RdPu-6-2},mark=square*\\%
 RdPu-6-3!70!black, every mark/.append style={solid,fill=RdPu-6-3},mark=triangle*\\%
 RdPu-6-4!70!black, every mark/.append style={solid,fill=RdPu-6-4},mark=diamond*\\%
 RdPu-6-5!70!black, every mark/.append style={solid,fill=RdPu-6-5},mark=pentagon*\\%
 RdPu-6-6!70!black, every mark/.append style={solid,fill=RdPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-7}{%
 RdPu-7-1!70!black, every mark/.append style={solid,fill=RdPu-7-1},mark=*\\%
 RdPu-7-2!70!black, every mark/.append style={solid,fill=RdPu-7-2},mark=square*\\%
 RdPu-7-3!70!black, every mark/.append style={solid,fill=RdPu-7-3},mark=triangle*\\%
 RdPu-7-4!70!black, every mark/.append style={solid,fill=RdPu-7-4},mark=diamond*\\%
 RdPu-7-5!70!black, every mark/.append style={solid,fill=RdPu-7-5},mark=pentagon*\\%
 RdPu-7-6!70!black, every mark/.append style={solid,fill=RdPu-7-6},mark=x\\%
 RdPu-7-7!70!black, every mark/.append style={solid,fill=RdPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-8}{%
 RdPu-8-1!70!black, every mark/.append style={solid,fill=RdPu-8-1},mark=*\\%
 RdPu-8-2!70!black, every mark/.append style={solid,fill=RdPu-8-2},mark=square*\\%
 RdPu-8-3!70!black, every mark/.append style={solid,fill=RdPu-8-3},mark=triangle*\\%
 RdPu-8-4!70!black, every mark/.append style={solid,fill=RdPu-8-4},mark=diamond*\\%
 RdPu-8-5!70!black, every mark/.append style={solid,fill=RdPu-8-5},mark=pentagon*\\%
 RdPu-8-6!70!black, every mark/.append style={solid,fill=RdPu-8-6},mark=x\\%
 RdPu-8-7!70!black, every mark/.append style={solid,fill=RdPu-8-7},mark=+\\%
 RdPu-8-8!70!black, every mark/.append style={solid,fill=RdPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-9}{%
 RdPu-9-1!70!black, every mark/.append style={solid,fill=RdPu-9-1},mark=*\\%
 RdPu-9-2!70!black, every mark/.append style={solid,fill=RdPu-9-2},mark=square*\\%
 RdPu-9-3!70!black, every mark/.append style={solid,fill=RdPu-9-3},mark=triangle*\\%
 RdPu-9-4!70!black, every mark/.append style={solid,fill=RdPu-9-4},mark=diamond*\\%
 RdPu-9-5!70!black, every mark/.append style={solid,fill=RdPu-9-5},mark=pentagon*\\%
 RdPu-9-6!70!black, every mark/.append style={solid,fill=RdPu-9-6},mark=x\\%
 RdPu-9-7!70!black, every mark/.append style={solid,fill=RdPu-9-7},mark=+\\%
 RdPu-9-8!70!black, every mark/.append style={solid,fill=RdPu-9-8},mark=star\\%
 RdPu-9-9!70!black, every mark/.append style={solid,fill=RdPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-3}{%
 PuRd-3-1!70!black, every mark/.append style={solid,fill=PuRd-3-1},mark=*\\%
 PuRd-3-2!70!black, every mark/.append style={solid,fill=PuRd-3-2},mark=square*\\%
 PuRd-3-3!70!black, every mark/.append style={solid,fill=PuRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-4}{%
 PuRd-4-1!70!black, every mark/.append style={solid,fill=PuRd-4-1},mark=*\\%
 PuRd-4-2!70!black, every mark/.append style={solid,fill=PuRd-4-2},mark=square*\\%
 PuRd-4-3!70!black, every mark/.append style={solid,fill=PuRd-4-3},mark=triangle*\\%
 PuRd-4-4!70!black, every mark/.append style={solid,fill=PuRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-5}{%
 PuRd-5-1!70!black, every mark/.append style={solid,fill=PuRd-5-1},mark=*\\%
 PuRd-5-2!70!black, every mark/.append style={solid,fill=PuRd-5-2},mark=square*\\%
 PuRd-5-3!70!black, every mark/.append style={solid,fill=PuRd-5-3},mark=triangle*\\%
 PuRd-5-4!70!black, every mark/.append style={solid,fill=PuRd-5-4},mark=diamond*\\%
 PuRd-5-5!70!black, every mark/.append style={solid,fill=PuRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-6}{%
 PuRd-6-1!70!black, every mark/.append style={solid,fill=PuRd-6-1},mark=*\\%
 PuRd-6-2!70!black, every mark/.append style={solid,fill=PuRd-6-2},mark=square*\\%
 PuRd-6-3!70!black, every mark/.append style={solid,fill=PuRd-6-3},mark=triangle*\\%
 PuRd-6-4!70!black, every mark/.append style={solid,fill=PuRd-6-4},mark=diamond*\\%
 PuRd-6-5!70!black, every mark/.append style={solid,fill=PuRd-6-5},mark=pentagon*\\%
 PuRd-6-6!70!black, every mark/.append style={solid,fill=PuRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-7}{%
 PuRd-7-1!70!black, every mark/.append style={solid,fill=PuRd-7-1},mark=*\\%
 PuRd-7-2!70!black, every mark/.append style={solid,fill=PuRd-7-2},mark=square*\\%
 PuRd-7-3!70!black, every mark/.append style={solid,fill=PuRd-7-3},mark=triangle*\\%
 PuRd-7-4!70!black, every mark/.append style={solid,fill=PuRd-7-4},mark=diamond*\\%
 PuRd-7-5!70!black, every mark/.append style={solid,fill=PuRd-7-5},mark=pentagon*\\%
 PuRd-7-6!70!black, every mark/.append style={solid,fill=PuRd-7-6},mark=x\\%
 PuRd-7-7!70!black, every mark/.append style={solid,fill=PuRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-8}{%
 PuRd-8-1!70!black, every mark/.append style={solid,fill=PuRd-8-1},mark=*\\%
 PuRd-8-2!70!black, every mark/.append style={solid,fill=PuRd-8-2},mark=square*\\%
 PuRd-8-3!70!black, every mark/.append style={solid,fill=PuRd-8-3},mark=triangle*\\%
 PuRd-8-4!70!black, every mark/.append style={solid,fill=PuRd-8-4},mark=diamond*\\%
 PuRd-8-5!70!black, every mark/.append style={solid,fill=PuRd-8-5},mark=pentagon*\\%
 PuRd-8-6!70!black, every mark/.append style={solid,fill=PuRd-8-6},mark=x\\%
 PuRd-8-7!70!black, every mark/.append style={solid,fill=PuRd-8-7},mark=+\\%
 PuRd-8-8!70!black, every mark/.append style={solid,fill=PuRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-9}{%
 PuRd-9-1!70!black, every mark/.append style={solid,fill=PuRd-9-1},mark=*\\%
 PuRd-9-2!70!black, every mark/.append style={solid,fill=PuRd-9-2},mark=square*\\%
 PuRd-9-3!70!black, every mark/.append style={solid,fill=PuRd-9-3},mark=triangle*\\%
 PuRd-9-4!70!black, every mark/.append style={solid,fill=PuRd-9-4},mark=diamond*\\%
 PuRd-9-5!70!black, every mark/.append style={solid,fill=PuRd-9-5},mark=pentagon*\\%
 PuRd-9-6!70!black, every mark/.append style={solid,fill=PuRd-9-6},mark=x\\%
 PuRd-9-7!70!black, every mark/.append style={solid,fill=PuRd-9-7},mark=+\\%
 PuRd-9-8!70!black, every mark/.append style={solid,fill=PuRd-9-8},mark=star\\%
 PuRd-9-9!70!black, every mark/.append style={solid,fill=PuRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-3}{%
 OrRd-3-1!70!black, every mark/.append style={solid,fill=OrRd-3-1},mark=*\\%
 OrRd-3-2!70!black, every mark/.append style={solid,fill=OrRd-3-2},mark=square*\\%
 OrRd-3-3!70!black, every mark/.append style={solid,fill=OrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-4}{%
 OrRd-4-1!70!black, every mark/.append style={solid,fill=OrRd-4-1},mark=*\\%
 OrRd-4-2!70!black, every mark/.append style={solid,fill=OrRd-4-2},mark=square*\\%
 OrRd-4-3!70!black, every mark/.append style={solid,fill=OrRd-4-3},mark=triangle*\\%
 OrRd-4-4!70!black, every mark/.append style={solid,fill=OrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-5}{%
 OrRd-5-1!70!black, every mark/.append style={solid,fill=OrRd-5-1},mark=*\\%
 OrRd-5-2!70!black, every mark/.append style={solid,fill=OrRd-5-2},mark=square*\\%
 OrRd-5-3!70!black, every mark/.append style={solid,fill=OrRd-5-3},mark=triangle*\\%
 OrRd-5-4!70!black, every mark/.append style={solid,fill=OrRd-5-4},mark=diamond*\\%
 OrRd-5-5!70!black, every mark/.append style={solid,fill=OrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-6}{%
 OrRd-6-1!70!black, every mark/.append style={solid,fill=OrRd-6-1},mark=*\\%
 OrRd-6-2!70!black, every mark/.append style={solid,fill=OrRd-6-2},mark=square*\\%
 OrRd-6-3!70!black, every mark/.append style={solid,fill=OrRd-6-3},mark=triangle*\\%
 OrRd-6-4!70!black, every mark/.append style={solid,fill=OrRd-6-4},mark=diamond*\\%
 OrRd-6-5!70!black, every mark/.append style={solid,fill=OrRd-6-5},mark=pentagon*\\%
 OrRd-6-6!70!black, every mark/.append style={solid,fill=OrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-7}{%
 OrRd-7-1!70!black, every mark/.append style={solid,fill=OrRd-7-1},mark=*\\%
 OrRd-7-2!70!black, every mark/.append style={solid,fill=OrRd-7-2},mark=square*\\%
 OrRd-7-3!70!black, every mark/.append style={solid,fill=OrRd-7-3},mark=triangle*\\%
 OrRd-7-4!70!black, every mark/.append style={solid,fill=OrRd-7-4},mark=diamond*\\%
 OrRd-7-5!70!black, every mark/.append style={solid,fill=OrRd-7-5},mark=pentagon*\\%
 OrRd-7-6!70!black, every mark/.append style={solid,fill=OrRd-7-6},mark=x\\%
 OrRd-7-7!70!black, every mark/.append style={solid,fill=OrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-8}{%
 OrRd-8-1!70!black, every mark/.append style={solid,fill=OrRd-8-1},mark=*\\%
 OrRd-8-2!70!black, every mark/.append style={solid,fill=OrRd-8-2},mark=square*\\%
 OrRd-8-3!70!black, every mark/.append style={solid,fill=OrRd-8-3},mark=triangle*\\%
 OrRd-8-4!70!black, every mark/.append style={solid,fill=OrRd-8-4},mark=diamond*\\%
 OrRd-8-5!70!black, every mark/.append style={solid,fill=OrRd-8-5},mark=pentagon*\\%
 OrRd-8-6!70!black, every mark/.append style={solid,fill=OrRd-8-6},mark=x\\%
 OrRd-8-7!70!black, every mark/.append style={solid,fill=OrRd-8-7},mark=+\\%
 OrRd-8-8!70!black, every mark/.append style={solid,fill=OrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-9}{%
 OrRd-9-1!70!black, every mark/.append style={solid,fill=OrRd-9-1},mark=*\\%
 OrRd-9-2!70!black, every mark/.append style={solid,fill=OrRd-9-2},mark=square*\\%
 OrRd-9-3!70!black, every mark/.append style={solid,fill=OrRd-9-3},mark=triangle*\\%
 OrRd-9-4!70!black, every mark/.append style={solid,fill=OrRd-9-4},mark=diamond*\\%
 OrRd-9-5!70!black, every mark/.append style={solid,fill=OrRd-9-5},mark=pentagon*\\%
 OrRd-9-6!70!black, every mark/.append style={solid,fill=OrRd-9-6},mark=x\\%
 OrRd-9-7!70!black, every mark/.append style={solid,fill=OrRd-9-7},mark=+\\%
 OrRd-9-8!70!black, every mark/.append style={solid,fill=OrRd-9-8},mark=star\\%
 OrRd-9-9!70!black, every mark/.append style={solid,fill=OrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-3}{%
 YlOrRd-3-1!70!black, every mark/.append style={solid,fill=YlOrRd-3-1},mark=*\\%
 YlOrRd-3-2!70!black, every mark/.append style={solid,fill=YlOrRd-3-2},mark=square*\\%
 YlOrRd-3-3!70!black, every mark/.append style={solid,fill=YlOrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-4}{%
 YlOrRd-4-1!70!black, every mark/.append style={solid,fill=YlOrRd-4-1},mark=*\\%
 YlOrRd-4-2!70!black, every mark/.append style={solid,fill=YlOrRd-4-2},mark=square*\\%
 YlOrRd-4-3!70!black, every mark/.append style={solid,fill=YlOrRd-4-3},mark=triangle*\\%
 YlOrRd-4-4!70!black, every mark/.append style={solid,fill=YlOrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-5}{%
 YlOrRd-5-1!70!black, every mark/.append style={solid,fill=YlOrRd-5-1},mark=*\\%
 YlOrRd-5-2!70!black, every mark/.append style={solid,fill=YlOrRd-5-2},mark=square*\\%
 YlOrRd-5-3!70!black, every mark/.append style={solid,fill=YlOrRd-5-3},mark=triangle*\\%
 YlOrRd-5-4!70!black, every mark/.append style={solid,fill=YlOrRd-5-4},mark=diamond*\\%
 YlOrRd-5-5!70!black, every mark/.append style={solid,fill=YlOrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-6}{%
 YlOrRd-6-1!70!black, every mark/.append style={solid,fill=YlOrRd-6-1},mark=*\\%
 YlOrRd-6-2!70!black, every mark/.append style={solid,fill=YlOrRd-6-2},mark=square*\\%
 YlOrRd-6-3!70!black, every mark/.append style={solid,fill=YlOrRd-6-3},mark=triangle*\\%
 YlOrRd-6-4!70!black, every mark/.append style={solid,fill=YlOrRd-6-4},mark=diamond*\\%
 YlOrRd-6-5!70!black, every mark/.append style={solid,fill=YlOrRd-6-5},mark=pentagon*\\%
 YlOrRd-6-6!70!black, every mark/.append style={solid,fill=YlOrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-7}{%
 YlOrRd-7-1!70!black, every mark/.append style={solid,fill=YlOrRd-7-1},mark=*\\%
 YlOrRd-7-2!70!black, every mark/.append style={solid,fill=YlOrRd-7-2},mark=square*\\%
 YlOrRd-7-3!70!black, every mark/.append style={solid,fill=YlOrRd-7-3},mark=triangle*\\%
 YlOrRd-7-4!70!black, every mark/.append style={solid,fill=YlOrRd-7-4},mark=diamond*\\%
 YlOrRd-7-5!70!black, every mark/.append style={solid,fill=YlOrRd-7-5},mark=pentagon*\\%
 YlOrRd-7-6!70!black, every mark/.append style={solid,fill=YlOrRd-7-6},mark=x\\%
 YlOrRd-7-7!70!black, every mark/.append style={solid,fill=YlOrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-8}{%
 YlOrRd-8-1!70!black, every mark/.append style={solid,fill=YlOrRd-8-1},mark=*\\%
 YlOrRd-8-2!70!black, every mark/.append style={solid,fill=YlOrRd-8-2},mark=square*\\%
 YlOrRd-8-3!70!black, every mark/.append style={solid,fill=YlOrRd-8-3},mark=triangle*\\%
 YlOrRd-8-4!70!black, every mark/.append style={solid,fill=YlOrRd-8-4},mark=diamond*\\%
 YlOrRd-8-5!70!black, every mark/.append style={solid,fill=YlOrRd-8-5},mark=pentagon*\\%
 YlOrRd-8-6!70!black, every mark/.append style={solid,fill=YlOrRd-8-6},mark=x\\%
 YlOrRd-8-7!70!black, every mark/.append style={solid,fill=YlOrRd-8-7},mark=+\\%
 YlOrRd-8-8!70!black, every mark/.append style={solid,fill=YlOrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-9}{%
 YlOrRd-9-1!70!black, every mark/.append style={solid,fill=YlOrRd-9-1},mark=*\\%
 YlOrRd-9-2!70!black, every mark/.append style={solid,fill=YlOrRd-9-2},mark=square*\\%
 YlOrRd-9-3!70!black, every mark/.append style={solid,fill=YlOrRd-9-3},mark=triangle*\\%
 YlOrRd-9-4!70!black, every mark/.append style={solid,fill=YlOrRd-9-4},mark=diamond*\\%
 YlOrRd-9-5!70!black, every mark/.append style={solid,fill=YlOrRd-9-5},mark=pentagon*\\%
 YlOrRd-9-6!70!black, every mark/.append style={solid,fill=YlOrRd-9-6},mark=x\\%
 YlOrRd-9-7!70!black, every mark/.append style={solid,fill=YlOrRd-9-7},mark=+\\%
 YlOrRd-9-8!70!black, every mark/.append style={solid,fill=YlOrRd-9-8},mark=star\\%
 YlOrRd-9-9!70!black, every mark/.append style={solid,fill=YlOrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-3}{%
 YlOrBr-3-1!70!black, every mark/.append style={solid,fill=YlOrBr-3-1},mark=*\\%
 YlOrBr-3-2!70!black, every mark/.append style={solid,fill=YlOrBr-3-2},mark=square*\\%
 YlOrBr-3-3!70!black, every mark/.append style={solid,fill=YlOrBr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-4}{%
 YlOrBr-4-1!70!black, every mark/.append style={solid,fill=YlOrBr-4-1},mark=*\\%
 YlOrBr-4-2!70!black, every mark/.append style={solid,fill=YlOrBr-4-2},mark=square*\\%
 YlOrBr-4-3!70!black, every mark/.append style={solid,fill=YlOrBr-4-3},mark=triangle*\\%
 YlOrBr-4-4!70!black, every mark/.append style={solid,fill=YlOrBr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-5}{%
 YlOrBr-5-1!70!black, every mark/.append style={solid,fill=YlOrBr-5-1},mark=*\\%
 YlOrBr-5-2!70!black, every mark/.append style={solid,fill=YlOrBr-5-2},mark=square*\\%
 YlOrBr-5-3!70!black, every mark/.append style={solid,fill=YlOrBr-5-3},mark=triangle*\\%
 YlOrBr-5-4!70!black, every mark/.append style={solid,fill=YlOrBr-5-4},mark=diamond*\\%
 YlOrBr-5-5!70!black, every mark/.append style={solid,fill=YlOrBr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-6}{%
 YlOrBr-6-1!70!black, every mark/.append style={solid,fill=YlOrBr-6-1},mark=*\\%
 YlOrBr-6-2!70!black, every mark/.append style={solid,fill=YlOrBr-6-2},mark=square*\\%
 YlOrBr-6-3!70!black, every mark/.append style={solid,fill=YlOrBr-6-3},mark=triangle*\\%
 YlOrBr-6-4!70!black, every mark/.append style={solid,fill=YlOrBr-6-4},mark=diamond*\\%
 YlOrBr-6-5!70!black, every mark/.append style={solid,fill=YlOrBr-6-5},mark=pentagon*\\%
 YlOrBr-6-6!70!black, every mark/.append style={solid,fill=YlOrBr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-7}{%
 YlOrBr-7-1!70!black, every mark/.append style={solid,fill=YlOrBr-7-1},mark=*\\%
 YlOrBr-7-2!70!black, every mark/.append style={solid,fill=YlOrBr-7-2},mark=square*\\%
 YlOrBr-7-3!70!black, every mark/.append style={solid,fill=YlOrBr-7-3},mark=triangle*\\%
 YlOrBr-7-4!70!black, every mark/.append style={solid,fill=YlOrBr-7-4},mark=diamond*\\%
 YlOrBr-7-5!70!black, every mark/.append style={solid,fill=YlOrBr-7-5},mark=pentagon*\\%
 YlOrBr-7-6!70!black, every mark/.append style={solid,fill=YlOrBr-7-6},mark=x\\%
 YlOrBr-7-7!70!black, every mark/.append style={solid,fill=YlOrBr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-8}{%
 YlOrBr-8-1!70!black, every mark/.append style={solid,fill=YlOrBr-8-1},mark=*\\%
 YlOrBr-8-2!70!black, every mark/.append style={solid,fill=YlOrBr-8-2},mark=square*\\%
 YlOrBr-8-3!70!black, every mark/.append style={solid,fill=YlOrBr-8-3},mark=triangle*\\%
 YlOrBr-8-4!70!black, every mark/.append style={solid,fill=YlOrBr-8-4},mark=diamond*\\%
 YlOrBr-8-5!70!black, every mark/.append style={solid,fill=YlOrBr-8-5},mark=pentagon*\\%
 YlOrBr-8-6!70!black, every mark/.append style={solid,fill=YlOrBr-8-6},mark=x\\%
 YlOrBr-8-7!70!black, every mark/.append style={solid,fill=YlOrBr-8-7},mark=+\\%
 YlOrBr-8-8!70!black, every mark/.append style={solid,fill=YlOrBr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-9}{%
 YlOrBr-9-1!70!black, every mark/.append style={solid,fill=YlOrBr-9-1},mark=*\\%
 YlOrBr-9-2!70!black, every mark/.append style={solid,fill=YlOrBr-9-2},mark=square*\\%
 YlOrBr-9-3!70!black, every mark/.append style={solid,fill=YlOrBr-9-3},mark=triangle*\\%
 YlOrBr-9-4!70!black, every mark/.append style={solid,fill=YlOrBr-9-4},mark=diamond*\\%
 YlOrBr-9-5!70!black, every mark/.append style={solid,fill=YlOrBr-9-5},mark=pentagon*\\%
 YlOrBr-9-6!70!black, every mark/.append style={solid,fill=YlOrBr-9-6},mark=x\\%
 YlOrBr-9-7!70!black, every mark/.append style={solid,fill=YlOrBr-9-7},mark=+\\%
 YlOrBr-9-8!70!black, every mark/.append style={solid,fill=YlOrBr-9-8},mark=star\\%
 YlOrBr-9-9!70!black, every mark/.append style={solid,fill=YlOrBr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-3}{%
 Purples-3-1!70!black, every mark/.append style={solid,fill=Purples-3-1},mark=*\\%
 Purples-3-2!70!black, every mark/.append style={solid,fill=Purples-3-2},mark=square*\\%
 Purples-3-3!70!black, every mark/.append style={solid,fill=Purples-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-4}{%
 Purples-4-1!70!black, every mark/.append style={solid,fill=Purples-4-1},mark=*\\%
 Purples-4-2!70!black, every mark/.append style={solid,fill=Purples-4-2},mark=square*\\%
 Purples-4-3!70!black, every mark/.append style={solid,fill=Purples-4-3},mark=triangle*\\%
 Purples-4-4!70!black, every mark/.append style={solid,fill=Purples-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-5}{%
 Purples-5-1!70!black, every mark/.append style={solid,fill=Purples-5-1},mark=*\\%
 Purples-5-2!70!black, every mark/.append style={solid,fill=Purples-5-2},mark=square*\\%
 Purples-5-3!70!black, every mark/.append style={solid,fill=Purples-5-3},mark=triangle*\\%
 Purples-5-4!70!black, every mark/.append style={solid,fill=Purples-5-4},mark=diamond*\\%
 Purples-5-5!70!black, every mark/.append style={solid,fill=Purples-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-6}{%
 Purples-6-1!70!black, every mark/.append style={solid,fill=Purples-6-1},mark=*\\%
 Purples-6-2!70!black, every mark/.append style={solid,fill=Purples-6-2},mark=square*\\%
 Purples-6-3!70!black, every mark/.append style={solid,fill=Purples-6-3},mark=triangle*\\%
 Purples-6-4!70!black, every mark/.append style={solid,fill=Purples-6-4},mark=diamond*\\%
 Purples-6-5!70!black, every mark/.append style={solid,fill=Purples-6-5},mark=pentagon*\\%
 Purples-6-6!70!black, every mark/.append style={solid,fill=Purples-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-7}{%
 Purples-7-1!70!black, every mark/.append style={solid,fill=Purples-7-1},mark=*\\%
 Purples-7-2!70!black, every mark/.append style={solid,fill=Purples-7-2},mark=square*\\%
 Purples-7-3!70!black, every mark/.append style={solid,fill=Purples-7-3},mark=triangle*\\%
 Purples-7-4!70!black, every mark/.append style={solid,fill=Purples-7-4},mark=diamond*\\%
 Purples-7-5!70!black, every mark/.append style={solid,fill=Purples-7-5},mark=pentagon*\\%
 Purples-7-6!70!black, every mark/.append style={solid,fill=Purples-7-6},mark=x\\%
 Purples-7-7!70!black, every mark/.append style={solid,fill=Purples-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-8}{%
 Purples-8-1!70!black, every mark/.append style={solid,fill=Purples-8-1},mark=*\\%
 Purples-8-2!70!black, every mark/.append style={solid,fill=Purples-8-2},mark=square*\\%
 Purples-8-3!70!black, every mark/.append style={solid,fill=Purples-8-3},mark=triangle*\\%
 Purples-8-4!70!black, every mark/.append style={solid,fill=Purples-8-4},mark=diamond*\\%
 Purples-8-5!70!black, every mark/.append style={solid,fill=Purples-8-5},mark=pentagon*\\%
 Purples-8-6!70!black, every mark/.append style={solid,fill=Purples-8-6},mark=x\\%
 Purples-8-7!70!black, every mark/.append style={solid,fill=Purples-8-7},mark=+\\%
 Purples-8-8!70!black, every mark/.append style={solid,fill=Purples-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-9}{%
 Purples-9-1!70!black, every mark/.append style={solid,fill=Purples-9-1},mark=*\\%
 Purples-9-2!70!black, every mark/.append style={solid,fill=Purples-9-2},mark=square*\\%
 Purples-9-3!70!black, every mark/.append style={solid,fill=Purples-9-3},mark=triangle*\\%
 Purples-9-4!70!black, every mark/.append style={solid,fill=Purples-9-4},mark=diamond*\\%
 Purples-9-5!70!black, every mark/.append style={solid,fill=Purples-9-5},mark=pentagon*\\%
 Purples-9-6!70!black, every mark/.append style={solid,fill=Purples-9-6},mark=x\\%
 Purples-9-7!70!black, every mark/.append style={solid,fill=Purples-9-7},mark=+\\%
 Purples-9-8!70!black, every mark/.append style={solid,fill=Purples-9-8},mark=star\\%
 Purples-9-9!70!black, every mark/.append style={solid,fill=Purples-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-3}{%
 Blues-3-1!70!black, every mark/.append style={solid,fill=Blues-3-1},mark=*\\%
 Blues-3-2!70!black, every mark/.append style={solid,fill=Blues-3-2},mark=square*\\%
 Blues-3-3!70!black, every mark/.append style={solid,fill=Blues-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-4}{%
 Blues-4-1!70!black, every mark/.append style={solid,fill=Blues-4-1},mark=*\\%
 Blues-4-2!70!black, every mark/.append style={solid,fill=Blues-4-2},mark=square*\\%
 Blues-4-3!70!black, every mark/.append style={solid,fill=Blues-4-3},mark=triangle*\\%
 Blues-4-4!70!black, every mark/.append style={solid,fill=Blues-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-5}{%
 Blues-5-1!70!black, every mark/.append style={solid,fill=Blues-5-1},mark=*\\%
 Blues-5-2!70!black, every mark/.append style={solid,fill=Blues-5-2},mark=square*\\%
 Blues-5-3!70!black, every mark/.append style={solid,fill=Blues-5-3},mark=triangle*\\%
 Blues-5-4!70!black, every mark/.append style={solid,fill=Blues-5-4},mark=diamond*\\%
 Blues-5-5!70!black, every mark/.append style={solid,fill=Blues-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-6}{%
 Blues-6-1!70!black, every mark/.append style={solid,fill=Blues-6-1},mark=*\\%
 Blues-6-2!70!black, every mark/.append style={solid,fill=Blues-6-2},mark=square*\\%
 Blues-6-3!70!black, every mark/.append style={solid,fill=Blues-6-3},mark=triangle*\\%
 Blues-6-4!70!black, every mark/.append style={solid,fill=Blues-6-4},mark=diamond*\\%
 Blues-6-5!70!black, every mark/.append style={solid,fill=Blues-6-5},mark=pentagon*\\%
 Blues-6-6!70!black, every mark/.append style={solid,fill=Blues-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-7}{%
 Blues-7-1!70!black, every mark/.append style={solid,fill=Blues-7-1},mark=*\\%
 Blues-7-2!70!black, every mark/.append style={solid,fill=Blues-7-2},mark=square*\\%
 Blues-7-3!70!black, every mark/.append style={solid,fill=Blues-7-3},mark=triangle*\\%
 Blues-7-4!70!black, every mark/.append style={solid,fill=Blues-7-4},mark=diamond*\\%
 Blues-7-5!70!black, every mark/.append style={solid,fill=Blues-7-5},mark=pentagon*\\%
 Blues-7-6!70!black, every mark/.append style={solid,fill=Blues-7-6},mark=x\\%
 Blues-7-7!70!black, every mark/.append style={solid,fill=Blues-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-8}{%
 Blues-8-1!70!black, every mark/.append style={solid,fill=Blues-8-1},mark=*\\%
 Blues-8-2!70!black, every mark/.append style={solid,fill=Blues-8-2},mark=square*\\%
 Blues-8-3!70!black, every mark/.append style={solid,fill=Blues-8-3},mark=triangle*\\%
 Blues-8-4!70!black, every mark/.append style={solid,fill=Blues-8-4},mark=diamond*\\%
 Blues-8-5!70!black, every mark/.append style={solid,fill=Blues-8-5},mark=pentagon*\\%
 Blues-8-6!70!black, every mark/.append style={solid,fill=Blues-8-6},mark=x\\%
 Blues-8-7!70!black, every mark/.append style={solid,fill=Blues-8-7},mark=+\\%
 Blues-8-8!70!black, every mark/.append style={solid,fill=Blues-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-9}{%
 Blues-9-1!70!black, every mark/.append style={solid,fill=Blues-9-1},mark=*\\%
 Blues-9-2!70!black, every mark/.append style={solid,fill=Blues-9-2},mark=square*\\%
 Blues-9-3!70!black, every mark/.append style={solid,fill=Blues-9-3},mark=triangle*\\%
 Blues-9-4!70!black, every mark/.append style={solid,fill=Blues-9-4},mark=diamond*\\%
 Blues-9-5!70!black, every mark/.append style={solid,fill=Blues-9-5},mark=pentagon*\\%
 Blues-9-6!70!black, every mark/.append style={solid,fill=Blues-9-6},mark=x\\%
 Blues-9-7!70!black, every mark/.append style={solid,fill=Blues-9-7},mark=+\\%
 Blues-9-8!70!black, every mark/.append style={solid,fill=Blues-9-8},mark=star\\%
 Blues-9-9!70!black, every mark/.append style={solid,fill=Blues-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-3}{%
 Greens-3-1!70!black, every mark/.append style={solid,fill=Greens-3-1},mark=*\\%
 Greens-3-2!70!black, every mark/.append style={solid,fill=Greens-3-2},mark=square*\\%
 Greens-3-3!70!black, every mark/.append style={solid,fill=Greens-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-4}{%
 Greens-4-1!70!black, every mark/.append style={solid,fill=Greens-4-1},mark=*\\%
 Greens-4-2!70!black, every mark/.append style={solid,fill=Greens-4-2},mark=square*\\%
 Greens-4-3!70!black, every mark/.append style={solid,fill=Greens-4-3},mark=triangle*\\%
 Greens-4-4!70!black, every mark/.append style={solid,fill=Greens-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-5}{%
 Greens-5-1!70!black, every mark/.append style={solid,fill=Greens-5-1},mark=*\\%
 Greens-5-2!70!black, every mark/.append style={solid,fill=Greens-5-2},mark=square*\\%
 Greens-5-3!70!black, every mark/.append style={solid,fill=Greens-5-3},mark=triangle*\\%
 Greens-5-4!70!black, every mark/.append style={solid,fill=Greens-5-4},mark=diamond*\\%
 Greens-5-5!70!black, every mark/.append style={solid,fill=Greens-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-6}{%
 Greens-6-1!70!black, every mark/.append style={solid,fill=Greens-6-1},mark=*\\%
 Greens-6-2!70!black, every mark/.append style={solid,fill=Greens-6-2},mark=square*\\%
 Greens-6-3!70!black, every mark/.append style={solid,fill=Greens-6-3},mark=triangle*\\%
 Greens-6-4!70!black, every mark/.append style={solid,fill=Greens-6-4},mark=diamond*\\%
 Greens-6-5!70!black, every mark/.append style={solid,fill=Greens-6-5},mark=pentagon*\\%
 Greens-6-6!70!black, every mark/.append style={solid,fill=Greens-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-7}{%
 Greens-7-1!70!black, every mark/.append style={solid,fill=Greens-7-1},mark=*\\%
 Greens-7-2!70!black, every mark/.append style={solid,fill=Greens-7-2},mark=square*\\%
 Greens-7-3!70!black, every mark/.append style={solid,fill=Greens-7-3},mark=triangle*\\%
 Greens-7-4!70!black, every mark/.append style={solid,fill=Greens-7-4},mark=diamond*\\%
 Greens-7-5!70!black, every mark/.append style={solid,fill=Greens-7-5},mark=pentagon*\\%
 Greens-7-6!70!black, every mark/.append style={solid,fill=Greens-7-6},mark=x\\%
 Greens-7-7!70!black, every mark/.append style={solid,fill=Greens-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-8}{%
 Greens-8-1!70!black, every mark/.append style={solid,fill=Greens-8-1},mark=*\\%
 Greens-8-2!70!black, every mark/.append style={solid,fill=Greens-8-2},mark=square*\\%
 Greens-8-3!70!black, every mark/.append style={solid,fill=Greens-8-3},mark=triangle*\\%
 Greens-8-4!70!black, every mark/.append style={solid,fill=Greens-8-4},mark=diamond*\\%
 Greens-8-5!70!black, every mark/.append style={solid,fill=Greens-8-5},mark=pentagon*\\%
 Greens-8-6!70!black, every mark/.append style={solid,fill=Greens-8-6},mark=x\\%
 Greens-8-7!70!black, every mark/.append style={solid,fill=Greens-8-7},mark=+\\%
 Greens-8-8!70!black, every mark/.append style={solid,fill=Greens-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-9}{%
 Greens-9-1!70!black, every mark/.append style={solid,fill=Greens-9-1},mark=*\\%
 Greens-9-2!70!black, every mark/.append style={solid,fill=Greens-9-2},mark=square*\\%
 Greens-9-3!70!black, every mark/.append style={solid,fill=Greens-9-3},mark=triangle*\\%
 Greens-9-4!70!black, every mark/.append style={solid,fill=Greens-9-4},mark=diamond*\\%
 Greens-9-5!70!black, every mark/.append style={solid,fill=Greens-9-5},mark=pentagon*\\%
 Greens-9-6!70!black, every mark/.append style={solid,fill=Greens-9-6},mark=x\\%
 Greens-9-7!70!black, every mark/.append style={solid,fill=Greens-9-7},mark=+\\%
 Greens-9-8!70!black, every mark/.append style={solid,fill=Greens-9-8},mark=star\\%
 Greens-9-9!70!black, every mark/.append style={solid,fill=Greens-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-3}{%
 Oranges-3-1!70!black, every mark/.append style={solid,fill=Oranges-3-1},mark=*\\%
 Oranges-3-2!70!black, every mark/.append style={solid,fill=Oranges-3-2},mark=square*\\%
 Oranges-3-3!70!black, every mark/.append style={solid,fill=Oranges-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-4}{%
 Oranges-4-1!70!black, every mark/.append style={solid,fill=Oranges-4-1},mark=*\\%
 Oranges-4-2!70!black, every mark/.append style={solid,fill=Oranges-4-2},mark=square*\\%
 Oranges-4-3!70!black, every mark/.append style={solid,fill=Oranges-4-3},mark=triangle*\\%
 Oranges-4-4!70!black, every mark/.append style={solid,fill=Oranges-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-5}{%
 Oranges-5-1!70!black, every mark/.append style={solid,fill=Oranges-5-1},mark=*\\%
 Oranges-5-2!70!black, every mark/.append style={solid,fill=Oranges-5-2},mark=square*\\%
 Oranges-5-3!70!black, every mark/.append style={solid,fill=Oranges-5-3},mark=triangle*\\%
 Oranges-5-4!70!black, every mark/.append style={solid,fill=Oranges-5-4},mark=diamond*\\%
 Oranges-5-5!70!black, every mark/.append style={solid,fill=Oranges-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-6}{%
 Oranges-6-1!70!black, every mark/.append style={solid,fill=Oranges-6-1},mark=*\\%
 Oranges-6-2!70!black, every mark/.append style={solid,fill=Oranges-6-2},mark=square*\\%
 Oranges-6-3!70!black, every mark/.append style={solid,fill=Oranges-6-3},mark=triangle*\\%
 Oranges-6-4!70!black, every mark/.append style={solid,fill=Oranges-6-4},mark=diamond*\\%
 Oranges-6-5!70!black, every mark/.append style={solid,fill=Oranges-6-5},mark=pentagon*\\%
 Oranges-6-6!70!black, every mark/.append style={solid,fill=Oranges-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-7}{%
 Oranges-7-1!70!black, every mark/.append style={solid,fill=Oranges-7-1},mark=*\\%
 Oranges-7-2!70!black, every mark/.append style={solid,fill=Oranges-7-2},mark=square*\\%
 Oranges-7-3!70!black, every mark/.append style={solid,fill=Oranges-7-3},mark=triangle*\\%
 Oranges-7-4!70!black, every mark/.append style={solid,fill=Oranges-7-4},mark=diamond*\\%
 Oranges-7-5!70!black, every mark/.append style={solid,fill=Oranges-7-5},mark=pentagon*\\%
 Oranges-7-6!70!black, every mark/.append style={solid,fill=Oranges-7-6},mark=x\\%
 Oranges-7-7!70!black, every mark/.append style={solid,fill=Oranges-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-8}{%
 Oranges-8-1!70!black, every mark/.append style={solid,fill=Oranges-8-1},mark=*\\%
 Oranges-8-2!70!black, every mark/.append style={solid,fill=Oranges-8-2},mark=square*\\%
 Oranges-8-3!70!black, every mark/.append style={solid,fill=Oranges-8-3},mark=triangle*\\%
 Oranges-8-4!70!black, every mark/.append style={solid,fill=Oranges-8-4},mark=diamond*\\%
 Oranges-8-5!70!black, every mark/.append style={solid,fill=Oranges-8-5},mark=pentagon*\\%
 Oranges-8-6!70!black, every mark/.append style={solid,fill=Oranges-8-6},mark=x\\%
 Oranges-8-7!70!black, every mark/.append style={solid,fill=Oranges-8-7},mark=+\\%
 Oranges-8-8!70!black, every mark/.append style={solid,fill=Oranges-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-9}{%
 Oranges-9-1!70!black, every mark/.append style={solid,fill=Oranges-9-1},mark=*\\%
 Oranges-9-2!70!black, every mark/.append style={solid,fill=Oranges-9-2},mark=square*\\%
 Oranges-9-3!70!black, every mark/.append style={solid,fill=Oranges-9-3},mark=triangle*\\%
 Oranges-9-4!70!black, every mark/.append style={solid,fill=Oranges-9-4},mark=diamond*\\%
 Oranges-9-5!70!black, every mark/.append style={solid,fill=Oranges-9-5},mark=pentagon*\\%
 Oranges-9-6!70!black, every mark/.append style={solid,fill=Oranges-9-6},mark=x\\%
 Oranges-9-7!70!black, every mark/.append style={solid,fill=Oranges-9-7},mark=+\\%
 Oranges-9-8!70!black, every mark/.append style={solid,fill=Oranges-9-8},mark=star\\%
 Oranges-9-9!70!black, every mark/.append style={solid,fill=Oranges-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-3}{%
 Reds-3-1!70!black, every mark/.append style={solid,fill=Reds-3-1},mark=*\\%
 Reds-3-2!70!black, every mark/.append style={solid,fill=Reds-3-2},mark=square*\\%
 Reds-3-3!70!black, every mark/.append style={solid,fill=Reds-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-4}{%
 Reds-4-1!70!black, every mark/.append style={solid,fill=Reds-4-1},mark=*\\%
 Reds-4-2!70!black, every mark/.append style={solid,fill=Reds-4-2},mark=square*\\%
 Reds-4-3!70!black, every mark/.append style={solid,fill=Reds-4-3},mark=triangle*\\%
 Reds-4-4!70!black, every mark/.append style={solid,fill=Reds-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-5}{%
 Reds-5-1!70!black, every mark/.append style={solid,fill=Reds-5-1},mark=*\\%
 Reds-5-2!70!black, every mark/.append style={solid,fill=Reds-5-2},mark=square*\\%
 Reds-5-3!70!black, every mark/.append style={solid,fill=Reds-5-3},mark=triangle*\\%
 Reds-5-4!70!black, every mark/.append style={solid,fill=Reds-5-4},mark=diamond*\\%
 Reds-5-5!70!black, every mark/.append style={solid,fill=Reds-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-6}{%
 Reds-6-1!70!black, every mark/.append style={solid,fill=Reds-6-1},mark=*\\%
 Reds-6-2!70!black, every mark/.append style={solid,fill=Reds-6-2},mark=square*\\%
 Reds-6-3!70!black, every mark/.append style={solid,fill=Reds-6-3},mark=triangle*\\%
 Reds-6-4!70!black, every mark/.append style={solid,fill=Reds-6-4},mark=diamond*\\%
 Reds-6-5!70!black, every mark/.append style={solid,fill=Reds-6-5},mark=pentagon*\\%
 Reds-6-6!70!black, every mark/.append style={solid,fill=Reds-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-7}{%
 Reds-7-1!70!black, every mark/.append style={solid,fill=Reds-7-1},mark=*\\%
 Reds-7-2!70!black, every mark/.append style={solid,fill=Reds-7-2},mark=square*\\%
 Reds-7-3!70!black, every mark/.append style={solid,fill=Reds-7-3},mark=triangle*\\%
 Reds-7-4!70!black, every mark/.append style={solid,fill=Reds-7-4},mark=diamond*\\%
 Reds-7-5!70!black, every mark/.append style={solid,fill=Reds-7-5},mark=pentagon*\\%
 Reds-7-6!70!black, every mark/.append style={solid,fill=Reds-7-6},mark=x\\%
 Reds-7-7!70!black, every mark/.append style={solid,fill=Reds-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-8}{%
 Reds-8-1!70!black, every mark/.append style={solid,fill=Reds-8-1},mark=*\\%
 Reds-8-2!70!black, every mark/.append style={solid,fill=Reds-8-2},mark=square*\\%
 Reds-8-3!70!black, every mark/.append style={solid,fill=Reds-8-3},mark=triangle*\\%
 Reds-8-4!70!black, every mark/.append style={solid,fill=Reds-8-4},mark=diamond*\\%
 Reds-8-5!70!black, every mark/.append style={solid,fill=Reds-8-5},mark=pentagon*\\%
 Reds-8-6!70!black, every mark/.append style={solid,fill=Reds-8-6},mark=x\\%
 Reds-8-7!70!black, every mark/.append style={solid,fill=Reds-8-7},mark=+\\%
 Reds-8-8!70!black, every mark/.append style={solid,fill=Reds-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-9}{%
 Reds-9-1!70!black, every mark/.append style={solid,fill=Reds-9-1},mark=*\\%
 Reds-9-2!70!black, every mark/.append style={solid,fill=Reds-9-2},mark=square*\\%
 Reds-9-3!70!black, every mark/.append style={solid,fill=Reds-9-3},mark=triangle*\\%
 Reds-9-4!70!black, every mark/.append style={solid,fill=Reds-9-4},mark=diamond*\\%
 Reds-9-5!70!black, every mark/.append style={solid,fill=Reds-9-5},mark=pentagon*\\%
 Reds-9-6!70!black, every mark/.append style={solid,fill=Reds-9-6},mark=x\\%
 Reds-9-7!70!black, every mark/.append style={solid,fill=Reds-9-7},mark=+\\%
 Reds-9-8!70!black, every mark/.append style={solid,fill=Reds-9-8},mark=star\\%
 Reds-9-9!70!black, every mark/.append style={solid,fill=Reds-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-3}{%
 Greys-3-1!70!black, every mark/.append style={solid,fill=Greys-3-1},mark=*\\%
 Greys-3-2!70!black, every mark/.append style={solid,fill=Greys-3-2},mark=square*\\%
 Greys-3-3!70!black, every mark/.append style={solid,fill=Greys-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-4}{%
 Greys-4-1!70!black, every mark/.append style={solid,fill=Greys-4-1},mark=*\\%
 Greys-4-2!70!black, every mark/.append style={solid,fill=Greys-4-2},mark=square*\\%
 Greys-4-3!70!black, every mark/.append style={solid,fill=Greys-4-3},mark=triangle*\\%
 Greys-4-4!70!black, every mark/.append style={solid,fill=Greys-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-5}{%
 Greys-5-1!70!black, every mark/.append style={solid,fill=Greys-5-1},mark=*\\%
 Greys-5-2!70!black, every mark/.append style={solid,fill=Greys-5-2},mark=square*\\%
 Greys-5-3!70!black, every mark/.append style={solid,fill=Greys-5-3},mark=triangle*\\%
 Greys-5-4!70!black, every mark/.append style={solid,fill=Greys-5-4},mark=diamond*\\%
 Greys-5-5!70!black, every mark/.append style={solid,fill=Greys-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-6}{%
 Greys-6-1!70!black, every mark/.append style={solid,fill=Greys-6-1},mark=*\\%
 Greys-6-2!70!black, every mark/.append style={solid,fill=Greys-6-2},mark=square*\\%
 Greys-6-3!70!black, every mark/.append style={solid,fill=Greys-6-3},mark=triangle*\\%
 Greys-6-4!70!black, every mark/.append style={solid,fill=Greys-6-4},mark=diamond*\\%
 Greys-6-5!70!black, every mark/.append style={solid,fill=Greys-6-5},mark=pentagon*\\%
 Greys-6-6!70!black, every mark/.append style={solid,fill=Greys-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-7}{%
 Greys-7-1!70!black, every mark/.append style={solid,fill=Greys-7-1},mark=*\\%
 Greys-7-2!70!black, every mark/.append style={solid,fill=Greys-7-2},mark=square*\\%
 Greys-7-3!70!black, every mark/.append style={solid,fill=Greys-7-3},mark=triangle*\\%
 Greys-7-4!70!black, every mark/.append style={solid,fill=Greys-7-4},mark=diamond*\\%
 Greys-7-5!70!black, every mark/.append style={solid,fill=Greys-7-5},mark=pentagon*\\%
 Greys-7-6!70!black, every mark/.append style={solid,fill=Greys-7-6},mark=x\\%
 Greys-7-7!70!black, every mark/.append style={solid,fill=Greys-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-8}{%
 Greys-8-1!70!black, every mark/.append style={solid,fill=Greys-8-1},mark=*\\%
 Greys-8-2!70!black, every mark/.append style={solid,fill=Greys-8-2},mark=square*\\%
 Greys-8-3!70!black, every mark/.append style={solid,fill=Greys-8-3},mark=triangle*\\%
 Greys-8-4!70!black, every mark/.append style={solid,fill=Greys-8-4},mark=diamond*\\%
 Greys-8-5!70!black, every mark/.append style={solid,fill=Greys-8-5},mark=pentagon*\\%
 Greys-8-6!70!black, every mark/.append style={solid,fill=Greys-8-6},mark=x\\%
 Greys-8-7!70!black, every mark/.append style={solid,fill=Greys-8-7},mark=+\\%
 Greys-8-8!70!black, every mark/.append style={solid,fill=Greys-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-9}{%
 Greys-9-1!70!black, every mark/.append style={solid,fill=Greys-9-1},mark=*\\%
 Greys-9-2!70!black, every mark/.append style={solid,fill=Greys-9-2},mark=square*\\%
 Greys-9-3!70!black, every mark/.append style={solid,fill=Greys-9-3},mark=triangle*\\%
 Greys-9-4!70!black, every mark/.append style={solid,fill=Greys-9-4},mark=diamond*\\%
 Greys-9-5!70!black, every mark/.append style={solid,fill=Greys-9-5},mark=pentagon*\\%
 Greys-9-6!70!black, every mark/.append style={solid,fill=Greys-9-6},mark=x\\%
 Greys-9-7!70!black, every mark/.append style={solid,fill=Greys-9-7},mark=+\\%
 Greys-9-8!70!black, every mark/.append style={solid,fill=Greys-9-8},mark=star\\%
 Greys-9-9!70!black, every mark/.append style={solid,fill=Greys-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-3}{%
 PuOr-3-1!70!black, every mark/.append style={solid,fill=PuOr-3-1},mark=*\\%
 PuOr-3-2!70!black, every mark/.append style={solid,fill=PuOr-3-2},mark=square*\\%
 PuOr-3-3!70!black, every mark/.append style={solid,fill=PuOr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-4}{%
 PuOr-4-1!70!black, every mark/.append style={solid,fill=PuOr-4-1},mark=*\\%
 PuOr-4-2!70!black, every mark/.append style={solid,fill=PuOr-4-2},mark=square*\\%
 PuOr-4-3!70!black, every mark/.append style={solid,fill=PuOr-4-3},mark=triangle*\\%
 PuOr-4-4!70!black, every mark/.append style={solid,fill=PuOr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-5}{%
 PuOr-5-1!70!black, every mark/.append style={solid,fill=PuOr-5-1},mark=*\\%
 PuOr-5-2!70!black, every mark/.append style={solid,fill=PuOr-5-2},mark=square*\\%
 PuOr-5-3!70!black, every mark/.append style={solid,fill=PuOr-5-3},mark=triangle*\\%
 PuOr-5-4!70!black, every mark/.append style={solid,fill=PuOr-5-4},mark=diamond*\\%
 PuOr-5-5!70!black, every mark/.append style={solid,fill=PuOr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-6}{%
 PuOr-6-1!70!black, every mark/.append style={solid,fill=PuOr-6-1},mark=*\\%
 PuOr-6-2!70!black, every mark/.append style={solid,fill=PuOr-6-2},mark=square*\\%
 PuOr-6-3!70!black, every mark/.append style={solid,fill=PuOr-6-3},mark=triangle*\\%
 PuOr-6-4!70!black, every mark/.append style={solid,fill=PuOr-6-4},mark=diamond*\\%
 PuOr-6-5!70!black, every mark/.append style={solid,fill=PuOr-6-5},mark=pentagon*\\%
 PuOr-6-6!70!black, every mark/.append style={solid,fill=PuOr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-7}{%
 PuOr-7-1!70!black, every mark/.append style={solid,fill=PuOr-7-1},mark=*\\%
 PuOr-7-2!70!black, every mark/.append style={solid,fill=PuOr-7-2},mark=square*\\%
 PuOr-7-3!70!black, every mark/.append style={solid,fill=PuOr-7-3},mark=triangle*\\%
 PuOr-7-4!70!black, every mark/.append style={solid,fill=PuOr-7-4},mark=diamond*\\%
 PuOr-7-5!70!black, every mark/.append style={solid,fill=PuOr-7-5},mark=pentagon*\\%
 PuOr-7-6!70!black, every mark/.append style={solid,fill=PuOr-7-6},mark=x\\%
 PuOr-7-7!70!black, every mark/.append style={solid,fill=PuOr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-8}{%
 PuOr-8-1!70!black, every mark/.append style={solid,fill=PuOr-8-1},mark=*\\%
 PuOr-8-2!70!black, every mark/.append style={solid,fill=PuOr-8-2},mark=square*\\%
 PuOr-8-3!70!black, every mark/.append style={solid,fill=PuOr-8-3},mark=triangle*\\%
 PuOr-8-4!70!black, every mark/.append style={solid,fill=PuOr-8-4},mark=diamond*\\%
 PuOr-8-5!70!black, every mark/.append style={solid,fill=PuOr-8-5},mark=pentagon*\\%
 PuOr-8-6!70!black, every mark/.append style={solid,fill=PuOr-8-6},mark=x\\%
 PuOr-8-7!70!black, every mark/.append style={solid,fill=PuOr-8-7},mark=+\\%
 PuOr-8-8!70!black, every mark/.append style={solid,fill=PuOr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-9}{%
 PuOr-9-1!70!black, every mark/.append style={solid,fill=PuOr-9-1},mark=*\\%
 PuOr-9-2!70!black, every mark/.append style={solid,fill=PuOr-9-2},mark=square*\\%
 PuOr-9-3!70!black, every mark/.append style={solid,fill=PuOr-9-3},mark=triangle*\\%
 PuOr-9-4!70!black, every mark/.append style={solid,fill=PuOr-9-4},mark=diamond*\\%
 PuOr-9-5!70!black, every mark/.append style={solid,fill=PuOr-9-5},mark=pentagon*\\%
 PuOr-9-6!70!black, every mark/.append style={solid,fill=PuOr-9-6},mark=x\\%
 PuOr-9-7!70!black, every mark/.append style={solid,fill=PuOr-9-7},mark=+\\%
 PuOr-9-8!70!black, every mark/.append style={solid,fill=PuOr-9-8},mark=star\\%
 PuOr-9-9!70!black, every mark/.append style={solid,fill=PuOr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-10}{%
 PuOr-10-1!70!black, every mark/.append style={solid,fill=PuOr-10-1},mark=*\\%
 PuOr-10-2!70!black, every mark/.append style={solid,fill=PuOr-10-2},mark=square*\\%
 PuOr-10-3!70!black, every mark/.append style={solid,fill=PuOr-10-3},mark=triangle*\\%
 PuOr-10-4!70!black, every mark/.append style={solid,fill=PuOr-10-4},mark=diamond*\\%
 PuOr-10-5!70!black, every mark/.append style={solid,fill=PuOr-10-5},mark=pentagon*\\%
 PuOr-10-6!70!black, every mark/.append style={solid,fill=PuOr-10-6},mark=x\\%
 PuOr-10-7!70!black, every mark/.append style={solid,fill=PuOr-10-7},mark=+\\%
 PuOr-10-8!70!black, every mark/.append style={solid,fill=PuOr-10-8},mark=star\\%
 PuOr-10-9!70!black, every mark/.append style={solid,fill=PuOr-10-9},mark=oplus*\\%
 PuOr-10-10!70!black, every mark/.append style={solid,fill=PuOr-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-11}{%
 PuOr-11-1!70!black, every mark/.append style={solid,fill=PuOr-11-1},mark=*\\%
 PuOr-11-2!70!black, every mark/.append style={solid,fill=PuOr-11-2},mark=square*\\%
 PuOr-11-3!70!black, every mark/.append style={solid,fill=PuOr-11-3},mark=triangle*\\%
 PuOr-11-4!70!black, every mark/.append style={solid,fill=PuOr-11-4},mark=diamond*\\%
 PuOr-11-5!70!black, every mark/.append style={solid,fill=PuOr-11-5},mark=pentagon*\\%
 PuOr-11-6!70!black, every mark/.append style={solid,fill=PuOr-11-6},mark=x\\%
 PuOr-11-7!70!black, every mark/.append style={solid,fill=PuOr-11-7},mark=+\\%
 PuOr-11-8!70!black, every mark/.append style={solid,fill=PuOr-11-8},mark=star\\%
 PuOr-11-9!70!black, every mark/.append style={solid,fill=PuOr-11-9},mark=oplus*\\%
 PuOr-11-10!70!black, every mark/.append style={solid,fill=PuOr-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-3}{%
 BrBG-3-1!70!black, every mark/.append style={solid,fill=BrBG-3-1},mark=*\\%
 BrBG-3-2!70!black, every mark/.append style={solid,fill=BrBG-3-2},mark=square*\\%
 BrBG-3-3!70!black, every mark/.append style={solid,fill=BrBG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-4}{%
 BrBG-4-1!70!black, every mark/.append style={solid,fill=BrBG-4-1},mark=*\\%
 BrBG-4-2!70!black, every mark/.append style={solid,fill=BrBG-4-2},mark=square*\\%
 BrBG-4-3!70!black, every mark/.append style={solid,fill=BrBG-4-3},mark=triangle*\\%
 BrBG-4-4!70!black, every mark/.append style={solid,fill=BrBG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-5}{%
 BrBG-5-1!70!black, every mark/.append style={solid,fill=BrBG-5-1},mark=*\\%
 BrBG-5-2!70!black, every mark/.append style={solid,fill=BrBG-5-2},mark=square*\\%
 BrBG-5-3!70!black, every mark/.append style={solid,fill=BrBG-5-3},mark=triangle*\\%
 BrBG-5-4!70!black, every mark/.append style={solid,fill=BrBG-5-4},mark=diamond*\\%
 BrBG-5-5!70!black, every mark/.append style={solid,fill=BrBG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-6}{%
 BrBG-6-1!70!black, every mark/.append style={solid,fill=BrBG-6-1},mark=*\\%
 BrBG-6-2!70!black, every mark/.append style={solid,fill=BrBG-6-2},mark=square*\\%
 BrBG-6-3!70!black, every mark/.append style={solid,fill=BrBG-6-3},mark=triangle*\\%
 BrBG-6-4!70!black, every mark/.append style={solid,fill=BrBG-6-4},mark=diamond*\\%
 BrBG-6-5!70!black, every mark/.append style={solid,fill=BrBG-6-5},mark=pentagon*\\%
 BrBG-6-6!70!black, every mark/.append style={solid,fill=BrBG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-7}{%
 BrBG-7-1!70!black, every mark/.append style={solid,fill=BrBG-7-1},mark=*\\%
 BrBG-7-2!70!black, every mark/.append style={solid,fill=BrBG-7-2},mark=square*\\%
 BrBG-7-3!70!black, every mark/.append style={solid,fill=BrBG-7-3},mark=triangle*\\%
 BrBG-7-4!70!black, every mark/.append style={solid,fill=BrBG-7-4},mark=diamond*\\%
 BrBG-7-5!70!black, every mark/.append style={solid,fill=BrBG-7-5},mark=pentagon*\\%
 BrBG-7-6!70!black, every mark/.append style={solid,fill=BrBG-7-6},mark=x\\%
 BrBG-7-7!70!black, every mark/.append style={solid,fill=BrBG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-8}{%
 BrBG-8-1!70!black, every mark/.append style={solid,fill=BrBG-8-1},mark=*\\%
 BrBG-8-2!70!black, every mark/.append style={solid,fill=BrBG-8-2},mark=square*\\%
 BrBG-8-3!70!black, every mark/.append style={solid,fill=BrBG-8-3},mark=triangle*\\%
 BrBG-8-4!70!black, every mark/.append style={solid,fill=BrBG-8-4},mark=diamond*\\%
 BrBG-8-5!70!black, every mark/.append style={solid,fill=BrBG-8-5},mark=pentagon*\\%
 BrBG-8-6!70!black, every mark/.append style={solid,fill=BrBG-8-6},mark=x\\%
 BrBG-8-7!70!black, every mark/.append style={solid,fill=BrBG-8-7},mark=+\\%
 BrBG-8-8!70!black, every mark/.append style={solid,fill=BrBG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-9}{%
 BrBG-9-1!70!black, every mark/.append style={solid,fill=BrBG-9-1},mark=*\\%
 BrBG-9-2!70!black, every mark/.append style={solid,fill=BrBG-9-2},mark=square*\\%
 BrBG-9-3!70!black, every mark/.append style={solid,fill=BrBG-9-3},mark=triangle*\\%
 BrBG-9-4!70!black, every mark/.append style={solid,fill=BrBG-9-4},mark=diamond*\\%
 BrBG-9-5!70!black, every mark/.append style={solid,fill=BrBG-9-5},mark=pentagon*\\%
 BrBG-9-6!70!black, every mark/.append style={solid,fill=BrBG-9-6},mark=x\\%
 BrBG-9-7!70!black, every mark/.append style={solid,fill=BrBG-9-7},mark=+\\%
 BrBG-9-8!70!black, every mark/.append style={solid,fill=BrBG-9-8},mark=star\\%
 BrBG-9-9!70!black, every mark/.append style={solid,fill=BrBG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-10}{%
 BrBG-10-1!70!black, every mark/.append style={solid,fill=BrBG-10-1},mark=*\\%
 BrBG-10-2!70!black, every mark/.append style={solid,fill=BrBG-10-2},mark=square*\\%
 BrBG-10-3!70!black, every mark/.append style={solid,fill=BrBG-10-3},mark=triangle*\\%
 BrBG-10-4!70!black, every mark/.append style={solid,fill=BrBG-10-4},mark=diamond*\\%
 BrBG-10-5!70!black, every mark/.append style={solid,fill=BrBG-10-5},mark=pentagon*\\%
 BrBG-10-6!70!black, every mark/.append style={solid,fill=BrBG-10-6},mark=x\\%
 BrBG-10-7!70!black, every mark/.append style={solid,fill=BrBG-10-7},mark=+\\%
 BrBG-10-8!70!black, every mark/.append style={solid,fill=BrBG-10-8},mark=star\\%
 BrBG-10-9!70!black, every mark/.append style={solid,fill=BrBG-10-9},mark=oplus*\\%
 BrBG-10-10!70!black, every mark/.append style={solid,fill=BrBG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-11}{%
 BrBG-11-1!70!black, every mark/.append style={solid,fill=BrBG-11-1},mark=*\\%
 BrBG-11-2!70!black, every mark/.append style={solid,fill=BrBG-11-2},mark=square*\\%
 BrBG-11-3!70!black, every mark/.append style={solid,fill=BrBG-11-3},mark=triangle*\\%
 BrBG-11-4!70!black, every mark/.append style={solid,fill=BrBG-11-4},mark=diamond*\\%
 BrBG-11-5!70!black, every mark/.append style={solid,fill=BrBG-11-5},mark=pentagon*\\%
 BrBG-11-6!70!black, every mark/.append style={solid,fill=BrBG-11-6},mark=x\\%
 BrBG-11-7!70!black, every mark/.append style={solid,fill=BrBG-11-7},mark=+\\%
 BrBG-11-8!70!black, every mark/.append style={solid,fill=BrBG-11-8},mark=star\\%
 BrBG-11-9!70!black, every mark/.append style={solid,fill=BrBG-11-9},mark=oplus*\\%
 BrBG-11-10!70!black, every mark/.append style={solid,fill=BrBG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-3}{%
 PRGn-3-1!70!black, every mark/.append style={solid,fill=PRGn-3-1},mark=*\\%
 PRGn-3-2!70!black, every mark/.append style={solid,fill=PRGn-3-2},mark=square*\\%
 PRGn-3-3!70!black, every mark/.append style={solid,fill=PRGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-4}{%
 PRGn-4-1!70!black, every mark/.append style={solid,fill=PRGn-4-1},mark=*\\%
 PRGn-4-2!70!black, every mark/.append style={solid,fill=PRGn-4-2},mark=square*\\%
 PRGn-4-3!70!black, every mark/.append style={solid,fill=PRGn-4-3},mark=triangle*\\%
 PRGn-4-4!70!black, every mark/.append style={solid,fill=PRGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-5}{%
 PRGn-5-1!70!black, every mark/.append style={solid,fill=PRGn-5-1},mark=*\\%
 PRGn-5-2!70!black, every mark/.append style={solid,fill=PRGn-5-2},mark=square*\\%
 PRGn-5-3!70!black, every mark/.append style={solid,fill=PRGn-5-3},mark=triangle*\\%
 PRGn-5-4!70!black, every mark/.append style={solid,fill=PRGn-5-4},mark=diamond*\\%
 PRGn-5-5!70!black, every mark/.append style={solid,fill=PRGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-6}{%
 PRGn-6-1!70!black, every mark/.append style={solid,fill=PRGn-6-1},mark=*\\%
 PRGn-6-2!70!black, every mark/.append style={solid,fill=PRGn-6-2},mark=square*\\%
 PRGn-6-3!70!black, every mark/.append style={solid,fill=PRGn-6-3},mark=triangle*\\%
 PRGn-6-4!70!black, every mark/.append style={solid,fill=PRGn-6-4},mark=diamond*\\%
 PRGn-6-5!70!black, every mark/.append style={solid,fill=PRGn-6-5},mark=pentagon*\\%
 PRGn-6-6!70!black, every mark/.append style={solid,fill=PRGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-7}{%
 PRGn-7-1!70!black, every mark/.append style={solid,fill=PRGn-7-1},mark=*\\%
 PRGn-7-2!70!black, every mark/.append style={solid,fill=PRGn-7-2},mark=square*\\%
 PRGn-7-3!70!black, every mark/.append style={solid,fill=PRGn-7-3},mark=triangle*\\%
 PRGn-7-4!70!black, every mark/.append style={solid,fill=PRGn-7-4},mark=diamond*\\%
 PRGn-7-5!70!black, every mark/.append style={solid,fill=PRGn-7-5},mark=pentagon*\\%
 PRGn-7-6!70!black, every mark/.append style={solid,fill=PRGn-7-6},mark=x\\%
 PRGn-7-7!70!black, every mark/.append style={solid,fill=PRGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-8}{%
 PRGn-8-1!70!black, every mark/.append style={solid,fill=PRGn-8-1},mark=*\\%
 PRGn-8-2!70!black, every mark/.append style={solid,fill=PRGn-8-2},mark=square*\\%
 PRGn-8-3!70!black, every mark/.append style={solid,fill=PRGn-8-3},mark=triangle*\\%
 PRGn-8-4!70!black, every mark/.append style={solid,fill=PRGn-8-4},mark=diamond*\\%
 PRGn-8-5!70!black, every mark/.append style={solid,fill=PRGn-8-5},mark=pentagon*\\%
 PRGn-8-6!70!black, every mark/.append style={solid,fill=PRGn-8-6},mark=x\\%
 PRGn-8-7!70!black, every mark/.append style={solid,fill=PRGn-8-7},mark=+\\%
 PRGn-8-8!70!black, every mark/.append style={solid,fill=PRGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-9}{%
 PRGn-9-1!70!black, every mark/.append style={solid,fill=PRGn-9-1},mark=*\\%
 PRGn-9-2!70!black, every mark/.append style={solid,fill=PRGn-9-2},mark=square*\\%
 PRGn-9-3!70!black, every mark/.append style={solid,fill=PRGn-9-3},mark=triangle*\\%
 PRGn-9-4!70!black, every mark/.append style={solid,fill=PRGn-9-4},mark=diamond*\\%
 PRGn-9-5!70!black, every mark/.append style={solid,fill=PRGn-9-5},mark=pentagon*\\%
 PRGn-9-6!70!black, every mark/.append style={solid,fill=PRGn-9-6},mark=x\\%
 PRGn-9-7!70!black, every mark/.append style={solid,fill=PRGn-9-7},mark=+\\%
 PRGn-9-8!70!black, every mark/.append style={solid,fill=PRGn-9-8},mark=star\\%
 PRGn-9-9!70!black, every mark/.append style={solid,fill=PRGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-10}{%
 PRGn-10-1!70!black, every mark/.append style={solid,fill=PRGn-10-1},mark=*\\%
 PRGn-10-2!70!black, every mark/.append style={solid,fill=PRGn-10-2},mark=square*\\%
 PRGn-10-3!70!black, every mark/.append style={solid,fill=PRGn-10-3},mark=triangle*\\%
 PRGn-10-4!70!black, every mark/.append style={solid,fill=PRGn-10-4},mark=diamond*\\%
 PRGn-10-5!70!black, every mark/.append style={solid,fill=PRGn-10-5},mark=pentagon*\\%
 PRGn-10-6!70!black, every mark/.append style={solid,fill=PRGn-10-6},mark=x\\%
 PRGn-10-7!70!black, every mark/.append style={solid,fill=PRGn-10-7},mark=+\\%
 PRGn-10-8!70!black, every mark/.append style={solid,fill=PRGn-10-8},mark=star\\%
 PRGn-10-9!70!black, every mark/.append style={solid,fill=PRGn-10-9},mark=oplus*\\%
 PRGn-10-10!70!black, every mark/.append style={solid,fill=PRGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-11}{%
 PRGn-11-1!70!black, every mark/.append style={solid,fill=PRGn-11-1},mark=*\\%
 PRGn-11-2!70!black, every mark/.append style={solid,fill=PRGn-11-2},mark=square*\\%
 PRGn-11-3!70!black, every mark/.append style={solid,fill=PRGn-11-3},mark=triangle*\\%
 PRGn-11-4!70!black, every mark/.append style={solid,fill=PRGn-11-4},mark=diamond*\\%
 PRGn-11-5!70!black, every mark/.append style={solid,fill=PRGn-11-5},mark=pentagon*\\%
 PRGn-11-6!70!black, every mark/.append style={solid,fill=PRGn-11-6},mark=x\\%
 PRGn-11-7!70!black, every mark/.append style={solid,fill=PRGn-11-7},mark=+\\%
 PRGn-11-8!70!black, every mark/.append style={solid,fill=PRGn-11-8},mark=star\\%
 PRGn-11-9!70!black, every mark/.append style={solid,fill=PRGn-11-9},mark=oplus*\\%
 PRGn-11-10!70!black, every mark/.append style={solid,fill=PRGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-3}{%
 PiYG-3-1!70!black, every mark/.append style={solid,fill=PiYG-3-1},mark=*\\%
 PiYG-3-2!70!black, every mark/.append style={solid,fill=PiYG-3-2},mark=square*\\%
 PiYG-3-3!70!black, every mark/.append style={solid,fill=PiYG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-4}{%
 PiYG-4-1!70!black, every mark/.append style={solid,fill=PiYG-4-1},mark=*\\%
 PiYG-4-2!70!black, every mark/.append style={solid,fill=PiYG-4-2},mark=square*\\%
 PiYG-4-3!70!black, every mark/.append style={solid,fill=PiYG-4-3},mark=triangle*\\%
 PiYG-4-4!70!black, every mark/.append style={solid,fill=PiYG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-5}{%
 PiYG-5-1!70!black, every mark/.append style={solid,fill=PiYG-5-1},mark=*\\%
 PiYG-5-2!70!black, every mark/.append style={solid,fill=PiYG-5-2},mark=square*\\%
 PiYG-5-3!70!black, every mark/.append style={solid,fill=PiYG-5-3},mark=triangle*\\%
 PiYG-5-4!70!black, every mark/.append style={solid,fill=PiYG-5-4},mark=diamond*\\%
 PiYG-5-5!70!black, every mark/.append style={solid,fill=PiYG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-6}{%
 PiYG-6-1!70!black, every mark/.append style={solid,fill=PiYG-6-1},mark=*\\%
 PiYG-6-2!70!black, every mark/.append style={solid,fill=PiYG-6-2},mark=square*\\%
 PiYG-6-3!70!black, every mark/.append style={solid,fill=PiYG-6-3},mark=triangle*\\%
 PiYG-6-4!70!black, every mark/.append style={solid,fill=PiYG-6-4},mark=diamond*\\%
 PiYG-6-5!70!black, every mark/.append style={solid,fill=PiYG-6-5},mark=pentagon*\\%
 PiYG-6-6!70!black, every mark/.append style={solid,fill=PiYG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-7}{%
 PiYG-7-1!70!black, every mark/.append style={solid,fill=PiYG-7-1},mark=*\\%
 PiYG-7-2!70!black, every mark/.append style={solid,fill=PiYG-7-2},mark=square*\\%
 PiYG-7-3!70!black, every mark/.append style={solid,fill=PiYG-7-3},mark=triangle*\\%
 PiYG-7-4!70!black, every mark/.append style={solid,fill=PiYG-7-4},mark=diamond*\\%
 PiYG-7-5!70!black, every mark/.append style={solid,fill=PiYG-7-5},mark=pentagon*\\%
 PiYG-7-6!70!black, every mark/.append style={solid,fill=PiYG-7-6},mark=x\\%
 PiYG-7-7!70!black, every mark/.append style={solid,fill=PiYG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-8}{%
 PiYG-8-1!70!black, every mark/.append style={solid,fill=PiYG-8-1},mark=*\\%
 PiYG-8-2!70!black, every mark/.append style={solid,fill=PiYG-8-2},mark=square*\\%
 PiYG-8-3!70!black, every mark/.append style={solid,fill=PiYG-8-3},mark=triangle*\\%
 PiYG-8-4!70!black, every mark/.append style={solid,fill=PiYG-8-4},mark=diamond*\\%
 PiYG-8-5!70!black, every mark/.append style={solid,fill=PiYG-8-5},mark=pentagon*\\%
 PiYG-8-6!70!black, every mark/.append style={solid,fill=PiYG-8-6},mark=x\\%
 PiYG-8-7!70!black, every mark/.append style={solid,fill=PiYG-8-7},mark=+\\%
 PiYG-8-8!70!black, every mark/.append style={solid,fill=PiYG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-9}{%
 PiYG-9-1!70!black, every mark/.append style={solid,fill=PiYG-9-1},mark=*\\%
 PiYG-9-2!70!black, every mark/.append style={solid,fill=PiYG-9-2},mark=square*\\%
 PiYG-9-3!70!black, every mark/.append style={solid,fill=PiYG-9-3},mark=triangle*\\%
 PiYG-9-4!70!black, every mark/.append style={solid,fill=PiYG-9-4},mark=diamond*\\%
 PiYG-9-5!70!black, every mark/.append style={solid,fill=PiYG-9-5},mark=pentagon*\\%
 PiYG-9-6!70!black, every mark/.append style={solid,fill=PiYG-9-6},mark=x\\%
 PiYG-9-7!70!black, every mark/.append style={solid,fill=PiYG-9-7},mark=+\\%
 PiYG-9-8!70!black, every mark/.append style={solid,fill=PiYG-9-8},mark=star\\%
 PiYG-9-9!70!black, every mark/.append style={solid,fill=PiYG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-10}{%
 PiYG-10-1!70!black, every mark/.append style={solid,fill=PiYG-10-1},mark=*\\%
 PiYG-10-2!70!black, every mark/.append style={solid,fill=PiYG-10-2},mark=square*\\%
 PiYG-10-3!70!black, every mark/.append style={solid,fill=PiYG-10-3},mark=triangle*\\%
 PiYG-10-4!70!black, every mark/.append style={solid,fill=PiYG-10-4},mark=diamond*\\%
 PiYG-10-5!70!black, every mark/.append style={solid,fill=PiYG-10-5},mark=pentagon*\\%
 PiYG-10-6!70!black, every mark/.append style={solid,fill=PiYG-10-6},mark=x\\%
 PiYG-10-7!70!black, every mark/.append style={solid,fill=PiYG-10-7},mark=+\\%
 PiYG-10-8!70!black, every mark/.append style={solid,fill=PiYG-10-8},mark=star\\%
 PiYG-10-9!70!black, every mark/.append style={solid,fill=PiYG-10-9},mark=oplus*\\%
 PiYG-10-10!70!black, every mark/.append style={solid,fill=PiYG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-11}{%
 PiYG-11-1!70!black, every mark/.append style={solid,fill=PiYG-11-1},mark=*\\%
 PiYG-11-2!70!black, every mark/.append style={solid,fill=PiYG-11-2},mark=square*\\%
 PiYG-11-3!70!black, every mark/.append style={solid,fill=PiYG-11-3},mark=triangle*\\%
 PiYG-11-4!70!black, every mark/.append style={solid,fill=PiYG-11-4},mark=diamond*\\%
 PiYG-11-5!70!black, every mark/.append style={solid,fill=PiYG-11-5},mark=pentagon*\\%
 PiYG-11-6!70!black, every mark/.append style={solid,fill=PiYG-11-6},mark=x\\%
 PiYG-11-7!70!black, every mark/.append style={solid,fill=PiYG-11-7},mark=+\\%
 PiYG-11-8!70!black, every mark/.append style={solid,fill=PiYG-11-8},mark=star\\%
 PiYG-11-9!70!black, every mark/.append style={solid,fill=PiYG-11-9},mark=oplus*\\%
 PiYG-11-10!70!black, every mark/.append style={solid,fill=PiYG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-3}{%
 RdBu-3-1!70!black, every mark/.append style={solid,fill=RdBu-3-1},mark=*\\%
 RdBu-3-2!70!black, every mark/.append style={solid,fill=RdBu-3-2},mark=square*\\%
 RdBu-3-3!70!black, every mark/.append style={solid,fill=RdBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-4}{%
 RdBu-4-1!70!black, every mark/.append style={solid,fill=RdBu-4-1},mark=*\\%
 RdBu-4-2!70!black, every mark/.append style={solid,fill=RdBu-4-2},mark=square*\\%
 RdBu-4-3!70!black, every mark/.append style={solid,fill=RdBu-4-3},mark=triangle*\\%
 RdBu-4-4!70!black, every mark/.append style={solid,fill=RdBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-5}{%
 RdBu-5-1!70!black, every mark/.append style={solid,fill=RdBu-5-1},mark=*\\%
 RdBu-5-2!70!black, every mark/.append style={solid,fill=RdBu-5-2},mark=square*\\%
 RdBu-5-3!70!black, every mark/.append style={solid,fill=RdBu-5-3},mark=triangle*\\%
 RdBu-5-4!70!black, every mark/.append style={solid,fill=RdBu-5-4},mark=diamond*\\%
 RdBu-5-5!70!black, every mark/.append style={solid,fill=RdBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-6}{%
 RdBu-6-1!70!black, every mark/.append style={solid,fill=RdBu-6-1},mark=*\\%
 RdBu-6-2!70!black, every mark/.append style={solid,fill=RdBu-6-2},mark=square*\\%
 RdBu-6-3!70!black, every mark/.append style={solid,fill=RdBu-6-3},mark=triangle*\\%
 RdBu-6-4!70!black, every mark/.append style={solid,fill=RdBu-6-4},mark=diamond*\\%
 RdBu-6-5!70!black, every mark/.append style={solid,fill=RdBu-6-5},mark=pentagon*\\%
 RdBu-6-6!70!black, every mark/.append style={solid,fill=RdBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-7}{%
 RdBu-7-1!70!black, every mark/.append style={solid,fill=RdBu-7-1},mark=*\\%
 RdBu-7-2!70!black, every mark/.append style={solid,fill=RdBu-7-2},mark=square*\\%
 RdBu-7-3!70!black, every mark/.append style={solid,fill=RdBu-7-3},mark=triangle*\\%
 RdBu-7-4!70!black, every mark/.append style={solid,fill=RdBu-7-4},mark=diamond*\\%
 RdBu-7-5!70!black, every mark/.append style={solid,fill=RdBu-7-5},mark=pentagon*\\%
 RdBu-7-6!70!black, every mark/.append style={solid,fill=RdBu-7-6},mark=x\\%
 RdBu-7-7!70!black, every mark/.append style={solid,fill=RdBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-8}{%
 RdBu-8-1!70!black, every mark/.append style={solid,fill=RdBu-8-1},mark=*\\%
 RdBu-8-2!70!black, every mark/.append style={solid,fill=RdBu-8-2},mark=square*\\%
 RdBu-8-3!70!black, every mark/.append style={solid,fill=RdBu-8-3},mark=triangle*\\%
 RdBu-8-4!70!black, every mark/.append style={solid,fill=RdBu-8-4},mark=diamond*\\%
 RdBu-8-5!70!black, every mark/.append style={solid,fill=RdBu-8-5},mark=pentagon*\\%
 RdBu-8-6!70!black, every mark/.append style={solid,fill=RdBu-8-6},mark=x\\%
 RdBu-8-7!70!black, every mark/.append style={solid,fill=RdBu-8-7},mark=+\\%
 RdBu-8-8!70!black, every mark/.append style={solid,fill=RdBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-9}{%
 RdBu-9-1!70!black, every mark/.append style={solid,fill=RdBu-9-1},mark=*\\%
 RdBu-9-2!70!black, every mark/.append style={solid,fill=RdBu-9-2},mark=square*\\%
 RdBu-9-3!70!black, every mark/.append style={solid,fill=RdBu-9-3},mark=triangle*\\%
 RdBu-9-4!70!black, every mark/.append style={solid,fill=RdBu-9-4},mark=diamond*\\%
 RdBu-9-5!70!black, every mark/.append style={solid,fill=RdBu-9-5},mark=pentagon*\\%
 RdBu-9-6!70!black, every mark/.append style={solid,fill=RdBu-9-6},mark=x\\%
 RdBu-9-7!70!black, every mark/.append style={solid,fill=RdBu-9-7},mark=+\\%
 RdBu-9-8!70!black, every mark/.append style={solid,fill=RdBu-9-8},mark=star\\%
 RdBu-9-9!70!black, every mark/.append style={solid,fill=RdBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-10}{%
 RdBu-10-1!70!black, every mark/.append style={solid,fill=RdBu-10-1},mark=*\\%
 RdBu-10-2!70!black, every mark/.append style={solid,fill=RdBu-10-2},mark=square*\\%
 RdBu-10-3!70!black, every mark/.append style={solid,fill=RdBu-10-3},mark=triangle*\\%
 RdBu-10-4!70!black, every mark/.append style={solid,fill=RdBu-10-4},mark=diamond*\\%
 RdBu-10-5!70!black, every mark/.append style={solid,fill=RdBu-10-5},mark=pentagon*\\%
 RdBu-10-6!70!black, every mark/.append style={solid,fill=RdBu-10-6},mark=x\\%
 RdBu-10-7!70!black, every mark/.append style={solid,fill=RdBu-10-7},mark=+\\%
 RdBu-10-8!70!black, every mark/.append style={solid,fill=RdBu-10-8},mark=star\\%
 RdBu-10-9!70!black, every mark/.append style={solid,fill=RdBu-10-9},mark=oplus*\\%
 RdBu-10-10!70!black, every mark/.append style={solid,fill=RdBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-11}{%
 RdBu-11-1!70!black, every mark/.append style={solid,fill=RdBu-11-1},mark=*\\%
 RdBu-11-2!70!black, every mark/.append style={solid,fill=RdBu-11-2},mark=square*\\%
 RdBu-11-3!70!black, every mark/.append style={solid,fill=RdBu-11-3},mark=triangle*\\%
 RdBu-11-4!70!black, every mark/.append style={solid,fill=RdBu-11-4},mark=diamond*\\%
 RdBu-11-5!70!black, every mark/.append style={solid,fill=RdBu-11-5},mark=pentagon*\\%
 RdBu-11-6!70!black, every mark/.append style={solid,fill=RdBu-11-6},mark=x\\%
 RdBu-11-7!70!black, every mark/.append style={solid,fill=RdBu-11-7},mark=+\\%
 RdBu-11-8!70!black, every mark/.append style={solid,fill=RdBu-11-8},mark=star\\%
 RdBu-11-9!70!black, every mark/.append style={solid,fill=RdBu-11-9},mark=oplus*\\%
 RdBu-11-10!70!black, every mark/.append style={solid,fill=RdBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-3}{%
 RdGy-3-1!70!black, every mark/.append style={solid,fill=RdGy-3-1},mark=*\\%
 RdGy-3-2!70!black, every mark/.append style={solid,fill=RdGy-3-2},mark=square*\\%
 RdGy-3-3!70!black, every mark/.append style={solid,fill=RdGy-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-4}{%
 RdGy-4-1!70!black, every mark/.append style={solid,fill=RdGy-4-1},mark=*\\%
 RdGy-4-2!70!black, every mark/.append style={solid,fill=RdGy-4-2},mark=square*\\%
 RdGy-4-3!70!black, every mark/.append style={solid,fill=RdGy-4-3},mark=triangle*\\%
 RdGy-4-4!70!black, every mark/.append style={solid,fill=RdGy-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-5}{%
 RdGy-5-1!70!black, every mark/.append style={solid,fill=RdGy-5-1},mark=*\\%
 RdGy-5-2!70!black, every mark/.append style={solid,fill=RdGy-5-2},mark=square*\\%
 RdGy-5-3!70!black, every mark/.append style={solid,fill=RdGy-5-3},mark=triangle*\\%
 RdGy-5-4!70!black, every mark/.append style={solid,fill=RdGy-5-4},mark=diamond*\\%
 RdGy-5-5!70!black, every mark/.append style={solid,fill=RdGy-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-6}{%
 RdGy-6-1!70!black, every mark/.append style={solid,fill=RdGy-6-1},mark=*\\%
 RdGy-6-2!70!black, every mark/.append style={solid,fill=RdGy-6-2},mark=square*\\%
 RdGy-6-3!70!black, every mark/.append style={solid,fill=RdGy-6-3},mark=triangle*\\%
 RdGy-6-4!70!black, every mark/.append style={solid,fill=RdGy-6-4},mark=diamond*\\%
 RdGy-6-5!70!black, every mark/.append style={solid,fill=RdGy-6-5},mark=pentagon*\\%
 RdGy-6-6!70!black, every mark/.append style={solid,fill=RdGy-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-7}{%
 RdGy-7-1!70!black, every mark/.append style={solid,fill=RdGy-7-1},mark=*\\%
 RdGy-7-2!70!black, every mark/.append style={solid,fill=RdGy-7-2},mark=square*\\%
 RdGy-7-3!70!black, every mark/.append style={solid,fill=RdGy-7-3},mark=triangle*\\%
 RdGy-7-4!70!black, every mark/.append style={solid,fill=RdGy-7-4},mark=diamond*\\%
 RdGy-7-5!70!black, every mark/.append style={solid,fill=RdGy-7-5},mark=pentagon*\\%
 RdGy-7-6!70!black, every mark/.append style={solid,fill=RdGy-7-6},mark=x\\%
 RdGy-7-7!70!black, every mark/.append style={solid,fill=RdGy-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-8}{%
 RdGy-8-1!70!black, every mark/.append style={solid,fill=RdGy-8-1},mark=*\\%
 RdGy-8-2!70!black, every mark/.append style={solid,fill=RdGy-8-2},mark=square*\\%
 RdGy-8-3!70!black, every mark/.append style={solid,fill=RdGy-8-3},mark=triangle*\\%
 RdGy-8-4!70!black, every mark/.append style={solid,fill=RdGy-8-4},mark=diamond*\\%
 RdGy-8-5!70!black, every mark/.append style={solid,fill=RdGy-8-5},mark=pentagon*\\%
 RdGy-8-6!70!black, every mark/.append style={solid,fill=RdGy-8-6},mark=x\\%
 RdGy-8-7!70!black, every mark/.append style={solid,fill=RdGy-8-7},mark=+\\%
 RdGy-8-8!70!black, every mark/.append style={solid,fill=RdGy-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-9}{%
 RdGy-9-1!70!black, every mark/.append style={solid,fill=RdGy-9-1},mark=*\\%
 RdGy-9-2!70!black, every mark/.append style={solid,fill=RdGy-9-2},mark=square*\\%
 RdGy-9-3!70!black, every mark/.append style={solid,fill=RdGy-9-3},mark=triangle*\\%
 RdGy-9-4!70!black, every mark/.append style={solid,fill=RdGy-9-4},mark=diamond*\\%
 RdGy-9-5!70!black, every mark/.append style={solid,fill=RdGy-9-5},mark=pentagon*\\%
 RdGy-9-6!70!black, every mark/.append style={solid,fill=RdGy-9-6},mark=x\\%
 RdGy-9-7!70!black, every mark/.append style={solid,fill=RdGy-9-7},mark=+\\%
 RdGy-9-8!70!black, every mark/.append style={solid,fill=RdGy-9-8},mark=star\\%
 RdGy-9-9!70!black, every mark/.append style={solid,fill=RdGy-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-10}{%
 RdGy-10-1!70!black, every mark/.append style={solid,fill=RdGy-10-1},mark=*\\%
 RdGy-10-2!70!black, every mark/.append style={solid,fill=RdGy-10-2},mark=square*\\%
 RdGy-10-3!70!black, every mark/.append style={solid,fill=RdGy-10-3},mark=triangle*\\%
 RdGy-10-4!70!black, every mark/.append style={solid,fill=RdGy-10-4},mark=diamond*\\%
 RdGy-10-5!70!black, every mark/.append style={solid,fill=RdGy-10-5},mark=pentagon*\\%
 RdGy-10-6!70!black, every mark/.append style={solid,fill=RdGy-10-6},mark=x\\%
 RdGy-10-7!70!black, every mark/.append style={solid,fill=RdGy-10-7},mark=+\\%
 RdGy-10-8!70!black, every mark/.append style={solid,fill=RdGy-10-8},mark=star\\%
 RdGy-10-9!70!black, every mark/.append style={solid,fill=RdGy-10-9},mark=oplus*\\%
 RdGy-10-10!70!black, every mark/.append style={solid,fill=RdGy-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-11}{%
 RdGy-11-1!70!black, every mark/.append style={solid,fill=RdGy-11-1},mark=*\\%
 RdGy-11-2!70!black, every mark/.append style={solid,fill=RdGy-11-2},mark=square*\\%
 RdGy-11-3!70!black, every mark/.append style={solid,fill=RdGy-11-3},mark=triangle*\\%
 RdGy-11-4!70!black, every mark/.append style={solid,fill=RdGy-11-4},mark=diamond*\\%
 RdGy-11-5!70!black, every mark/.append style={solid,fill=RdGy-11-5},mark=pentagon*\\%
 RdGy-11-6!70!black, every mark/.append style={solid,fill=RdGy-11-6},mark=x\\%
 RdGy-11-7!70!black, every mark/.append style={solid,fill=RdGy-11-7},mark=+\\%
 RdGy-11-8!70!black, every mark/.append style={solid,fill=RdGy-11-8},mark=star\\%
 RdGy-11-9!70!black, every mark/.append style={solid,fill=RdGy-11-9},mark=oplus*\\%
 RdGy-11-10!70!black, every mark/.append style={solid,fill=RdGy-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-3}{%
 RdYlBu-3-1!70!black, every mark/.append style={solid,fill=RdYlBu-3-1},mark=*\\%
 RdYlBu-3-2!70!black, every mark/.append style={solid,fill=RdYlBu-3-2},mark=square*\\%
 RdYlBu-3-3!70!black, every mark/.append style={solid,fill=RdYlBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-4}{%
 RdYlBu-4-1!70!black, every mark/.append style={solid,fill=RdYlBu-4-1},mark=*\\%
 RdYlBu-4-2!70!black, every mark/.append style={solid,fill=RdYlBu-4-2},mark=square*\\%
 RdYlBu-4-3!70!black, every mark/.append style={solid,fill=RdYlBu-4-3},mark=triangle*\\%
 RdYlBu-4-4!70!black, every mark/.append style={solid,fill=RdYlBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-5}{%
 RdYlBu-5-1!70!black, every mark/.append style={solid,fill=RdYlBu-5-1},mark=*\\%
 RdYlBu-5-2!70!black, every mark/.append style={solid,fill=RdYlBu-5-2},mark=square*\\%
 RdYlBu-5-3!70!black, every mark/.append style={solid,fill=RdYlBu-5-3},mark=triangle*\\%
 RdYlBu-5-4!70!black, every mark/.append style={solid,fill=RdYlBu-5-4},mark=diamond*\\%
 RdYlBu-5-5!70!black, every mark/.append style={solid,fill=RdYlBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-6}{%
 RdYlBu-6-1!70!black, every mark/.append style={solid,fill=RdYlBu-6-1},mark=*\\%
 RdYlBu-6-2!70!black, every mark/.append style={solid,fill=RdYlBu-6-2},mark=square*\\%
 RdYlBu-6-3!70!black, every mark/.append style={solid,fill=RdYlBu-6-3},mark=triangle*\\%
 RdYlBu-6-4!70!black, every mark/.append style={solid,fill=RdYlBu-6-4},mark=diamond*\\%
 RdYlBu-6-5!70!black, every mark/.append style={solid,fill=RdYlBu-6-5},mark=pentagon*\\%
 RdYlBu-6-6!70!black, every mark/.append style={solid,fill=RdYlBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-7}{%
 RdYlBu-7-1!70!black, every mark/.append style={solid,fill=RdYlBu-7-1},mark=*\\%
 RdYlBu-7-2!70!black, every mark/.append style={solid,fill=RdYlBu-7-2},mark=square*\\%
 RdYlBu-7-3!70!black, every mark/.append style={solid,fill=RdYlBu-7-3},mark=triangle*\\%
 RdYlBu-7-4!70!black, every mark/.append style={solid,fill=RdYlBu-7-4},mark=diamond*\\%
 RdYlBu-7-5!70!black, every mark/.append style={solid,fill=RdYlBu-7-5},mark=pentagon*\\%
 RdYlBu-7-6!70!black, every mark/.append style={solid,fill=RdYlBu-7-6},mark=x\\%
 RdYlBu-7-7!70!black, every mark/.append style={solid,fill=RdYlBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-8}{%
 RdYlBu-8-1!70!black, every mark/.append style={solid,fill=RdYlBu-8-1},mark=*\\%
 RdYlBu-8-2!70!black, every mark/.append style={solid,fill=RdYlBu-8-2},mark=square*\\%
 RdYlBu-8-3!70!black, every mark/.append style={solid,fill=RdYlBu-8-3},mark=triangle*\\%
 RdYlBu-8-4!70!black, every mark/.append style={solid,fill=RdYlBu-8-4},mark=diamond*\\%
 RdYlBu-8-5!70!black, every mark/.append style={solid,fill=RdYlBu-8-5},mark=pentagon*\\%
 RdYlBu-8-6!70!black, every mark/.append style={solid,fill=RdYlBu-8-6},mark=x\\%
 RdYlBu-8-7!70!black, every mark/.append style={solid,fill=RdYlBu-8-7},mark=+\\%
 RdYlBu-8-8!70!black, every mark/.append style={solid,fill=RdYlBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-9}{%
 RdYlBu-9-1!70!black, every mark/.append style={solid,fill=RdYlBu-9-1},mark=*\\%
 RdYlBu-9-2!70!black, every mark/.append style={solid,fill=RdYlBu-9-2},mark=square*\\%
 RdYlBu-9-3!70!black, every mark/.append style={solid,fill=RdYlBu-9-3},mark=triangle*\\%
 RdYlBu-9-4!70!black, every mark/.append style={solid,fill=RdYlBu-9-4},mark=diamond*\\%
 RdYlBu-9-5!70!black, every mark/.append style={solid,fill=RdYlBu-9-5},mark=pentagon*\\%
 RdYlBu-9-6!70!black, every mark/.append style={solid,fill=RdYlBu-9-6},mark=x\\%
 RdYlBu-9-7!70!black, every mark/.append style={solid,fill=RdYlBu-9-7},mark=+\\%
 RdYlBu-9-8!70!black, every mark/.append style={solid,fill=RdYlBu-9-8},mark=star\\%
 RdYlBu-9-9!70!black, every mark/.append style={solid,fill=RdYlBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-10}{%
 RdYlBu-10-1!70!black, every mark/.append style={solid,fill=RdYlBu-10-1},mark=*\\%
 RdYlBu-10-2!70!black, every mark/.append style={solid,fill=RdYlBu-10-2},mark=square*\\%
 RdYlBu-10-3!70!black, every mark/.append style={solid,fill=RdYlBu-10-3},mark=triangle*\\%
 RdYlBu-10-4!70!black, every mark/.append style={solid,fill=RdYlBu-10-4},mark=diamond*\\%
 RdYlBu-10-5!70!black, every mark/.append style={solid,fill=RdYlBu-10-5},mark=pentagon*\\%
 RdYlBu-10-6!70!black, every mark/.append style={solid,fill=RdYlBu-10-6},mark=x\\%
 RdYlBu-10-7!70!black, every mark/.append style={solid,fill=RdYlBu-10-7},mark=+\\%
 RdYlBu-10-8!70!black, every mark/.append style={solid,fill=RdYlBu-10-8},mark=star\\%
 RdYlBu-10-9!70!black, every mark/.append style={solid,fill=RdYlBu-10-9},mark=oplus*\\%
 RdYlBu-10-10!70!black, every mark/.append style={solid,fill=RdYlBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-11}{%
 RdYlBu-11-1!70!black, every mark/.append style={solid,fill=RdYlBu-11-1},mark=*\\%
 RdYlBu-11-2!70!black, every mark/.append style={solid,fill=RdYlBu-11-2},mark=square*\\%
 RdYlBu-11-3!70!black, every mark/.append style={solid,fill=RdYlBu-11-3},mark=triangle*\\%
 RdYlBu-11-4!70!black, every mark/.append style={solid,fill=RdYlBu-11-4},mark=diamond*\\%
 RdYlBu-11-5!70!black, every mark/.append style={solid,fill=RdYlBu-11-5},mark=pentagon*\\%
 RdYlBu-11-6!70!black, every mark/.append style={solid,fill=RdYlBu-11-6},mark=x\\%
 RdYlBu-11-7!70!black, every mark/.append style={solid,fill=RdYlBu-11-7},mark=+\\%
 RdYlBu-11-8!70!black, every mark/.append style={solid,fill=RdYlBu-11-8},mark=star\\%
 RdYlBu-11-9!70!black, every mark/.append style={solid,fill=RdYlBu-11-9},mark=oplus*\\%
 RdYlBu-11-10!70!black, every mark/.append style={solid,fill=RdYlBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-3}{%
 Spectral-3-1!70!black, every mark/.append style={solid,fill=Spectral-3-1},mark=*\\%
 Spectral-3-2!70!black, every mark/.append style={solid,fill=Spectral-3-2},mark=square*\\%
 Spectral-3-3!70!black, every mark/.append style={solid,fill=Spectral-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-4}{%
 Spectral-4-1!70!black, every mark/.append style={solid,fill=Spectral-4-1},mark=*\\%
 Spectral-4-2!70!black, every mark/.append style={solid,fill=Spectral-4-2},mark=square*\\%
 Spectral-4-3!70!black, every mark/.append style={solid,fill=Spectral-4-3},mark=triangle*\\%
 Spectral-4-4!70!black, every mark/.append style={solid,fill=Spectral-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-5}{%
 Spectral-5-1!70!black, every mark/.append style={solid,fill=Spectral-5-1},mark=*\\%
 Spectral-5-2!70!black, every mark/.append style={solid,fill=Spectral-5-2},mark=square*\\%
 Spectral-5-3!70!black, every mark/.append style={solid,fill=Spectral-5-3},mark=triangle*\\%
 Spectral-5-4!70!black, every mark/.append style={solid,fill=Spectral-5-4},mark=diamond*\\%
 Spectral-5-5!70!black, every mark/.append style={solid,fill=Spectral-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-6}{%
 Spectral-6-1!70!black, every mark/.append style={solid,fill=Spectral-6-1},mark=*\\%
 Spectral-6-2!70!black, every mark/.append style={solid,fill=Spectral-6-2},mark=square*\\%
 Spectral-6-3!70!black, every mark/.append style={solid,fill=Spectral-6-3},mark=triangle*\\%
 Spectral-6-4!70!black, every mark/.append style={solid,fill=Spectral-6-4},mark=diamond*\\%
 Spectral-6-5!70!black, every mark/.append style={solid,fill=Spectral-6-5},mark=pentagon*\\%
 Spectral-6-6!70!black, every mark/.append style={solid,fill=Spectral-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-7}{%
 Spectral-7-1!70!black, every mark/.append style={solid,fill=Spectral-7-1},mark=*\\%
 Spectral-7-2!70!black, every mark/.append style={solid,fill=Spectral-7-2},mark=square*\\%
 Spectral-7-3!70!black, every mark/.append style={solid,fill=Spectral-7-3},mark=triangle*\\%
 Spectral-7-4!70!black, every mark/.append style={solid,fill=Spectral-7-4},mark=diamond*\\%
 Spectral-7-5!70!black, every mark/.append style={solid,fill=Spectral-7-5},mark=pentagon*\\%
 Spectral-7-6!70!black, every mark/.append style={solid,fill=Spectral-7-6},mark=x\\%
 Spectral-7-7!70!black, every mark/.append style={solid,fill=Spectral-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-8}{%
 Spectral-8-1!70!black, every mark/.append style={solid,fill=Spectral-8-1},mark=*\\%
 Spectral-8-2!70!black, every mark/.append style={solid,fill=Spectral-8-2},mark=square*\\%
 Spectral-8-3!70!black, every mark/.append style={solid,fill=Spectral-8-3},mark=triangle*\\%
 Spectral-8-4!70!black, every mark/.append style={solid,fill=Spectral-8-4},mark=diamond*\\%
 Spectral-8-5!70!black, every mark/.append style={solid,fill=Spectral-8-5},mark=pentagon*\\%
 Spectral-8-6!70!black, every mark/.append style={solid,fill=Spectral-8-6},mark=x\\%
 Spectral-8-7!70!black, every mark/.append style={solid,fill=Spectral-8-7},mark=+\\%
 Spectral-8-8!70!black, every mark/.append style={solid,fill=Spectral-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-9}{%
 Spectral-9-1!70!black, every mark/.append style={solid,fill=Spectral-9-1},mark=*\\%
 Spectral-9-2!70!black, every mark/.append style={solid,fill=Spectral-9-2},mark=square*\\%
 Spectral-9-3!70!black, every mark/.append style={solid,fill=Spectral-9-3},mark=triangle*\\%
 Spectral-9-4!70!black, every mark/.append style={solid,fill=Spectral-9-4},mark=diamond*\\%
 Spectral-9-5!70!black, every mark/.append style={solid,fill=Spectral-9-5},mark=pentagon*\\%
 Spectral-9-6!70!black, every mark/.append style={solid,fill=Spectral-9-6},mark=x\\%
 Spectral-9-7!70!black, every mark/.append style={solid,fill=Spectral-9-7},mark=+\\%
 Spectral-9-8!70!black, every mark/.append style={solid,fill=Spectral-9-8},mark=star\\%
 Spectral-9-9!70!black, every mark/.append style={solid,fill=Spectral-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-10}{%
 Spectral-10-1!70!black, every mark/.append style={solid,fill=Spectral-10-1},mark=*\\%
 Spectral-10-2!70!black, every mark/.append style={solid,fill=Spectral-10-2},mark=square*\\%
 Spectral-10-3!70!black, every mark/.append style={solid,fill=Spectral-10-3},mark=triangle*\\%
 Spectral-10-4!70!black, every mark/.append style={solid,fill=Spectral-10-4},mark=diamond*\\%
 Spectral-10-5!70!black, every mark/.append style={solid,fill=Spectral-10-5},mark=pentagon*\\%
 Spectral-10-6!70!black, every mark/.append style={solid,fill=Spectral-10-6},mark=x\\%
 Spectral-10-7!70!black, every mark/.append style={solid,fill=Spectral-10-7},mark=+\\%
 Spectral-10-8!70!black, every mark/.append style={solid,fill=Spectral-10-8},mark=star\\%
 Spectral-10-9!70!black, every mark/.append style={solid,fill=Spectral-10-9},mark=oplus*\\%
 Spectral-10-10!70!black, every mark/.append style={solid,fill=Spectral-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-11}{%
 Spectral-11-1!70!black, every mark/.append style={solid,fill=Spectral-11-1},mark=*\\%
 Spectral-11-2!70!black, every mark/.append style={solid,fill=Spectral-11-2},mark=square*\\%
 Spectral-11-3!70!black, every mark/.append style={solid,fill=Spectral-11-3},mark=triangle*\\%
 Spectral-11-4!70!black, every mark/.append style={solid,fill=Spectral-11-4},mark=diamond*\\%
 Spectral-11-5!70!black, every mark/.append style={solid,fill=Spectral-11-5},mark=pentagon*\\%
 Spectral-11-6!70!black, every mark/.append style={solid,fill=Spectral-11-6},mark=x\\%
 Spectral-11-7!70!black, every mark/.append style={solid,fill=Spectral-11-7},mark=+\\%
 Spectral-11-8!70!black, every mark/.append style={solid,fill=Spectral-11-8},mark=star\\%
 Spectral-11-9!70!black, every mark/.append style={solid,fill=Spectral-11-9},mark=oplus*\\%
 Spectral-11-10!70!black, every mark/.append style={solid,fill=Spectral-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-3}{%
 RdYlGn-3-1!70!black, every mark/.append style={solid,fill=RdYlGn-3-1},mark=*\\%
 RdYlGn-3-2!70!black, every mark/.append style={solid,fill=RdYlGn-3-2},mark=square*\\%
 RdYlGn-3-3!70!black, every mark/.append style={solid,fill=RdYlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-4}{%
 RdYlGn-4-1!70!black, every mark/.append style={solid,fill=RdYlGn-4-1},mark=*\\%
 RdYlGn-4-2!70!black, every mark/.append style={solid,fill=RdYlGn-4-2},mark=square*\\%
 RdYlGn-4-3!70!black, every mark/.append style={solid,fill=RdYlGn-4-3},mark=triangle*\\%
 RdYlGn-4-4!70!black, every mark/.append style={solid,fill=RdYlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-5}{%
 RdYlGn-5-1!70!black, every mark/.append style={solid,fill=RdYlGn-5-1},mark=*\\%
 RdYlGn-5-2!70!black, every mark/.append style={solid,fill=RdYlGn-5-2},mark=square*\\%
 RdYlGn-5-3!70!black, every mark/.append style={solid,fill=RdYlGn-5-3},mark=triangle*\\%
 RdYlGn-5-4!70!black, every mark/.append style={solid,fill=RdYlGn-5-4},mark=diamond*\\%
 RdYlGn-5-5!70!black, every mark/.append style={solid,fill=RdYlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-6}{%
 RdYlGn-6-1!70!black, every mark/.append style={solid,fill=RdYlGn-6-1},mark=*\\%
 RdYlGn-6-2!70!black, every mark/.append style={solid,fill=RdYlGn-6-2},mark=square*\\%
 RdYlGn-6-3!70!black, every mark/.append style={solid,fill=RdYlGn-6-3},mark=triangle*\\%
 RdYlGn-6-4!70!black, every mark/.append style={solid,fill=RdYlGn-6-4},mark=diamond*\\%
 RdYlGn-6-5!70!black, every mark/.append style={solid,fill=RdYlGn-6-5},mark=pentagon*\\%
 RdYlGn-6-6!70!black, every mark/.append style={solid,fill=RdYlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-7}{%
 RdYlGn-7-1!70!black, every mark/.append style={solid,fill=RdYlGn-7-1},mark=*\\%
 RdYlGn-7-2!70!black, every mark/.append style={solid,fill=RdYlGn-7-2},mark=square*\\%
 RdYlGn-7-3!70!black, every mark/.append style={solid,fill=RdYlGn-7-3},mark=triangle*\\%
 RdYlGn-7-4!70!black, every mark/.append style={solid,fill=RdYlGn-7-4},mark=diamond*\\%
 RdYlGn-7-5!70!black, every mark/.append style={solid,fill=RdYlGn-7-5},mark=pentagon*\\%
 RdYlGn-7-6!70!black, every mark/.append style={solid,fill=RdYlGn-7-6},mark=x\\%
 RdYlGn-7-7!70!black, every mark/.append style={solid,fill=RdYlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-8}{%
 RdYlGn-8-1!70!black, every mark/.append style={solid,fill=RdYlGn-8-1},mark=*\\%
 RdYlGn-8-2!70!black, every mark/.append style={solid,fill=RdYlGn-8-2},mark=square*\\%
 RdYlGn-8-3!70!black, every mark/.append style={solid,fill=RdYlGn-8-3},mark=triangle*\\%
 RdYlGn-8-4!70!black, every mark/.append style={solid,fill=RdYlGn-8-4},mark=diamond*\\%
 RdYlGn-8-5!70!black, every mark/.append style={solid,fill=RdYlGn-8-5},mark=pentagon*\\%
 RdYlGn-8-6!70!black, every mark/.append style={solid,fill=RdYlGn-8-6},mark=x\\%
 RdYlGn-8-7!70!black, every mark/.append style={solid,fill=RdYlGn-8-7},mark=+\\%
 RdYlGn-8-8!70!black, every mark/.append style={solid,fill=RdYlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-9}{%
 RdYlGn-9-1!70!black, every mark/.append style={solid,fill=RdYlGn-9-1},mark=*\\%
 RdYlGn-9-2!70!black, every mark/.append style={solid,fill=RdYlGn-9-2},mark=square*\\%
 RdYlGn-9-3!70!black, every mark/.append style={solid,fill=RdYlGn-9-3},mark=triangle*\\%
 RdYlGn-9-4!70!black, every mark/.append style={solid,fill=RdYlGn-9-4},mark=diamond*\\%
 RdYlGn-9-5!70!black, every mark/.append style={solid,fill=RdYlGn-9-5},mark=pentagon*\\%
 RdYlGn-9-6!70!black, every mark/.append style={solid,fill=RdYlGn-9-6},mark=x\\%
 RdYlGn-9-7!70!black, every mark/.append style={solid,fill=RdYlGn-9-7},mark=+\\%
 RdYlGn-9-8!70!black, every mark/.append style={solid,fill=RdYlGn-9-8},mark=star\\%
 RdYlGn-9-9!70!black, every mark/.append style={solid,fill=RdYlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-10}{%
 RdYlGn-10-1!70!black, every mark/.append style={solid,fill=RdYlGn-10-1},mark=*\\%
 RdYlGn-10-2!70!black, every mark/.append style={solid,fill=RdYlGn-10-2},mark=square*\\%
 RdYlGn-10-3!70!black, every mark/.append style={solid,fill=RdYlGn-10-3},mark=triangle*\\%
 RdYlGn-10-4!70!black, every mark/.append style={solid,fill=RdYlGn-10-4},mark=diamond*\\%
 RdYlGn-10-5!70!black, every mark/.append style={solid,fill=RdYlGn-10-5},mark=pentagon*\\%
 RdYlGn-10-6!70!black, every mark/.append style={solid,fill=RdYlGn-10-6},mark=x\\%
 RdYlGn-10-7!70!black, every mark/.append style={solid,fill=RdYlGn-10-7},mark=+\\%
 RdYlGn-10-8!70!black, every mark/.append style={solid,fill=RdYlGn-10-8},mark=star\\%
 RdYlGn-10-9!70!black, every mark/.append style={solid,fill=RdYlGn-10-9},mark=oplus*\\%
 RdYlGn-10-10!70!black, every mark/.append style={solid,fill=RdYlGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-11}{%
 RdYlGn-11-1!70!black, every mark/.append style={solid,fill=RdYlGn-11-1},mark=*\\%
 RdYlGn-11-2!70!black, every mark/.append style={solid,fill=RdYlGn-11-2},mark=square*\\%
 RdYlGn-11-3!70!black, every mark/.append style={solid,fill=RdYlGn-11-3},mark=triangle*\\%
 RdYlGn-11-4!70!black, every mark/.append style={solid,fill=RdYlGn-11-4},mark=diamond*\\%
 RdYlGn-11-5!70!black, every mark/.append style={solid,fill=RdYlGn-11-5},mark=pentagon*\\%
 RdYlGn-11-6!70!black, every mark/.append style={solid,fill=RdYlGn-11-6},mark=x\\%
 RdYlGn-11-7!70!black, every mark/.append style={solid,fill=RdYlGn-11-7},mark=+\\%
 RdYlGn-11-8!70!black, every mark/.append style={solid,fill=RdYlGn-11-8},mark=star\\%
 RdYlGn-11-9!70!black, every mark/.append style={solid,fill=RdYlGn-11-9},mark=oplus*\\%
 RdYlGn-11-10!70!black, every mark/.append style={solid,fill=RdYlGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-3}{%
 Set3-3-1!70!black, every mark/.append style={solid,fill=Set3-3-1},mark=*\\%
 Set3-3-2!70!black, every mark/.append style={solid,fill=Set3-3-2},mark=square*\\%
 Set3-3-3!70!black, every mark/.append style={solid,fill=Set3-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-4}{%
 Set3-4-1!70!black, every mark/.append style={solid,fill=Set3-4-1},mark=*\\%
 Set3-4-2!70!black, every mark/.append style={solid,fill=Set3-4-2},mark=square*\\%
 Set3-4-3!70!black, every mark/.append style={solid,fill=Set3-4-3},mark=triangle*\\%
 Set3-4-4!70!black, every mark/.append style={solid,fill=Set3-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-5}{%
 Set3-5-1!70!black, every mark/.append style={solid,fill=Set3-5-1},mark=*\\%
 Set3-5-2!70!black, every mark/.append style={solid,fill=Set3-5-2},mark=square*\\%
 Set3-5-3!70!black, every mark/.append style={solid,fill=Set3-5-3},mark=triangle*\\%
 Set3-5-4!70!black, every mark/.append style={solid,fill=Set3-5-4},mark=diamond*\\%
 Set3-5-5!70!black, every mark/.append style={solid,fill=Set3-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-6}{%
 Set3-6-1!70!black, every mark/.append style={solid,fill=Set3-6-1},mark=*\\%
 Set3-6-2!70!black, every mark/.append style={solid,fill=Set3-6-2},mark=square*\\%
 Set3-6-3!70!black, every mark/.append style={solid,fill=Set3-6-3},mark=triangle*\\%
 Set3-6-4!70!black, every mark/.append style={solid,fill=Set3-6-4},mark=diamond*\\%
 Set3-6-5!70!black, every mark/.append style={solid,fill=Set3-6-5},mark=pentagon*\\%
 Set3-6-6!70!black, every mark/.append style={solid,fill=Set3-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-7}{%
 Set3-7-1!70!black, every mark/.append style={solid,fill=Set3-7-1},mark=*\\%
 Set3-7-2!70!black, every mark/.append style={solid,fill=Set3-7-2},mark=square*\\%
 Set3-7-3!70!black, every mark/.append style={solid,fill=Set3-7-3},mark=triangle*\\%
 Set3-7-4!70!black, every mark/.append style={solid,fill=Set3-7-4},mark=diamond*\\%
 Set3-7-5!70!black, every mark/.append style={solid,fill=Set3-7-5},mark=pentagon*\\%
 Set3-7-6!70!black, every mark/.append style={solid,fill=Set3-7-6},mark=x\\%
 Set3-7-7!70!black, every mark/.append style={solid,fill=Set3-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-8}{%
 Set3-8-1!70!black, every mark/.append style={solid,fill=Set3-8-1},mark=*\\%
 Set3-8-2!70!black, every mark/.append style={solid,fill=Set3-8-2},mark=square*\\%
 Set3-8-3!70!black, every mark/.append style={solid,fill=Set3-8-3},mark=triangle*\\%
 Set3-8-4!70!black, every mark/.append style={solid,fill=Set3-8-4},mark=diamond*\\%
 Set3-8-5!70!black, every mark/.append style={solid,fill=Set3-8-5},mark=pentagon*\\%
 Set3-8-6!70!black, every mark/.append style={solid,fill=Set3-8-6},mark=x\\%
 Set3-8-7!70!black, every mark/.append style={solid,fill=Set3-8-7},mark=+\\%
 Set3-8-8!70!black, every mark/.append style={solid,fill=Set3-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-9}{%
 Set3-9-1!70!black, every mark/.append style={solid,fill=Set3-9-1},mark=*\\%
 Set3-9-2!70!black, every mark/.append style={solid,fill=Set3-9-2},mark=square*\\%
 Set3-9-3!70!black, every mark/.append style={solid,fill=Set3-9-3},mark=triangle*\\%
 Set3-9-4!70!black, every mark/.append style={solid,fill=Set3-9-4},mark=diamond*\\%
 Set3-9-5!70!black, every mark/.append style={solid,fill=Set3-9-5},mark=pentagon*\\%
 Set3-9-6!70!black, every mark/.append style={solid,fill=Set3-9-6},mark=x\\%
 Set3-9-7!70!black, every mark/.append style={solid,fill=Set3-9-7},mark=+\\%
 Set3-9-8!70!black, every mark/.append style={solid,fill=Set3-9-8},mark=star\\%
 Set3-9-9!70!black, every mark/.append style={solid,fill=Set3-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-10}{%
 Set3-10-1!70!black, every mark/.append style={solid,fill=Set3-10-1},mark=*\\%
 Set3-10-2!70!black, every mark/.append style={solid,fill=Set3-10-2},mark=square*\\%
 Set3-10-3!70!black, every mark/.append style={solid,fill=Set3-10-3},mark=triangle*\\%
 Set3-10-4!70!black, every mark/.append style={solid,fill=Set3-10-4},mark=diamond*\\%
 Set3-10-5!70!black, every mark/.append style={solid,fill=Set3-10-5},mark=pentagon*\\%
 Set3-10-6!70!black, every mark/.append style={solid,fill=Set3-10-6},mark=x\\%
 Set3-10-7!70!black, every mark/.append style={solid,fill=Set3-10-7},mark=+\\%
 Set3-10-8!70!black, every mark/.append style={solid,fill=Set3-10-8},mark=star\\%
 Set3-10-9!70!black, every mark/.append style={solid,fill=Set3-10-9},mark=oplus*\\%
 Set3-10-10!70!black, every mark/.append style={solid,fill=Set3-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-11}{%
 Set3-11-1!70!black, every mark/.append style={solid,fill=Set3-11-1},mark=*\\%
 Set3-11-2!70!black, every mark/.append style={solid,fill=Set3-11-2},mark=square*\\%
 Set3-11-3!70!black, every mark/.append style={solid,fill=Set3-11-3},mark=triangle*\\%
 Set3-11-4!70!black, every mark/.append style={solid,fill=Set3-11-4},mark=diamond*\\%
 Set3-11-5!70!black, every mark/.append style={solid,fill=Set3-11-5},mark=pentagon*\\%
 Set3-11-6!70!black, every mark/.append style={solid,fill=Set3-11-6},mark=x\\%
 Set3-11-7!70!black, every mark/.append style={solid,fill=Set3-11-7},mark=+\\%
 Set3-11-8!70!black, every mark/.append style={solid,fill=Set3-11-8},mark=star\\%
 Set3-11-9!70!black, every mark/.append style={solid,fill=Set3-11-9},mark=oplus*\\%
 Set3-11-10!70!black, every mark/.append style={solid,fill=Set3-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-12}{%
 Set3-12-1!70!black, every mark/.append style={solid,fill=Set3-12-1},mark=*\\%
 Set3-12-2!70!black, every mark/.append style={solid,fill=Set3-12-2},mark=square*\\%
 Set3-12-3!70!black, every mark/.append style={solid,fill=Set3-12-3},mark=triangle*\\%
 Set3-12-4!70!black, every mark/.append style={solid,fill=Set3-12-4},mark=diamond*\\%
 Set3-12-5!70!black, every mark/.append style={solid,fill=Set3-12-5},mark=pentagon*\\%
 Set3-12-6!70!black, every mark/.append style={solid,fill=Set3-12-6},mark=x\\%
 Set3-12-7!70!black, every mark/.append style={solid,fill=Set3-12-7},mark=+\\%
 Set3-12-8!70!black, every mark/.append style={solid,fill=Set3-12-8},mark=star\\%
 Set3-12-9!70!black, every mark/.append style={solid,fill=Set3-12-9},mark=oplus*\\%
 Set3-12-10!70!black, every mark/.append style={solid,fill=Set3-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-3}{%
 Pastel1-3-1!70!black, every mark/.append style={solid,fill=Pastel1-3-1},mark=*\\%
 Pastel1-3-2!70!black, every mark/.append style={solid,fill=Pastel1-3-2},mark=square*\\%
 Pastel1-3-3!70!black, every mark/.append style={solid,fill=Pastel1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-4}{%
 Pastel1-4-1!70!black, every mark/.append style={solid,fill=Pastel1-4-1},mark=*\\%
 Pastel1-4-2!70!black, every mark/.append style={solid,fill=Pastel1-4-2},mark=square*\\%
 Pastel1-4-3!70!black, every mark/.append style={solid,fill=Pastel1-4-3},mark=triangle*\\%
 Pastel1-4-4!70!black, every mark/.append style={solid,fill=Pastel1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-5}{%
 Pastel1-5-1!70!black, every mark/.append style={solid,fill=Pastel1-5-1},mark=*\\%
 Pastel1-5-2!70!black, every mark/.append style={solid,fill=Pastel1-5-2},mark=square*\\%
 Pastel1-5-3!70!black, every mark/.append style={solid,fill=Pastel1-5-3},mark=triangle*\\%
 Pastel1-5-4!70!black, every mark/.append style={solid,fill=Pastel1-5-4},mark=diamond*\\%
 Pastel1-5-5!70!black, every mark/.append style={solid,fill=Pastel1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-6}{%
 Pastel1-6-1!70!black, every mark/.append style={solid,fill=Pastel1-6-1},mark=*\\%
 Pastel1-6-2!70!black, every mark/.append style={solid,fill=Pastel1-6-2},mark=square*\\%
 Pastel1-6-3!70!black, every mark/.append style={solid,fill=Pastel1-6-3},mark=triangle*\\%
 Pastel1-6-4!70!black, every mark/.append style={solid,fill=Pastel1-6-4},mark=diamond*\\%
 Pastel1-6-5!70!black, every mark/.append style={solid,fill=Pastel1-6-5},mark=pentagon*\\%
 Pastel1-6-6!70!black, every mark/.append style={solid,fill=Pastel1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-7}{%
 Pastel1-7-1!70!black, every mark/.append style={solid,fill=Pastel1-7-1},mark=*\\%
 Pastel1-7-2!70!black, every mark/.append style={solid,fill=Pastel1-7-2},mark=square*\\%
 Pastel1-7-3!70!black, every mark/.append style={solid,fill=Pastel1-7-3},mark=triangle*\\%
 Pastel1-7-4!70!black, every mark/.append style={solid,fill=Pastel1-7-4},mark=diamond*\\%
 Pastel1-7-5!70!black, every mark/.append style={solid,fill=Pastel1-7-5},mark=pentagon*\\%
 Pastel1-7-6!70!black, every mark/.append style={solid,fill=Pastel1-7-6},mark=x\\%
 Pastel1-7-7!70!black, every mark/.append style={solid,fill=Pastel1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-8}{%
 Pastel1-8-1!70!black, every mark/.append style={solid,fill=Pastel1-8-1},mark=*\\%
 Pastel1-8-2!70!black, every mark/.append style={solid,fill=Pastel1-8-2},mark=square*\\%
 Pastel1-8-3!70!black, every mark/.append style={solid,fill=Pastel1-8-3},mark=triangle*\\%
 Pastel1-8-4!70!black, every mark/.append style={solid,fill=Pastel1-8-4},mark=diamond*\\%
 Pastel1-8-5!70!black, every mark/.append style={solid,fill=Pastel1-8-5},mark=pentagon*\\%
 Pastel1-8-6!70!black, every mark/.append style={solid,fill=Pastel1-8-6},mark=x\\%
 Pastel1-8-7!70!black, every mark/.append style={solid,fill=Pastel1-8-7},mark=+\\%
 Pastel1-8-8!70!black, every mark/.append style={solid,fill=Pastel1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-9}{%
 Pastel1-9-1!70!black, every mark/.append style={solid,fill=Pastel1-9-1},mark=*\\%
 Pastel1-9-2!70!black, every mark/.append style={solid,fill=Pastel1-9-2},mark=square*\\%
 Pastel1-9-3!70!black, every mark/.append style={solid,fill=Pastel1-9-3},mark=triangle*\\%
 Pastel1-9-4!70!black, every mark/.append style={solid,fill=Pastel1-9-4},mark=diamond*\\%
 Pastel1-9-5!70!black, every mark/.append style={solid,fill=Pastel1-9-5},mark=pentagon*\\%
 Pastel1-9-6!70!black, every mark/.append style={solid,fill=Pastel1-9-6},mark=x\\%
 Pastel1-9-7!70!black, every mark/.append style={solid,fill=Pastel1-9-7},mark=+\\%
 Pastel1-9-8!70!black, every mark/.append style={solid,fill=Pastel1-9-8},mark=star\\%
 Pastel1-9-9!70!black, every mark/.append style={solid,fill=Pastel1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-3}{%
 Set1-3-1!70!black, every mark/.append style={solid,fill=Set1-3-1},mark=*\\%
 Set1-3-2!70!black, every mark/.append style={solid,fill=Set1-3-2},mark=square*\\%
 Set1-3-3!70!black, every mark/.append style={solid,fill=Set1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-4}{%
 Set1-4-1!70!black, every mark/.append style={solid,fill=Set1-4-1},mark=*\\%
 Set1-4-2!70!black, every mark/.append style={solid,fill=Set1-4-2},mark=square*\\%
 Set1-4-3!70!black, every mark/.append style={solid,fill=Set1-4-3},mark=triangle*\\%
 Set1-4-4!70!black, every mark/.append style={solid,fill=Set1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-5}{%
 Set1-5-1!70!black, every mark/.append style={solid,fill=Set1-5-1},mark=*\\%
 Set1-5-2!70!black, every mark/.append style={solid,fill=Set1-5-2},mark=square*\\%
 Set1-5-3!70!black, every mark/.append style={solid,fill=Set1-5-3},mark=triangle*\\%
 Set1-5-4!70!black, every mark/.append style={solid,fill=Set1-5-4},mark=diamond*\\%
 Set1-5-5!70!black, every mark/.append style={solid,fill=Set1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-6}{%
 Set1-6-1!70!black, every mark/.append style={solid,fill=Set1-6-1},mark=*\\%
 Set1-6-2!70!black, every mark/.append style={solid,fill=Set1-6-2},mark=square*\\%
 Set1-6-3!70!black, every mark/.append style={solid,fill=Set1-6-3},mark=triangle*\\%
 Set1-6-4!70!black, every mark/.append style={solid,fill=Set1-6-4},mark=diamond*\\%
 Set1-6-5!70!black, every mark/.append style={solid,fill=Set1-6-5},mark=pentagon*\\%
 Set1-6-6!70!black, every mark/.append style={solid,fill=Set1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-7}{%
 Set1-7-1!70!black, every mark/.append style={solid,fill=Set1-7-1},mark=*\\%
 Set1-7-2!70!black, every mark/.append style={solid,fill=Set1-7-2},mark=square*\\%
 Set1-7-3!70!black, every mark/.append style={solid,fill=Set1-7-3},mark=triangle*\\%
 Set1-7-4!70!black, every mark/.append style={solid,fill=Set1-7-4},mark=diamond*\\%
 Set1-7-5!70!black, every mark/.append style={solid,fill=Set1-7-5},mark=pentagon*\\%
 Set1-7-6!70!black, every mark/.append style={solid,fill=Set1-7-6},mark=x\\%
 Set1-7-7!70!black, every mark/.append style={solid,fill=Set1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-8}{%
 Set1-8-1!70!black, every mark/.append style={solid,fill=Set1-8-1},mark=*\\%
 Set1-8-2!70!black, every mark/.append style={solid,fill=Set1-8-2},mark=square*\\%
 Set1-8-3!70!black, every mark/.append style={solid,fill=Set1-8-3},mark=triangle*\\%
 Set1-8-4!70!black, every mark/.append style={solid,fill=Set1-8-4},mark=diamond*\\%
 Set1-8-5!70!black, every mark/.append style={solid,fill=Set1-8-5},mark=pentagon*\\%
 Set1-8-6!70!black, every mark/.append style={solid,fill=Set1-8-6},mark=x\\%
 Set1-8-7!70!black, every mark/.append style={solid,fill=Set1-8-7},mark=+\\%
 Set1-8-8!70!black, every mark/.append style={solid,fill=Set1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-9}{%
 Set1-9-1!70!black, every mark/.append style={solid,fill=Set1-9-1},mark=*\\%
 Set1-9-2!70!black, every mark/.append style={solid,fill=Set1-9-2},mark=square*\\%
 Set1-9-3!70!black, every mark/.append style={solid,fill=Set1-9-3},mark=triangle*\\%
 Set1-9-4!70!black, every mark/.append style={solid,fill=Set1-9-4},mark=diamond*\\%
 Set1-9-5!70!black, every mark/.append style={solid,fill=Set1-9-5},mark=pentagon*\\%
 Set1-9-6!70!black, every mark/.append style={solid,fill=Set1-9-6},mark=x\\%
 Set1-9-7!70!black, every mark/.append style={solid,fill=Set1-9-7},mark=+\\%
 Set1-9-8!70!black, every mark/.append style={solid,fill=Set1-9-8},mark=star\\%
 Set1-9-9!70!black, every mark/.append style={solid,fill=Set1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-3}{%
 Pastel2-3-1!70!black, every mark/.append style={solid,fill=Pastel2-3-1},mark=*\\%
 Pastel2-3-2!70!black, every mark/.append style={solid,fill=Pastel2-3-2},mark=square*\\%
 Pastel2-3-3!70!black, every mark/.append style={solid,fill=Pastel2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-4}{%
 Pastel2-4-1!70!black, every mark/.append style={solid,fill=Pastel2-4-1},mark=*\\%
 Pastel2-4-2!70!black, every mark/.append style={solid,fill=Pastel2-4-2},mark=square*\\%
 Pastel2-4-3!70!black, every mark/.append style={solid,fill=Pastel2-4-3},mark=triangle*\\%
 Pastel2-4-4!70!black, every mark/.append style={solid,fill=Pastel2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-5}{%
 Pastel2-5-1!70!black, every mark/.append style={solid,fill=Pastel2-5-1},mark=*\\%
 Pastel2-5-2!70!black, every mark/.append style={solid,fill=Pastel2-5-2},mark=square*\\%
 Pastel2-5-3!70!black, every mark/.append style={solid,fill=Pastel2-5-3},mark=triangle*\\%
 Pastel2-5-4!70!black, every mark/.append style={solid,fill=Pastel2-5-4},mark=diamond*\\%
 Pastel2-5-5!70!black, every mark/.append style={solid,fill=Pastel2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-6}{%
 Pastel2-6-1!70!black, every mark/.append style={solid,fill=Pastel2-6-1},mark=*\\%
 Pastel2-6-2!70!black, every mark/.append style={solid,fill=Pastel2-6-2},mark=square*\\%
 Pastel2-6-3!70!black, every mark/.append style={solid,fill=Pastel2-6-3},mark=triangle*\\%
 Pastel2-6-4!70!black, every mark/.append style={solid,fill=Pastel2-6-4},mark=diamond*\\%
 Pastel2-6-5!70!black, every mark/.append style={solid,fill=Pastel2-6-5},mark=pentagon*\\%
 Pastel2-6-6!70!black, every mark/.append style={solid,fill=Pastel2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-7}{%
 Pastel2-7-1!70!black, every mark/.append style={solid,fill=Pastel2-7-1},mark=*\\%
 Pastel2-7-2!70!black, every mark/.append style={solid,fill=Pastel2-7-2},mark=square*\\%
 Pastel2-7-3!70!black, every mark/.append style={solid,fill=Pastel2-7-3},mark=triangle*\\%
 Pastel2-7-4!70!black, every mark/.append style={solid,fill=Pastel2-7-4},mark=diamond*\\%
 Pastel2-7-5!70!black, every mark/.append style={solid,fill=Pastel2-7-5},mark=pentagon*\\%
 Pastel2-7-6!70!black, every mark/.append style={solid,fill=Pastel2-7-6},mark=x\\%
 Pastel2-7-7!70!black, every mark/.append style={solid,fill=Pastel2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-8}{%
 Pastel2-8-1!70!black, every mark/.append style={solid,fill=Pastel2-8-1},mark=*\\%
 Pastel2-8-2!70!black, every mark/.append style={solid,fill=Pastel2-8-2},mark=square*\\%
 Pastel2-8-3!70!black, every mark/.append style={solid,fill=Pastel2-8-3},mark=triangle*\\%
 Pastel2-8-4!70!black, every mark/.append style={solid,fill=Pastel2-8-4},mark=diamond*\\%
 Pastel2-8-5!70!black, every mark/.append style={solid,fill=Pastel2-8-5},mark=pentagon*\\%
 Pastel2-8-6!70!black, every mark/.append style={solid,fill=Pastel2-8-6},mark=x\\%
 Pastel2-8-7!70!black, every mark/.append style={solid,fill=Pastel2-8-7},mark=+\\%
 Pastel2-8-8!70!black, every mark/.append style={solid,fill=Pastel2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-3}{%
 Set2-3-1!70!black, every mark/.append style={solid,fill=Set2-3-1},mark=*\\%
 Set2-3-2!70!black, every mark/.append style={solid,fill=Set2-3-2},mark=square*\\%
 Set2-3-3!70!black, every mark/.append style={solid,fill=Set2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-4}{%
 Set2-4-1!70!black, every mark/.append style={solid,fill=Set2-4-1},mark=*\\%
 Set2-4-2!70!black, every mark/.append style={solid,fill=Set2-4-2},mark=square*\\%
 Set2-4-3!70!black, every mark/.append style={solid,fill=Set2-4-3},mark=triangle*\\%
 Set2-4-4!70!black, every mark/.append style={solid,fill=Set2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-5}{%
 Set2-5-1!70!black, every mark/.append style={solid,fill=Set2-5-1},mark=*\\%
 Set2-5-2!70!black, every mark/.append style={solid,fill=Set2-5-2},mark=square*\\%
 Set2-5-3!70!black, every mark/.append style={solid,fill=Set2-5-3},mark=triangle*\\%
 Set2-5-4!70!black, every mark/.append style={solid,fill=Set2-5-4},mark=diamond*\\%
 Set2-5-5!70!black, every mark/.append style={solid,fill=Set2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-6}{%
 Set2-6-1!70!black, every mark/.append style={solid,fill=Set2-6-1},mark=*\\%
 Set2-6-2!70!black, every mark/.append style={solid,fill=Set2-6-2},mark=square*\\%
 Set2-6-3!70!black, every mark/.append style={solid,fill=Set2-6-3},mark=triangle*\\%
 Set2-6-4!70!black, every mark/.append style={solid,fill=Set2-6-4},mark=diamond*\\%
 Set2-6-5!70!black, every mark/.append style={solid,fill=Set2-6-5},mark=pentagon*\\%
 Set2-6-6!70!black, every mark/.append style={solid,fill=Set2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-7}{%
 Set2-7-1!70!black, every mark/.append style={solid,fill=Set2-7-1},mark=*\\%
 Set2-7-2!70!black, every mark/.append style={solid,fill=Set2-7-2},mark=square*\\%
 Set2-7-3!70!black, every mark/.append style={solid,fill=Set2-7-3},mark=triangle*\\%
 Set2-7-4!70!black, every mark/.append style={solid,fill=Set2-7-4},mark=diamond*\\%
 Set2-7-5!70!black, every mark/.append style={solid,fill=Set2-7-5},mark=pentagon*\\%
 Set2-7-6!70!black, every mark/.append style={solid,fill=Set2-7-6},mark=x\\%
 Set2-7-7!70!black, every mark/.append style={solid,fill=Set2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-8}{%
 Set2-8-1!70!black, every mark/.append style={solid,fill=Set2-8-1},mark=*\\%
 Set2-8-2!70!black, every mark/.append style={solid,fill=Set2-8-2},mark=square*\\%
 Set2-8-3!70!black, every mark/.append style={solid,fill=Set2-8-3},mark=triangle*\\%
 Set2-8-4!70!black, every mark/.append style={solid,fill=Set2-8-4},mark=diamond*\\%
 Set2-8-5!70!black, every mark/.append style={solid,fill=Set2-8-5},mark=pentagon*\\%
 Set2-8-6!70!black, every mark/.append style={solid,fill=Set2-8-6},mark=x\\%
 Set2-8-7!70!black, every mark/.append style={solid,fill=Set2-8-7},mark=+\\%
 Set2-8-8!70!black, every mark/.append style={solid,fill=Set2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-3}{%
 Dark2-3-1!70!black, every mark/.append style={solid,fill=Dark2-3-1},mark=*\\%
 Dark2-3-2!70!black, every mark/.append style={solid,fill=Dark2-3-2},mark=square*\\%
 Dark2-3-3!70!black, every mark/.append style={solid,fill=Dark2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-4}{%
 Dark2-4-1!70!black, every mark/.append style={solid,fill=Dark2-4-1},mark=*\\%
 Dark2-4-2!70!black, every mark/.append style={solid,fill=Dark2-4-2},mark=square*\\%
 Dark2-4-3!70!black, every mark/.append style={solid,fill=Dark2-4-3},mark=triangle*\\%
 Dark2-4-4!70!black, every mark/.append style={solid,fill=Dark2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-5}{%
 Dark2-5-1!70!black, every mark/.append style={solid,fill=Dark2-5-1},mark=*\\%
 Dark2-5-2!70!black, every mark/.append style={solid,fill=Dark2-5-2},mark=square*\\%
 Dark2-5-3!70!black, every mark/.append style={solid,fill=Dark2-5-3},mark=triangle*\\%
 Dark2-5-4!70!black, every mark/.append style={solid,fill=Dark2-5-4},mark=diamond*\\%
 Dark2-5-5!70!black, every mark/.append style={solid,fill=Dark2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-6}{%
 Dark2-6-1!70!black, every mark/.append style={solid,fill=Dark2-6-1},mark=*\\%
 Dark2-6-2!70!black, every mark/.append style={solid,fill=Dark2-6-2},mark=square*\\%
 Dark2-6-3!70!black, every mark/.append style={solid,fill=Dark2-6-3},mark=triangle*\\%
 Dark2-6-4!70!black, every mark/.append style={solid,fill=Dark2-6-4},mark=diamond*\\%
 Dark2-6-5!70!black, every mark/.append style={solid,fill=Dark2-6-5},mark=pentagon*\\%
 Dark2-6-6!70!black, every mark/.append style={solid,fill=Dark2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-7}{%
 Dark2-7-1!70!black, every mark/.append style={solid,fill=Dark2-7-1},mark=*\\%
 Dark2-7-2!70!black, every mark/.append style={solid,fill=Dark2-7-2},mark=square*\\%
 Dark2-7-3!70!black, every mark/.append style={solid,fill=Dark2-7-3},mark=triangle*\\%
 Dark2-7-4!70!black, every mark/.append style={solid,fill=Dark2-7-4},mark=diamond*\\%
 Dark2-7-5!70!black, every mark/.append style={solid,fill=Dark2-7-5},mark=pentagon*\\%
 Dark2-7-6!70!black, every mark/.append style={solid,fill=Dark2-7-6},mark=x\\%
 Dark2-7-7!70!black, every mark/.append style={solid,fill=Dark2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-8}{%
 Dark2-8-1!70!black, every mark/.append style={solid,fill=Dark2-8-1},mark=*\\%
 Dark2-8-2!70!black, every mark/.append style={solid,fill=Dark2-8-2},mark=square*\\%
 Dark2-8-3!70!black, every mark/.append style={solid,fill=Dark2-8-3},mark=triangle*\\%
 Dark2-8-4!70!black, every mark/.append style={solid,fill=Dark2-8-4},mark=diamond*\\%
 Dark2-8-5!70!black, every mark/.append style={solid,fill=Dark2-8-5},mark=pentagon*\\%
 Dark2-8-6!70!black, every mark/.append style={solid,fill=Dark2-8-6},mark=x\\%
 Dark2-8-7!70!black, every mark/.append style={solid,fill=Dark2-8-7},mark=+\\%
 Dark2-8-8!70!black, every mark/.append style={solid,fill=Dark2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-3}{%
 Paired-3-1!70!black, every mark/.append style={solid,fill=Paired-3-1},mark=*\\%
 Paired-3-2!70!black, every mark/.append style={solid,fill=Paired-3-2},mark=square*\\%
 Paired-3-3!70!black, every mark/.append style={solid,fill=Paired-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-4}{%
 Paired-4-1!70!black, every mark/.append style={solid,fill=Paired-4-1},mark=*\\%
 Paired-4-2!70!black, every mark/.append style={solid,fill=Paired-4-2},mark=square*\\%
 Paired-4-3!70!black, every mark/.append style={solid,fill=Paired-4-3},mark=triangle*\\%
 Paired-4-4!70!black, every mark/.append style={solid,fill=Paired-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-5}{%
 Paired-5-1!70!black, every mark/.append style={solid,fill=Paired-5-1},mark=*\\%
 Paired-5-2!70!black, every mark/.append style={solid,fill=Paired-5-2},mark=square*\\%
 Paired-5-3!70!black, every mark/.append style={solid,fill=Paired-5-3},mark=triangle*\\%
 Paired-5-4!70!black, every mark/.append style={solid,fill=Paired-5-4},mark=diamond*\\%
 Paired-5-5!70!black, every mark/.append style={solid,fill=Paired-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-6}{%
 Paired-6-1!70!black, every mark/.append style={solid,fill=Paired-6-1},mark=*\\%
 Paired-6-2!70!black, every mark/.append style={solid,fill=Paired-6-2},mark=square*\\%
 Paired-6-3!70!black, every mark/.append style={solid,fill=Paired-6-3},mark=triangle*\\%
 Paired-6-4!70!black, every mark/.append style={solid,fill=Paired-6-4},mark=diamond*\\%
 Paired-6-5!70!black, every mark/.append style={solid,fill=Paired-6-5},mark=pentagon*\\%
 Paired-6-6!70!black, every mark/.append style={solid,fill=Paired-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-7}{%
 Paired-7-1!70!black, every mark/.append style={solid,fill=Paired-7-1},mark=*\\%
 Paired-7-2!70!black, every mark/.append style={solid,fill=Paired-7-2},mark=square*\\%
 Paired-7-3!70!black, every mark/.append style={solid,fill=Paired-7-3},mark=triangle*\\%
 Paired-7-4!70!black, every mark/.append style={solid,fill=Paired-7-4},mark=diamond*\\%
 Paired-7-5!70!black, every mark/.append style={solid,fill=Paired-7-5},mark=pentagon*\\%
 Paired-7-6!70!black, every mark/.append style={solid,fill=Paired-7-6},mark=x\\%
 Paired-7-7!70!black, every mark/.append style={solid,fill=Paired-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-8}{%
 Paired-8-1!70!black, every mark/.append style={solid,fill=Paired-8-1},mark=*\\%
 Paired-8-2!70!black, every mark/.append style={solid,fill=Paired-8-2},mark=square*\\%
 Paired-8-3!70!black, every mark/.append style={solid,fill=Paired-8-3},mark=triangle*\\%
 Paired-8-4!70!black, every mark/.append style={solid,fill=Paired-8-4},mark=diamond*\\%
 Paired-8-5!70!black, every mark/.append style={solid,fill=Paired-8-5},mark=pentagon*\\%
 Paired-8-6!70!black, every mark/.append style={solid,fill=Paired-8-6},mark=x\\%
 Paired-8-7!70!black, every mark/.append style={solid,fill=Paired-8-7},mark=+\\%
 Paired-8-8!70!black, every mark/.append style={solid,fill=Paired-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-9}{%
 Paired-9-1!70!black, every mark/.append style={solid,fill=Paired-9-1},mark=*\\%
 Paired-9-2!70!black, every mark/.append style={solid,fill=Paired-9-2},mark=square*\\%
 Paired-9-3!70!black, every mark/.append style={solid,fill=Paired-9-3},mark=triangle*\\%
 Paired-9-4!70!black, every mark/.append style={solid,fill=Paired-9-4},mark=diamond*\\%
 Paired-9-5!70!black, every mark/.append style={solid,fill=Paired-9-5},mark=pentagon*\\%
 Paired-9-6!70!black, every mark/.append style={solid,fill=Paired-9-6},mark=x\\%
 Paired-9-7!70!black, every mark/.append style={solid,fill=Paired-9-7},mark=+\\%
 Paired-9-8!70!black, every mark/.append style={solid,fill=Paired-9-8},mark=star\\%
 Paired-9-9!70!black, every mark/.append style={solid,fill=Paired-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-10}{%
 Paired-10-1!70!black, every mark/.append style={solid,fill=Paired-10-1},mark=*\\%
 Paired-10-2!70!black, every mark/.append style={solid,fill=Paired-10-2},mark=square*\\%
 Paired-10-3!70!black, every mark/.append style={solid,fill=Paired-10-3},mark=triangle*\\%
 Paired-10-4!70!black, every mark/.append style={solid,fill=Paired-10-4},mark=diamond*\\%
 Paired-10-5!70!black, every mark/.append style={solid,fill=Paired-10-5},mark=pentagon*\\%
 Paired-10-6!70!black, every mark/.append style={solid,fill=Paired-10-6},mark=x\\%
 Paired-10-7!70!black, every mark/.append style={solid,fill=Paired-10-7},mark=+\\%
 Paired-10-8!70!black, every mark/.append style={solid,fill=Paired-10-8},mark=star\\%
 Paired-10-9!70!black, every mark/.append style={solid,fill=Paired-10-9},mark=oplus*\\%
 Paired-10-10!70!black, every mark/.append style={solid,fill=Paired-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-11}{%
 Paired-11-1!70!black, every mark/.append style={solid,fill=Paired-11-1},mark=*\\%
 Paired-11-2!70!black, every mark/.append style={solid,fill=Paired-11-2},mark=square*\\%
 Paired-11-3!70!black, every mark/.append style={solid,fill=Paired-11-3},mark=triangle*\\%
 Paired-11-4!70!black, every mark/.append style={solid,fill=Paired-11-4},mark=diamond*\\%
 Paired-11-5!70!black, every mark/.append style={solid,fill=Paired-11-5},mark=pentagon*\\%
 Paired-11-6!70!black, every mark/.append style={solid,fill=Paired-11-6},mark=x\\%
 Paired-11-7!70!black, every mark/.append style={solid,fill=Paired-11-7},mark=+\\%
 Paired-11-8!70!black, every mark/.append style={solid,fill=Paired-11-8},mark=star\\%
 Paired-11-9!70!black, every mark/.append style={solid,fill=Paired-11-9},mark=oplus*\\%
 Paired-11-10!70!black, every mark/.append style={solid,fill=Paired-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-12}{%
 Paired-12-1!70!black, every mark/.append style={solid,fill=Paired-12-1},mark=*\\%
 Paired-12-2!70!black, every mark/.append style={solid,fill=Paired-12-2},mark=square*\\%
 Paired-12-3!70!black, every mark/.append style={solid,fill=Paired-12-3},mark=triangle*\\%
 Paired-12-4!70!black, every mark/.append style={solid,fill=Paired-12-4},mark=diamond*\\%
 Paired-12-5!70!black, every mark/.append style={solid,fill=Paired-12-5},mark=pentagon*\\%
 Paired-12-6!70!black, every mark/.append style={solid,fill=Paired-12-6},mark=x\\%
 Paired-12-7!70!black, every mark/.append style={solid,fill=Paired-12-7},mark=+\\%
 Paired-12-8!70!black, every mark/.append style={solid,fill=Paired-12-8},mark=star\\%
 Paired-12-9!70!black, every mark/.append style={solid,fill=Paired-12-9},mark=oplus*\\%
 Paired-12-10!70!black, every mark/.append style={solid,fill=Paired-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-3}{%
 Accent-3-1!70!black, every mark/.append style={solid,fill=Accent-3-1},mark=*\\%
 Accent-3-2!70!black, every mark/.append style={solid,fill=Accent-3-2},mark=square*\\%
 Accent-3-3!70!black, every mark/.append style={solid,fill=Accent-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-4}{%
 Accent-4-1!70!black, every mark/.append style={solid,fill=Accent-4-1},mark=*\\%
 Accent-4-2!70!black, every mark/.append style={solid,fill=Accent-4-2},mark=square*\\%
 Accent-4-3!70!black, every mark/.append style={solid,fill=Accent-4-3},mark=triangle*\\%
 Accent-4-4!70!black, every mark/.append style={solid,fill=Accent-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-5}{%
 Accent-5-1!70!black, every mark/.append style={solid,fill=Accent-5-1},mark=*\\%
 Accent-5-2!70!black, every mark/.append style={solid,fill=Accent-5-2},mark=square*\\%
 Accent-5-3!70!black, every mark/.append style={solid,fill=Accent-5-3},mark=triangle*\\%
 Accent-5-4!70!black, every mark/.append style={solid,fill=Accent-5-4},mark=diamond*\\%
 Accent-5-5!70!black, every mark/.append style={solid,fill=Accent-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-6}{%
 Accent-6-1!70!black, every mark/.append style={solid,fill=Accent-6-1},mark=*\\%
 Accent-6-2!70!black, every mark/.append style={solid,fill=Accent-6-2},mark=square*\\%
 Accent-6-3!70!black, every mark/.append style={solid,fill=Accent-6-3},mark=triangle*\\%
 Accent-6-4!70!black, every mark/.append style={solid,fill=Accent-6-4},mark=diamond*\\%
 Accent-6-5!70!black, every mark/.append style={solid,fill=Accent-6-5},mark=pentagon*\\%
 Accent-6-6!70!black, every mark/.append style={solid,fill=Accent-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-7}{%
 Accent-7-1!70!black, every mark/.append style={solid,fill=Accent-7-1},mark=*\\%
 Accent-7-2!70!black, every mark/.append style={solid,fill=Accent-7-2},mark=square*\\%
 Accent-7-3!70!black, every mark/.append style={solid,fill=Accent-7-3},mark=triangle*\\%
 Accent-7-4!70!black, every mark/.append style={solid,fill=Accent-7-4},mark=diamond*\\%
 Accent-7-5!70!black, every mark/.append style={solid,fill=Accent-7-5},mark=pentagon*\\%
 Accent-7-6!70!black, every mark/.append style={solid,fill=Accent-7-6},mark=x\\%
 Accent-7-7!70!black, every mark/.append style={solid,fill=Accent-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-8}{%
 Accent-8-1!70!black, every mark/.append style={solid,fill=Accent-8-1},mark=*\\%
 Accent-8-2!70!black, every mark/.append style={solid,fill=Accent-8-2},mark=square*\\%
 Accent-8-3!70!black, every mark/.append style={solid,fill=Accent-8-3},mark=triangle*\\%
 Accent-8-4!70!black, every mark/.append style={solid,fill=Accent-8-4},mark=diamond*\\%
 Accent-8-5!70!black, every mark/.append style={solid,fill=Accent-8-5},mark=pentagon*\\%
 Accent-8-6!70!black, every mark/.append style={solid,fill=Accent-8-6},mark=x\\%
 Accent-8-7!70!black, every mark/.append style={solid,fill=Accent-8-7},mark=+\\%
 Accent-8-8!70!black, every mark/.append style={solid,fill=Accent-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-3}{%
 YlGn-3-1!70, every mark/.append style={solid,fill=YlGn-3-1},mark=*\\%
 YlGn-3-2!70, every mark/.append style={solid,fill=YlGn-3-2},mark=square*\\%
 YlGn-3-3!70, every mark/.append style={solid,fill=YlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-4}{%
 YlGn-4-1!70, every mark/.append style={solid,fill=YlGn-4-1},mark=*\\%
 YlGn-4-2!70, every mark/.append style={solid,fill=YlGn-4-2},mark=square*\\%
 YlGn-4-3!70, every mark/.append style={solid,fill=YlGn-4-3},mark=triangle*\\%
 YlGn-4-4!70, every mark/.append style={solid,fill=YlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-5}{%
 YlGn-5-1!70, every mark/.append style={solid,fill=YlGn-5-1},mark=*\\%
 YlGn-5-2!70, every mark/.append style={solid,fill=YlGn-5-2},mark=square*\\%
 YlGn-5-3!70, every mark/.append style={solid,fill=YlGn-5-3},mark=triangle*\\%
 YlGn-5-4!70, every mark/.append style={solid,fill=YlGn-5-4},mark=diamond*\\%
 YlGn-5-5!70, every mark/.append style={solid,fill=YlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-6}{%
 YlGn-6-1!70, every mark/.append style={solid,fill=YlGn-6-1},mark=*\\%
 YlGn-6-2!70, every mark/.append style={solid,fill=YlGn-6-2},mark=square*\\%
 YlGn-6-3!70, every mark/.append style={solid,fill=YlGn-6-3},mark=triangle*\\%
 YlGn-6-4!70, every mark/.append style={solid,fill=YlGn-6-4},mark=diamond*\\%
 YlGn-6-5!70, every mark/.append style={solid,fill=YlGn-6-5},mark=pentagon*\\%
 YlGn-6-6!70, every mark/.append style={solid,fill=YlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-7}{%
 YlGn-7-1!70, every mark/.append style={solid,fill=YlGn-7-1},mark=*\\%
 YlGn-7-2!70, every mark/.append style={solid,fill=YlGn-7-2},mark=square*\\%
 YlGn-7-3!70, every mark/.append style={solid,fill=YlGn-7-3},mark=triangle*\\%
 YlGn-7-4!70, every mark/.append style={solid,fill=YlGn-7-4},mark=diamond*\\%
 YlGn-7-5!70, every mark/.append style={solid,fill=YlGn-7-5},mark=pentagon*\\%
 YlGn-7-6!70, every mark/.append style={solid,fill=YlGn-7-6},mark=x\\%
 YlGn-7-7!70, every mark/.append style={solid,fill=YlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-8}{%
 YlGn-8-1!70, every mark/.append style={solid,fill=YlGn-8-1},mark=*\\%
 YlGn-8-2!70, every mark/.append style={solid,fill=YlGn-8-2},mark=square*\\%
 YlGn-8-3!70, every mark/.append style={solid,fill=YlGn-8-3},mark=triangle*\\%
 YlGn-8-4!70, every mark/.append style={solid,fill=YlGn-8-4},mark=diamond*\\%
 YlGn-8-5!70, every mark/.append style={solid,fill=YlGn-8-5},mark=pentagon*\\%
 YlGn-8-6!70, every mark/.append style={solid,fill=YlGn-8-6},mark=x\\%
 YlGn-8-7!70, every mark/.append style={solid,fill=YlGn-8-7},mark=+\\%
 YlGn-8-8!70, every mark/.append style={solid,fill=YlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-9}{%
 YlGn-9-1!70, every mark/.append style={solid,fill=YlGn-9-1},mark=*\\%
 YlGn-9-2!70, every mark/.append style={solid,fill=YlGn-9-2},mark=square*\\%
 YlGn-9-3!70, every mark/.append style={solid,fill=YlGn-9-3},mark=triangle*\\%
 YlGn-9-4!70, every mark/.append style={solid,fill=YlGn-9-4},mark=diamond*\\%
 YlGn-9-5!70, every mark/.append style={solid,fill=YlGn-9-5},mark=pentagon*\\%
 YlGn-9-6!70, every mark/.append style={solid,fill=YlGn-9-6},mark=x\\%
 YlGn-9-7!70, every mark/.append style={solid,fill=YlGn-9-7},mark=+\\%
 YlGn-9-8!70, every mark/.append style={solid,fill=YlGn-9-8},mark=star\\%
 YlGn-9-9!70, every mark/.append style={solid,fill=YlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-3}{%
 YlGnBu-3-1!70, every mark/.append style={solid,fill=YlGnBu-3-1},mark=*\\%
 YlGnBu-3-2!70, every mark/.append style={solid,fill=YlGnBu-3-2},mark=square*\\%
 YlGnBu-3-3!70, every mark/.append style={solid,fill=YlGnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-4}{%
 YlGnBu-4-1!70, every mark/.append style={solid,fill=YlGnBu-4-1},mark=*\\%
 YlGnBu-4-2!70, every mark/.append style={solid,fill=YlGnBu-4-2},mark=square*\\%
 YlGnBu-4-3!70, every mark/.append style={solid,fill=YlGnBu-4-3},mark=triangle*\\%
 YlGnBu-4-4!70, every mark/.append style={solid,fill=YlGnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-5}{%
 YlGnBu-5-1!70, every mark/.append style={solid,fill=YlGnBu-5-1},mark=*\\%
 YlGnBu-5-2!70, every mark/.append style={solid,fill=YlGnBu-5-2},mark=square*\\%
 YlGnBu-5-3!70, every mark/.append style={solid,fill=YlGnBu-5-3},mark=triangle*\\%
 YlGnBu-5-4!70, every mark/.append style={solid,fill=YlGnBu-5-4},mark=diamond*\\%
 YlGnBu-5-5!70, every mark/.append style={solid,fill=YlGnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-6}{%
 YlGnBu-6-1!70, every mark/.append style={solid,fill=YlGnBu-6-1},mark=*\\%
 YlGnBu-6-2!70, every mark/.append style={solid,fill=YlGnBu-6-2},mark=square*\\%
 YlGnBu-6-3!70, every mark/.append style={solid,fill=YlGnBu-6-3},mark=triangle*\\%
 YlGnBu-6-4!70, every mark/.append style={solid,fill=YlGnBu-6-4},mark=diamond*\\%
 YlGnBu-6-5!70, every mark/.append style={solid,fill=YlGnBu-6-5},mark=pentagon*\\%
 YlGnBu-6-6!70, every mark/.append style={solid,fill=YlGnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-7}{%
 YlGnBu-7-1!70, every mark/.append style={solid,fill=YlGnBu-7-1},mark=*\\%
 YlGnBu-7-2!70, every mark/.append style={solid,fill=YlGnBu-7-2},mark=square*\\%
 YlGnBu-7-3!70, every mark/.append style={solid,fill=YlGnBu-7-3},mark=triangle*\\%
 YlGnBu-7-4!70, every mark/.append style={solid,fill=YlGnBu-7-4},mark=diamond*\\%
 YlGnBu-7-5!70, every mark/.append style={solid,fill=YlGnBu-7-5},mark=pentagon*\\%
 YlGnBu-7-6!70, every mark/.append style={solid,fill=YlGnBu-7-6},mark=x\\%
 YlGnBu-7-7!70, every mark/.append style={solid,fill=YlGnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-8}{%
 YlGnBu-8-1!70, every mark/.append style={solid,fill=YlGnBu-8-1},mark=*\\%
 YlGnBu-8-2!70, every mark/.append style={solid,fill=YlGnBu-8-2},mark=square*\\%
 YlGnBu-8-3!70, every mark/.append style={solid,fill=YlGnBu-8-3},mark=triangle*\\%
 YlGnBu-8-4!70, every mark/.append style={solid,fill=YlGnBu-8-4},mark=diamond*\\%
 YlGnBu-8-5!70, every mark/.append style={solid,fill=YlGnBu-8-5},mark=pentagon*\\%
 YlGnBu-8-6!70, every mark/.append style={solid,fill=YlGnBu-8-6},mark=x\\%
 YlGnBu-8-7!70, every mark/.append style={solid,fill=YlGnBu-8-7},mark=+\\%
 YlGnBu-8-8!70, every mark/.append style={solid,fill=YlGnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-9}{%
 YlGnBu-9-1!70, every mark/.append style={solid,fill=YlGnBu-9-1},mark=*\\%
 YlGnBu-9-2!70, every mark/.append style={solid,fill=YlGnBu-9-2},mark=square*\\%
 YlGnBu-9-3!70, every mark/.append style={solid,fill=YlGnBu-9-3},mark=triangle*\\%
 YlGnBu-9-4!70, every mark/.append style={solid,fill=YlGnBu-9-4},mark=diamond*\\%
 YlGnBu-9-5!70, every mark/.append style={solid,fill=YlGnBu-9-5},mark=pentagon*\\%
 YlGnBu-9-6!70, every mark/.append style={solid,fill=YlGnBu-9-6},mark=x\\%
 YlGnBu-9-7!70, every mark/.append style={solid,fill=YlGnBu-9-7},mark=+\\%
 YlGnBu-9-8!70, every mark/.append style={solid,fill=YlGnBu-9-8},mark=star\\%
 YlGnBu-9-9!70, every mark/.append style={solid,fill=YlGnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-3}{%
 GnBu-3-1!70, every mark/.append style={solid,fill=GnBu-3-1},mark=*\\%
 GnBu-3-2!70, every mark/.append style={solid,fill=GnBu-3-2},mark=square*\\%
 GnBu-3-3!70, every mark/.append style={solid,fill=GnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-4}{%
 GnBu-4-1!70, every mark/.append style={solid,fill=GnBu-4-1},mark=*\\%
 GnBu-4-2!70, every mark/.append style={solid,fill=GnBu-4-2},mark=square*\\%
 GnBu-4-3!70, every mark/.append style={solid,fill=GnBu-4-3},mark=triangle*\\%
 GnBu-4-4!70, every mark/.append style={solid,fill=GnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-5}{%
 GnBu-5-1!70, every mark/.append style={solid,fill=GnBu-5-1},mark=*\\%
 GnBu-5-2!70, every mark/.append style={solid,fill=GnBu-5-2},mark=square*\\%
 GnBu-5-3!70, every mark/.append style={solid,fill=GnBu-5-3},mark=triangle*\\%
 GnBu-5-4!70, every mark/.append style={solid,fill=GnBu-5-4},mark=diamond*\\%
 GnBu-5-5!70, every mark/.append style={solid,fill=GnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-6}{%
 GnBu-6-1!70, every mark/.append style={solid,fill=GnBu-6-1},mark=*\\%
 GnBu-6-2!70, every mark/.append style={solid,fill=GnBu-6-2},mark=square*\\%
 GnBu-6-3!70, every mark/.append style={solid,fill=GnBu-6-3},mark=triangle*\\%
 GnBu-6-4!70, every mark/.append style={solid,fill=GnBu-6-4},mark=diamond*\\%
 GnBu-6-5!70, every mark/.append style={solid,fill=GnBu-6-5},mark=pentagon*\\%
 GnBu-6-6!70, every mark/.append style={solid,fill=GnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-7}{%
 GnBu-7-1!70, every mark/.append style={solid,fill=GnBu-7-1},mark=*\\%
 GnBu-7-2!70, every mark/.append style={solid,fill=GnBu-7-2},mark=square*\\%
 GnBu-7-3!70, every mark/.append style={solid,fill=GnBu-7-3},mark=triangle*\\%
 GnBu-7-4!70, every mark/.append style={solid,fill=GnBu-7-4},mark=diamond*\\%
 GnBu-7-5!70, every mark/.append style={solid,fill=GnBu-7-5},mark=pentagon*\\%
 GnBu-7-6!70, every mark/.append style={solid,fill=GnBu-7-6},mark=x\\%
 GnBu-7-7!70, every mark/.append style={solid,fill=GnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-8}{%
 GnBu-8-1!70, every mark/.append style={solid,fill=GnBu-8-1},mark=*\\%
 GnBu-8-2!70, every mark/.append style={solid,fill=GnBu-8-2},mark=square*\\%
 GnBu-8-3!70, every mark/.append style={solid,fill=GnBu-8-3},mark=triangle*\\%
 GnBu-8-4!70, every mark/.append style={solid,fill=GnBu-8-4},mark=diamond*\\%
 GnBu-8-5!70, every mark/.append style={solid,fill=GnBu-8-5},mark=pentagon*\\%
 GnBu-8-6!70, every mark/.append style={solid,fill=GnBu-8-6},mark=x\\%
 GnBu-8-7!70, every mark/.append style={solid,fill=GnBu-8-7},mark=+\\%
 GnBu-8-8!70, every mark/.append style={solid,fill=GnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-9}{%
 GnBu-9-1!70, every mark/.append style={solid,fill=GnBu-9-1},mark=*\\%
 GnBu-9-2!70, every mark/.append style={solid,fill=GnBu-9-2},mark=square*\\%
 GnBu-9-3!70, every mark/.append style={solid,fill=GnBu-9-3},mark=triangle*\\%
 GnBu-9-4!70, every mark/.append style={solid,fill=GnBu-9-4},mark=diamond*\\%
 GnBu-9-5!70, every mark/.append style={solid,fill=GnBu-9-5},mark=pentagon*\\%
 GnBu-9-6!70, every mark/.append style={solid,fill=GnBu-9-6},mark=x\\%
 GnBu-9-7!70, every mark/.append style={solid,fill=GnBu-9-7},mark=+\\%
 GnBu-9-8!70, every mark/.append style={solid,fill=GnBu-9-8},mark=star\\%
 GnBu-9-9!70, every mark/.append style={solid,fill=GnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-3}{%
 BuGn-3-1!70, every mark/.append style={solid,fill=BuGn-3-1},mark=*\\%
 BuGn-3-2!70, every mark/.append style={solid,fill=BuGn-3-2},mark=square*\\%
 BuGn-3-3!70, every mark/.append style={solid,fill=BuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-4}{%
 BuGn-4-1!70, every mark/.append style={solid,fill=BuGn-4-1},mark=*\\%
 BuGn-4-2!70, every mark/.append style={solid,fill=BuGn-4-2},mark=square*\\%
 BuGn-4-3!70, every mark/.append style={solid,fill=BuGn-4-3},mark=triangle*\\%
 BuGn-4-4!70, every mark/.append style={solid,fill=BuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-5}{%
 BuGn-5-1!70, every mark/.append style={solid,fill=BuGn-5-1},mark=*\\%
 BuGn-5-2!70, every mark/.append style={solid,fill=BuGn-5-2},mark=square*\\%
 BuGn-5-3!70, every mark/.append style={solid,fill=BuGn-5-3},mark=triangle*\\%
 BuGn-5-4!70, every mark/.append style={solid,fill=BuGn-5-4},mark=diamond*\\%
 BuGn-5-5!70, every mark/.append style={solid,fill=BuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-6}{%
 BuGn-6-1!70, every mark/.append style={solid,fill=BuGn-6-1},mark=*\\%
 BuGn-6-2!70, every mark/.append style={solid,fill=BuGn-6-2},mark=square*\\%
 BuGn-6-3!70, every mark/.append style={solid,fill=BuGn-6-3},mark=triangle*\\%
 BuGn-6-4!70, every mark/.append style={solid,fill=BuGn-6-4},mark=diamond*\\%
 BuGn-6-5!70, every mark/.append style={solid,fill=BuGn-6-5},mark=pentagon*\\%
 BuGn-6-6!70, every mark/.append style={solid,fill=BuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-7}{%
 BuGn-7-1!70, every mark/.append style={solid,fill=BuGn-7-1},mark=*\\%
 BuGn-7-2!70, every mark/.append style={solid,fill=BuGn-7-2},mark=square*\\%
 BuGn-7-3!70, every mark/.append style={solid,fill=BuGn-7-3},mark=triangle*\\%
 BuGn-7-4!70, every mark/.append style={solid,fill=BuGn-7-4},mark=diamond*\\%
 BuGn-7-5!70, every mark/.append style={solid,fill=BuGn-7-5},mark=pentagon*\\%
 BuGn-7-6!70, every mark/.append style={solid,fill=BuGn-7-6},mark=x\\%
 BuGn-7-7!70, every mark/.append style={solid,fill=BuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-8}{%
 BuGn-8-1!70, every mark/.append style={solid,fill=BuGn-8-1},mark=*\\%
 BuGn-8-2!70, every mark/.append style={solid,fill=BuGn-8-2},mark=square*\\%
 BuGn-8-3!70, every mark/.append style={solid,fill=BuGn-8-3},mark=triangle*\\%
 BuGn-8-4!70, every mark/.append style={solid,fill=BuGn-8-4},mark=diamond*\\%
 BuGn-8-5!70, every mark/.append style={solid,fill=BuGn-8-5},mark=pentagon*\\%
 BuGn-8-6!70, every mark/.append style={solid,fill=BuGn-8-6},mark=x\\%
 BuGn-8-7!70, every mark/.append style={solid,fill=BuGn-8-7},mark=+\\%
 BuGn-8-8!70, every mark/.append style={solid,fill=BuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-9}{%
 BuGn-9-1!70, every mark/.append style={solid,fill=BuGn-9-1},mark=*\\%
 BuGn-9-2!70, every mark/.append style={solid,fill=BuGn-9-2},mark=square*\\%
 BuGn-9-3!70, every mark/.append style={solid,fill=BuGn-9-3},mark=triangle*\\%
 BuGn-9-4!70, every mark/.append style={solid,fill=BuGn-9-4},mark=diamond*\\%
 BuGn-9-5!70, every mark/.append style={solid,fill=BuGn-9-5},mark=pentagon*\\%
 BuGn-9-6!70, every mark/.append style={solid,fill=BuGn-9-6},mark=x\\%
 BuGn-9-7!70, every mark/.append style={solid,fill=BuGn-9-7},mark=+\\%
 BuGn-9-8!70, every mark/.append style={solid,fill=BuGn-9-8},mark=star\\%
 BuGn-9-9!70, every mark/.append style={solid,fill=BuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-3}{%
 PuBuGn-3-1!70, every mark/.append style={solid,fill=PuBuGn-3-1},mark=*\\%
 PuBuGn-3-2!70, every mark/.append style={solid,fill=PuBuGn-3-2},mark=square*\\%
 PuBuGn-3-3!70, every mark/.append style={solid,fill=PuBuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-4}{%
 PuBuGn-4-1!70, every mark/.append style={solid,fill=PuBuGn-4-1},mark=*\\%
 PuBuGn-4-2!70, every mark/.append style={solid,fill=PuBuGn-4-2},mark=square*\\%
 PuBuGn-4-3!70, every mark/.append style={solid,fill=PuBuGn-4-3},mark=triangle*\\%
 PuBuGn-4-4!70, every mark/.append style={solid,fill=PuBuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-5}{%
 PuBuGn-5-1!70, every mark/.append style={solid,fill=PuBuGn-5-1},mark=*\\%
 PuBuGn-5-2!70, every mark/.append style={solid,fill=PuBuGn-5-2},mark=square*\\%
 PuBuGn-5-3!70, every mark/.append style={solid,fill=PuBuGn-5-3},mark=triangle*\\%
 PuBuGn-5-4!70, every mark/.append style={solid,fill=PuBuGn-5-4},mark=diamond*\\%
 PuBuGn-5-5!70, every mark/.append style={solid,fill=PuBuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-6}{%
 PuBuGn-6-1!70, every mark/.append style={solid,fill=PuBuGn-6-1},mark=*\\%
 PuBuGn-6-2!70, every mark/.append style={solid,fill=PuBuGn-6-2},mark=square*\\%
 PuBuGn-6-3!70, every mark/.append style={solid,fill=PuBuGn-6-3},mark=triangle*\\%
 PuBuGn-6-4!70, every mark/.append style={solid,fill=PuBuGn-6-4},mark=diamond*\\%
 PuBuGn-6-5!70, every mark/.append style={solid,fill=PuBuGn-6-5},mark=pentagon*\\%
 PuBuGn-6-6!70, every mark/.append style={solid,fill=PuBuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-7}{%
 PuBuGn-7-1!70, every mark/.append style={solid,fill=PuBuGn-7-1},mark=*\\%
 PuBuGn-7-2!70, every mark/.append style={solid,fill=PuBuGn-7-2},mark=square*\\%
 PuBuGn-7-3!70, every mark/.append style={solid,fill=PuBuGn-7-3},mark=triangle*\\%
 PuBuGn-7-4!70, every mark/.append style={solid,fill=PuBuGn-7-4},mark=diamond*\\%
 PuBuGn-7-5!70, every mark/.append style={solid,fill=PuBuGn-7-5},mark=pentagon*\\%
 PuBuGn-7-6!70, every mark/.append style={solid,fill=PuBuGn-7-6},mark=x\\%
 PuBuGn-7-7!70, every mark/.append style={solid,fill=PuBuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-8}{%
 PuBuGn-8-1!70, every mark/.append style={solid,fill=PuBuGn-8-1},mark=*\\%
 PuBuGn-8-2!70, every mark/.append style={solid,fill=PuBuGn-8-2},mark=square*\\%
 PuBuGn-8-3!70, every mark/.append style={solid,fill=PuBuGn-8-3},mark=triangle*\\%
 PuBuGn-8-4!70, every mark/.append style={solid,fill=PuBuGn-8-4},mark=diamond*\\%
 PuBuGn-8-5!70, every mark/.append style={solid,fill=PuBuGn-8-5},mark=pentagon*\\%
 PuBuGn-8-6!70, every mark/.append style={solid,fill=PuBuGn-8-6},mark=x\\%
 PuBuGn-8-7!70, every mark/.append style={solid,fill=PuBuGn-8-7},mark=+\\%
 PuBuGn-8-8!70, every mark/.append style={solid,fill=PuBuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-9}{%
 PuBuGn-9-1!70, every mark/.append style={solid,fill=PuBuGn-9-1},mark=*\\%
 PuBuGn-9-2!70, every mark/.append style={solid,fill=PuBuGn-9-2},mark=square*\\%
 PuBuGn-9-3!70, every mark/.append style={solid,fill=PuBuGn-9-3},mark=triangle*\\%
 PuBuGn-9-4!70, every mark/.append style={solid,fill=PuBuGn-9-4},mark=diamond*\\%
 PuBuGn-9-5!70, every mark/.append style={solid,fill=PuBuGn-9-5},mark=pentagon*\\%
 PuBuGn-9-6!70, every mark/.append style={solid,fill=PuBuGn-9-6},mark=x\\%
 PuBuGn-9-7!70, every mark/.append style={solid,fill=PuBuGn-9-7},mark=+\\%
 PuBuGn-9-8!70, every mark/.append style={solid,fill=PuBuGn-9-8},mark=star\\%
 PuBuGn-9-9!70, every mark/.append style={solid,fill=PuBuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-3}{%
 PuBu-3-1!70, every mark/.append style={solid,fill=PuBu-3-1},mark=*\\%
 PuBu-3-2!70, every mark/.append style={solid,fill=PuBu-3-2},mark=square*\\%
 PuBu-3-3!70, every mark/.append style={solid,fill=PuBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-4}{%
 PuBu-4-1!70, every mark/.append style={solid,fill=PuBu-4-1},mark=*\\%
 PuBu-4-2!70, every mark/.append style={solid,fill=PuBu-4-2},mark=square*\\%
 PuBu-4-3!70, every mark/.append style={solid,fill=PuBu-4-3},mark=triangle*\\%
 PuBu-4-4!70, every mark/.append style={solid,fill=PuBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-5}{%
 PuBu-5-1!70, every mark/.append style={solid,fill=PuBu-5-1},mark=*\\%
 PuBu-5-2!70, every mark/.append style={solid,fill=PuBu-5-2},mark=square*\\%
 PuBu-5-3!70, every mark/.append style={solid,fill=PuBu-5-3},mark=triangle*\\%
 PuBu-5-4!70, every mark/.append style={solid,fill=PuBu-5-4},mark=diamond*\\%
 PuBu-5-5!70, every mark/.append style={solid,fill=PuBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-6}{%
 PuBu-6-1!70, every mark/.append style={solid,fill=PuBu-6-1},mark=*\\%
 PuBu-6-2!70, every mark/.append style={solid,fill=PuBu-6-2},mark=square*\\%
 PuBu-6-3!70, every mark/.append style={solid,fill=PuBu-6-3},mark=triangle*\\%
 PuBu-6-4!70, every mark/.append style={solid,fill=PuBu-6-4},mark=diamond*\\%
 PuBu-6-5!70, every mark/.append style={solid,fill=PuBu-6-5},mark=pentagon*\\%
 PuBu-6-6!70, every mark/.append style={solid,fill=PuBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-7}{%
 PuBu-7-1!70, every mark/.append style={solid,fill=PuBu-7-1},mark=*\\%
 PuBu-7-2!70, every mark/.append style={solid,fill=PuBu-7-2},mark=square*\\%
 PuBu-7-3!70, every mark/.append style={solid,fill=PuBu-7-3},mark=triangle*\\%
 PuBu-7-4!70, every mark/.append style={solid,fill=PuBu-7-4},mark=diamond*\\%
 PuBu-7-5!70, every mark/.append style={solid,fill=PuBu-7-5},mark=pentagon*\\%
 PuBu-7-6!70, every mark/.append style={solid,fill=PuBu-7-6},mark=x\\%
 PuBu-7-7!70, every mark/.append style={solid,fill=PuBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-8}{%
 PuBu-8-1!70, every mark/.append style={solid,fill=PuBu-8-1},mark=*\\%
 PuBu-8-2!70, every mark/.append style={solid,fill=PuBu-8-2},mark=square*\\%
 PuBu-8-3!70, every mark/.append style={solid,fill=PuBu-8-3},mark=triangle*\\%
 PuBu-8-4!70, every mark/.append style={solid,fill=PuBu-8-4},mark=diamond*\\%
 PuBu-8-5!70, every mark/.append style={solid,fill=PuBu-8-5},mark=pentagon*\\%
 PuBu-8-6!70, every mark/.append style={solid,fill=PuBu-8-6},mark=x\\%
 PuBu-8-7!70, every mark/.append style={solid,fill=PuBu-8-7},mark=+\\%
 PuBu-8-8!70, every mark/.append style={solid,fill=PuBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-9}{%
 PuBu-9-1!70, every mark/.append style={solid,fill=PuBu-9-1},mark=*\\%
 PuBu-9-2!70, every mark/.append style={solid,fill=PuBu-9-2},mark=square*\\%
 PuBu-9-3!70, every mark/.append style={solid,fill=PuBu-9-3},mark=triangle*\\%
 PuBu-9-4!70, every mark/.append style={solid,fill=PuBu-9-4},mark=diamond*\\%
 PuBu-9-5!70, every mark/.append style={solid,fill=PuBu-9-5},mark=pentagon*\\%
 PuBu-9-6!70, every mark/.append style={solid,fill=PuBu-9-6},mark=x\\%
 PuBu-9-7!70, every mark/.append style={solid,fill=PuBu-9-7},mark=+\\%
 PuBu-9-8!70, every mark/.append style={solid,fill=PuBu-9-8},mark=star\\%
 PuBu-9-9!70, every mark/.append style={solid,fill=PuBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-3}{%
 BuPu-3-1!70, every mark/.append style={solid,fill=BuPu-3-1},mark=*\\%
 BuPu-3-2!70, every mark/.append style={solid,fill=BuPu-3-2},mark=square*\\%
 BuPu-3-3!70, every mark/.append style={solid,fill=BuPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-4}{%
 BuPu-4-1!70, every mark/.append style={solid,fill=BuPu-4-1},mark=*\\%
 BuPu-4-2!70, every mark/.append style={solid,fill=BuPu-4-2},mark=square*\\%
 BuPu-4-3!70, every mark/.append style={solid,fill=BuPu-4-3},mark=triangle*\\%
 BuPu-4-4!70, every mark/.append style={solid,fill=BuPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-5}{%
 BuPu-5-1!70, every mark/.append style={solid,fill=BuPu-5-1},mark=*\\%
 BuPu-5-2!70, every mark/.append style={solid,fill=BuPu-5-2},mark=square*\\%
 BuPu-5-3!70, every mark/.append style={solid,fill=BuPu-5-3},mark=triangle*\\%
 BuPu-5-4!70, every mark/.append style={solid,fill=BuPu-5-4},mark=diamond*\\%
 BuPu-5-5!70, every mark/.append style={solid,fill=BuPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-6}{%
 BuPu-6-1!70, every mark/.append style={solid,fill=BuPu-6-1},mark=*\\%
 BuPu-6-2!70, every mark/.append style={solid,fill=BuPu-6-2},mark=square*\\%
 BuPu-6-3!70, every mark/.append style={solid,fill=BuPu-6-3},mark=triangle*\\%
 BuPu-6-4!70, every mark/.append style={solid,fill=BuPu-6-4},mark=diamond*\\%
 BuPu-6-5!70, every mark/.append style={solid,fill=BuPu-6-5},mark=pentagon*\\%
 BuPu-6-6!70, every mark/.append style={solid,fill=BuPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-7}{%
 BuPu-7-1!70, every mark/.append style={solid,fill=BuPu-7-1},mark=*\\%
 BuPu-7-2!70, every mark/.append style={solid,fill=BuPu-7-2},mark=square*\\%
 BuPu-7-3!70, every mark/.append style={solid,fill=BuPu-7-3},mark=triangle*\\%
 BuPu-7-4!70, every mark/.append style={solid,fill=BuPu-7-4},mark=diamond*\\%
 BuPu-7-5!70, every mark/.append style={solid,fill=BuPu-7-5},mark=pentagon*\\%
 BuPu-7-6!70, every mark/.append style={solid,fill=BuPu-7-6},mark=x\\%
 BuPu-7-7!70, every mark/.append style={solid,fill=BuPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-8}{%
 BuPu-8-1!70, every mark/.append style={solid,fill=BuPu-8-1},mark=*\\%
 BuPu-8-2!70, every mark/.append style={solid,fill=BuPu-8-2},mark=square*\\%
 BuPu-8-3!70, every mark/.append style={solid,fill=BuPu-8-3},mark=triangle*\\%
 BuPu-8-4!70, every mark/.append style={solid,fill=BuPu-8-4},mark=diamond*\\%
 BuPu-8-5!70, every mark/.append style={solid,fill=BuPu-8-5},mark=pentagon*\\%
 BuPu-8-6!70, every mark/.append style={solid,fill=BuPu-8-6},mark=x\\%
 BuPu-8-7!70, every mark/.append style={solid,fill=BuPu-8-7},mark=+\\%
 BuPu-8-8!70, every mark/.append style={solid,fill=BuPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-9}{%
 BuPu-9-1!70, every mark/.append style={solid,fill=BuPu-9-1},mark=*\\%
 BuPu-9-2!70, every mark/.append style={solid,fill=BuPu-9-2},mark=square*\\%
 BuPu-9-3!70, every mark/.append style={solid,fill=BuPu-9-3},mark=triangle*\\%
 BuPu-9-4!70, every mark/.append style={solid,fill=BuPu-9-4},mark=diamond*\\%
 BuPu-9-5!70, every mark/.append style={solid,fill=BuPu-9-5},mark=pentagon*\\%
 BuPu-9-6!70, every mark/.append style={solid,fill=BuPu-9-6},mark=x\\%
 BuPu-9-7!70, every mark/.append style={solid,fill=BuPu-9-7},mark=+\\%
 BuPu-9-8!70, every mark/.append style={solid,fill=BuPu-9-8},mark=star\\%
 BuPu-9-9!70, every mark/.append style={solid,fill=BuPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-3}{%
 RdPu-3-1!70, every mark/.append style={solid,fill=RdPu-3-1},mark=*\\%
 RdPu-3-2!70, every mark/.append style={solid,fill=RdPu-3-2},mark=square*\\%
 RdPu-3-3!70, every mark/.append style={solid,fill=RdPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-4}{%
 RdPu-4-1!70, every mark/.append style={solid,fill=RdPu-4-1},mark=*\\%
 RdPu-4-2!70, every mark/.append style={solid,fill=RdPu-4-2},mark=square*\\%
 RdPu-4-3!70, every mark/.append style={solid,fill=RdPu-4-3},mark=triangle*\\%
 RdPu-4-4!70, every mark/.append style={solid,fill=RdPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-5}{%
 RdPu-5-1!70, every mark/.append style={solid,fill=RdPu-5-1},mark=*\\%
 RdPu-5-2!70, every mark/.append style={solid,fill=RdPu-5-2},mark=square*\\%
 RdPu-5-3!70, every mark/.append style={solid,fill=RdPu-5-3},mark=triangle*\\%
 RdPu-5-4!70, every mark/.append style={solid,fill=RdPu-5-4},mark=diamond*\\%
 RdPu-5-5!70, every mark/.append style={solid,fill=RdPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-6}{%
 RdPu-6-1!70, every mark/.append style={solid,fill=RdPu-6-1},mark=*\\%
 RdPu-6-2!70, every mark/.append style={solid,fill=RdPu-6-2},mark=square*\\%
 RdPu-6-3!70, every mark/.append style={solid,fill=RdPu-6-3},mark=triangle*\\%
 RdPu-6-4!70, every mark/.append style={solid,fill=RdPu-6-4},mark=diamond*\\%
 RdPu-6-5!70, every mark/.append style={solid,fill=RdPu-6-5},mark=pentagon*\\%
 RdPu-6-6!70, every mark/.append style={solid,fill=RdPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-7}{%
 RdPu-7-1!70, every mark/.append style={solid,fill=RdPu-7-1},mark=*\\%
 RdPu-7-2!70, every mark/.append style={solid,fill=RdPu-7-2},mark=square*\\%
 RdPu-7-3!70, every mark/.append style={solid,fill=RdPu-7-3},mark=triangle*\\%
 RdPu-7-4!70, every mark/.append style={solid,fill=RdPu-7-4},mark=diamond*\\%
 RdPu-7-5!70, every mark/.append style={solid,fill=RdPu-7-5},mark=pentagon*\\%
 RdPu-7-6!70, every mark/.append style={solid,fill=RdPu-7-6},mark=x\\%
 RdPu-7-7!70, every mark/.append style={solid,fill=RdPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-8}{%
 RdPu-8-1!70, every mark/.append style={solid,fill=RdPu-8-1},mark=*\\%
 RdPu-8-2!70, every mark/.append style={solid,fill=RdPu-8-2},mark=square*\\%
 RdPu-8-3!70, every mark/.append style={solid,fill=RdPu-8-3},mark=triangle*\\%
 RdPu-8-4!70, every mark/.append style={solid,fill=RdPu-8-4},mark=diamond*\\%
 RdPu-8-5!70, every mark/.append style={solid,fill=RdPu-8-5},mark=pentagon*\\%
 RdPu-8-6!70, every mark/.append style={solid,fill=RdPu-8-6},mark=x\\%
 RdPu-8-7!70, every mark/.append style={solid,fill=RdPu-8-7},mark=+\\%
 RdPu-8-8!70, every mark/.append style={solid,fill=RdPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-9}{%
 RdPu-9-1!70, every mark/.append style={solid,fill=RdPu-9-1},mark=*\\%
 RdPu-9-2!70, every mark/.append style={solid,fill=RdPu-9-2},mark=square*\\%
 RdPu-9-3!70, every mark/.append style={solid,fill=RdPu-9-3},mark=triangle*\\%
 RdPu-9-4!70, every mark/.append style={solid,fill=RdPu-9-4},mark=diamond*\\%
 RdPu-9-5!70, every mark/.append style={solid,fill=RdPu-9-5},mark=pentagon*\\%
 RdPu-9-6!70, every mark/.append style={solid,fill=RdPu-9-6},mark=x\\%
 RdPu-9-7!70, every mark/.append style={solid,fill=RdPu-9-7},mark=+\\%
 RdPu-9-8!70, every mark/.append style={solid,fill=RdPu-9-8},mark=star\\%
 RdPu-9-9!70, every mark/.append style={solid,fill=RdPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-3}{%
 PuRd-3-1!70, every mark/.append style={solid,fill=PuRd-3-1},mark=*\\%
 PuRd-3-2!70, every mark/.append style={solid,fill=PuRd-3-2},mark=square*\\%
 PuRd-3-3!70, every mark/.append style={solid,fill=PuRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-4}{%
 PuRd-4-1!70, every mark/.append style={solid,fill=PuRd-4-1},mark=*\\%
 PuRd-4-2!70, every mark/.append style={solid,fill=PuRd-4-2},mark=square*\\%
 PuRd-4-3!70, every mark/.append style={solid,fill=PuRd-4-3},mark=triangle*\\%
 PuRd-4-4!70, every mark/.append style={solid,fill=PuRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-5}{%
 PuRd-5-1!70, every mark/.append style={solid,fill=PuRd-5-1},mark=*\\%
 PuRd-5-2!70, every mark/.append style={solid,fill=PuRd-5-2},mark=square*\\%
 PuRd-5-3!70, every mark/.append style={solid,fill=PuRd-5-3},mark=triangle*\\%
 PuRd-5-4!70, every mark/.append style={solid,fill=PuRd-5-4},mark=diamond*\\%
 PuRd-5-5!70, every mark/.append style={solid,fill=PuRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-6}{%
 PuRd-6-1!70, every mark/.append style={solid,fill=PuRd-6-1},mark=*\\%
 PuRd-6-2!70, every mark/.append style={solid,fill=PuRd-6-2},mark=square*\\%
 PuRd-6-3!70, every mark/.append style={solid,fill=PuRd-6-3},mark=triangle*\\%
 PuRd-6-4!70, every mark/.append style={solid,fill=PuRd-6-4},mark=diamond*\\%
 PuRd-6-5!70, every mark/.append style={solid,fill=PuRd-6-5},mark=pentagon*\\%
 PuRd-6-6!70, every mark/.append style={solid,fill=PuRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-7}{%
 PuRd-7-1!70, every mark/.append style={solid,fill=PuRd-7-1},mark=*\\%
 PuRd-7-2!70, every mark/.append style={solid,fill=PuRd-7-2},mark=square*\\%
 PuRd-7-3!70, every mark/.append style={solid,fill=PuRd-7-3},mark=triangle*\\%
 PuRd-7-4!70, every mark/.append style={solid,fill=PuRd-7-4},mark=diamond*\\%
 PuRd-7-5!70, every mark/.append style={solid,fill=PuRd-7-5},mark=pentagon*\\%
 PuRd-7-6!70, every mark/.append style={solid,fill=PuRd-7-6},mark=x\\%
 PuRd-7-7!70, every mark/.append style={solid,fill=PuRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-8}{%
 PuRd-8-1!70, every mark/.append style={solid,fill=PuRd-8-1},mark=*\\%
 PuRd-8-2!70, every mark/.append style={solid,fill=PuRd-8-2},mark=square*\\%
 PuRd-8-3!70, every mark/.append style={solid,fill=PuRd-8-3},mark=triangle*\\%
 PuRd-8-4!70, every mark/.append style={solid,fill=PuRd-8-4},mark=diamond*\\%
 PuRd-8-5!70, every mark/.append style={solid,fill=PuRd-8-5},mark=pentagon*\\%
 PuRd-8-6!70, every mark/.append style={solid,fill=PuRd-8-6},mark=x\\%
 PuRd-8-7!70, every mark/.append style={solid,fill=PuRd-8-7},mark=+\\%
 PuRd-8-8!70, every mark/.append style={solid,fill=PuRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-9}{%
 PuRd-9-1!70, every mark/.append style={solid,fill=PuRd-9-1},mark=*\\%
 PuRd-9-2!70, every mark/.append style={solid,fill=PuRd-9-2},mark=square*\\%
 PuRd-9-3!70, every mark/.append style={solid,fill=PuRd-9-3},mark=triangle*\\%
 PuRd-9-4!70, every mark/.append style={solid,fill=PuRd-9-4},mark=diamond*\\%
 PuRd-9-5!70, every mark/.append style={solid,fill=PuRd-9-5},mark=pentagon*\\%
 PuRd-9-6!70, every mark/.append style={solid,fill=PuRd-9-6},mark=x\\%
 PuRd-9-7!70, every mark/.append style={solid,fill=PuRd-9-7},mark=+\\%
 PuRd-9-8!70, every mark/.append style={solid,fill=PuRd-9-8},mark=star\\%
 PuRd-9-9!70, every mark/.append style={solid,fill=PuRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-3}{%
 OrRd-3-1!70, every mark/.append style={solid,fill=OrRd-3-1},mark=*\\%
 OrRd-3-2!70, every mark/.append style={solid,fill=OrRd-3-2},mark=square*\\%
 OrRd-3-3!70, every mark/.append style={solid,fill=OrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-4}{%
 OrRd-4-1!70, every mark/.append style={solid,fill=OrRd-4-1},mark=*\\%
 OrRd-4-2!70, every mark/.append style={solid,fill=OrRd-4-2},mark=square*\\%
 OrRd-4-3!70, every mark/.append style={solid,fill=OrRd-4-3},mark=triangle*\\%
 OrRd-4-4!70, every mark/.append style={solid,fill=OrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-5}{%
 OrRd-5-1!70, every mark/.append style={solid,fill=OrRd-5-1},mark=*\\%
 OrRd-5-2!70, every mark/.append style={solid,fill=OrRd-5-2},mark=square*\\%
 OrRd-5-3!70, every mark/.append style={solid,fill=OrRd-5-3},mark=triangle*\\%
 OrRd-5-4!70, every mark/.append style={solid,fill=OrRd-5-4},mark=diamond*\\%
 OrRd-5-5!70, every mark/.append style={solid,fill=OrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-6}{%
 OrRd-6-1!70, every mark/.append style={solid,fill=OrRd-6-1},mark=*\\%
 OrRd-6-2!70, every mark/.append style={solid,fill=OrRd-6-2},mark=square*\\%
 OrRd-6-3!70, every mark/.append style={solid,fill=OrRd-6-3},mark=triangle*\\%
 OrRd-6-4!70, every mark/.append style={solid,fill=OrRd-6-4},mark=diamond*\\%
 OrRd-6-5!70, every mark/.append style={solid,fill=OrRd-6-5},mark=pentagon*\\%
 OrRd-6-6!70, every mark/.append style={solid,fill=OrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-7}{%
 OrRd-7-1!70, every mark/.append style={solid,fill=OrRd-7-1},mark=*\\%
 OrRd-7-2!70, every mark/.append style={solid,fill=OrRd-7-2},mark=square*\\%
 OrRd-7-3!70, every mark/.append style={solid,fill=OrRd-7-3},mark=triangle*\\%
 OrRd-7-4!70, every mark/.append style={solid,fill=OrRd-7-4},mark=diamond*\\%
 OrRd-7-5!70, every mark/.append style={solid,fill=OrRd-7-5},mark=pentagon*\\%
 OrRd-7-6!70, every mark/.append style={solid,fill=OrRd-7-6},mark=x\\%
 OrRd-7-7!70, every mark/.append style={solid,fill=OrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-8}{%
 OrRd-8-1!70, every mark/.append style={solid,fill=OrRd-8-1},mark=*\\%
 OrRd-8-2!70, every mark/.append style={solid,fill=OrRd-8-2},mark=square*\\%
 OrRd-8-3!70, every mark/.append style={solid,fill=OrRd-8-3},mark=triangle*\\%
 OrRd-8-4!70, every mark/.append style={solid,fill=OrRd-8-4},mark=diamond*\\%
 OrRd-8-5!70, every mark/.append style={solid,fill=OrRd-8-5},mark=pentagon*\\%
 OrRd-8-6!70, every mark/.append style={solid,fill=OrRd-8-6},mark=x\\%
 OrRd-8-7!70, every mark/.append style={solid,fill=OrRd-8-7},mark=+\\%
 OrRd-8-8!70, every mark/.append style={solid,fill=OrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-9}{%
 OrRd-9-1!70, every mark/.append style={solid,fill=OrRd-9-1},mark=*\\%
 OrRd-9-2!70, every mark/.append style={solid,fill=OrRd-9-2},mark=square*\\%
 OrRd-9-3!70, every mark/.append style={solid,fill=OrRd-9-3},mark=triangle*\\%
 OrRd-9-4!70, every mark/.append style={solid,fill=OrRd-9-4},mark=diamond*\\%
 OrRd-9-5!70, every mark/.append style={solid,fill=OrRd-9-5},mark=pentagon*\\%
 OrRd-9-6!70, every mark/.append style={solid,fill=OrRd-9-6},mark=x\\%
 OrRd-9-7!70, every mark/.append style={solid,fill=OrRd-9-7},mark=+\\%
 OrRd-9-8!70, every mark/.append style={solid,fill=OrRd-9-8},mark=star\\%
 OrRd-9-9!70, every mark/.append style={solid,fill=OrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-3}{%
 YlOrRd-3-1!70, every mark/.append style={solid,fill=YlOrRd-3-1},mark=*\\%
 YlOrRd-3-2!70, every mark/.append style={solid,fill=YlOrRd-3-2},mark=square*\\%
 YlOrRd-3-3!70, every mark/.append style={solid,fill=YlOrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-4}{%
 YlOrRd-4-1!70, every mark/.append style={solid,fill=YlOrRd-4-1},mark=*\\%
 YlOrRd-4-2!70, every mark/.append style={solid,fill=YlOrRd-4-2},mark=square*\\%
 YlOrRd-4-3!70, every mark/.append style={solid,fill=YlOrRd-4-3},mark=triangle*\\%
 YlOrRd-4-4!70, every mark/.append style={solid,fill=YlOrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-5}{%
 YlOrRd-5-1!70, every mark/.append style={solid,fill=YlOrRd-5-1},mark=*\\%
 YlOrRd-5-2!70, every mark/.append style={solid,fill=YlOrRd-5-2},mark=square*\\%
 YlOrRd-5-3!70, every mark/.append style={solid,fill=YlOrRd-5-3},mark=triangle*\\%
 YlOrRd-5-4!70, every mark/.append style={solid,fill=YlOrRd-5-4},mark=diamond*\\%
 YlOrRd-5-5!70, every mark/.append style={solid,fill=YlOrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-6}{%
 YlOrRd-6-1!70, every mark/.append style={solid,fill=YlOrRd-6-1},mark=*\\%
 YlOrRd-6-2!70, every mark/.append style={solid,fill=YlOrRd-6-2},mark=square*\\%
 YlOrRd-6-3!70, every mark/.append style={solid,fill=YlOrRd-6-3},mark=triangle*\\%
 YlOrRd-6-4!70, every mark/.append style={solid,fill=YlOrRd-6-4},mark=diamond*\\%
 YlOrRd-6-5!70, every mark/.append style={solid,fill=YlOrRd-6-5},mark=pentagon*\\%
 YlOrRd-6-6!70, every mark/.append style={solid,fill=YlOrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-7}{%
 YlOrRd-7-1!70, every mark/.append style={solid,fill=YlOrRd-7-1},mark=*\\%
 YlOrRd-7-2!70, every mark/.append style={solid,fill=YlOrRd-7-2},mark=square*\\%
 YlOrRd-7-3!70, every mark/.append style={solid,fill=YlOrRd-7-3},mark=triangle*\\%
 YlOrRd-7-4!70, every mark/.append style={solid,fill=YlOrRd-7-4},mark=diamond*\\%
 YlOrRd-7-5!70, every mark/.append style={solid,fill=YlOrRd-7-5},mark=pentagon*\\%
 YlOrRd-7-6!70, every mark/.append style={solid,fill=YlOrRd-7-6},mark=x\\%
 YlOrRd-7-7!70, every mark/.append style={solid,fill=YlOrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-8}{%
 YlOrRd-8-1!70, every mark/.append style={solid,fill=YlOrRd-8-1},mark=*\\%
 YlOrRd-8-2!70, every mark/.append style={solid,fill=YlOrRd-8-2},mark=square*\\%
 YlOrRd-8-3!70, every mark/.append style={solid,fill=YlOrRd-8-3},mark=triangle*\\%
 YlOrRd-8-4!70, every mark/.append style={solid,fill=YlOrRd-8-4},mark=diamond*\\%
 YlOrRd-8-5!70, every mark/.append style={solid,fill=YlOrRd-8-5},mark=pentagon*\\%
 YlOrRd-8-6!70, every mark/.append style={solid,fill=YlOrRd-8-6},mark=x\\%
 YlOrRd-8-7!70, every mark/.append style={solid,fill=YlOrRd-8-7},mark=+\\%
 YlOrRd-8-8!70, every mark/.append style={solid,fill=YlOrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-9}{%
 YlOrRd-9-1!70, every mark/.append style={solid,fill=YlOrRd-9-1},mark=*\\%
 YlOrRd-9-2!70, every mark/.append style={solid,fill=YlOrRd-9-2},mark=square*\\%
 YlOrRd-9-3!70, every mark/.append style={solid,fill=YlOrRd-9-3},mark=triangle*\\%
 YlOrRd-9-4!70, every mark/.append style={solid,fill=YlOrRd-9-4},mark=diamond*\\%
 YlOrRd-9-5!70, every mark/.append style={solid,fill=YlOrRd-9-5},mark=pentagon*\\%
 YlOrRd-9-6!70, every mark/.append style={solid,fill=YlOrRd-9-6},mark=x\\%
 YlOrRd-9-7!70, every mark/.append style={solid,fill=YlOrRd-9-7},mark=+\\%
 YlOrRd-9-8!70, every mark/.append style={solid,fill=YlOrRd-9-8},mark=star\\%
 YlOrRd-9-9!70, every mark/.append style={solid,fill=YlOrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-3}{%
 YlOrBr-3-1!70, every mark/.append style={solid,fill=YlOrBr-3-1},mark=*\\%
 YlOrBr-3-2!70, every mark/.append style={solid,fill=YlOrBr-3-2},mark=square*\\%
 YlOrBr-3-3!70, every mark/.append style={solid,fill=YlOrBr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-4}{%
 YlOrBr-4-1!70, every mark/.append style={solid,fill=YlOrBr-4-1},mark=*\\%
 YlOrBr-4-2!70, every mark/.append style={solid,fill=YlOrBr-4-2},mark=square*\\%
 YlOrBr-4-3!70, every mark/.append style={solid,fill=YlOrBr-4-3},mark=triangle*\\%
 YlOrBr-4-4!70, every mark/.append style={solid,fill=YlOrBr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-5}{%
 YlOrBr-5-1!70, every mark/.append style={solid,fill=YlOrBr-5-1},mark=*\\%
 YlOrBr-5-2!70, every mark/.append style={solid,fill=YlOrBr-5-2},mark=square*\\%
 YlOrBr-5-3!70, every mark/.append style={solid,fill=YlOrBr-5-3},mark=triangle*\\%
 YlOrBr-5-4!70, every mark/.append style={solid,fill=YlOrBr-5-4},mark=diamond*\\%
 YlOrBr-5-5!70, every mark/.append style={solid,fill=YlOrBr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-6}{%
 YlOrBr-6-1!70, every mark/.append style={solid,fill=YlOrBr-6-1},mark=*\\%
 YlOrBr-6-2!70, every mark/.append style={solid,fill=YlOrBr-6-2},mark=square*\\%
 YlOrBr-6-3!70, every mark/.append style={solid,fill=YlOrBr-6-3},mark=triangle*\\%
 YlOrBr-6-4!70, every mark/.append style={solid,fill=YlOrBr-6-4},mark=diamond*\\%
 YlOrBr-6-5!70, every mark/.append style={solid,fill=YlOrBr-6-5},mark=pentagon*\\%
 YlOrBr-6-6!70, every mark/.append style={solid,fill=YlOrBr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-7}{%
 YlOrBr-7-1!70, every mark/.append style={solid,fill=YlOrBr-7-1},mark=*\\%
 YlOrBr-7-2!70, every mark/.append style={solid,fill=YlOrBr-7-2},mark=square*\\%
 YlOrBr-7-3!70, every mark/.append style={solid,fill=YlOrBr-7-3},mark=triangle*\\%
 YlOrBr-7-4!70, every mark/.append style={solid,fill=YlOrBr-7-4},mark=diamond*\\%
 YlOrBr-7-5!70, every mark/.append style={solid,fill=YlOrBr-7-5},mark=pentagon*\\%
 YlOrBr-7-6!70, every mark/.append style={solid,fill=YlOrBr-7-6},mark=x\\%
 YlOrBr-7-7!70, every mark/.append style={solid,fill=YlOrBr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-8}{%
 YlOrBr-8-1!70, every mark/.append style={solid,fill=YlOrBr-8-1},mark=*\\%
 YlOrBr-8-2!70, every mark/.append style={solid,fill=YlOrBr-8-2},mark=square*\\%
 YlOrBr-8-3!70, every mark/.append style={solid,fill=YlOrBr-8-3},mark=triangle*\\%
 YlOrBr-8-4!70, every mark/.append style={solid,fill=YlOrBr-8-4},mark=diamond*\\%
 YlOrBr-8-5!70, every mark/.append style={solid,fill=YlOrBr-8-5},mark=pentagon*\\%
 YlOrBr-8-6!70, every mark/.append style={solid,fill=YlOrBr-8-6},mark=x\\%
 YlOrBr-8-7!70, every mark/.append style={solid,fill=YlOrBr-8-7},mark=+\\%
 YlOrBr-8-8!70, every mark/.append style={solid,fill=YlOrBr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-9}{%
 YlOrBr-9-1!70, every mark/.append style={solid,fill=YlOrBr-9-1},mark=*\\%
 YlOrBr-9-2!70, every mark/.append style={solid,fill=YlOrBr-9-2},mark=square*\\%
 YlOrBr-9-3!70, every mark/.append style={solid,fill=YlOrBr-9-3},mark=triangle*\\%
 YlOrBr-9-4!70, every mark/.append style={solid,fill=YlOrBr-9-4},mark=diamond*\\%
 YlOrBr-9-5!70, every mark/.append style={solid,fill=YlOrBr-9-5},mark=pentagon*\\%
 YlOrBr-9-6!70, every mark/.append style={solid,fill=YlOrBr-9-6},mark=x\\%
 YlOrBr-9-7!70, every mark/.append style={solid,fill=YlOrBr-9-7},mark=+\\%
 YlOrBr-9-8!70, every mark/.append style={solid,fill=YlOrBr-9-8},mark=star\\%
 YlOrBr-9-9!70, every mark/.append style={solid,fill=YlOrBr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-3}{%
 Purples-3-1!70, every mark/.append style={solid,fill=Purples-3-1},mark=*\\%
 Purples-3-2!70, every mark/.append style={solid,fill=Purples-3-2},mark=square*\\%
 Purples-3-3!70, every mark/.append style={solid,fill=Purples-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-4}{%
 Purples-4-1!70, every mark/.append style={solid,fill=Purples-4-1},mark=*\\%
 Purples-4-2!70, every mark/.append style={solid,fill=Purples-4-2},mark=square*\\%
 Purples-4-3!70, every mark/.append style={solid,fill=Purples-4-3},mark=triangle*\\%
 Purples-4-4!70, every mark/.append style={solid,fill=Purples-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-5}{%
 Purples-5-1!70, every mark/.append style={solid,fill=Purples-5-1},mark=*\\%
 Purples-5-2!70, every mark/.append style={solid,fill=Purples-5-2},mark=square*\\%
 Purples-5-3!70, every mark/.append style={solid,fill=Purples-5-3},mark=triangle*\\%
 Purples-5-4!70, every mark/.append style={solid,fill=Purples-5-4},mark=diamond*\\%
 Purples-5-5!70, every mark/.append style={solid,fill=Purples-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-6}{%
 Purples-6-1!70, every mark/.append style={solid,fill=Purples-6-1},mark=*\\%
 Purples-6-2!70, every mark/.append style={solid,fill=Purples-6-2},mark=square*\\%
 Purples-6-3!70, every mark/.append style={solid,fill=Purples-6-3},mark=triangle*\\%
 Purples-6-4!70, every mark/.append style={solid,fill=Purples-6-4},mark=diamond*\\%
 Purples-6-5!70, every mark/.append style={solid,fill=Purples-6-5},mark=pentagon*\\%
 Purples-6-6!70, every mark/.append style={solid,fill=Purples-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-7}{%
 Purples-7-1!70, every mark/.append style={solid,fill=Purples-7-1},mark=*\\%
 Purples-7-2!70, every mark/.append style={solid,fill=Purples-7-2},mark=square*\\%
 Purples-7-3!70, every mark/.append style={solid,fill=Purples-7-3},mark=triangle*\\%
 Purples-7-4!70, every mark/.append style={solid,fill=Purples-7-4},mark=diamond*\\%
 Purples-7-5!70, every mark/.append style={solid,fill=Purples-7-5},mark=pentagon*\\%
 Purples-7-6!70, every mark/.append style={solid,fill=Purples-7-6},mark=x\\%
 Purples-7-7!70, every mark/.append style={solid,fill=Purples-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-8}{%
 Purples-8-1!70, every mark/.append style={solid,fill=Purples-8-1},mark=*\\%
 Purples-8-2!70, every mark/.append style={solid,fill=Purples-8-2},mark=square*\\%
 Purples-8-3!70, every mark/.append style={solid,fill=Purples-8-3},mark=triangle*\\%
 Purples-8-4!70, every mark/.append style={solid,fill=Purples-8-4},mark=diamond*\\%
 Purples-8-5!70, every mark/.append style={solid,fill=Purples-8-5},mark=pentagon*\\%
 Purples-8-6!70, every mark/.append style={solid,fill=Purples-8-6},mark=x\\%
 Purples-8-7!70, every mark/.append style={solid,fill=Purples-8-7},mark=+\\%
 Purples-8-8!70, every mark/.append style={solid,fill=Purples-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-9}{%
 Purples-9-1!70, every mark/.append style={solid,fill=Purples-9-1},mark=*\\%
 Purples-9-2!70, every mark/.append style={solid,fill=Purples-9-2},mark=square*\\%
 Purples-9-3!70, every mark/.append style={solid,fill=Purples-9-3},mark=triangle*\\%
 Purples-9-4!70, every mark/.append style={solid,fill=Purples-9-4},mark=diamond*\\%
 Purples-9-5!70, every mark/.append style={solid,fill=Purples-9-5},mark=pentagon*\\%
 Purples-9-6!70, every mark/.append style={solid,fill=Purples-9-6},mark=x\\%
 Purples-9-7!70, every mark/.append style={solid,fill=Purples-9-7},mark=+\\%
 Purples-9-8!70, every mark/.append style={solid,fill=Purples-9-8},mark=star\\%
 Purples-9-9!70, every mark/.append style={solid,fill=Purples-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-3}{%
 Blues-3-1!70, every mark/.append style={solid,fill=Blues-3-1},mark=*\\%
 Blues-3-2!70, every mark/.append style={solid,fill=Blues-3-2},mark=square*\\%
 Blues-3-3!70, every mark/.append style={solid,fill=Blues-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-4}{%
 Blues-4-1!70, every mark/.append style={solid,fill=Blues-4-1},mark=*\\%
 Blues-4-2!70, every mark/.append style={solid,fill=Blues-4-2},mark=square*\\%
 Blues-4-3!70, every mark/.append style={solid,fill=Blues-4-3},mark=triangle*\\%
 Blues-4-4!70, every mark/.append style={solid,fill=Blues-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-5}{%
 Blues-5-1!70, every mark/.append style={solid,fill=Blues-5-1},mark=*\\%
 Blues-5-2!70, every mark/.append style={solid,fill=Blues-5-2},mark=square*\\%
 Blues-5-3!70, every mark/.append style={solid,fill=Blues-5-3},mark=triangle*\\%
 Blues-5-4!70, every mark/.append style={solid,fill=Blues-5-4},mark=diamond*\\%
 Blues-5-5!70, every mark/.append style={solid,fill=Blues-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-6}{%
 Blues-6-1!70, every mark/.append style={solid,fill=Blues-6-1},mark=*\\%
 Blues-6-2!70, every mark/.append style={solid,fill=Blues-6-2},mark=square*\\%
 Blues-6-3!70, every mark/.append style={solid,fill=Blues-6-3},mark=triangle*\\%
 Blues-6-4!70, every mark/.append style={solid,fill=Blues-6-4},mark=diamond*\\%
 Blues-6-5!70, every mark/.append style={solid,fill=Blues-6-5},mark=pentagon*\\%
 Blues-6-6!70, every mark/.append style={solid,fill=Blues-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-7}{%
 Blues-7-1!70, every mark/.append style={solid,fill=Blues-7-1},mark=*\\%
 Blues-7-2!70, every mark/.append style={solid,fill=Blues-7-2},mark=square*\\%
 Blues-7-3!70, every mark/.append style={solid,fill=Blues-7-3},mark=triangle*\\%
 Blues-7-4!70, every mark/.append style={solid,fill=Blues-7-4},mark=diamond*\\%
 Blues-7-5!70, every mark/.append style={solid,fill=Blues-7-5},mark=pentagon*\\%
 Blues-7-6!70, every mark/.append style={solid,fill=Blues-7-6},mark=x\\%
 Blues-7-7!70, every mark/.append style={solid,fill=Blues-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-8}{%
 Blues-8-1!70, every mark/.append style={solid,fill=Blues-8-1},mark=*\\%
 Blues-8-2!70, every mark/.append style={solid,fill=Blues-8-2},mark=square*\\%
 Blues-8-3!70, every mark/.append style={solid,fill=Blues-8-3},mark=triangle*\\%
 Blues-8-4!70, every mark/.append style={solid,fill=Blues-8-4},mark=diamond*\\%
 Blues-8-5!70, every mark/.append style={solid,fill=Blues-8-5},mark=pentagon*\\%
 Blues-8-6!70, every mark/.append style={solid,fill=Blues-8-6},mark=x\\%
 Blues-8-7!70, every mark/.append style={solid,fill=Blues-8-7},mark=+\\%
 Blues-8-8!70, every mark/.append style={solid,fill=Blues-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-9}{%
 Blues-9-1!70, every mark/.append style={solid,fill=Blues-9-1},mark=*\\%
 Blues-9-2!70, every mark/.append style={solid,fill=Blues-9-2},mark=square*\\%
 Blues-9-3!70, every mark/.append style={solid,fill=Blues-9-3},mark=triangle*\\%
 Blues-9-4!70, every mark/.append style={solid,fill=Blues-9-4},mark=diamond*\\%
 Blues-9-5!70, every mark/.append style={solid,fill=Blues-9-5},mark=pentagon*\\%
 Blues-9-6!70, every mark/.append style={solid,fill=Blues-9-6},mark=x\\%
 Blues-9-7!70, every mark/.append style={solid,fill=Blues-9-7},mark=+\\%
 Blues-9-8!70, every mark/.append style={solid,fill=Blues-9-8},mark=star\\%
 Blues-9-9!70, every mark/.append style={solid,fill=Blues-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-3}{%
 Greens-3-1!70, every mark/.append style={solid,fill=Greens-3-1},mark=*\\%
 Greens-3-2!70, every mark/.append style={solid,fill=Greens-3-2},mark=square*\\%
 Greens-3-3!70, every mark/.append style={solid,fill=Greens-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-4}{%
 Greens-4-1!70, every mark/.append style={solid,fill=Greens-4-1},mark=*\\%
 Greens-4-2!70, every mark/.append style={solid,fill=Greens-4-2},mark=square*\\%
 Greens-4-3!70, every mark/.append style={solid,fill=Greens-4-3},mark=triangle*\\%
 Greens-4-4!70, every mark/.append style={solid,fill=Greens-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-5}{%
 Greens-5-1!70, every mark/.append style={solid,fill=Greens-5-1},mark=*\\%
 Greens-5-2!70, every mark/.append style={solid,fill=Greens-5-2},mark=square*\\%
 Greens-5-3!70, every mark/.append style={solid,fill=Greens-5-3},mark=triangle*\\%
 Greens-5-4!70, every mark/.append style={solid,fill=Greens-5-4},mark=diamond*\\%
 Greens-5-5!70, every mark/.append style={solid,fill=Greens-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-6}{%
 Greens-6-1!70, every mark/.append style={solid,fill=Greens-6-1},mark=*\\%
 Greens-6-2!70, every mark/.append style={solid,fill=Greens-6-2},mark=square*\\%
 Greens-6-3!70, every mark/.append style={solid,fill=Greens-6-3},mark=triangle*\\%
 Greens-6-4!70, every mark/.append style={solid,fill=Greens-6-4},mark=diamond*\\%
 Greens-6-5!70, every mark/.append style={solid,fill=Greens-6-5},mark=pentagon*\\%
 Greens-6-6!70, every mark/.append style={solid,fill=Greens-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-7}{%
 Greens-7-1!70, every mark/.append style={solid,fill=Greens-7-1},mark=*\\%
 Greens-7-2!70, every mark/.append style={solid,fill=Greens-7-2},mark=square*\\%
 Greens-7-3!70, every mark/.append style={solid,fill=Greens-7-3},mark=triangle*\\%
 Greens-7-4!70, every mark/.append style={solid,fill=Greens-7-4},mark=diamond*\\%
 Greens-7-5!70, every mark/.append style={solid,fill=Greens-7-5},mark=pentagon*\\%
 Greens-7-6!70, every mark/.append style={solid,fill=Greens-7-6},mark=x\\%
 Greens-7-7!70, every mark/.append style={solid,fill=Greens-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-8}{%
 Greens-8-1!70, every mark/.append style={solid,fill=Greens-8-1},mark=*\\%
 Greens-8-2!70, every mark/.append style={solid,fill=Greens-8-2},mark=square*\\%
 Greens-8-3!70, every mark/.append style={solid,fill=Greens-8-3},mark=triangle*\\%
 Greens-8-4!70, every mark/.append style={solid,fill=Greens-8-4},mark=diamond*\\%
 Greens-8-5!70, every mark/.append style={solid,fill=Greens-8-5},mark=pentagon*\\%
 Greens-8-6!70, every mark/.append style={solid,fill=Greens-8-6},mark=x\\%
 Greens-8-7!70, every mark/.append style={solid,fill=Greens-8-7},mark=+\\%
 Greens-8-8!70, every mark/.append style={solid,fill=Greens-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-9}{%
 Greens-9-1!70, every mark/.append style={solid,fill=Greens-9-1},mark=*\\%
 Greens-9-2!70, every mark/.append style={solid,fill=Greens-9-2},mark=square*\\%
 Greens-9-3!70, every mark/.append style={solid,fill=Greens-9-3},mark=triangle*\\%
 Greens-9-4!70, every mark/.append style={solid,fill=Greens-9-4},mark=diamond*\\%
 Greens-9-5!70, every mark/.append style={solid,fill=Greens-9-5},mark=pentagon*\\%
 Greens-9-6!70, every mark/.append style={solid,fill=Greens-9-6},mark=x\\%
 Greens-9-7!70, every mark/.append style={solid,fill=Greens-9-7},mark=+\\%
 Greens-9-8!70, every mark/.append style={solid,fill=Greens-9-8},mark=star\\%
 Greens-9-9!70, every mark/.append style={solid,fill=Greens-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-3}{%
 Oranges-3-1!70, every mark/.append style={solid,fill=Oranges-3-1},mark=*\\%
 Oranges-3-2!70, every mark/.append style={solid,fill=Oranges-3-2},mark=square*\\%
 Oranges-3-3!70, every mark/.append style={solid,fill=Oranges-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-4}{%
 Oranges-4-1!70, every mark/.append style={solid,fill=Oranges-4-1},mark=*\\%
 Oranges-4-2!70, every mark/.append style={solid,fill=Oranges-4-2},mark=square*\\%
 Oranges-4-3!70, every mark/.append style={solid,fill=Oranges-4-3},mark=triangle*\\%
 Oranges-4-4!70, every mark/.append style={solid,fill=Oranges-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-5}{%
 Oranges-5-1!70, every mark/.append style={solid,fill=Oranges-5-1},mark=*\\%
 Oranges-5-2!70, every mark/.append style={solid,fill=Oranges-5-2},mark=square*\\%
 Oranges-5-3!70, every mark/.append style={solid,fill=Oranges-5-3},mark=triangle*\\%
 Oranges-5-4!70, every mark/.append style={solid,fill=Oranges-5-4},mark=diamond*\\%
 Oranges-5-5!70, every mark/.append style={solid,fill=Oranges-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-6}{%
 Oranges-6-1!70, every mark/.append style={solid,fill=Oranges-6-1},mark=*\\%
 Oranges-6-2!70, every mark/.append style={solid,fill=Oranges-6-2},mark=square*\\%
 Oranges-6-3!70, every mark/.append style={solid,fill=Oranges-6-3},mark=triangle*\\%
 Oranges-6-4!70, every mark/.append style={solid,fill=Oranges-6-4},mark=diamond*\\%
 Oranges-6-5!70, every mark/.append style={solid,fill=Oranges-6-5},mark=pentagon*\\%
 Oranges-6-6!70, every mark/.append style={solid,fill=Oranges-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-7}{%
 Oranges-7-1!70, every mark/.append style={solid,fill=Oranges-7-1},mark=*\\%
 Oranges-7-2!70, every mark/.append style={solid,fill=Oranges-7-2},mark=square*\\%
 Oranges-7-3!70, every mark/.append style={solid,fill=Oranges-7-3},mark=triangle*\\%
 Oranges-7-4!70, every mark/.append style={solid,fill=Oranges-7-4},mark=diamond*\\%
 Oranges-7-5!70, every mark/.append style={solid,fill=Oranges-7-5},mark=pentagon*\\%
 Oranges-7-6!70, every mark/.append style={solid,fill=Oranges-7-6},mark=x\\%
 Oranges-7-7!70, every mark/.append style={solid,fill=Oranges-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-8}{%
 Oranges-8-1!70, every mark/.append style={solid,fill=Oranges-8-1},mark=*\\%
 Oranges-8-2!70, every mark/.append style={solid,fill=Oranges-8-2},mark=square*\\%
 Oranges-8-3!70, every mark/.append style={solid,fill=Oranges-8-3},mark=triangle*\\%
 Oranges-8-4!70, every mark/.append style={solid,fill=Oranges-8-4},mark=diamond*\\%
 Oranges-8-5!70, every mark/.append style={solid,fill=Oranges-8-5},mark=pentagon*\\%
 Oranges-8-6!70, every mark/.append style={solid,fill=Oranges-8-6},mark=x\\%
 Oranges-8-7!70, every mark/.append style={solid,fill=Oranges-8-7},mark=+\\%
 Oranges-8-8!70, every mark/.append style={solid,fill=Oranges-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-9}{%
 Oranges-9-1!70, every mark/.append style={solid,fill=Oranges-9-1},mark=*\\%
 Oranges-9-2!70, every mark/.append style={solid,fill=Oranges-9-2},mark=square*\\%
 Oranges-9-3!70, every mark/.append style={solid,fill=Oranges-9-3},mark=triangle*\\%
 Oranges-9-4!70, every mark/.append style={solid,fill=Oranges-9-4},mark=diamond*\\%
 Oranges-9-5!70, every mark/.append style={solid,fill=Oranges-9-5},mark=pentagon*\\%
 Oranges-9-6!70, every mark/.append style={solid,fill=Oranges-9-6},mark=x\\%
 Oranges-9-7!70, every mark/.append style={solid,fill=Oranges-9-7},mark=+\\%
 Oranges-9-8!70, every mark/.append style={solid,fill=Oranges-9-8},mark=star\\%
 Oranges-9-9!70, every mark/.append style={solid,fill=Oranges-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-3}{%
 Reds-3-1!70, every mark/.append style={solid,fill=Reds-3-1},mark=*\\%
 Reds-3-2!70, every mark/.append style={solid,fill=Reds-3-2},mark=square*\\%
 Reds-3-3!70, every mark/.append style={solid,fill=Reds-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-4}{%
 Reds-4-1!70, every mark/.append style={solid,fill=Reds-4-1},mark=*\\%
 Reds-4-2!70, every mark/.append style={solid,fill=Reds-4-2},mark=square*\\%
 Reds-4-3!70, every mark/.append style={solid,fill=Reds-4-3},mark=triangle*\\%
 Reds-4-4!70, every mark/.append style={solid,fill=Reds-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-5}{%
 Reds-5-1!70, every mark/.append style={solid,fill=Reds-5-1},mark=*\\%
 Reds-5-2!70, every mark/.append style={solid,fill=Reds-5-2},mark=square*\\%
 Reds-5-3!70, every mark/.append style={solid,fill=Reds-5-3},mark=triangle*\\%
 Reds-5-4!70, every mark/.append style={solid,fill=Reds-5-4},mark=diamond*\\%
 Reds-5-5!70, every mark/.append style={solid,fill=Reds-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-6}{%
 Reds-6-1!70, every mark/.append style={solid,fill=Reds-6-1},mark=*\\%
 Reds-6-2!70, every mark/.append style={solid,fill=Reds-6-2},mark=square*\\%
 Reds-6-3!70, every mark/.append style={solid,fill=Reds-6-3},mark=triangle*\\%
 Reds-6-4!70, every mark/.append style={solid,fill=Reds-6-4},mark=diamond*\\%
 Reds-6-5!70, every mark/.append style={solid,fill=Reds-6-5},mark=pentagon*\\%
 Reds-6-6!70, every mark/.append style={solid,fill=Reds-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-7}{%
 Reds-7-1!70, every mark/.append style={solid,fill=Reds-7-1},mark=*\\%
 Reds-7-2!70, every mark/.append style={solid,fill=Reds-7-2},mark=square*\\%
 Reds-7-3!70, every mark/.append style={solid,fill=Reds-7-3},mark=triangle*\\%
 Reds-7-4!70, every mark/.append style={solid,fill=Reds-7-4},mark=diamond*\\%
 Reds-7-5!70, every mark/.append style={solid,fill=Reds-7-5},mark=pentagon*\\%
 Reds-7-6!70, every mark/.append style={solid,fill=Reds-7-6},mark=x\\%
 Reds-7-7!70, every mark/.append style={solid,fill=Reds-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-8}{%
 Reds-8-1!70, every mark/.append style={solid,fill=Reds-8-1},mark=*\\%
 Reds-8-2!70, every mark/.append style={solid,fill=Reds-8-2},mark=square*\\%
 Reds-8-3!70, every mark/.append style={solid,fill=Reds-8-3},mark=triangle*\\%
 Reds-8-4!70, every mark/.append style={solid,fill=Reds-8-4},mark=diamond*\\%
 Reds-8-5!70, every mark/.append style={solid,fill=Reds-8-5},mark=pentagon*\\%
 Reds-8-6!70, every mark/.append style={solid,fill=Reds-8-6},mark=x\\%
 Reds-8-7!70, every mark/.append style={solid,fill=Reds-8-7},mark=+\\%
 Reds-8-8!70, every mark/.append style={solid,fill=Reds-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-9}{%
 Reds-9-1!70, every mark/.append style={solid,fill=Reds-9-1},mark=*\\%
 Reds-9-2!70, every mark/.append style={solid,fill=Reds-9-2},mark=square*\\%
 Reds-9-3!70, every mark/.append style={solid,fill=Reds-9-3},mark=triangle*\\%
 Reds-9-4!70, every mark/.append style={solid,fill=Reds-9-4},mark=diamond*\\%
 Reds-9-5!70, every mark/.append style={solid,fill=Reds-9-5},mark=pentagon*\\%
 Reds-9-6!70, every mark/.append style={solid,fill=Reds-9-6},mark=x\\%
 Reds-9-7!70, every mark/.append style={solid,fill=Reds-9-7},mark=+\\%
 Reds-9-8!70, every mark/.append style={solid,fill=Reds-9-8},mark=star\\%
 Reds-9-9!70, every mark/.append style={solid,fill=Reds-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-3}{%
 Greys-3-1!70, every mark/.append style={solid,fill=Greys-3-1},mark=*\\%
 Greys-3-2!70, every mark/.append style={solid,fill=Greys-3-2},mark=square*\\%
 Greys-3-3!70, every mark/.append style={solid,fill=Greys-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-4}{%
 Greys-4-1!70, every mark/.append style={solid,fill=Greys-4-1},mark=*\\%
 Greys-4-2!70, every mark/.append style={solid,fill=Greys-4-2},mark=square*\\%
 Greys-4-3!70, every mark/.append style={solid,fill=Greys-4-3},mark=triangle*\\%
 Greys-4-4!70, every mark/.append style={solid,fill=Greys-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-5}{%
 Greys-5-1!70, every mark/.append style={solid,fill=Greys-5-1},mark=*\\%
 Greys-5-2!70, every mark/.append style={solid,fill=Greys-5-2},mark=square*\\%
 Greys-5-3!70, every mark/.append style={solid,fill=Greys-5-3},mark=triangle*\\%
 Greys-5-4!70, every mark/.append style={solid,fill=Greys-5-4},mark=diamond*\\%
 Greys-5-5!70, every mark/.append style={solid,fill=Greys-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-6}{%
 Greys-6-1!70, every mark/.append style={solid,fill=Greys-6-1},mark=*\\%
 Greys-6-2!70, every mark/.append style={solid,fill=Greys-6-2},mark=square*\\%
 Greys-6-3!70, every mark/.append style={solid,fill=Greys-6-3},mark=triangle*\\%
 Greys-6-4!70, every mark/.append style={solid,fill=Greys-6-4},mark=diamond*\\%
 Greys-6-5!70, every mark/.append style={solid,fill=Greys-6-5},mark=pentagon*\\%
 Greys-6-6!70, every mark/.append style={solid,fill=Greys-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-7}{%
 Greys-7-1!70, every mark/.append style={solid,fill=Greys-7-1},mark=*\\%
 Greys-7-2!70, every mark/.append style={solid,fill=Greys-7-2},mark=square*\\%
 Greys-7-3!70, every mark/.append style={solid,fill=Greys-7-3},mark=triangle*\\%
 Greys-7-4!70, every mark/.append style={solid,fill=Greys-7-4},mark=diamond*\\%
 Greys-7-5!70, every mark/.append style={solid,fill=Greys-7-5},mark=pentagon*\\%
 Greys-7-6!70, every mark/.append style={solid,fill=Greys-7-6},mark=x\\%
 Greys-7-7!70, every mark/.append style={solid,fill=Greys-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-8}{%
 Greys-8-1!70, every mark/.append style={solid,fill=Greys-8-1},mark=*\\%
 Greys-8-2!70, every mark/.append style={solid,fill=Greys-8-2},mark=square*\\%
 Greys-8-3!70, every mark/.append style={solid,fill=Greys-8-3},mark=triangle*\\%
 Greys-8-4!70, every mark/.append style={solid,fill=Greys-8-4},mark=diamond*\\%
 Greys-8-5!70, every mark/.append style={solid,fill=Greys-8-5},mark=pentagon*\\%
 Greys-8-6!70, every mark/.append style={solid,fill=Greys-8-6},mark=x\\%
 Greys-8-7!70, every mark/.append style={solid,fill=Greys-8-7},mark=+\\%
 Greys-8-8!70, every mark/.append style={solid,fill=Greys-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-9}{%
 Greys-9-1!70, every mark/.append style={solid,fill=Greys-9-1},mark=*\\%
 Greys-9-2!70, every mark/.append style={solid,fill=Greys-9-2},mark=square*\\%
 Greys-9-3!70, every mark/.append style={solid,fill=Greys-9-3},mark=triangle*\\%
 Greys-9-4!70, every mark/.append style={solid,fill=Greys-9-4},mark=diamond*\\%
 Greys-9-5!70, every mark/.append style={solid,fill=Greys-9-5},mark=pentagon*\\%
 Greys-9-6!70, every mark/.append style={solid,fill=Greys-9-6},mark=x\\%
 Greys-9-7!70, every mark/.append style={solid,fill=Greys-9-7},mark=+\\%
 Greys-9-8!70, every mark/.append style={solid,fill=Greys-9-8},mark=star\\%
 Greys-9-9!70, every mark/.append style={solid,fill=Greys-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-3}{%
 PuOr-3-1!70, every mark/.append style={solid,fill=PuOr-3-1},mark=*\\%
 PuOr-3-2!70, every mark/.append style={solid,fill=PuOr-3-2},mark=square*\\%
 PuOr-3-3!70, every mark/.append style={solid,fill=PuOr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-4}{%
 PuOr-4-1!70, every mark/.append style={solid,fill=PuOr-4-1},mark=*\\%
 PuOr-4-2!70, every mark/.append style={solid,fill=PuOr-4-2},mark=square*\\%
 PuOr-4-3!70, every mark/.append style={solid,fill=PuOr-4-3},mark=triangle*\\%
 PuOr-4-4!70, every mark/.append style={solid,fill=PuOr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-5}{%
 PuOr-5-1!70, every mark/.append style={solid,fill=PuOr-5-1},mark=*\\%
 PuOr-5-2!70, every mark/.append style={solid,fill=PuOr-5-2},mark=square*\\%
 PuOr-5-3!70, every mark/.append style={solid,fill=PuOr-5-3},mark=triangle*\\%
 PuOr-5-4!70, every mark/.append style={solid,fill=PuOr-5-4},mark=diamond*\\%
 PuOr-5-5!70, every mark/.append style={solid,fill=PuOr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-6}{%
 PuOr-6-1!70, every mark/.append style={solid,fill=PuOr-6-1},mark=*\\%
 PuOr-6-2!70, every mark/.append style={solid,fill=PuOr-6-2},mark=square*\\%
 PuOr-6-3!70, every mark/.append style={solid,fill=PuOr-6-3},mark=triangle*\\%
 PuOr-6-4!70, every mark/.append style={solid,fill=PuOr-6-4},mark=diamond*\\%
 PuOr-6-5!70, every mark/.append style={solid,fill=PuOr-6-5},mark=pentagon*\\%
 PuOr-6-6!70, every mark/.append style={solid,fill=PuOr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-7}{%
 PuOr-7-1!70, every mark/.append style={solid,fill=PuOr-7-1},mark=*\\%
 PuOr-7-2!70, every mark/.append style={solid,fill=PuOr-7-2},mark=square*\\%
 PuOr-7-3!70, every mark/.append style={solid,fill=PuOr-7-3},mark=triangle*\\%
 PuOr-7-4!70, every mark/.append style={solid,fill=PuOr-7-4},mark=diamond*\\%
 PuOr-7-5!70, every mark/.append style={solid,fill=PuOr-7-5},mark=pentagon*\\%
 PuOr-7-6!70, every mark/.append style={solid,fill=PuOr-7-6},mark=x\\%
 PuOr-7-7!70, every mark/.append style={solid,fill=PuOr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-8}{%
 PuOr-8-1!70, every mark/.append style={solid,fill=PuOr-8-1},mark=*\\%
 PuOr-8-2!70, every mark/.append style={solid,fill=PuOr-8-2},mark=square*\\%
 PuOr-8-3!70, every mark/.append style={solid,fill=PuOr-8-3},mark=triangle*\\%
 PuOr-8-4!70, every mark/.append style={solid,fill=PuOr-8-4},mark=diamond*\\%
 PuOr-8-5!70, every mark/.append style={solid,fill=PuOr-8-5},mark=pentagon*\\%
 PuOr-8-6!70, every mark/.append style={solid,fill=PuOr-8-6},mark=x\\%
 PuOr-8-7!70, every mark/.append style={solid,fill=PuOr-8-7},mark=+\\%
 PuOr-8-8!70, every mark/.append style={solid,fill=PuOr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-9}{%
 PuOr-9-1!70, every mark/.append style={solid,fill=PuOr-9-1},mark=*\\%
 PuOr-9-2!70, every mark/.append style={solid,fill=PuOr-9-2},mark=square*\\%
 PuOr-9-3!70, every mark/.append style={solid,fill=PuOr-9-3},mark=triangle*\\%
 PuOr-9-4!70, every mark/.append style={solid,fill=PuOr-9-4},mark=diamond*\\%
 PuOr-9-5!70, every mark/.append style={solid,fill=PuOr-9-5},mark=pentagon*\\%
 PuOr-9-6!70, every mark/.append style={solid,fill=PuOr-9-6},mark=x\\%
 PuOr-9-7!70, every mark/.append style={solid,fill=PuOr-9-7},mark=+\\%
 PuOr-9-8!70, every mark/.append style={solid,fill=PuOr-9-8},mark=star\\%
 PuOr-9-9!70, every mark/.append style={solid,fill=PuOr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-10}{%
 PuOr-10-1!70, every mark/.append style={solid,fill=PuOr-10-1},mark=*\\%
 PuOr-10-2!70, every mark/.append style={solid,fill=PuOr-10-2},mark=square*\\%
 PuOr-10-3!70, every mark/.append style={solid,fill=PuOr-10-3},mark=triangle*\\%
 PuOr-10-4!70, every mark/.append style={solid,fill=PuOr-10-4},mark=diamond*\\%
 PuOr-10-5!70, every mark/.append style={solid,fill=PuOr-10-5},mark=pentagon*\\%
 PuOr-10-6!70, every mark/.append style={solid,fill=PuOr-10-6},mark=x\\%
 PuOr-10-7!70, every mark/.append style={solid,fill=PuOr-10-7},mark=+\\%
 PuOr-10-8!70, every mark/.append style={solid,fill=PuOr-10-8},mark=star\\%
 PuOr-10-9!70, every mark/.append style={solid,fill=PuOr-10-9},mark=oplus*\\%
 PuOr-10-10!70, every mark/.append style={solid,fill=PuOr-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-11}{%
 PuOr-11-1!70, every mark/.append style={solid,fill=PuOr-11-1},mark=*\\%
 PuOr-11-2!70, every mark/.append style={solid,fill=PuOr-11-2},mark=square*\\%
 PuOr-11-3!70, every mark/.append style={solid,fill=PuOr-11-3},mark=triangle*\\%
 PuOr-11-4!70, every mark/.append style={solid,fill=PuOr-11-4},mark=diamond*\\%
 PuOr-11-5!70, every mark/.append style={solid,fill=PuOr-11-5},mark=pentagon*\\%
 PuOr-11-6!70, every mark/.append style={solid,fill=PuOr-11-6},mark=x\\%
 PuOr-11-7!70, every mark/.append style={solid,fill=PuOr-11-7},mark=+\\%
 PuOr-11-8!70, every mark/.append style={solid,fill=PuOr-11-8},mark=star\\%
 PuOr-11-9!70, every mark/.append style={solid,fill=PuOr-11-9},mark=oplus*\\%
 PuOr-11-10!70, every mark/.append style={solid,fill=PuOr-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-3}{%
 BrBG-3-1!70, every mark/.append style={solid,fill=BrBG-3-1},mark=*\\%
 BrBG-3-2!70, every mark/.append style={solid,fill=BrBG-3-2},mark=square*\\%
 BrBG-3-3!70, every mark/.append style={solid,fill=BrBG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-4}{%
 BrBG-4-1!70, every mark/.append style={solid,fill=BrBG-4-1},mark=*\\%
 BrBG-4-2!70, every mark/.append style={solid,fill=BrBG-4-2},mark=square*\\%
 BrBG-4-3!70, every mark/.append style={solid,fill=BrBG-4-3},mark=triangle*\\%
 BrBG-4-4!70, every mark/.append style={solid,fill=BrBG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-5}{%
 BrBG-5-1!70, every mark/.append style={solid,fill=BrBG-5-1},mark=*\\%
 BrBG-5-2!70, every mark/.append style={solid,fill=BrBG-5-2},mark=square*\\%
 BrBG-5-3!70, every mark/.append style={solid,fill=BrBG-5-3},mark=triangle*\\%
 BrBG-5-4!70, every mark/.append style={solid,fill=BrBG-5-4},mark=diamond*\\%
 BrBG-5-5!70, every mark/.append style={solid,fill=BrBG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-6}{%
 BrBG-6-1!70, every mark/.append style={solid,fill=BrBG-6-1},mark=*\\%
 BrBG-6-2!70, every mark/.append style={solid,fill=BrBG-6-2},mark=square*\\%
 BrBG-6-3!70, every mark/.append style={solid,fill=BrBG-6-3},mark=triangle*\\%
 BrBG-6-4!70, every mark/.append style={solid,fill=BrBG-6-4},mark=diamond*\\%
 BrBG-6-5!70, every mark/.append style={solid,fill=BrBG-6-5},mark=pentagon*\\%
 BrBG-6-6!70, every mark/.append style={solid,fill=BrBG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-7}{%
 BrBG-7-1!70, every mark/.append style={solid,fill=BrBG-7-1},mark=*\\%
 BrBG-7-2!70, every mark/.append style={solid,fill=BrBG-7-2},mark=square*\\%
 BrBG-7-3!70, every mark/.append style={solid,fill=BrBG-7-3},mark=triangle*\\%
 BrBG-7-4!70, every mark/.append style={solid,fill=BrBG-7-4},mark=diamond*\\%
 BrBG-7-5!70, every mark/.append style={solid,fill=BrBG-7-5},mark=pentagon*\\%
 BrBG-7-6!70, every mark/.append style={solid,fill=BrBG-7-6},mark=x\\%
 BrBG-7-7!70, every mark/.append style={solid,fill=BrBG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-8}{%
 BrBG-8-1!70, every mark/.append style={solid,fill=BrBG-8-1},mark=*\\%
 BrBG-8-2!70, every mark/.append style={solid,fill=BrBG-8-2},mark=square*\\%
 BrBG-8-3!70, every mark/.append style={solid,fill=BrBG-8-3},mark=triangle*\\%
 BrBG-8-4!70, every mark/.append style={solid,fill=BrBG-8-4},mark=diamond*\\%
 BrBG-8-5!70, every mark/.append style={solid,fill=BrBG-8-5},mark=pentagon*\\%
 BrBG-8-6!70, every mark/.append style={solid,fill=BrBG-8-6},mark=x\\%
 BrBG-8-7!70, every mark/.append style={solid,fill=BrBG-8-7},mark=+\\%
 BrBG-8-8!70, every mark/.append style={solid,fill=BrBG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-9}{%
 BrBG-9-1!70, every mark/.append style={solid,fill=BrBG-9-1},mark=*\\%
 BrBG-9-2!70, every mark/.append style={solid,fill=BrBG-9-2},mark=square*\\%
 BrBG-9-3!70, every mark/.append style={solid,fill=BrBG-9-3},mark=triangle*\\%
 BrBG-9-4!70, every mark/.append style={solid,fill=BrBG-9-4},mark=diamond*\\%
 BrBG-9-5!70, every mark/.append style={solid,fill=BrBG-9-5},mark=pentagon*\\%
 BrBG-9-6!70, every mark/.append style={solid,fill=BrBG-9-6},mark=x\\%
 BrBG-9-7!70, every mark/.append style={solid,fill=BrBG-9-7},mark=+\\%
 BrBG-9-8!70, every mark/.append style={solid,fill=BrBG-9-8},mark=star\\%
 BrBG-9-9!70, every mark/.append style={solid,fill=BrBG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-10}{%
 BrBG-10-1!70, every mark/.append style={solid,fill=BrBG-10-1},mark=*\\%
 BrBG-10-2!70, every mark/.append style={solid,fill=BrBG-10-2},mark=square*\\%
 BrBG-10-3!70, every mark/.append style={solid,fill=BrBG-10-3},mark=triangle*\\%
 BrBG-10-4!70, every mark/.append style={solid,fill=BrBG-10-4},mark=diamond*\\%
 BrBG-10-5!70, every mark/.append style={solid,fill=BrBG-10-5},mark=pentagon*\\%
 BrBG-10-6!70, every mark/.append style={solid,fill=BrBG-10-6},mark=x\\%
 BrBG-10-7!70, every mark/.append style={solid,fill=BrBG-10-7},mark=+\\%
 BrBG-10-8!70, every mark/.append style={solid,fill=BrBG-10-8},mark=star\\%
 BrBG-10-9!70, every mark/.append style={solid,fill=BrBG-10-9},mark=oplus*\\%
 BrBG-10-10!70, every mark/.append style={solid,fill=BrBG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-11}{%
 BrBG-11-1!70, every mark/.append style={solid,fill=BrBG-11-1},mark=*\\%
 BrBG-11-2!70, every mark/.append style={solid,fill=BrBG-11-2},mark=square*\\%
 BrBG-11-3!70, every mark/.append style={solid,fill=BrBG-11-3},mark=triangle*\\%
 BrBG-11-4!70, every mark/.append style={solid,fill=BrBG-11-4},mark=diamond*\\%
 BrBG-11-5!70, every mark/.append style={solid,fill=BrBG-11-5},mark=pentagon*\\%
 BrBG-11-6!70, every mark/.append style={solid,fill=BrBG-11-6},mark=x\\%
 BrBG-11-7!70, every mark/.append style={solid,fill=BrBG-11-7},mark=+\\%
 BrBG-11-8!70, every mark/.append style={solid,fill=BrBG-11-8},mark=star\\%
 BrBG-11-9!70, every mark/.append style={solid,fill=BrBG-11-9},mark=oplus*\\%
 BrBG-11-10!70, every mark/.append style={solid,fill=BrBG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-3}{%
 PRGn-3-1!70, every mark/.append style={solid,fill=PRGn-3-1},mark=*\\%
 PRGn-3-2!70, every mark/.append style={solid,fill=PRGn-3-2},mark=square*\\%
 PRGn-3-3!70, every mark/.append style={solid,fill=PRGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-4}{%
 PRGn-4-1!70, every mark/.append style={solid,fill=PRGn-4-1},mark=*\\%
 PRGn-4-2!70, every mark/.append style={solid,fill=PRGn-4-2},mark=square*\\%
 PRGn-4-3!70, every mark/.append style={solid,fill=PRGn-4-3},mark=triangle*\\%
 PRGn-4-4!70, every mark/.append style={solid,fill=PRGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-5}{%
 PRGn-5-1!70, every mark/.append style={solid,fill=PRGn-5-1},mark=*\\%
 PRGn-5-2!70, every mark/.append style={solid,fill=PRGn-5-2},mark=square*\\%
 PRGn-5-3!70, every mark/.append style={solid,fill=PRGn-5-3},mark=triangle*\\%
 PRGn-5-4!70, every mark/.append style={solid,fill=PRGn-5-4},mark=diamond*\\%
 PRGn-5-5!70, every mark/.append style={solid,fill=PRGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-6}{%
 PRGn-6-1!70, every mark/.append style={solid,fill=PRGn-6-1},mark=*\\%
 PRGn-6-2!70, every mark/.append style={solid,fill=PRGn-6-2},mark=square*\\%
 PRGn-6-3!70, every mark/.append style={solid,fill=PRGn-6-3},mark=triangle*\\%
 PRGn-6-4!70, every mark/.append style={solid,fill=PRGn-6-4},mark=diamond*\\%
 PRGn-6-5!70, every mark/.append style={solid,fill=PRGn-6-5},mark=pentagon*\\%
 PRGn-6-6!70, every mark/.append style={solid,fill=PRGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-7}{%
 PRGn-7-1!70, every mark/.append style={solid,fill=PRGn-7-1},mark=*\\%
 PRGn-7-2!70, every mark/.append style={solid,fill=PRGn-7-2},mark=square*\\%
 PRGn-7-3!70, every mark/.append style={solid,fill=PRGn-7-3},mark=triangle*\\%
 PRGn-7-4!70, every mark/.append style={solid,fill=PRGn-7-4},mark=diamond*\\%
 PRGn-7-5!70, every mark/.append style={solid,fill=PRGn-7-5},mark=pentagon*\\%
 PRGn-7-6!70, every mark/.append style={solid,fill=PRGn-7-6},mark=x\\%
 PRGn-7-7!70, every mark/.append style={solid,fill=PRGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-8}{%
 PRGn-8-1!70, every mark/.append style={solid,fill=PRGn-8-1},mark=*\\%
 PRGn-8-2!70, every mark/.append style={solid,fill=PRGn-8-2},mark=square*\\%
 PRGn-8-3!70, every mark/.append style={solid,fill=PRGn-8-3},mark=triangle*\\%
 PRGn-8-4!70, every mark/.append style={solid,fill=PRGn-8-4},mark=diamond*\\%
 PRGn-8-5!70, every mark/.append style={solid,fill=PRGn-8-5},mark=pentagon*\\%
 PRGn-8-6!70, every mark/.append style={solid,fill=PRGn-8-6},mark=x\\%
 PRGn-8-7!70, every mark/.append style={solid,fill=PRGn-8-7},mark=+\\%
 PRGn-8-8!70, every mark/.append style={solid,fill=PRGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-9}{%
 PRGn-9-1!70, every mark/.append style={solid,fill=PRGn-9-1},mark=*\\%
 PRGn-9-2!70, every mark/.append style={solid,fill=PRGn-9-2},mark=square*\\%
 PRGn-9-3!70, every mark/.append style={solid,fill=PRGn-9-3},mark=triangle*\\%
 PRGn-9-4!70, every mark/.append style={solid,fill=PRGn-9-4},mark=diamond*\\%
 PRGn-9-5!70, every mark/.append style={solid,fill=PRGn-9-5},mark=pentagon*\\%
 PRGn-9-6!70, every mark/.append style={solid,fill=PRGn-9-6},mark=x\\%
 PRGn-9-7!70, every mark/.append style={solid,fill=PRGn-9-7},mark=+\\%
 PRGn-9-8!70, every mark/.append style={solid,fill=PRGn-9-8},mark=star\\%
 PRGn-9-9!70, every mark/.append style={solid,fill=PRGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-10}{%
 PRGn-10-1!70, every mark/.append style={solid,fill=PRGn-10-1},mark=*\\%
 PRGn-10-2!70, every mark/.append style={solid,fill=PRGn-10-2},mark=square*\\%
 PRGn-10-3!70, every mark/.append style={solid,fill=PRGn-10-3},mark=triangle*\\%
 PRGn-10-4!70, every mark/.append style={solid,fill=PRGn-10-4},mark=diamond*\\%
 PRGn-10-5!70, every mark/.append style={solid,fill=PRGn-10-5},mark=pentagon*\\%
 PRGn-10-6!70, every mark/.append style={solid,fill=PRGn-10-6},mark=x\\%
 PRGn-10-7!70, every mark/.append style={solid,fill=PRGn-10-7},mark=+\\%
 PRGn-10-8!70, every mark/.append style={solid,fill=PRGn-10-8},mark=star\\%
 PRGn-10-9!70, every mark/.append style={solid,fill=PRGn-10-9},mark=oplus*\\%
 PRGn-10-10!70, every mark/.append style={solid,fill=PRGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-11}{%
 PRGn-11-1!70, every mark/.append style={solid,fill=PRGn-11-1},mark=*\\%
 PRGn-11-2!70, every mark/.append style={solid,fill=PRGn-11-2},mark=square*\\%
 PRGn-11-3!70, every mark/.append style={solid,fill=PRGn-11-3},mark=triangle*\\%
 PRGn-11-4!70, every mark/.append style={solid,fill=PRGn-11-4},mark=diamond*\\%
 PRGn-11-5!70, every mark/.append style={solid,fill=PRGn-11-5},mark=pentagon*\\%
 PRGn-11-6!70, every mark/.append style={solid,fill=PRGn-11-6},mark=x\\%
 PRGn-11-7!70, every mark/.append style={solid,fill=PRGn-11-7},mark=+\\%
 PRGn-11-8!70, every mark/.append style={solid,fill=PRGn-11-8},mark=star\\%
 PRGn-11-9!70, every mark/.append style={solid,fill=PRGn-11-9},mark=oplus*\\%
 PRGn-11-10!70, every mark/.append style={solid,fill=PRGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-3}{%
 PiYG-3-1!70, every mark/.append style={solid,fill=PiYG-3-1},mark=*\\%
 PiYG-3-2!70, every mark/.append style={solid,fill=PiYG-3-2},mark=square*\\%
 PiYG-3-3!70, every mark/.append style={solid,fill=PiYG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-4}{%
 PiYG-4-1!70, every mark/.append style={solid,fill=PiYG-4-1},mark=*\\%
 PiYG-4-2!70, every mark/.append style={solid,fill=PiYG-4-2},mark=square*\\%
 PiYG-4-3!70, every mark/.append style={solid,fill=PiYG-4-3},mark=triangle*\\%
 PiYG-4-4!70, every mark/.append style={solid,fill=PiYG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-5}{%
 PiYG-5-1!70, every mark/.append style={solid,fill=PiYG-5-1},mark=*\\%
 PiYG-5-2!70, every mark/.append style={solid,fill=PiYG-5-2},mark=square*\\%
 PiYG-5-3!70, every mark/.append style={solid,fill=PiYG-5-3},mark=triangle*\\%
 PiYG-5-4!70, every mark/.append style={solid,fill=PiYG-5-4},mark=diamond*\\%
 PiYG-5-5!70, every mark/.append style={solid,fill=PiYG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-6}{%
 PiYG-6-1!70, every mark/.append style={solid,fill=PiYG-6-1},mark=*\\%
 PiYG-6-2!70, every mark/.append style={solid,fill=PiYG-6-2},mark=square*\\%
 PiYG-6-3!70, every mark/.append style={solid,fill=PiYG-6-3},mark=triangle*\\%
 PiYG-6-4!70, every mark/.append style={solid,fill=PiYG-6-4},mark=diamond*\\%
 PiYG-6-5!70, every mark/.append style={solid,fill=PiYG-6-5},mark=pentagon*\\%
 PiYG-6-6!70, every mark/.append style={solid,fill=PiYG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-7}{%
 PiYG-7-1!70, every mark/.append style={solid,fill=PiYG-7-1},mark=*\\%
 PiYG-7-2!70, every mark/.append style={solid,fill=PiYG-7-2},mark=square*\\%
 PiYG-7-3!70, every mark/.append style={solid,fill=PiYG-7-3},mark=triangle*\\%
 PiYG-7-4!70, every mark/.append style={solid,fill=PiYG-7-4},mark=diamond*\\%
 PiYG-7-5!70, every mark/.append style={solid,fill=PiYG-7-5},mark=pentagon*\\%
 PiYG-7-6!70, every mark/.append style={solid,fill=PiYG-7-6},mark=x\\%
 PiYG-7-7!70, every mark/.append style={solid,fill=PiYG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-8}{%
 PiYG-8-1!70, every mark/.append style={solid,fill=PiYG-8-1},mark=*\\%
 PiYG-8-2!70, every mark/.append style={solid,fill=PiYG-8-2},mark=square*\\%
 PiYG-8-3!70, every mark/.append style={solid,fill=PiYG-8-3},mark=triangle*\\%
 PiYG-8-4!70, every mark/.append style={solid,fill=PiYG-8-4},mark=diamond*\\%
 PiYG-8-5!70, every mark/.append style={solid,fill=PiYG-8-5},mark=pentagon*\\%
 PiYG-8-6!70, every mark/.append style={solid,fill=PiYG-8-6},mark=x\\%
 PiYG-8-7!70, every mark/.append style={solid,fill=PiYG-8-7},mark=+\\%
 PiYG-8-8!70, every mark/.append style={solid,fill=PiYG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-9}{%
 PiYG-9-1!70, every mark/.append style={solid,fill=PiYG-9-1},mark=*\\%
 PiYG-9-2!70, every mark/.append style={solid,fill=PiYG-9-2},mark=square*\\%
 PiYG-9-3!70, every mark/.append style={solid,fill=PiYG-9-3},mark=triangle*\\%
 PiYG-9-4!70, every mark/.append style={solid,fill=PiYG-9-4},mark=diamond*\\%
 PiYG-9-5!70, every mark/.append style={solid,fill=PiYG-9-5},mark=pentagon*\\%
 PiYG-9-6!70, every mark/.append style={solid,fill=PiYG-9-6},mark=x\\%
 PiYG-9-7!70, every mark/.append style={solid,fill=PiYG-9-7},mark=+\\%
 PiYG-9-8!70, every mark/.append style={solid,fill=PiYG-9-8},mark=star\\%
 PiYG-9-9!70, every mark/.append style={solid,fill=PiYG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-10}{%
 PiYG-10-1!70, every mark/.append style={solid,fill=PiYG-10-1},mark=*\\%
 PiYG-10-2!70, every mark/.append style={solid,fill=PiYG-10-2},mark=square*\\%
 PiYG-10-3!70, every mark/.append style={solid,fill=PiYG-10-3},mark=triangle*\\%
 PiYG-10-4!70, every mark/.append style={solid,fill=PiYG-10-4},mark=diamond*\\%
 PiYG-10-5!70, every mark/.append style={solid,fill=PiYG-10-5},mark=pentagon*\\%
 PiYG-10-6!70, every mark/.append style={solid,fill=PiYG-10-6},mark=x\\%
 PiYG-10-7!70, every mark/.append style={solid,fill=PiYG-10-7},mark=+\\%
 PiYG-10-8!70, every mark/.append style={solid,fill=PiYG-10-8},mark=star\\%
 PiYG-10-9!70, every mark/.append style={solid,fill=PiYG-10-9},mark=oplus*\\%
 PiYG-10-10!70, every mark/.append style={solid,fill=PiYG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-11}{%
 PiYG-11-1!70, every mark/.append style={solid,fill=PiYG-11-1},mark=*\\%
 PiYG-11-2!70, every mark/.append style={solid,fill=PiYG-11-2},mark=square*\\%
 PiYG-11-3!70, every mark/.append style={solid,fill=PiYG-11-3},mark=triangle*\\%
 PiYG-11-4!70, every mark/.append style={solid,fill=PiYG-11-4},mark=diamond*\\%
 PiYG-11-5!70, every mark/.append style={solid,fill=PiYG-11-5},mark=pentagon*\\%
 PiYG-11-6!70, every mark/.append style={solid,fill=PiYG-11-6},mark=x\\%
 PiYG-11-7!70, every mark/.append style={solid,fill=PiYG-11-7},mark=+\\%
 PiYG-11-8!70, every mark/.append style={solid,fill=PiYG-11-8},mark=star\\%
 PiYG-11-9!70, every mark/.append style={solid,fill=PiYG-11-9},mark=oplus*\\%
 PiYG-11-10!70, every mark/.append style={solid,fill=PiYG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-3}{%
 RdBu-3-1!70, every mark/.append style={solid,fill=RdBu-3-1},mark=*\\%
 RdBu-3-2!70, every mark/.append style={solid,fill=RdBu-3-2},mark=square*\\%
 RdBu-3-3!70, every mark/.append style={solid,fill=RdBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-4}{%
 RdBu-4-1!70, every mark/.append style={solid,fill=RdBu-4-1},mark=*\\%
 RdBu-4-2!70, every mark/.append style={solid,fill=RdBu-4-2},mark=square*\\%
 RdBu-4-3!70, every mark/.append style={solid,fill=RdBu-4-3},mark=triangle*\\%
 RdBu-4-4!70, every mark/.append style={solid,fill=RdBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-5}{%
 RdBu-5-1!70, every mark/.append style={solid,fill=RdBu-5-1},mark=*\\%
 RdBu-5-2!70, every mark/.append style={solid,fill=RdBu-5-2},mark=square*\\%
 RdBu-5-3!70, every mark/.append style={solid,fill=RdBu-5-3},mark=triangle*\\%
 RdBu-5-4!70, every mark/.append style={solid,fill=RdBu-5-4},mark=diamond*\\%
 RdBu-5-5!70, every mark/.append style={solid,fill=RdBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-6}{%
 RdBu-6-1!70, every mark/.append style={solid,fill=RdBu-6-1},mark=*\\%
 RdBu-6-2!70, every mark/.append style={solid,fill=RdBu-6-2},mark=square*\\%
 RdBu-6-3!70, every mark/.append style={solid,fill=RdBu-6-3},mark=triangle*\\%
 RdBu-6-4!70, every mark/.append style={solid,fill=RdBu-6-4},mark=diamond*\\%
 RdBu-6-5!70, every mark/.append style={solid,fill=RdBu-6-5},mark=pentagon*\\%
 RdBu-6-6!70, every mark/.append style={solid,fill=RdBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-7}{%
 RdBu-7-1!70, every mark/.append style={solid,fill=RdBu-7-1},mark=*\\%
 RdBu-7-2!70, every mark/.append style={solid,fill=RdBu-7-2},mark=square*\\%
 RdBu-7-3!70, every mark/.append style={solid,fill=RdBu-7-3},mark=triangle*\\%
 RdBu-7-4!70, every mark/.append style={solid,fill=RdBu-7-4},mark=diamond*\\%
 RdBu-7-5!70, every mark/.append style={solid,fill=RdBu-7-5},mark=pentagon*\\%
 RdBu-7-6!70, every mark/.append style={solid,fill=RdBu-7-6},mark=x\\%
 RdBu-7-7!70, every mark/.append style={solid,fill=RdBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-8}{%
 RdBu-8-1!70, every mark/.append style={solid,fill=RdBu-8-1},mark=*\\%
 RdBu-8-2!70, every mark/.append style={solid,fill=RdBu-8-2},mark=square*\\%
 RdBu-8-3!70, every mark/.append style={solid,fill=RdBu-8-3},mark=triangle*\\%
 RdBu-8-4!70, every mark/.append style={solid,fill=RdBu-8-4},mark=diamond*\\%
 RdBu-8-5!70, every mark/.append style={solid,fill=RdBu-8-5},mark=pentagon*\\%
 RdBu-8-6!70, every mark/.append style={solid,fill=RdBu-8-6},mark=x\\%
 RdBu-8-7!70, every mark/.append style={solid,fill=RdBu-8-7},mark=+\\%
 RdBu-8-8!70, every mark/.append style={solid,fill=RdBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-9}{%
 RdBu-9-1!70, every mark/.append style={solid,fill=RdBu-9-1},mark=*\\%
 RdBu-9-2!70, every mark/.append style={solid,fill=RdBu-9-2},mark=square*\\%
 RdBu-9-3!70, every mark/.append style={solid,fill=RdBu-9-3},mark=triangle*\\%
 RdBu-9-4!70, every mark/.append style={solid,fill=RdBu-9-4},mark=diamond*\\%
 RdBu-9-5!70, every mark/.append style={solid,fill=RdBu-9-5},mark=pentagon*\\%
 RdBu-9-6!70, every mark/.append style={solid,fill=RdBu-9-6},mark=x\\%
 RdBu-9-7!70, every mark/.append style={solid,fill=RdBu-9-7},mark=+\\%
 RdBu-9-8!70, every mark/.append style={solid,fill=RdBu-9-8},mark=star\\%
 RdBu-9-9!70, every mark/.append style={solid,fill=RdBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-10}{%
 RdBu-10-1!70, every mark/.append style={solid,fill=RdBu-10-1},mark=*\\%
 RdBu-10-2!70, every mark/.append style={solid,fill=RdBu-10-2},mark=square*\\%
 RdBu-10-3!70, every mark/.append style={solid,fill=RdBu-10-3},mark=triangle*\\%
 RdBu-10-4!70, every mark/.append style={solid,fill=RdBu-10-4},mark=diamond*\\%
 RdBu-10-5!70, every mark/.append style={solid,fill=RdBu-10-5},mark=pentagon*\\%
 RdBu-10-6!70, every mark/.append style={solid,fill=RdBu-10-6},mark=x\\%
 RdBu-10-7!70, every mark/.append style={solid,fill=RdBu-10-7},mark=+\\%
 RdBu-10-8!70, every mark/.append style={solid,fill=RdBu-10-8},mark=star\\%
 RdBu-10-9!70, every mark/.append style={solid,fill=RdBu-10-9},mark=oplus*\\%
 RdBu-10-10!70, every mark/.append style={solid,fill=RdBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-11}{%
 RdBu-11-1!70, every mark/.append style={solid,fill=RdBu-11-1},mark=*\\%
 RdBu-11-2!70, every mark/.append style={solid,fill=RdBu-11-2},mark=square*\\%
 RdBu-11-3!70, every mark/.append style={solid,fill=RdBu-11-3},mark=triangle*\\%
 RdBu-11-4!70, every mark/.append style={solid,fill=RdBu-11-4},mark=diamond*\\%
 RdBu-11-5!70, every mark/.append style={solid,fill=RdBu-11-5},mark=pentagon*\\%
 RdBu-11-6!70, every mark/.append style={solid,fill=RdBu-11-6},mark=x\\%
 RdBu-11-7!70, every mark/.append style={solid,fill=RdBu-11-7},mark=+\\%
 RdBu-11-8!70, every mark/.append style={solid,fill=RdBu-11-8},mark=star\\%
 RdBu-11-9!70, every mark/.append style={solid,fill=RdBu-11-9},mark=oplus*\\%
 RdBu-11-10!70, every mark/.append style={solid,fill=RdBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-3}{%
 RdGy-3-1!70, every mark/.append style={solid,fill=RdGy-3-1},mark=*\\%
 RdGy-3-2!70, every mark/.append style={solid,fill=RdGy-3-2},mark=square*\\%
 RdGy-3-3!70, every mark/.append style={solid,fill=RdGy-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-4}{%
 RdGy-4-1!70, every mark/.append style={solid,fill=RdGy-4-1},mark=*\\%
 RdGy-4-2!70, every mark/.append style={solid,fill=RdGy-4-2},mark=square*\\%
 RdGy-4-3!70, every mark/.append style={solid,fill=RdGy-4-3},mark=triangle*\\%
 RdGy-4-4!70, every mark/.append style={solid,fill=RdGy-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-5}{%
 RdGy-5-1!70, every mark/.append style={solid,fill=RdGy-5-1},mark=*\\%
 RdGy-5-2!70, every mark/.append style={solid,fill=RdGy-5-2},mark=square*\\%
 RdGy-5-3!70, every mark/.append style={solid,fill=RdGy-5-3},mark=triangle*\\%
 RdGy-5-4!70, every mark/.append style={solid,fill=RdGy-5-4},mark=diamond*\\%
 RdGy-5-5!70, every mark/.append style={solid,fill=RdGy-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-6}{%
 RdGy-6-1!70, every mark/.append style={solid,fill=RdGy-6-1},mark=*\\%
 RdGy-6-2!70, every mark/.append style={solid,fill=RdGy-6-2},mark=square*\\%
 RdGy-6-3!70, every mark/.append style={solid,fill=RdGy-6-3},mark=triangle*\\%
 RdGy-6-4!70, every mark/.append style={solid,fill=RdGy-6-4},mark=diamond*\\%
 RdGy-6-5!70, every mark/.append style={solid,fill=RdGy-6-5},mark=pentagon*\\%
 RdGy-6-6!70, every mark/.append style={solid,fill=RdGy-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-7}{%
 RdGy-7-1!70, every mark/.append style={solid,fill=RdGy-7-1},mark=*\\%
 RdGy-7-2!70, every mark/.append style={solid,fill=RdGy-7-2},mark=square*\\%
 RdGy-7-3!70, every mark/.append style={solid,fill=RdGy-7-3},mark=triangle*\\%
 RdGy-7-4!70, every mark/.append style={solid,fill=RdGy-7-4},mark=diamond*\\%
 RdGy-7-5!70, every mark/.append style={solid,fill=RdGy-7-5},mark=pentagon*\\%
 RdGy-7-6!70, every mark/.append style={solid,fill=RdGy-7-6},mark=x\\%
 RdGy-7-7!70, every mark/.append style={solid,fill=RdGy-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-8}{%
 RdGy-8-1!70, every mark/.append style={solid,fill=RdGy-8-1},mark=*\\%
 RdGy-8-2!70, every mark/.append style={solid,fill=RdGy-8-2},mark=square*\\%
 RdGy-8-3!70, every mark/.append style={solid,fill=RdGy-8-3},mark=triangle*\\%
 RdGy-8-4!70, every mark/.append style={solid,fill=RdGy-8-4},mark=diamond*\\%
 RdGy-8-5!70, every mark/.append style={solid,fill=RdGy-8-5},mark=pentagon*\\%
 RdGy-8-6!70, every mark/.append style={solid,fill=RdGy-8-6},mark=x\\%
 RdGy-8-7!70, every mark/.append style={solid,fill=RdGy-8-7},mark=+\\%
 RdGy-8-8!70, every mark/.append style={solid,fill=RdGy-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-9}{%
 RdGy-9-1!70, every mark/.append style={solid,fill=RdGy-9-1},mark=*\\%
 RdGy-9-2!70, every mark/.append style={solid,fill=RdGy-9-2},mark=square*\\%
 RdGy-9-3!70, every mark/.append style={solid,fill=RdGy-9-3},mark=triangle*\\%
 RdGy-9-4!70, every mark/.append style={solid,fill=RdGy-9-4},mark=diamond*\\%
 RdGy-9-5!70, every mark/.append style={solid,fill=RdGy-9-5},mark=pentagon*\\%
 RdGy-9-6!70, every mark/.append style={solid,fill=RdGy-9-6},mark=x\\%
 RdGy-9-7!70, every mark/.append style={solid,fill=RdGy-9-7},mark=+\\%
 RdGy-9-8!70, every mark/.append style={solid,fill=RdGy-9-8},mark=star\\%
 RdGy-9-9!70, every mark/.append style={solid,fill=RdGy-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-10}{%
 RdGy-10-1!70, every mark/.append style={solid,fill=RdGy-10-1},mark=*\\%
 RdGy-10-2!70, every mark/.append style={solid,fill=RdGy-10-2},mark=square*\\%
 RdGy-10-3!70, every mark/.append style={solid,fill=RdGy-10-3},mark=triangle*\\%
 RdGy-10-4!70, every mark/.append style={solid,fill=RdGy-10-4},mark=diamond*\\%
 RdGy-10-5!70, every mark/.append style={solid,fill=RdGy-10-5},mark=pentagon*\\%
 RdGy-10-6!70, every mark/.append style={solid,fill=RdGy-10-6},mark=x\\%
 RdGy-10-7!70, every mark/.append style={solid,fill=RdGy-10-7},mark=+\\%
 RdGy-10-8!70, every mark/.append style={solid,fill=RdGy-10-8},mark=star\\%
 RdGy-10-9!70, every mark/.append style={solid,fill=RdGy-10-9},mark=oplus*\\%
 RdGy-10-10!70, every mark/.append style={solid,fill=RdGy-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-11}{%
 RdGy-11-1!70, every mark/.append style={solid,fill=RdGy-11-1},mark=*\\%
 RdGy-11-2!70, every mark/.append style={solid,fill=RdGy-11-2},mark=square*\\%
 RdGy-11-3!70, every mark/.append style={solid,fill=RdGy-11-3},mark=triangle*\\%
 RdGy-11-4!70, every mark/.append style={solid,fill=RdGy-11-4},mark=diamond*\\%
 RdGy-11-5!70, every mark/.append style={solid,fill=RdGy-11-5},mark=pentagon*\\%
 RdGy-11-6!70, every mark/.append style={solid,fill=RdGy-11-6},mark=x\\%
 RdGy-11-7!70, every mark/.append style={solid,fill=RdGy-11-7},mark=+\\%
 RdGy-11-8!70, every mark/.append style={solid,fill=RdGy-11-8},mark=star\\%
 RdGy-11-9!70, every mark/.append style={solid,fill=RdGy-11-9},mark=oplus*\\%
 RdGy-11-10!70, every mark/.append style={solid,fill=RdGy-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-3}{%
 RdYlBu-3-1!70, every mark/.append style={solid,fill=RdYlBu-3-1},mark=*\\%
 RdYlBu-3-2!70, every mark/.append style={solid,fill=RdYlBu-3-2},mark=square*\\%
 RdYlBu-3-3!70, every mark/.append style={solid,fill=RdYlBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-4}{%
 RdYlBu-4-1!70, every mark/.append style={solid,fill=RdYlBu-4-1},mark=*\\%
 RdYlBu-4-2!70, every mark/.append style={solid,fill=RdYlBu-4-2},mark=square*\\%
 RdYlBu-4-3!70, every mark/.append style={solid,fill=RdYlBu-4-3},mark=triangle*\\%
 RdYlBu-4-4!70, every mark/.append style={solid,fill=RdYlBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-5}{%
 RdYlBu-5-1!70, every mark/.append style={solid,fill=RdYlBu-5-1},mark=*\\%
 RdYlBu-5-2!70, every mark/.append style={solid,fill=RdYlBu-5-2},mark=square*\\%
 RdYlBu-5-3!70, every mark/.append style={solid,fill=RdYlBu-5-3},mark=triangle*\\%
 RdYlBu-5-4!70, every mark/.append style={solid,fill=RdYlBu-5-4},mark=diamond*\\%
 RdYlBu-5-5!70, every mark/.append style={solid,fill=RdYlBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-6}{%
 RdYlBu-6-1!70, every mark/.append style={solid,fill=RdYlBu-6-1},mark=*\\%
 RdYlBu-6-2!70, every mark/.append style={solid,fill=RdYlBu-6-2},mark=square*\\%
 RdYlBu-6-3!70, every mark/.append style={solid,fill=RdYlBu-6-3},mark=triangle*\\%
 RdYlBu-6-4!70, every mark/.append style={solid,fill=RdYlBu-6-4},mark=diamond*\\%
 RdYlBu-6-5!70, every mark/.append style={solid,fill=RdYlBu-6-5},mark=pentagon*\\%
 RdYlBu-6-6!70, every mark/.append style={solid,fill=RdYlBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-7}{%
 RdYlBu-7-1!70, every mark/.append style={solid,fill=RdYlBu-7-1},mark=*\\%
 RdYlBu-7-2!70, every mark/.append style={solid,fill=RdYlBu-7-2},mark=square*\\%
 RdYlBu-7-3!70, every mark/.append style={solid,fill=RdYlBu-7-3},mark=triangle*\\%
 RdYlBu-7-4!70, every mark/.append style={solid,fill=RdYlBu-7-4},mark=diamond*\\%
 RdYlBu-7-5!70, every mark/.append style={solid,fill=RdYlBu-7-5},mark=pentagon*\\%
 RdYlBu-7-6!70, every mark/.append style={solid,fill=RdYlBu-7-6},mark=x\\%
 RdYlBu-7-7!70, every mark/.append style={solid,fill=RdYlBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-8}{%
 RdYlBu-8-1!70, every mark/.append style={solid,fill=RdYlBu-8-1},mark=*\\%
 RdYlBu-8-2!70, every mark/.append style={solid,fill=RdYlBu-8-2},mark=square*\\%
 RdYlBu-8-3!70, every mark/.append style={solid,fill=RdYlBu-8-3},mark=triangle*\\%
 RdYlBu-8-4!70, every mark/.append style={solid,fill=RdYlBu-8-4},mark=diamond*\\%
 RdYlBu-8-5!70, every mark/.append style={solid,fill=RdYlBu-8-5},mark=pentagon*\\%
 RdYlBu-8-6!70, every mark/.append style={solid,fill=RdYlBu-8-6},mark=x\\%
 RdYlBu-8-7!70, every mark/.append style={solid,fill=RdYlBu-8-7},mark=+\\%
 RdYlBu-8-8!70, every mark/.append style={solid,fill=RdYlBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-9}{%
 RdYlBu-9-1!70, every mark/.append style={solid,fill=RdYlBu-9-1},mark=*\\%
 RdYlBu-9-2!70, every mark/.append style={solid,fill=RdYlBu-9-2},mark=square*\\%
 RdYlBu-9-3!70, every mark/.append style={solid,fill=RdYlBu-9-3},mark=triangle*\\%
 RdYlBu-9-4!70, every mark/.append style={solid,fill=RdYlBu-9-4},mark=diamond*\\%
 RdYlBu-9-5!70, every mark/.append style={solid,fill=RdYlBu-9-5},mark=pentagon*\\%
 RdYlBu-9-6!70, every mark/.append style={solid,fill=RdYlBu-9-6},mark=x\\%
 RdYlBu-9-7!70, every mark/.append style={solid,fill=RdYlBu-9-7},mark=+\\%
 RdYlBu-9-8!70, every mark/.append style={solid,fill=RdYlBu-9-8},mark=star\\%
 RdYlBu-9-9!70, every mark/.append style={solid,fill=RdYlBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-10}{%
 RdYlBu-10-1!70, every mark/.append style={solid,fill=RdYlBu-10-1},mark=*\\%
 RdYlBu-10-2!70, every mark/.append style={solid,fill=RdYlBu-10-2},mark=square*\\%
 RdYlBu-10-3!70, every mark/.append style={solid,fill=RdYlBu-10-3},mark=triangle*\\%
 RdYlBu-10-4!70, every mark/.append style={solid,fill=RdYlBu-10-4},mark=diamond*\\%
 RdYlBu-10-5!70, every mark/.append style={solid,fill=RdYlBu-10-5},mark=pentagon*\\%
 RdYlBu-10-6!70, every mark/.append style={solid,fill=RdYlBu-10-6},mark=x\\%
 RdYlBu-10-7!70, every mark/.append style={solid,fill=RdYlBu-10-7},mark=+\\%
 RdYlBu-10-8!70, every mark/.append style={solid,fill=RdYlBu-10-8},mark=star\\%
 RdYlBu-10-9!70, every mark/.append style={solid,fill=RdYlBu-10-9},mark=oplus*\\%
 RdYlBu-10-10!70, every mark/.append style={solid,fill=RdYlBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-11}{%
 RdYlBu-11-1!70, every mark/.append style={solid,fill=RdYlBu-11-1},mark=*\\%
 RdYlBu-11-2!70, every mark/.append style={solid,fill=RdYlBu-11-2},mark=square*\\%
 RdYlBu-11-3!70, every mark/.append style={solid,fill=RdYlBu-11-3},mark=triangle*\\%
 RdYlBu-11-4!70, every mark/.append style={solid,fill=RdYlBu-11-4},mark=diamond*\\%
 RdYlBu-11-5!70, every mark/.append style={solid,fill=RdYlBu-11-5},mark=pentagon*\\%
 RdYlBu-11-6!70, every mark/.append style={solid,fill=RdYlBu-11-6},mark=x\\%
 RdYlBu-11-7!70, every mark/.append style={solid,fill=RdYlBu-11-7},mark=+\\%
 RdYlBu-11-8!70, every mark/.append style={solid,fill=RdYlBu-11-8},mark=star\\%
 RdYlBu-11-9!70, every mark/.append style={solid,fill=RdYlBu-11-9},mark=oplus*\\%
 RdYlBu-11-10!70, every mark/.append style={solid,fill=RdYlBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-3}{%
 Spectral-3-1!70, every mark/.append style={solid,fill=Spectral-3-1},mark=*\\%
 Spectral-3-2!70, every mark/.append style={solid,fill=Spectral-3-2},mark=square*\\%
 Spectral-3-3!70, every mark/.append style={solid,fill=Spectral-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-4}{%
 Spectral-4-1!70, every mark/.append style={solid,fill=Spectral-4-1},mark=*\\%
 Spectral-4-2!70, every mark/.append style={solid,fill=Spectral-4-2},mark=square*\\%
 Spectral-4-3!70, every mark/.append style={solid,fill=Spectral-4-3},mark=triangle*\\%
 Spectral-4-4!70, every mark/.append style={solid,fill=Spectral-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-5}{%
 Spectral-5-1!70, every mark/.append style={solid,fill=Spectral-5-1},mark=*\\%
 Spectral-5-2!70, every mark/.append style={solid,fill=Spectral-5-2},mark=square*\\%
 Spectral-5-3!70, every mark/.append style={solid,fill=Spectral-5-3},mark=triangle*\\%
 Spectral-5-4!70, every mark/.append style={solid,fill=Spectral-5-4},mark=diamond*\\%
 Spectral-5-5!70, every mark/.append style={solid,fill=Spectral-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-6}{%
 Spectral-6-1!70, every mark/.append style={solid,fill=Spectral-6-1},mark=*\\%
 Spectral-6-2!70, every mark/.append style={solid,fill=Spectral-6-2},mark=square*\\%
 Spectral-6-3!70, every mark/.append style={solid,fill=Spectral-6-3},mark=triangle*\\%
 Spectral-6-4!70, every mark/.append style={solid,fill=Spectral-6-4},mark=diamond*\\%
 Spectral-6-5!70, every mark/.append style={solid,fill=Spectral-6-5},mark=pentagon*\\%
 Spectral-6-6!70, every mark/.append style={solid,fill=Spectral-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-7}{%
 Spectral-7-1!70, every mark/.append style={solid,fill=Spectral-7-1},mark=*\\%
 Spectral-7-2!70, every mark/.append style={solid,fill=Spectral-7-2},mark=square*\\%
 Spectral-7-3!70, every mark/.append style={solid,fill=Spectral-7-3},mark=triangle*\\%
 Spectral-7-4!70, every mark/.append style={solid,fill=Spectral-7-4},mark=diamond*\\%
 Spectral-7-5!70, every mark/.append style={solid,fill=Spectral-7-5},mark=pentagon*\\%
 Spectral-7-6!70, every mark/.append style={solid,fill=Spectral-7-6},mark=x\\%
 Spectral-7-7!70, every mark/.append style={solid,fill=Spectral-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-8}{%
 Spectral-8-1!70, every mark/.append style={solid,fill=Spectral-8-1},mark=*\\%
 Spectral-8-2!70, every mark/.append style={solid,fill=Spectral-8-2},mark=square*\\%
 Spectral-8-3!70, every mark/.append style={solid,fill=Spectral-8-3},mark=triangle*\\%
 Spectral-8-4!70, every mark/.append style={solid,fill=Spectral-8-4},mark=diamond*\\%
 Spectral-8-5!70, every mark/.append style={solid,fill=Spectral-8-5},mark=pentagon*\\%
 Spectral-8-6!70, every mark/.append style={solid,fill=Spectral-8-6},mark=x\\%
 Spectral-8-7!70, every mark/.append style={solid,fill=Spectral-8-7},mark=+\\%
 Spectral-8-8!70, every mark/.append style={solid,fill=Spectral-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-9}{%
 Spectral-9-1!70, every mark/.append style={solid,fill=Spectral-9-1},mark=*\\%
 Spectral-9-2!70, every mark/.append style={solid,fill=Spectral-9-2},mark=square*\\%
 Spectral-9-3!70, every mark/.append style={solid,fill=Spectral-9-3},mark=triangle*\\%
 Spectral-9-4!70, every mark/.append style={solid,fill=Spectral-9-4},mark=diamond*\\%
 Spectral-9-5!70, every mark/.append style={solid,fill=Spectral-9-5},mark=pentagon*\\%
 Spectral-9-6!70, every mark/.append style={solid,fill=Spectral-9-6},mark=x\\%
 Spectral-9-7!70, every mark/.append style={solid,fill=Spectral-9-7},mark=+\\%
 Spectral-9-8!70, every mark/.append style={solid,fill=Spectral-9-8},mark=star\\%
 Spectral-9-9!70, every mark/.append style={solid,fill=Spectral-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-10}{%
 Spectral-10-1!70, every mark/.append style={solid,fill=Spectral-10-1},mark=*\\%
 Spectral-10-2!70, every mark/.append style={solid,fill=Spectral-10-2},mark=square*\\%
 Spectral-10-3!70, every mark/.append style={solid,fill=Spectral-10-3},mark=triangle*\\%
 Spectral-10-4!70, every mark/.append style={solid,fill=Spectral-10-4},mark=diamond*\\%
 Spectral-10-5!70, every mark/.append style={solid,fill=Spectral-10-5},mark=pentagon*\\%
 Spectral-10-6!70, every mark/.append style={solid,fill=Spectral-10-6},mark=x\\%
 Spectral-10-7!70, every mark/.append style={solid,fill=Spectral-10-7},mark=+\\%
 Spectral-10-8!70, every mark/.append style={solid,fill=Spectral-10-8},mark=star\\%
 Spectral-10-9!70, every mark/.append style={solid,fill=Spectral-10-9},mark=oplus*\\%
 Spectral-10-10!70, every mark/.append style={solid,fill=Spectral-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-11}{%
 Spectral-11-1!70, every mark/.append style={solid,fill=Spectral-11-1},mark=*\\%
 Spectral-11-2!70, every mark/.append style={solid,fill=Spectral-11-2},mark=square*\\%
 Spectral-11-3!70, every mark/.append style={solid,fill=Spectral-11-3},mark=triangle*\\%
 Spectral-11-4!70, every mark/.append style={solid,fill=Spectral-11-4},mark=diamond*\\%
 Spectral-11-5!70, every mark/.append style={solid,fill=Spectral-11-5},mark=pentagon*\\%
 Spectral-11-6!70, every mark/.append style={solid,fill=Spectral-11-6},mark=x\\%
 Spectral-11-7!70, every mark/.append style={solid,fill=Spectral-11-7},mark=+\\%
 Spectral-11-8!70, every mark/.append style={solid,fill=Spectral-11-8},mark=star\\%
 Spectral-11-9!70, every mark/.append style={solid,fill=Spectral-11-9},mark=oplus*\\%
 Spectral-11-10!70, every mark/.append style={solid,fill=Spectral-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-3}{%
 RdYlGn-3-1!70, every mark/.append style={solid,fill=RdYlGn-3-1},mark=*\\%
 RdYlGn-3-2!70, every mark/.append style={solid,fill=RdYlGn-3-2},mark=square*\\%
 RdYlGn-3-3!70, every mark/.append style={solid,fill=RdYlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-4}{%
 RdYlGn-4-1!70, every mark/.append style={solid,fill=RdYlGn-4-1},mark=*\\%
 RdYlGn-4-2!70, every mark/.append style={solid,fill=RdYlGn-4-2},mark=square*\\%
 RdYlGn-4-3!70, every mark/.append style={solid,fill=RdYlGn-4-3},mark=triangle*\\%
 RdYlGn-4-4!70, every mark/.append style={solid,fill=RdYlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-5}{%
 RdYlGn-5-1!70, every mark/.append style={solid,fill=RdYlGn-5-1},mark=*\\%
 RdYlGn-5-2!70, every mark/.append style={solid,fill=RdYlGn-5-2},mark=square*\\%
 RdYlGn-5-3!70, every mark/.append style={solid,fill=RdYlGn-5-3},mark=triangle*\\%
 RdYlGn-5-4!70, every mark/.append style={solid,fill=RdYlGn-5-4},mark=diamond*\\%
 RdYlGn-5-5!70, every mark/.append style={solid,fill=RdYlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-6}{%
 RdYlGn-6-1!70, every mark/.append style={solid,fill=RdYlGn-6-1},mark=*\\%
 RdYlGn-6-2!70, every mark/.append style={solid,fill=RdYlGn-6-2},mark=square*\\%
 RdYlGn-6-3!70, every mark/.append style={solid,fill=RdYlGn-6-3},mark=triangle*\\%
 RdYlGn-6-4!70, every mark/.append style={solid,fill=RdYlGn-6-4},mark=diamond*\\%
 RdYlGn-6-5!70, every mark/.append style={solid,fill=RdYlGn-6-5},mark=pentagon*\\%
 RdYlGn-6-6!70, every mark/.append style={solid,fill=RdYlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-7}{%
 RdYlGn-7-1!70, every mark/.append style={solid,fill=RdYlGn-7-1},mark=*\\%
 RdYlGn-7-2!70, every mark/.append style={solid,fill=RdYlGn-7-2},mark=square*\\%
 RdYlGn-7-3!70, every mark/.append style={solid,fill=RdYlGn-7-3},mark=triangle*\\%
 RdYlGn-7-4!70, every mark/.append style={solid,fill=RdYlGn-7-4},mark=diamond*\\%
 RdYlGn-7-5!70, every mark/.append style={solid,fill=RdYlGn-7-5},mark=pentagon*\\%
 RdYlGn-7-6!70, every mark/.append style={solid,fill=RdYlGn-7-6},mark=x\\%
 RdYlGn-7-7!70, every mark/.append style={solid,fill=RdYlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-8}{%
 RdYlGn-8-1!70, every mark/.append style={solid,fill=RdYlGn-8-1},mark=*\\%
 RdYlGn-8-2!70, every mark/.append style={solid,fill=RdYlGn-8-2},mark=square*\\%
 RdYlGn-8-3!70, every mark/.append style={solid,fill=RdYlGn-8-3},mark=triangle*\\%
 RdYlGn-8-4!70, every mark/.append style={solid,fill=RdYlGn-8-4},mark=diamond*\\%
 RdYlGn-8-5!70, every mark/.append style={solid,fill=RdYlGn-8-5},mark=pentagon*\\%
 RdYlGn-8-6!70, every mark/.append style={solid,fill=RdYlGn-8-6},mark=x\\%
 RdYlGn-8-7!70, every mark/.append style={solid,fill=RdYlGn-8-7},mark=+\\%
 RdYlGn-8-8!70, every mark/.append style={solid,fill=RdYlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-9}{%
 RdYlGn-9-1!70, every mark/.append style={solid,fill=RdYlGn-9-1},mark=*\\%
 RdYlGn-9-2!70, every mark/.append style={solid,fill=RdYlGn-9-2},mark=square*\\%
 RdYlGn-9-3!70, every mark/.append style={solid,fill=RdYlGn-9-3},mark=triangle*\\%
 RdYlGn-9-4!70, every mark/.append style={solid,fill=RdYlGn-9-4},mark=diamond*\\%
 RdYlGn-9-5!70, every mark/.append style={solid,fill=RdYlGn-9-5},mark=pentagon*\\%
 RdYlGn-9-6!70, every mark/.append style={solid,fill=RdYlGn-9-6},mark=x\\%
 RdYlGn-9-7!70, every mark/.append style={solid,fill=RdYlGn-9-7},mark=+\\%
 RdYlGn-9-8!70, every mark/.append style={solid,fill=RdYlGn-9-8},mark=star\\%
 RdYlGn-9-9!70, every mark/.append style={solid,fill=RdYlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-10}{%
 RdYlGn-10-1!70, every mark/.append style={solid,fill=RdYlGn-10-1},mark=*\\%
 RdYlGn-10-2!70, every mark/.append style={solid,fill=RdYlGn-10-2},mark=square*\\%
 RdYlGn-10-3!70, every mark/.append style={solid,fill=RdYlGn-10-3},mark=triangle*\\%
 RdYlGn-10-4!70, every mark/.append style={solid,fill=RdYlGn-10-4},mark=diamond*\\%
 RdYlGn-10-5!70, every mark/.append style={solid,fill=RdYlGn-10-5},mark=pentagon*\\%
 RdYlGn-10-6!70, every mark/.append style={solid,fill=RdYlGn-10-6},mark=x\\%
 RdYlGn-10-7!70, every mark/.append style={solid,fill=RdYlGn-10-7},mark=+\\%
 RdYlGn-10-8!70, every mark/.append style={solid,fill=RdYlGn-10-8},mark=star\\%
 RdYlGn-10-9!70, every mark/.append style={solid,fill=RdYlGn-10-9},mark=oplus*\\%
 RdYlGn-10-10!70, every mark/.append style={solid,fill=RdYlGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-11}{%
 RdYlGn-11-1!70, every mark/.append style={solid,fill=RdYlGn-11-1},mark=*\\%
 RdYlGn-11-2!70, every mark/.append style={solid,fill=RdYlGn-11-2},mark=square*\\%
 RdYlGn-11-3!70, every mark/.append style={solid,fill=RdYlGn-11-3},mark=triangle*\\%
 RdYlGn-11-4!70, every mark/.append style={solid,fill=RdYlGn-11-4},mark=diamond*\\%
 RdYlGn-11-5!70, every mark/.append style={solid,fill=RdYlGn-11-5},mark=pentagon*\\%
 RdYlGn-11-6!70, every mark/.append style={solid,fill=RdYlGn-11-6},mark=x\\%
 RdYlGn-11-7!70, every mark/.append style={solid,fill=RdYlGn-11-7},mark=+\\%
 RdYlGn-11-8!70, every mark/.append style={solid,fill=RdYlGn-11-8},mark=star\\%
 RdYlGn-11-9!70, every mark/.append style={solid,fill=RdYlGn-11-9},mark=oplus*\\%
 RdYlGn-11-10!70, every mark/.append style={solid,fill=RdYlGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-3}{%
 Set3-3-1!70, every mark/.append style={solid,fill=Set3-3-1},mark=*\\%
 Set3-3-2!70, every mark/.append style={solid,fill=Set3-3-2},mark=square*\\%
 Set3-3-3!70, every mark/.append style={solid,fill=Set3-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-4}{%
 Set3-4-1!70, every mark/.append style={solid,fill=Set3-4-1},mark=*\\%
 Set3-4-2!70, every mark/.append style={solid,fill=Set3-4-2},mark=square*\\%
 Set3-4-3!70, every mark/.append style={solid,fill=Set3-4-3},mark=triangle*\\%
 Set3-4-4!70, every mark/.append style={solid,fill=Set3-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-5}{%
 Set3-5-1!70, every mark/.append style={solid,fill=Set3-5-1},mark=*\\%
 Set3-5-2!70, every mark/.append style={solid,fill=Set3-5-2},mark=square*\\%
 Set3-5-3!70, every mark/.append style={solid,fill=Set3-5-3},mark=triangle*\\%
 Set3-5-4!70, every mark/.append style={solid,fill=Set3-5-4},mark=diamond*\\%
 Set3-5-5!70, every mark/.append style={solid,fill=Set3-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-6}{%
 Set3-6-1!70, every mark/.append style={solid,fill=Set3-6-1},mark=*\\%
 Set3-6-2!70, every mark/.append style={solid,fill=Set3-6-2},mark=square*\\%
 Set3-6-3!70, every mark/.append style={solid,fill=Set3-6-3},mark=triangle*\\%
 Set3-6-4!70, every mark/.append style={solid,fill=Set3-6-4},mark=diamond*\\%
 Set3-6-5!70, every mark/.append style={solid,fill=Set3-6-5},mark=pentagon*\\%
 Set3-6-6!70, every mark/.append style={solid,fill=Set3-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-7}{%
 Set3-7-1!70, every mark/.append style={solid,fill=Set3-7-1},mark=*\\%
 Set3-7-2!70, every mark/.append style={solid,fill=Set3-7-2},mark=square*\\%
 Set3-7-3!70, every mark/.append style={solid,fill=Set3-7-3},mark=triangle*\\%
 Set3-7-4!70, every mark/.append style={solid,fill=Set3-7-4},mark=diamond*\\%
 Set3-7-5!70, every mark/.append style={solid,fill=Set3-7-5},mark=pentagon*\\%
 Set3-7-6!70, every mark/.append style={solid,fill=Set3-7-6},mark=x\\%
 Set3-7-7!70, every mark/.append style={solid,fill=Set3-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-8}{%
 Set3-8-1!70, every mark/.append style={solid,fill=Set3-8-1},mark=*\\%
 Set3-8-2!70, every mark/.append style={solid,fill=Set3-8-2},mark=square*\\%
 Set3-8-3!70, every mark/.append style={solid,fill=Set3-8-3},mark=triangle*\\%
 Set3-8-4!70, every mark/.append style={solid,fill=Set3-8-4},mark=diamond*\\%
 Set3-8-5!70, every mark/.append style={solid,fill=Set3-8-5},mark=pentagon*\\%
 Set3-8-6!70, every mark/.append style={solid,fill=Set3-8-6},mark=x\\%
 Set3-8-7!70, every mark/.append style={solid,fill=Set3-8-7},mark=+\\%
 Set3-8-8!70, every mark/.append style={solid,fill=Set3-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-9}{%
 Set3-9-1!70, every mark/.append style={solid,fill=Set3-9-1},mark=*\\%
 Set3-9-2!70, every mark/.append style={solid,fill=Set3-9-2},mark=square*\\%
 Set3-9-3!70, every mark/.append style={solid,fill=Set3-9-3},mark=triangle*\\%
 Set3-9-4!70, every mark/.append style={solid,fill=Set3-9-4},mark=diamond*\\%
 Set3-9-5!70, every mark/.append style={solid,fill=Set3-9-5},mark=pentagon*\\%
 Set3-9-6!70, every mark/.append style={solid,fill=Set3-9-6},mark=x\\%
 Set3-9-7!70, every mark/.append style={solid,fill=Set3-9-7},mark=+\\%
 Set3-9-8!70, every mark/.append style={solid,fill=Set3-9-8},mark=star\\%
 Set3-9-9!70, every mark/.append style={solid,fill=Set3-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-10}{%
 Set3-10-1!70, every mark/.append style={solid,fill=Set3-10-1},mark=*\\%
 Set3-10-2!70, every mark/.append style={solid,fill=Set3-10-2},mark=square*\\%
 Set3-10-3!70, every mark/.append style={solid,fill=Set3-10-3},mark=triangle*\\%
 Set3-10-4!70, every mark/.append style={solid,fill=Set3-10-4},mark=diamond*\\%
 Set3-10-5!70, every mark/.append style={solid,fill=Set3-10-5},mark=pentagon*\\%
 Set3-10-6!70, every mark/.append style={solid,fill=Set3-10-6},mark=x\\%
 Set3-10-7!70, every mark/.append style={solid,fill=Set3-10-7},mark=+\\%
 Set3-10-8!70, every mark/.append style={solid,fill=Set3-10-8},mark=star\\%
 Set3-10-9!70, every mark/.append style={solid,fill=Set3-10-9},mark=oplus*\\%
 Set3-10-10!70, every mark/.append style={solid,fill=Set3-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-11}{%
 Set3-11-1!70, every mark/.append style={solid,fill=Set3-11-1},mark=*\\%
 Set3-11-2!70, every mark/.append style={solid,fill=Set3-11-2},mark=square*\\%
 Set3-11-3!70, every mark/.append style={solid,fill=Set3-11-3},mark=triangle*\\%
 Set3-11-4!70, every mark/.append style={solid,fill=Set3-11-4},mark=diamond*\\%
 Set3-11-5!70, every mark/.append style={solid,fill=Set3-11-5},mark=pentagon*\\%
 Set3-11-6!70, every mark/.append style={solid,fill=Set3-11-6},mark=x\\%
 Set3-11-7!70, every mark/.append style={solid,fill=Set3-11-7},mark=+\\%
 Set3-11-8!70, every mark/.append style={solid,fill=Set3-11-8},mark=star\\%
 Set3-11-9!70, every mark/.append style={solid,fill=Set3-11-9},mark=oplus*\\%
 Set3-11-10!70, every mark/.append style={solid,fill=Set3-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-12}{%
 Set3-12-1!70, every mark/.append style={solid,fill=Set3-12-1},mark=*\\%
 Set3-12-2!70, every mark/.append style={solid,fill=Set3-12-2},mark=square*\\%
 Set3-12-3!70, every mark/.append style={solid,fill=Set3-12-3},mark=triangle*\\%
 Set3-12-4!70, every mark/.append style={solid,fill=Set3-12-4},mark=diamond*\\%
 Set3-12-5!70, every mark/.append style={solid,fill=Set3-12-5},mark=pentagon*\\%
 Set3-12-6!70, every mark/.append style={solid,fill=Set3-12-6},mark=x\\%
 Set3-12-7!70, every mark/.append style={solid,fill=Set3-12-7},mark=+\\%
 Set3-12-8!70, every mark/.append style={solid,fill=Set3-12-8},mark=star\\%
 Set3-12-9!70, every mark/.append style={solid,fill=Set3-12-9},mark=oplus*\\%
 Set3-12-10!70, every mark/.append style={solid,fill=Set3-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-3}{%
 Pastel1-3-1!70, every mark/.append style={solid,fill=Pastel1-3-1},mark=*\\%
 Pastel1-3-2!70, every mark/.append style={solid,fill=Pastel1-3-2},mark=square*\\%
 Pastel1-3-3!70, every mark/.append style={solid,fill=Pastel1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-4}{%
 Pastel1-4-1!70, every mark/.append style={solid,fill=Pastel1-4-1},mark=*\\%
 Pastel1-4-2!70, every mark/.append style={solid,fill=Pastel1-4-2},mark=square*\\%
 Pastel1-4-3!70, every mark/.append style={solid,fill=Pastel1-4-3},mark=triangle*\\%
 Pastel1-4-4!70, every mark/.append style={solid,fill=Pastel1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-5}{%
 Pastel1-5-1!70, every mark/.append style={solid,fill=Pastel1-5-1},mark=*\\%
 Pastel1-5-2!70, every mark/.append style={solid,fill=Pastel1-5-2},mark=square*\\%
 Pastel1-5-3!70, every mark/.append style={solid,fill=Pastel1-5-3},mark=triangle*\\%
 Pastel1-5-4!70, every mark/.append style={solid,fill=Pastel1-5-4},mark=diamond*\\%
 Pastel1-5-5!70, every mark/.append style={solid,fill=Pastel1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-6}{%
 Pastel1-6-1!70, every mark/.append style={solid,fill=Pastel1-6-1},mark=*\\%
 Pastel1-6-2!70, every mark/.append style={solid,fill=Pastel1-6-2},mark=square*\\%
 Pastel1-6-3!70, every mark/.append style={solid,fill=Pastel1-6-3},mark=triangle*\\%
 Pastel1-6-4!70, every mark/.append style={solid,fill=Pastel1-6-4},mark=diamond*\\%
 Pastel1-6-5!70, every mark/.append style={solid,fill=Pastel1-6-5},mark=pentagon*\\%
 Pastel1-6-6!70, every mark/.append style={solid,fill=Pastel1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-7}{%
 Pastel1-7-1!70, every mark/.append style={solid,fill=Pastel1-7-1},mark=*\\%
 Pastel1-7-2!70, every mark/.append style={solid,fill=Pastel1-7-2},mark=square*\\%
 Pastel1-7-3!70, every mark/.append style={solid,fill=Pastel1-7-3},mark=triangle*\\%
 Pastel1-7-4!70, every mark/.append style={solid,fill=Pastel1-7-4},mark=diamond*\\%
 Pastel1-7-5!70, every mark/.append style={solid,fill=Pastel1-7-5},mark=pentagon*\\%
 Pastel1-7-6!70, every mark/.append style={solid,fill=Pastel1-7-6},mark=x\\%
 Pastel1-7-7!70, every mark/.append style={solid,fill=Pastel1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-8}{%
 Pastel1-8-1!70, every mark/.append style={solid,fill=Pastel1-8-1},mark=*\\%
 Pastel1-8-2!70, every mark/.append style={solid,fill=Pastel1-8-2},mark=square*\\%
 Pastel1-8-3!70, every mark/.append style={solid,fill=Pastel1-8-3},mark=triangle*\\%
 Pastel1-8-4!70, every mark/.append style={solid,fill=Pastel1-8-4},mark=diamond*\\%
 Pastel1-8-5!70, every mark/.append style={solid,fill=Pastel1-8-5},mark=pentagon*\\%
 Pastel1-8-6!70, every mark/.append style={solid,fill=Pastel1-8-6},mark=x\\%
 Pastel1-8-7!70, every mark/.append style={solid,fill=Pastel1-8-7},mark=+\\%
 Pastel1-8-8!70, every mark/.append style={solid,fill=Pastel1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-9}{%
 Pastel1-9-1!70, every mark/.append style={solid,fill=Pastel1-9-1},mark=*\\%
 Pastel1-9-2!70, every mark/.append style={solid,fill=Pastel1-9-2},mark=square*\\%
 Pastel1-9-3!70, every mark/.append style={solid,fill=Pastel1-9-3},mark=triangle*\\%
 Pastel1-9-4!70, every mark/.append style={solid,fill=Pastel1-9-4},mark=diamond*\\%
 Pastel1-9-5!70, every mark/.append style={solid,fill=Pastel1-9-5},mark=pentagon*\\%
 Pastel1-9-6!70, every mark/.append style={solid,fill=Pastel1-9-6},mark=x\\%
 Pastel1-9-7!70, every mark/.append style={solid,fill=Pastel1-9-7},mark=+\\%
 Pastel1-9-8!70, every mark/.append style={solid,fill=Pastel1-9-8},mark=star\\%
 Pastel1-9-9!70, every mark/.append style={solid,fill=Pastel1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-3}{%
 Set1-3-1!70, every mark/.append style={solid,fill=Set1-3-1},mark=*\\%
 Set1-3-2!70, every mark/.append style={solid,fill=Set1-3-2},mark=square*\\%
 Set1-3-3!70, every mark/.append style={solid,fill=Set1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-4}{%
 Set1-4-1!70, every mark/.append style={solid,fill=Set1-4-1},mark=*\\%
 Set1-4-2!70, every mark/.append style={solid,fill=Set1-4-2},mark=square*\\%
 Set1-4-3!70, every mark/.append style={solid,fill=Set1-4-3},mark=triangle*\\%
 Set1-4-4!70, every mark/.append style={solid,fill=Set1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-5}{%
 Set1-5-1!70, every mark/.append style={solid,fill=Set1-5-1},mark=*\\%
 Set1-5-2!70, every mark/.append style={solid,fill=Set1-5-2},mark=square*\\%
 Set1-5-3!70, every mark/.append style={solid,fill=Set1-5-3},mark=triangle*\\%
 Set1-5-4!70, every mark/.append style={solid,fill=Set1-5-4},mark=diamond*\\%
 Set1-5-5!70, every mark/.append style={solid,fill=Set1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-6}{%
 Set1-6-1!70, every mark/.append style={solid,fill=Set1-6-1},mark=*\\%
 Set1-6-2!70, every mark/.append style={solid,fill=Set1-6-2},mark=square*\\%
 Set1-6-3!70, every mark/.append style={solid,fill=Set1-6-3},mark=triangle*\\%
 Set1-6-4!70, every mark/.append style={solid,fill=Set1-6-4},mark=diamond*\\%
 Set1-6-5!70, every mark/.append style={solid,fill=Set1-6-5},mark=pentagon*\\%
 Set1-6-6!70, every mark/.append style={solid,fill=Set1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-7}{%
 Set1-7-1!70, every mark/.append style={solid,fill=Set1-7-1},mark=*\\%
 Set1-7-2!70, every mark/.append style={solid,fill=Set1-7-2},mark=square*\\%
 Set1-7-3!70, every mark/.append style={solid,fill=Set1-7-3},mark=triangle*\\%
 Set1-7-4!70, every mark/.append style={solid,fill=Set1-7-4},mark=diamond*\\%
 Set1-7-5!70, every mark/.append style={solid,fill=Set1-7-5},mark=pentagon*\\%
 Set1-7-6!70, every mark/.append style={solid,fill=Set1-7-6},mark=x\\%
 Set1-7-7!70, every mark/.append style={solid,fill=Set1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-8}{%
 Set1-8-1!70, every mark/.append style={solid,fill=Set1-8-1},mark=*\\%
 Set1-8-2!70, every mark/.append style={solid,fill=Set1-8-2},mark=square*\\%
 Set1-8-3!70, every mark/.append style={solid,fill=Set1-8-3},mark=triangle*\\%
 Set1-8-4!70, every mark/.append style={solid,fill=Set1-8-4},mark=diamond*\\%
 Set1-8-5!70, every mark/.append style={solid,fill=Set1-8-5},mark=pentagon*\\%
 Set1-8-6!70, every mark/.append style={solid,fill=Set1-8-6},mark=x\\%
 Set1-8-7!70, every mark/.append style={solid,fill=Set1-8-7},mark=+\\%
 Set1-8-8!70, every mark/.append style={solid,fill=Set1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-9}{%
 Set1-9-1!70, every mark/.append style={solid,fill=Set1-9-1},mark=*\\%
 Set1-9-2!70, every mark/.append style={solid,fill=Set1-9-2},mark=square*\\%
 Set1-9-3!70, every mark/.append style={solid,fill=Set1-9-3},mark=triangle*\\%
 Set1-9-4!70, every mark/.append style={solid,fill=Set1-9-4},mark=diamond*\\%
 Set1-9-5!70, every mark/.append style={solid,fill=Set1-9-5},mark=pentagon*\\%
 Set1-9-6!70, every mark/.append style={solid,fill=Set1-9-6},mark=x\\%
 Set1-9-7!70, every mark/.append style={solid,fill=Set1-9-7},mark=+\\%
 Set1-9-8!70, every mark/.append style={solid,fill=Set1-9-8},mark=star\\%
 Set1-9-9!70, every mark/.append style={solid,fill=Set1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-3}{%
 Pastel2-3-1!70, every mark/.append style={solid,fill=Pastel2-3-1},mark=*\\%
 Pastel2-3-2!70, every mark/.append style={solid,fill=Pastel2-3-2},mark=square*\\%
 Pastel2-3-3!70, every mark/.append style={solid,fill=Pastel2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-4}{%
 Pastel2-4-1!70, every mark/.append style={solid,fill=Pastel2-4-1},mark=*\\%
 Pastel2-4-2!70, every mark/.append style={solid,fill=Pastel2-4-2},mark=square*\\%
 Pastel2-4-3!70, every mark/.append style={solid,fill=Pastel2-4-3},mark=triangle*\\%
 Pastel2-4-4!70, every mark/.append style={solid,fill=Pastel2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-5}{%
 Pastel2-5-1!70, every mark/.append style={solid,fill=Pastel2-5-1},mark=*\\%
 Pastel2-5-2!70, every mark/.append style={solid,fill=Pastel2-5-2},mark=square*\\%
 Pastel2-5-3!70, every mark/.append style={solid,fill=Pastel2-5-3},mark=triangle*\\%
 Pastel2-5-4!70, every mark/.append style={solid,fill=Pastel2-5-4},mark=diamond*\\%
 Pastel2-5-5!70, every mark/.append style={solid,fill=Pastel2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-6}{%
 Pastel2-6-1!70, every mark/.append style={solid,fill=Pastel2-6-1},mark=*\\%
 Pastel2-6-2!70, every mark/.append style={solid,fill=Pastel2-6-2},mark=square*\\%
 Pastel2-6-3!70, every mark/.append style={solid,fill=Pastel2-6-3},mark=triangle*\\%
 Pastel2-6-4!70, every mark/.append style={solid,fill=Pastel2-6-4},mark=diamond*\\%
 Pastel2-6-5!70, every mark/.append style={solid,fill=Pastel2-6-5},mark=pentagon*\\%
 Pastel2-6-6!70, every mark/.append style={solid,fill=Pastel2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-7}{%
 Pastel2-7-1!70, every mark/.append style={solid,fill=Pastel2-7-1},mark=*\\%
 Pastel2-7-2!70, every mark/.append style={solid,fill=Pastel2-7-2},mark=square*\\%
 Pastel2-7-3!70, every mark/.append style={solid,fill=Pastel2-7-3},mark=triangle*\\%
 Pastel2-7-4!70, every mark/.append style={solid,fill=Pastel2-7-4},mark=diamond*\\%
 Pastel2-7-5!70, every mark/.append style={solid,fill=Pastel2-7-5},mark=pentagon*\\%
 Pastel2-7-6!70, every mark/.append style={solid,fill=Pastel2-7-6},mark=x\\%
 Pastel2-7-7!70, every mark/.append style={solid,fill=Pastel2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-8}{%
 Pastel2-8-1!70, every mark/.append style={solid,fill=Pastel2-8-1},mark=*\\%
 Pastel2-8-2!70, every mark/.append style={solid,fill=Pastel2-8-2},mark=square*\\%
 Pastel2-8-3!70, every mark/.append style={solid,fill=Pastel2-8-3},mark=triangle*\\%
 Pastel2-8-4!70, every mark/.append style={solid,fill=Pastel2-8-4},mark=diamond*\\%
 Pastel2-8-5!70, every mark/.append style={solid,fill=Pastel2-8-5},mark=pentagon*\\%
 Pastel2-8-6!70, every mark/.append style={solid,fill=Pastel2-8-6},mark=x\\%
 Pastel2-8-7!70, every mark/.append style={solid,fill=Pastel2-8-7},mark=+\\%
 Pastel2-8-8!70, every mark/.append style={solid,fill=Pastel2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-3}{%
 Set2-3-1!70, every mark/.append style={solid,fill=Set2-3-1},mark=*\\%
 Set2-3-2!70, every mark/.append style={solid,fill=Set2-3-2},mark=square*\\%
 Set2-3-3!70, every mark/.append style={solid,fill=Set2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-4}{%
 Set2-4-1!70, every mark/.append style={solid,fill=Set2-4-1},mark=*\\%
 Set2-4-2!70, every mark/.append style={solid,fill=Set2-4-2},mark=square*\\%
 Set2-4-3!70, every mark/.append style={solid,fill=Set2-4-3},mark=triangle*\\%
 Set2-4-4!70, every mark/.append style={solid,fill=Set2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-5}{%
 Set2-5-1!70, every mark/.append style={solid,fill=Set2-5-1},mark=*\\%
 Set2-5-2!70, every mark/.append style={solid,fill=Set2-5-2},mark=square*\\%
 Set2-5-3!70, every mark/.append style={solid,fill=Set2-5-3},mark=triangle*\\%
 Set2-5-4!70, every mark/.append style={solid,fill=Set2-5-4},mark=diamond*\\%
 Set2-5-5!70, every mark/.append style={solid,fill=Set2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-6}{%
 Set2-6-1!70, every mark/.append style={solid,fill=Set2-6-1},mark=*\\%
 Set2-6-2!70, every mark/.append style={solid,fill=Set2-6-2},mark=square*\\%
 Set2-6-3!70, every mark/.append style={solid,fill=Set2-6-3},mark=triangle*\\%
 Set2-6-4!70, every mark/.append style={solid,fill=Set2-6-4},mark=diamond*\\%
 Set2-6-5!70, every mark/.append style={solid,fill=Set2-6-5},mark=pentagon*\\%
 Set2-6-6!70, every mark/.append style={solid,fill=Set2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-7}{%
 Set2-7-1!70, every mark/.append style={solid,fill=Set2-7-1},mark=*\\%
 Set2-7-2!70, every mark/.append style={solid,fill=Set2-7-2},mark=square*\\%
 Set2-7-3!70, every mark/.append style={solid,fill=Set2-7-3},mark=triangle*\\%
 Set2-7-4!70, every mark/.append style={solid,fill=Set2-7-4},mark=diamond*\\%
 Set2-7-5!70, every mark/.append style={solid,fill=Set2-7-5},mark=pentagon*\\%
 Set2-7-6!70, every mark/.append style={solid,fill=Set2-7-6},mark=x\\%
 Set2-7-7!70, every mark/.append style={solid,fill=Set2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-8}{%
 Set2-8-1!70, every mark/.append style={solid,fill=Set2-8-1},mark=*\\%
 Set2-8-2!70, every mark/.append style={solid,fill=Set2-8-2},mark=square*\\%
 Set2-8-3!70, every mark/.append style={solid,fill=Set2-8-3},mark=triangle*\\%
 Set2-8-4!70, every mark/.append style={solid,fill=Set2-8-4},mark=diamond*\\%
 Set2-8-5!70, every mark/.append style={solid,fill=Set2-8-5},mark=pentagon*\\%
 Set2-8-6!70, every mark/.append style={solid,fill=Set2-8-6},mark=x\\%
 Set2-8-7!70, every mark/.append style={solid,fill=Set2-8-7},mark=+\\%
 Set2-8-8!70, every mark/.append style={solid,fill=Set2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-3}{%
 Dark2-3-1!70, every mark/.append style={solid,fill=Dark2-3-1},mark=*\\%
 Dark2-3-2!70, every mark/.append style={solid,fill=Dark2-3-2},mark=square*\\%
 Dark2-3-3!70, every mark/.append style={solid,fill=Dark2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-4}{%
 Dark2-4-1!70, every mark/.append style={solid,fill=Dark2-4-1},mark=*\\%
 Dark2-4-2!70, every mark/.append style={solid,fill=Dark2-4-2},mark=square*\\%
 Dark2-4-3!70, every mark/.append style={solid,fill=Dark2-4-3},mark=triangle*\\%
 Dark2-4-4!70, every mark/.append style={solid,fill=Dark2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-5}{%
 Dark2-5-1!70, every mark/.append style={solid,fill=Dark2-5-1},mark=*\\%
 Dark2-5-2!70, every mark/.append style={solid,fill=Dark2-5-2},mark=square*\\%
 Dark2-5-3!70, every mark/.append style={solid,fill=Dark2-5-3},mark=triangle*\\%
 Dark2-5-4!70, every mark/.append style={solid,fill=Dark2-5-4},mark=diamond*\\%
 Dark2-5-5!70, every mark/.append style={solid,fill=Dark2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-6}{%
 Dark2-6-1!70, every mark/.append style={solid,fill=Dark2-6-1},mark=*\\%
 Dark2-6-2!70, every mark/.append style={solid,fill=Dark2-6-2},mark=square*\\%
 Dark2-6-3!70, every mark/.append style={solid,fill=Dark2-6-3},mark=triangle*\\%
 Dark2-6-4!70, every mark/.append style={solid,fill=Dark2-6-4},mark=diamond*\\%
 Dark2-6-5!70, every mark/.append style={solid,fill=Dark2-6-5},mark=pentagon*\\%
 Dark2-6-6!70, every mark/.append style={solid,fill=Dark2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-7}{%
 Dark2-7-1!70, every mark/.append style={solid,fill=Dark2-7-1},mark=*\\%
 Dark2-7-2!70, every mark/.append style={solid,fill=Dark2-7-2},mark=square*\\%
 Dark2-7-3!70, every mark/.append style={solid,fill=Dark2-7-3},mark=triangle*\\%
 Dark2-7-4!70, every mark/.append style={solid,fill=Dark2-7-4},mark=diamond*\\%
 Dark2-7-5!70, every mark/.append style={solid,fill=Dark2-7-5},mark=pentagon*\\%
 Dark2-7-6!70, every mark/.append style={solid,fill=Dark2-7-6},mark=x\\%
 Dark2-7-7!70, every mark/.append style={solid,fill=Dark2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-8}{%
 Dark2-8-1!70, every mark/.append style={solid,fill=Dark2-8-1},mark=*\\%
 Dark2-8-2!70, every mark/.append style={solid,fill=Dark2-8-2},mark=square*\\%
 Dark2-8-3!70, every mark/.append style={solid,fill=Dark2-8-3},mark=triangle*\\%
 Dark2-8-4!70, every mark/.append style={solid,fill=Dark2-8-4},mark=diamond*\\%
 Dark2-8-5!70, every mark/.append style={solid,fill=Dark2-8-5},mark=pentagon*\\%
 Dark2-8-6!70, every mark/.append style={solid,fill=Dark2-8-6},mark=x\\%
 Dark2-8-7!70, every mark/.append style={solid,fill=Dark2-8-7},mark=+\\%
 Dark2-8-8!70, every mark/.append style={solid,fill=Dark2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-3}{%
 Paired-3-1!70, every mark/.append style={solid,fill=Paired-3-1},mark=*\\%
 Paired-3-2!70, every mark/.append style={solid,fill=Paired-3-2},mark=square*\\%
 Paired-3-3!70, every mark/.append style={solid,fill=Paired-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-4}{%
 Paired-4-1!70, every mark/.append style={solid,fill=Paired-4-1},mark=*\\%
 Paired-4-2!70, every mark/.append style={solid,fill=Paired-4-2},mark=square*\\%
 Paired-4-3!70, every mark/.append style={solid,fill=Paired-4-3},mark=triangle*\\%
 Paired-4-4!70, every mark/.append style={solid,fill=Paired-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-5}{%
 Paired-5-1!70, every mark/.append style={solid,fill=Paired-5-1},mark=*\\%
 Paired-5-2!70, every mark/.append style={solid,fill=Paired-5-2},mark=square*\\%
 Paired-5-3!70, every mark/.append style={solid,fill=Paired-5-3},mark=triangle*\\%
 Paired-5-4!70, every mark/.append style={solid,fill=Paired-5-4},mark=diamond*\\%
 Paired-5-5!70, every mark/.append style={solid,fill=Paired-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-6}{%
 Paired-6-1!70, every mark/.append style={solid,fill=Paired-6-1},mark=*\\%
 Paired-6-2!70, every mark/.append style={solid,fill=Paired-6-2},mark=square*\\%
 Paired-6-3!70, every mark/.append style={solid,fill=Paired-6-3},mark=triangle*\\%
 Paired-6-4!70, every mark/.append style={solid,fill=Paired-6-4},mark=diamond*\\%
 Paired-6-5!70, every mark/.append style={solid,fill=Paired-6-5},mark=pentagon*\\%
 Paired-6-6!70, every mark/.append style={solid,fill=Paired-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-7}{%
 Paired-7-1!70, every mark/.append style={solid,fill=Paired-7-1},mark=*\\%
 Paired-7-2!70, every mark/.append style={solid,fill=Paired-7-2},mark=square*\\%
 Paired-7-3!70, every mark/.append style={solid,fill=Paired-7-3},mark=triangle*\\%
 Paired-7-4!70, every mark/.append style={solid,fill=Paired-7-4},mark=diamond*\\%
 Paired-7-5!70, every mark/.append style={solid,fill=Paired-7-5},mark=pentagon*\\%
 Paired-7-6!70, every mark/.append style={solid,fill=Paired-7-6},mark=x\\%
 Paired-7-7!70, every mark/.append style={solid,fill=Paired-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-8}{%
 Paired-8-1!70, every mark/.append style={solid,fill=Paired-8-1},mark=*\\%
 Paired-8-2!70, every mark/.append style={solid,fill=Paired-8-2},mark=square*\\%
 Paired-8-3!70, every mark/.append style={solid,fill=Paired-8-3},mark=triangle*\\%
 Paired-8-4!70, every mark/.append style={solid,fill=Paired-8-4},mark=diamond*\\%
 Paired-8-5!70, every mark/.append style={solid,fill=Paired-8-5},mark=pentagon*\\%
 Paired-8-6!70, every mark/.append style={solid,fill=Paired-8-6},mark=x\\%
 Paired-8-7!70, every mark/.append style={solid,fill=Paired-8-7},mark=+\\%
 Paired-8-8!70, every mark/.append style={solid,fill=Paired-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-9}{%
 Paired-9-1!70, every mark/.append style={solid,fill=Paired-9-1},mark=*\\%
 Paired-9-2!70, every mark/.append style={solid,fill=Paired-9-2},mark=square*\\%
 Paired-9-3!70, every mark/.append style={solid,fill=Paired-9-3},mark=triangle*\\%
 Paired-9-4!70, every mark/.append style={solid,fill=Paired-9-4},mark=diamond*\\%
 Paired-9-5!70, every mark/.append style={solid,fill=Paired-9-5},mark=pentagon*\\%
 Paired-9-6!70, every mark/.append style={solid,fill=Paired-9-6},mark=x\\%
 Paired-9-7!70, every mark/.append style={solid,fill=Paired-9-7},mark=+\\%
 Paired-9-8!70, every mark/.append style={solid,fill=Paired-9-8},mark=star\\%
 Paired-9-9!70, every mark/.append style={solid,fill=Paired-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-10}{%
 Paired-10-1!70, every mark/.append style={solid,fill=Paired-10-1},mark=*\\%
 Paired-10-2!70, every mark/.append style={solid,fill=Paired-10-2},mark=square*\\%
 Paired-10-3!70, every mark/.append style={solid,fill=Paired-10-3},mark=triangle*\\%
 Paired-10-4!70, every mark/.append style={solid,fill=Paired-10-4},mark=diamond*\\%
 Paired-10-5!70, every mark/.append style={solid,fill=Paired-10-5},mark=pentagon*\\%
 Paired-10-6!70, every mark/.append style={solid,fill=Paired-10-6},mark=x\\%
 Paired-10-7!70, every mark/.append style={solid,fill=Paired-10-7},mark=+\\%
 Paired-10-8!70, every mark/.append style={solid,fill=Paired-10-8},mark=star\\%
 Paired-10-9!70, every mark/.append style={solid,fill=Paired-10-9},mark=oplus*\\%
 Paired-10-10!70, every mark/.append style={solid,fill=Paired-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-11}{%
 Paired-11-1!70, every mark/.append style={solid,fill=Paired-11-1},mark=*\\%
 Paired-11-2!70, every mark/.append style={solid,fill=Paired-11-2},mark=square*\\%
 Paired-11-3!70, every mark/.append style={solid,fill=Paired-11-3},mark=triangle*\\%
 Paired-11-4!70, every mark/.append style={solid,fill=Paired-11-4},mark=diamond*\\%
 Paired-11-5!70, every mark/.append style={solid,fill=Paired-11-5},mark=pentagon*\\%
 Paired-11-6!70, every mark/.append style={solid,fill=Paired-11-6},mark=x\\%
 Paired-11-7!70, every mark/.append style={solid,fill=Paired-11-7},mark=+\\%
 Paired-11-8!70, every mark/.append style={solid,fill=Paired-11-8},mark=star\\%
 Paired-11-9!70, every mark/.append style={solid,fill=Paired-11-9},mark=oplus*\\%
 Paired-11-10!70, every mark/.append style={solid,fill=Paired-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-12}{%
 Paired-12-1!70, every mark/.append style={solid,fill=Paired-12-1},mark=*\\%
 Paired-12-2!70, every mark/.append style={solid,fill=Paired-12-2},mark=square*\\%
 Paired-12-3!70, every mark/.append style={solid,fill=Paired-12-3},mark=triangle*\\%
 Paired-12-4!70, every mark/.append style={solid,fill=Paired-12-4},mark=diamond*\\%
 Paired-12-5!70, every mark/.append style={solid,fill=Paired-12-5},mark=pentagon*\\%
 Paired-12-6!70, every mark/.append style={solid,fill=Paired-12-6},mark=x\\%
 Paired-12-7!70, every mark/.append style={solid,fill=Paired-12-7},mark=+\\%
 Paired-12-8!70, every mark/.append style={solid,fill=Paired-12-8},mark=star\\%
 Paired-12-9!70, every mark/.append style={solid,fill=Paired-12-9},mark=oplus*\\%
 Paired-12-10!70, every mark/.append style={solid,fill=Paired-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-3}{%
 Accent-3-1!70, every mark/.append style={solid,fill=Accent-3-1},mark=*\\%
 Accent-3-2!70, every mark/.append style={solid,fill=Accent-3-2},mark=square*\\%
 Accent-3-3!70, every mark/.append style={solid,fill=Accent-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-4}{%
 Accent-4-1!70, every mark/.append style={solid,fill=Accent-4-1},mark=*\\%
 Accent-4-2!70, every mark/.append style={solid,fill=Accent-4-2},mark=square*\\%
 Accent-4-3!70, every mark/.append style={solid,fill=Accent-4-3},mark=triangle*\\%
 Accent-4-4!70, every mark/.append style={solid,fill=Accent-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-5}{%
 Accent-5-1!70, every mark/.append style={solid,fill=Accent-5-1},mark=*\\%
 Accent-5-2!70, every mark/.append style={solid,fill=Accent-5-2},mark=square*\\%
 Accent-5-3!70, every mark/.append style={solid,fill=Accent-5-3},mark=triangle*\\%
 Accent-5-4!70, every mark/.append style={solid,fill=Accent-5-4},mark=diamond*\\%
 Accent-5-5!70, every mark/.append style={solid,fill=Accent-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-6}{%
 Accent-6-1!70, every mark/.append style={solid,fill=Accent-6-1},mark=*\\%
 Accent-6-2!70, every mark/.append style={solid,fill=Accent-6-2},mark=square*\\%
 Accent-6-3!70, every mark/.append style={solid,fill=Accent-6-3},mark=triangle*\\%
 Accent-6-4!70, every mark/.append style={solid,fill=Accent-6-4},mark=diamond*\\%
 Accent-6-5!70, every mark/.append style={solid,fill=Accent-6-5},mark=pentagon*\\%
 Accent-6-6!70, every mark/.append style={solid,fill=Accent-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-7}{%
 Accent-7-1!70, every mark/.append style={solid,fill=Accent-7-1},mark=*\\%
 Accent-7-2!70, every mark/.append style={solid,fill=Accent-7-2},mark=square*\\%
 Accent-7-3!70, every mark/.append style={solid,fill=Accent-7-3},mark=triangle*\\%
 Accent-7-4!70, every mark/.append style={solid,fill=Accent-7-4},mark=diamond*\\%
 Accent-7-5!70, every mark/.append style={solid,fill=Accent-7-5},mark=pentagon*\\%
 Accent-7-6!70, every mark/.append style={solid,fill=Accent-7-6},mark=x\\%
 Accent-7-7!70, every mark/.append style={solid,fill=Accent-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-8}{%
 Accent-8-1!70, every mark/.append style={solid,fill=Accent-8-1},mark=*\\%
 Accent-8-2!70, every mark/.append style={solid,fill=Accent-8-2},mark=square*\\%
 Accent-8-3!70, every mark/.append style={solid,fill=Accent-8-3},mark=triangle*\\%
 Accent-8-4!70, every mark/.append style={solid,fill=Accent-8-4},mark=diamond*\\%
 Accent-8-5!70, every mark/.append style={solid,fill=Accent-8-5},mark=pentagon*\\%
 Accent-8-6!70, every mark/.append style={solid,fill=Accent-8-6},mark=x\\%
 Accent-8-7!70, every mark/.append style={solid,fill=Accent-8-7},mark=+\\%
 Accent-8-8!70, every mark/.append style={solid,fill=Accent-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-3}{%
 YlGn-3-1,mark=x\\%
 YlGn-3-2,mark=+\\%
 YlGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-4}{%
 YlGn-4-1,mark=x\\%
 YlGn-4-2,mark=+\\%
 YlGn-4-3,mark=-\\%
 YlGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-5}{%
 YlGn-5-1,mark=x\\%
 YlGn-5-2,mark=+\\%
 YlGn-5-3,mark=-\\%
 YlGn-5-4,mark=|\\%
 YlGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-6}{%
 YlGn-6-1,mark=x\\%
 YlGn-6-2,mark=+\\%
 YlGn-6-3,mark=-\\%
 YlGn-6-4,mark=|\\%
 YlGn-6-5,mark=asterisk\\%
 YlGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-7}{%
 YlGn-7-1,mark=x\\%
 YlGn-7-2,mark=+\\%
 YlGn-7-3,mark=-\\%
 YlGn-7-4,mark=|\\%
 YlGn-7-5,mark=asterisk\\%
 YlGn-7-6,mark=star\\%
 YlGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-8}{%
 YlGn-8-1,mark=x\\%
 YlGn-8-2,mark=+\\%
 YlGn-8-3,mark=-\\%
 YlGn-8-4,mark=|\\%
 YlGn-8-5,mark=asterisk\\%
 YlGn-8-6,mark=star\\%
 YlGn-8-7,mark=10-pointed star\\%
 YlGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-9}{%
 YlGn-9-1,mark=x\\%
 YlGn-9-2,mark=+\\%
 YlGn-9-3,mark=-\\%
 YlGn-9-4,mark=|\\%
 YlGn-9-5,mark=asterisk\\%
 YlGn-9-6,mark=star\\%
 YlGn-9-7,mark=10-pointed star\\%
 YlGn-9-8,mark=Mercedes star\\%
 YlGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-3}{%
 YlGnBu-3-1,mark=x\\%
 YlGnBu-3-2,mark=+\\%
 YlGnBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-4}{%
 YlGnBu-4-1,mark=x\\%
 YlGnBu-4-2,mark=+\\%
 YlGnBu-4-3,mark=-\\%
 YlGnBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-5}{%
 YlGnBu-5-1,mark=x\\%
 YlGnBu-5-2,mark=+\\%
 YlGnBu-5-3,mark=-\\%
 YlGnBu-5-4,mark=|\\%
 YlGnBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-6}{%
 YlGnBu-6-1,mark=x\\%
 YlGnBu-6-2,mark=+\\%
 YlGnBu-6-3,mark=-\\%
 YlGnBu-6-4,mark=|\\%
 YlGnBu-6-5,mark=asterisk\\%
 YlGnBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-7}{%
 YlGnBu-7-1,mark=x\\%
 YlGnBu-7-2,mark=+\\%
 YlGnBu-7-3,mark=-\\%
 YlGnBu-7-4,mark=|\\%
 YlGnBu-7-5,mark=asterisk\\%
 YlGnBu-7-6,mark=star\\%
 YlGnBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-8}{%
 YlGnBu-8-1,mark=x\\%
 YlGnBu-8-2,mark=+\\%
 YlGnBu-8-3,mark=-\\%
 YlGnBu-8-4,mark=|\\%
 YlGnBu-8-5,mark=asterisk\\%
 YlGnBu-8-6,mark=star\\%
 YlGnBu-8-7,mark=10-pointed star\\%
 YlGnBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-9}{%
 YlGnBu-9-1,mark=x\\%
 YlGnBu-9-2,mark=+\\%
 YlGnBu-9-3,mark=-\\%
 YlGnBu-9-4,mark=|\\%
 YlGnBu-9-5,mark=asterisk\\%
 YlGnBu-9-6,mark=star\\%
 YlGnBu-9-7,mark=10-pointed star\\%
 YlGnBu-9-8,mark=Mercedes star\\%
 YlGnBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-3}{%
 GnBu-3-1,mark=x\\%
 GnBu-3-2,mark=+\\%
 GnBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-4}{%
 GnBu-4-1,mark=x\\%
 GnBu-4-2,mark=+\\%
 GnBu-4-3,mark=-\\%
 GnBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-5}{%
 GnBu-5-1,mark=x\\%
 GnBu-5-2,mark=+\\%
 GnBu-5-3,mark=-\\%
 GnBu-5-4,mark=|\\%
 GnBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-6}{%
 GnBu-6-1,mark=x\\%
 GnBu-6-2,mark=+\\%
 GnBu-6-3,mark=-\\%
 GnBu-6-4,mark=|\\%
 GnBu-6-5,mark=asterisk\\%
 GnBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-7}{%
 GnBu-7-1,mark=x\\%
 GnBu-7-2,mark=+\\%
 GnBu-7-3,mark=-\\%
 GnBu-7-4,mark=|\\%
 GnBu-7-5,mark=asterisk\\%
 GnBu-7-6,mark=star\\%
 GnBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-8}{%
 GnBu-8-1,mark=x\\%
 GnBu-8-2,mark=+\\%
 GnBu-8-3,mark=-\\%
 GnBu-8-4,mark=|\\%
 GnBu-8-5,mark=asterisk\\%
 GnBu-8-6,mark=star\\%
 GnBu-8-7,mark=10-pointed star\\%
 GnBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-9}{%
 GnBu-9-1,mark=x\\%
 GnBu-9-2,mark=+\\%
 GnBu-9-3,mark=-\\%
 GnBu-9-4,mark=|\\%
 GnBu-9-5,mark=asterisk\\%
 GnBu-9-6,mark=star\\%
 GnBu-9-7,mark=10-pointed star\\%
 GnBu-9-8,mark=Mercedes star\\%
 GnBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-3}{%
 BuGn-3-1,mark=x\\%
 BuGn-3-2,mark=+\\%
 BuGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-4}{%
 BuGn-4-1,mark=x\\%
 BuGn-4-2,mark=+\\%
 BuGn-4-3,mark=-\\%
 BuGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-5}{%
 BuGn-5-1,mark=x\\%
 BuGn-5-2,mark=+\\%
 BuGn-5-3,mark=-\\%
 BuGn-5-4,mark=|\\%
 BuGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-6}{%
 BuGn-6-1,mark=x\\%
 BuGn-6-2,mark=+\\%
 BuGn-6-3,mark=-\\%
 BuGn-6-4,mark=|\\%
 BuGn-6-5,mark=asterisk\\%
 BuGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-7}{%
 BuGn-7-1,mark=x\\%
 BuGn-7-2,mark=+\\%
 BuGn-7-3,mark=-\\%
 BuGn-7-4,mark=|\\%
 BuGn-7-5,mark=asterisk\\%
 BuGn-7-6,mark=star\\%
 BuGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-8}{%
 BuGn-8-1,mark=x\\%
 BuGn-8-2,mark=+\\%
 BuGn-8-3,mark=-\\%
 BuGn-8-4,mark=|\\%
 BuGn-8-5,mark=asterisk\\%
 BuGn-8-6,mark=star\\%
 BuGn-8-7,mark=10-pointed star\\%
 BuGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-9}{%
 BuGn-9-1,mark=x\\%
 BuGn-9-2,mark=+\\%
 BuGn-9-3,mark=-\\%
 BuGn-9-4,mark=|\\%
 BuGn-9-5,mark=asterisk\\%
 BuGn-9-6,mark=star\\%
 BuGn-9-7,mark=10-pointed star\\%
 BuGn-9-8,mark=Mercedes star\\%
 BuGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-3}{%
 PuBuGn-3-1,mark=x\\%
 PuBuGn-3-2,mark=+\\%
 PuBuGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-4}{%
 PuBuGn-4-1,mark=x\\%
 PuBuGn-4-2,mark=+\\%
 PuBuGn-4-3,mark=-\\%
 PuBuGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-5}{%
 PuBuGn-5-1,mark=x\\%
 PuBuGn-5-2,mark=+\\%
 PuBuGn-5-3,mark=-\\%
 PuBuGn-5-4,mark=|\\%
 PuBuGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-6}{%
 PuBuGn-6-1,mark=x\\%
 PuBuGn-6-2,mark=+\\%
 PuBuGn-6-3,mark=-\\%
 PuBuGn-6-4,mark=|\\%
 PuBuGn-6-5,mark=asterisk\\%
 PuBuGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-7}{%
 PuBuGn-7-1,mark=x\\%
 PuBuGn-7-2,mark=+\\%
 PuBuGn-7-3,mark=-\\%
 PuBuGn-7-4,mark=|\\%
 PuBuGn-7-5,mark=asterisk\\%
 PuBuGn-7-6,mark=star\\%
 PuBuGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-8}{%
 PuBuGn-8-1,mark=x\\%
 PuBuGn-8-2,mark=+\\%
 PuBuGn-8-3,mark=-\\%
 PuBuGn-8-4,mark=|\\%
 PuBuGn-8-5,mark=asterisk\\%
 PuBuGn-8-6,mark=star\\%
 PuBuGn-8-7,mark=10-pointed star\\%
 PuBuGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-9}{%
 PuBuGn-9-1,mark=x\\%
 PuBuGn-9-2,mark=+\\%
 PuBuGn-9-3,mark=-\\%
 PuBuGn-9-4,mark=|\\%
 PuBuGn-9-5,mark=asterisk\\%
 PuBuGn-9-6,mark=star\\%
 PuBuGn-9-7,mark=10-pointed star\\%
 PuBuGn-9-8,mark=Mercedes star\\%
 PuBuGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-3}{%
 PuBu-3-1,mark=x\\%
 PuBu-3-2,mark=+\\%
 PuBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-4}{%
 PuBu-4-1,mark=x\\%
 PuBu-4-2,mark=+\\%
 PuBu-4-3,mark=-\\%
 PuBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-5}{%
 PuBu-5-1,mark=x\\%
 PuBu-5-2,mark=+\\%
 PuBu-5-3,mark=-\\%
 PuBu-5-4,mark=|\\%
 PuBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-6}{%
 PuBu-6-1,mark=x\\%
 PuBu-6-2,mark=+\\%
 PuBu-6-3,mark=-\\%
 PuBu-6-4,mark=|\\%
 PuBu-6-5,mark=asterisk\\%
 PuBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-7}{%
 PuBu-7-1,mark=x\\%
 PuBu-7-2,mark=+\\%
 PuBu-7-3,mark=-\\%
 PuBu-7-4,mark=|\\%
 PuBu-7-5,mark=asterisk\\%
 PuBu-7-6,mark=star\\%
 PuBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-8}{%
 PuBu-8-1,mark=x\\%
 PuBu-8-2,mark=+\\%
 PuBu-8-3,mark=-\\%
 PuBu-8-4,mark=|\\%
 PuBu-8-5,mark=asterisk\\%
 PuBu-8-6,mark=star\\%
 PuBu-8-7,mark=10-pointed star\\%
 PuBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-9}{%
 PuBu-9-1,mark=x\\%
 PuBu-9-2,mark=+\\%
 PuBu-9-3,mark=-\\%
 PuBu-9-4,mark=|\\%
 PuBu-9-5,mark=asterisk\\%
 PuBu-9-6,mark=star\\%
 PuBu-9-7,mark=10-pointed star\\%
 PuBu-9-8,mark=Mercedes star\\%
 PuBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-3}{%
 BuPu-3-1,mark=x\\%
 BuPu-3-2,mark=+\\%
 BuPu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-4}{%
 BuPu-4-1,mark=x\\%
 BuPu-4-2,mark=+\\%
 BuPu-4-3,mark=-\\%
 BuPu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-5}{%
 BuPu-5-1,mark=x\\%
 BuPu-5-2,mark=+\\%
 BuPu-5-3,mark=-\\%
 BuPu-5-4,mark=|\\%
 BuPu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-6}{%
 BuPu-6-1,mark=x\\%
 BuPu-6-2,mark=+\\%
 BuPu-6-3,mark=-\\%
 BuPu-6-4,mark=|\\%
 BuPu-6-5,mark=asterisk\\%
 BuPu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-7}{%
 BuPu-7-1,mark=x\\%
 BuPu-7-2,mark=+\\%
 BuPu-7-3,mark=-\\%
 BuPu-7-4,mark=|\\%
 BuPu-7-5,mark=asterisk\\%
 BuPu-7-6,mark=star\\%
 BuPu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-8}{%
 BuPu-8-1,mark=x\\%
 BuPu-8-2,mark=+\\%
 BuPu-8-3,mark=-\\%
 BuPu-8-4,mark=|\\%
 BuPu-8-5,mark=asterisk\\%
 BuPu-8-6,mark=star\\%
 BuPu-8-7,mark=10-pointed star\\%
 BuPu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-9}{%
 BuPu-9-1,mark=x\\%
 BuPu-9-2,mark=+\\%
 BuPu-9-3,mark=-\\%
 BuPu-9-4,mark=|\\%
 BuPu-9-5,mark=asterisk\\%
 BuPu-9-6,mark=star\\%
 BuPu-9-7,mark=10-pointed star\\%
 BuPu-9-8,mark=Mercedes star\\%
 BuPu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-3}{%
 RdPu-3-1,mark=x\\%
 RdPu-3-2,mark=+\\%
 RdPu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-4}{%
 RdPu-4-1,mark=x\\%
 RdPu-4-2,mark=+\\%
 RdPu-4-3,mark=-\\%
 RdPu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-5}{%
 RdPu-5-1,mark=x\\%
 RdPu-5-2,mark=+\\%
 RdPu-5-3,mark=-\\%
 RdPu-5-4,mark=|\\%
 RdPu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-6}{%
 RdPu-6-1,mark=x\\%
 RdPu-6-2,mark=+\\%
 RdPu-6-3,mark=-\\%
 RdPu-6-4,mark=|\\%
 RdPu-6-5,mark=asterisk\\%
 RdPu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-7}{%
 RdPu-7-1,mark=x\\%
 RdPu-7-2,mark=+\\%
 RdPu-7-3,mark=-\\%
 RdPu-7-4,mark=|\\%
 RdPu-7-5,mark=asterisk\\%
 RdPu-7-6,mark=star\\%
 RdPu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-8}{%
 RdPu-8-1,mark=x\\%
 RdPu-8-2,mark=+\\%
 RdPu-8-3,mark=-\\%
 RdPu-8-4,mark=|\\%
 RdPu-8-5,mark=asterisk\\%
 RdPu-8-6,mark=star\\%
 RdPu-8-7,mark=10-pointed star\\%
 RdPu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-9}{%
 RdPu-9-1,mark=x\\%
 RdPu-9-2,mark=+\\%
 RdPu-9-3,mark=-\\%
 RdPu-9-4,mark=|\\%
 RdPu-9-5,mark=asterisk\\%
 RdPu-9-6,mark=star\\%
 RdPu-9-7,mark=10-pointed star\\%
 RdPu-9-8,mark=Mercedes star\\%
 RdPu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-3}{%
 PuRd-3-1,mark=x\\%
 PuRd-3-2,mark=+\\%
 PuRd-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-4}{%
 PuRd-4-1,mark=x\\%
 PuRd-4-2,mark=+\\%
 PuRd-4-3,mark=-\\%
 PuRd-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-5}{%
 PuRd-5-1,mark=x\\%
 PuRd-5-2,mark=+\\%
 PuRd-5-3,mark=-\\%
 PuRd-5-4,mark=|\\%
 PuRd-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-6}{%
 PuRd-6-1,mark=x\\%
 PuRd-6-2,mark=+\\%
 PuRd-6-3,mark=-\\%
 PuRd-6-4,mark=|\\%
 PuRd-6-5,mark=asterisk\\%
 PuRd-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-7}{%
 PuRd-7-1,mark=x\\%
 PuRd-7-2,mark=+\\%
 PuRd-7-3,mark=-\\%
 PuRd-7-4,mark=|\\%
 PuRd-7-5,mark=asterisk\\%
 PuRd-7-6,mark=star\\%
 PuRd-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-8}{%
 PuRd-8-1,mark=x\\%
 PuRd-8-2,mark=+\\%
 PuRd-8-3,mark=-\\%
 PuRd-8-4,mark=|\\%
 PuRd-8-5,mark=asterisk\\%
 PuRd-8-6,mark=star\\%
 PuRd-8-7,mark=10-pointed star\\%
 PuRd-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-9}{%
 PuRd-9-1,mark=x\\%
 PuRd-9-2,mark=+\\%
 PuRd-9-3,mark=-\\%
 PuRd-9-4,mark=|\\%
 PuRd-9-5,mark=asterisk\\%
 PuRd-9-6,mark=star\\%
 PuRd-9-7,mark=10-pointed star\\%
 PuRd-9-8,mark=Mercedes star\\%
 PuRd-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-3}{%
 OrRd-3-1,mark=x\\%
 OrRd-3-2,mark=+\\%
 OrRd-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-4}{%
 OrRd-4-1,mark=x\\%
 OrRd-4-2,mark=+\\%
 OrRd-4-3,mark=-\\%
 OrRd-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-5}{%
 OrRd-5-1,mark=x\\%
 OrRd-5-2,mark=+\\%
 OrRd-5-3,mark=-\\%
 OrRd-5-4,mark=|\\%
 OrRd-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-6}{%
 OrRd-6-1,mark=x\\%
 OrRd-6-2,mark=+\\%
 OrRd-6-3,mark=-\\%
 OrRd-6-4,mark=|\\%
 OrRd-6-5,mark=asterisk\\%
 OrRd-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-7}{%
 OrRd-7-1,mark=x\\%
 OrRd-7-2,mark=+\\%
 OrRd-7-3,mark=-\\%
 OrRd-7-4,mark=|\\%
 OrRd-7-5,mark=asterisk\\%
 OrRd-7-6,mark=star\\%
 OrRd-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-8}{%
 OrRd-8-1,mark=x\\%
 OrRd-8-2,mark=+\\%
 OrRd-8-3,mark=-\\%
 OrRd-8-4,mark=|\\%
 OrRd-8-5,mark=asterisk\\%
 OrRd-8-6,mark=star\\%
 OrRd-8-7,mark=10-pointed star\\%
 OrRd-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-9}{%
 OrRd-9-1,mark=x\\%
 OrRd-9-2,mark=+\\%
 OrRd-9-3,mark=-\\%
 OrRd-9-4,mark=|\\%
 OrRd-9-5,mark=asterisk\\%
 OrRd-9-6,mark=star\\%
 OrRd-9-7,mark=10-pointed star\\%
 OrRd-9-8,mark=Mercedes star\\%
 OrRd-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-3}{%
 YlOrRd-3-1,mark=x\\%
 YlOrRd-3-2,mark=+\\%
 YlOrRd-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-4}{%
 YlOrRd-4-1,mark=x\\%
 YlOrRd-4-2,mark=+\\%
 YlOrRd-4-3,mark=-\\%
 YlOrRd-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-5}{%
 YlOrRd-5-1,mark=x\\%
 YlOrRd-5-2,mark=+\\%
 YlOrRd-5-3,mark=-\\%
 YlOrRd-5-4,mark=|\\%
 YlOrRd-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-6}{%
 YlOrRd-6-1,mark=x\\%
 YlOrRd-6-2,mark=+\\%
 YlOrRd-6-3,mark=-\\%
 YlOrRd-6-4,mark=|\\%
 YlOrRd-6-5,mark=asterisk\\%
 YlOrRd-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-7}{%
 YlOrRd-7-1,mark=x\\%
 YlOrRd-7-2,mark=+\\%
 YlOrRd-7-3,mark=-\\%
 YlOrRd-7-4,mark=|\\%
 YlOrRd-7-5,mark=asterisk\\%
 YlOrRd-7-6,mark=star\\%
 YlOrRd-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-8}{%
 YlOrRd-8-1,mark=x\\%
 YlOrRd-8-2,mark=+\\%
 YlOrRd-8-3,mark=-\\%
 YlOrRd-8-4,mark=|\\%
 YlOrRd-8-5,mark=asterisk\\%
 YlOrRd-8-6,mark=star\\%
 YlOrRd-8-7,mark=10-pointed star\\%
 YlOrRd-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-9}{%
 YlOrRd-9-1,mark=x\\%
 YlOrRd-9-2,mark=+\\%
 YlOrRd-9-3,mark=-\\%
 YlOrRd-9-4,mark=|\\%
 YlOrRd-9-5,mark=asterisk\\%
 YlOrRd-9-6,mark=star\\%
 YlOrRd-9-7,mark=10-pointed star\\%
 YlOrRd-9-8,mark=Mercedes star\\%
 YlOrRd-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-3}{%
 YlOrBr-3-1,mark=x\\%
 YlOrBr-3-2,mark=+\\%
 YlOrBr-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-4}{%
 YlOrBr-4-1,mark=x\\%
 YlOrBr-4-2,mark=+\\%
 YlOrBr-4-3,mark=-\\%
 YlOrBr-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-5}{%
 YlOrBr-5-1,mark=x\\%
 YlOrBr-5-2,mark=+\\%
 YlOrBr-5-3,mark=-\\%
 YlOrBr-5-4,mark=|\\%
 YlOrBr-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-6}{%
 YlOrBr-6-1,mark=x\\%
 YlOrBr-6-2,mark=+\\%
 YlOrBr-6-3,mark=-\\%
 YlOrBr-6-4,mark=|\\%
 YlOrBr-6-5,mark=asterisk\\%
 YlOrBr-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-7}{%
 YlOrBr-7-1,mark=x\\%
 YlOrBr-7-2,mark=+\\%
 YlOrBr-7-3,mark=-\\%
 YlOrBr-7-4,mark=|\\%
 YlOrBr-7-5,mark=asterisk\\%
 YlOrBr-7-6,mark=star\\%
 YlOrBr-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-8}{%
 YlOrBr-8-1,mark=x\\%
 YlOrBr-8-2,mark=+\\%
 YlOrBr-8-3,mark=-\\%
 YlOrBr-8-4,mark=|\\%
 YlOrBr-8-5,mark=asterisk\\%
 YlOrBr-8-6,mark=star\\%
 YlOrBr-8-7,mark=10-pointed star\\%
 YlOrBr-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-9}{%
 YlOrBr-9-1,mark=x\\%
 YlOrBr-9-2,mark=+\\%
 YlOrBr-9-3,mark=-\\%
 YlOrBr-9-4,mark=|\\%
 YlOrBr-9-5,mark=asterisk\\%
 YlOrBr-9-6,mark=star\\%
 YlOrBr-9-7,mark=10-pointed star\\%
 YlOrBr-9-8,mark=Mercedes star\\%
 YlOrBr-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-3}{%
 Purples-3-1,mark=x\\%
 Purples-3-2,mark=+\\%
 Purples-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-4}{%
 Purples-4-1,mark=x\\%
 Purples-4-2,mark=+\\%
 Purples-4-3,mark=-\\%
 Purples-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-5}{%
 Purples-5-1,mark=x\\%
 Purples-5-2,mark=+\\%
 Purples-5-3,mark=-\\%
 Purples-5-4,mark=|\\%
 Purples-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-6}{%
 Purples-6-1,mark=x\\%
 Purples-6-2,mark=+\\%
 Purples-6-3,mark=-\\%
 Purples-6-4,mark=|\\%
 Purples-6-5,mark=asterisk\\%
 Purples-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-7}{%
 Purples-7-1,mark=x\\%
 Purples-7-2,mark=+\\%
 Purples-7-3,mark=-\\%
 Purples-7-4,mark=|\\%
 Purples-7-5,mark=asterisk\\%
 Purples-7-6,mark=star\\%
 Purples-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-8}{%
 Purples-8-1,mark=x\\%
 Purples-8-2,mark=+\\%
 Purples-8-3,mark=-\\%
 Purples-8-4,mark=|\\%
 Purples-8-5,mark=asterisk\\%
 Purples-8-6,mark=star\\%
 Purples-8-7,mark=10-pointed star\\%
 Purples-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-9}{%
 Purples-9-1,mark=x\\%
 Purples-9-2,mark=+\\%
 Purples-9-3,mark=-\\%
 Purples-9-4,mark=|\\%
 Purples-9-5,mark=asterisk\\%
 Purples-9-6,mark=star\\%
 Purples-9-7,mark=10-pointed star\\%
 Purples-9-8,mark=Mercedes star\\%
 Purples-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-3}{%
 Blues-3-1,mark=x\\%
 Blues-3-2,mark=+\\%
 Blues-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-4}{%
 Blues-4-1,mark=x\\%
 Blues-4-2,mark=+\\%
 Blues-4-3,mark=-\\%
 Blues-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-5}{%
 Blues-5-1,mark=x\\%
 Blues-5-2,mark=+\\%
 Blues-5-3,mark=-\\%
 Blues-5-4,mark=|\\%
 Blues-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-6}{%
 Blues-6-1,mark=x\\%
 Blues-6-2,mark=+\\%
 Blues-6-3,mark=-\\%
 Blues-6-4,mark=|\\%
 Blues-6-5,mark=asterisk\\%
 Blues-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-7}{%
 Blues-7-1,mark=x\\%
 Blues-7-2,mark=+\\%
 Blues-7-3,mark=-\\%
 Blues-7-4,mark=|\\%
 Blues-7-5,mark=asterisk\\%
 Blues-7-6,mark=star\\%
 Blues-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-8}{%
 Blues-8-1,mark=x\\%
 Blues-8-2,mark=+\\%
 Blues-8-3,mark=-\\%
 Blues-8-4,mark=|\\%
 Blues-8-5,mark=asterisk\\%
 Blues-8-6,mark=star\\%
 Blues-8-7,mark=10-pointed star\\%
 Blues-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-9}{%
 Blues-9-1,mark=x\\%
 Blues-9-2,mark=+\\%
 Blues-9-3,mark=-\\%
 Blues-9-4,mark=|\\%
 Blues-9-5,mark=asterisk\\%
 Blues-9-6,mark=star\\%
 Blues-9-7,mark=10-pointed star\\%
 Blues-9-8,mark=Mercedes star\\%
 Blues-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-3}{%
 Greens-3-1,mark=x\\%
 Greens-3-2,mark=+\\%
 Greens-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-4}{%
 Greens-4-1,mark=x\\%
 Greens-4-2,mark=+\\%
 Greens-4-3,mark=-\\%
 Greens-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-5}{%
 Greens-5-1,mark=x\\%
 Greens-5-2,mark=+\\%
 Greens-5-3,mark=-\\%
 Greens-5-4,mark=|\\%
 Greens-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-6}{%
 Greens-6-1,mark=x\\%
 Greens-6-2,mark=+\\%
 Greens-6-3,mark=-\\%
 Greens-6-4,mark=|\\%
 Greens-6-5,mark=asterisk\\%
 Greens-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-7}{%
 Greens-7-1,mark=x\\%
 Greens-7-2,mark=+\\%
 Greens-7-3,mark=-\\%
 Greens-7-4,mark=|\\%
 Greens-7-5,mark=asterisk\\%
 Greens-7-6,mark=star\\%
 Greens-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-8}{%
 Greens-8-1,mark=x\\%
 Greens-8-2,mark=+\\%
 Greens-8-3,mark=-\\%
 Greens-8-4,mark=|\\%
 Greens-8-5,mark=asterisk\\%
 Greens-8-6,mark=star\\%
 Greens-8-7,mark=10-pointed star\\%
 Greens-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-9}{%
 Greens-9-1,mark=x\\%
 Greens-9-2,mark=+\\%
 Greens-9-3,mark=-\\%
 Greens-9-4,mark=|\\%
 Greens-9-5,mark=asterisk\\%
 Greens-9-6,mark=star\\%
 Greens-9-7,mark=10-pointed star\\%
 Greens-9-8,mark=Mercedes star\\%
 Greens-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-3}{%
 Oranges-3-1,mark=x\\%
 Oranges-3-2,mark=+\\%
 Oranges-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-4}{%
 Oranges-4-1,mark=x\\%
 Oranges-4-2,mark=+\\%
 Oranges-4-3,mark=-\\%
 Oranges-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-5}{%
 Oranges-5-1,mark=x\\%
 Oranges-5-2,mark=+\\%
 Oranges-5-3,mark=-\\%
 Oranges-5-4,mark=|\\%
 Oranges-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-6}{%
 Oranges-6-1,mark=x\\%
 Oranges-6-2,mark=+\\%
 Oranges-6-3,mark=-\\%
 Oranges-6-4,mark=|\\%
 Oranges-6-5,mark=asterisk\\%
 Oranges-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-7}{%
 Oranges-7-1,mark=x\\%
 Oranges-7-2,mark=+\\%
 Oranges-7-3,mark=-\\%
 Oranges-7-4,mark=|\\%
 Oranges-7-5,mark=asterisk\\%
 Oranges-7-6,mark=star\\%
 Oranges-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-8}{%
 Oranges-8-1,mark=x\\%
 Oranges-8-2,mark=+\\%
 Oranges-8-3,mark=-\\%
 Oranges-8-4,mark=|\\%
 Oranges-8-5,mark=asterisk\\%
 Oranges-8-6,mark=star\\%
 Oranges-8-7,mark=10-pointed star\\%
 Oranges-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-9}{%
 Oranges-9-1,mark=x\\%
 Oranges-9-2,mark=+\\%
 Oranges-9-3,mark=-\\%
 Oranges-9-4,mark=|\\%
 Oranges-9-5,mark=asterisk\\%
 Oranges-9-6,mark=star\\%
 Oranges-9-7,mark=10-pointed star\\%
 Oranges-9-8,mark=Mercedes star\\%
 Oranges-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-3}{%
 Reds-3-1,mark=x\\%
 Reds-3-2,mark=+\\%
 Reds-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-4}{%
 Reds-4-1,mark=x\\%
 Reds-4-2,mark=+\\%
 Reds-4-3,mark=-\\%
 Reds-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-5}{%
 Reds-5-1,mark=x\\%
 Reds-5-2,mark=+\\%
 Reds-5-3,mark=-\\%
 Reds-5-4,mark=|\\%
 Reds-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-6}{%
 Reds-6-1,mark=x\\%
 Reds-6-2,mark=+\\%
 Reds-6-3,mark=-\\%
 Reds-6-4,mark=|\\%
 Reds-6-5,mark=asterisk\\%
 Reds-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-7}{%
 Reds-7-1,mark=x\\%
 Reds-7-2,mark=+\\%
 Reds-7-3,mark=-\\%
 Reds-7-4,mark=|\\%
 Reds-7-5,mark=asterisk\\%
 Reds-7-6,mark=star\\%
 Reds-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-8}{%
 Reds-8-1,mark=x\\%
 Reds-8-2,mark=+\\%
 Reds-8-3,mark=-\\%
 Reds-8-4,mark=|\\%
 Reds-8-5,mark=asterisk\\%
 Reds-8-6,mark=star\\%
 Reds-8-7,mark=10-pointed star\\%
 Reds-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-9}{%
 Reds-9-1,mark=x\\%
 Reds-9-2,mark=+\\%
 Reds-9-3,mark=-\\%
 Reds-9-4,mark=|\\%
 Reds-9-5,mark=asterisk\\%
 Reds-9-6,mark=star\\%
 Reds-9-7,mark=10-pointed star\\%
 Reds-9-8,mark=Mercedes star\\%
 Reds-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-3}{%
 Greys-3-1,mark=x\\%
 Greys-3-2,mark=+\\%
 Greys-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-4}{%
 Greys-4-1,mark=x\\%
 Greys-4-2,mark=+\\%
 Greys-4-3,mark=-\\%
 Greys-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-5}{%
 Greys-5-1,mark=x\\%
 Greys-5-2,mark=+\\%
 Greys-5-3,mark=-\\%
 Greys-5-4,mark=|\\%
 Greys-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-6}{%
 Greys-6-1,mark=x\\%
 Greys-6-2,mark=+\\%
 Greys-6-3,mark=-\\%
 Greys-6-4,mark=|\\%
 Greys-6-5,mark=asterisk\\%
 Greys-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-7}{%
 Greys-7-1,mark=x\\%
 Greys-7-2,mark=+\\%
 Greys-7-3,mark=-\\%
 Greys-7-4,mark=|\\%
 Greys-7-5,mark=asterisk\\%
 Greys-7-6,mark=star\\%
 Greys-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-8}{%
 Greys-8-1,mark=x\\%
 Greys-8-2,mark=+\\%
 Greys-8-3,mark=-\\%
 Greys-8-4,mark=|\\%
 Greys-8-5,mark=asterisk\\%
 Greys-8-6,mark=star\\%
 Greys-8-7,mark=10-pointed star\\%
 Greys-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-9}{%
 Greys-9-1,mark=x\\%
 Greys-9-2,mark=+\\%
 Greys-9-3,mark=-\\%
 Greys-9-4,mark=|\\%
 Greys-9-5,mark=asterisk\\%
 Greys-9-6,mark=star\\%
 Greys-9-7,mark=10-pointed star\\%
 Greys-9-8,mark=Mercedes star\\%
 Greys-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-3}{%
 PuOr-3-1,mark=x\\%
 PuOr-3-2,mark=+\\%
 PuOr-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-4}{%
 PuOr-4-1,mark=x\\%
 PuOr-4-2,mark=+\\%
 PuOr-4-3,mark=-\\%
 PuOr-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-5}{%
 PuOr-5-1,mark=x\\%
 PuOr-5-2,mark=+\\%
 PuOr-5-3,mark=-\\%
 PuOr-5-4,mark=|\\%
 PuOr-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-6}{%
 PuOr-6-1,mark=x\\%
 PuOr-6-2,mark=+\\%
 PuOr-6-3,mark=-\\%
 PuOr-6-4,mark=|\\%
 PuOr-6-5,mark=asterisk\\%
 PuOr-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-7}{%
 PuOr-7-1,mark=x\\%
 PuOr-7-2,mark=+\\%
 PuOr-7-3,mark=-\\%
 PuOr-7-4,mark=|\\%
 PuOr-7-5,mark=asterisk\\%
 PuOr-7-6,mark=star\\%
 PuOr-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-8}{%
 PuOr-8-1,mark=x\\%
 PuOr-8-2,mark=+\\%
 PuOr-8-3,mark=-\\%
 PuOr-8-4,mark=|\\%
 PuOr-8-5,mark=asterisk\\%
 PuOr-8-6,mark=star\\%
 PuOr-8-7,mark=10-pointed star\\%
 PuOr-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-9}{%
 PuOr-9-1,mark=x\\%
 PuOr-9-2,mark=+\\%
 PuOr-9-3,mark=-\\%
 PuOr-9-4,mark=|\\%
 PuOr-9-5,mark=asterisk\\%
 PuOr-9-6,mark=star\\%
 PuOr-9-7,mark=10-pointed star\\%
 PuOr-9-8,mark=Mercedes star\\%
 PuOr-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-10}{%
 PuOr-10-1,mark=x\\%
 PuOr-10-2,mark=+\\%
 PuOr-10-3,mark=-\\%
 PuOr-10-4,mark=|\\%
 PuOr-10-5,mark=asterisk\\%
 PuOr-10-6,mark=star\\%
 PuOr-10-7,mark=10-pointed star\\%
 PuOr-10-8,mark=Mercedes star\\%
 PuOr-10-9,mark=Mercedes star flipped\\%
 PuOr-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-11}{%
 PuOr-11-1,mark=x\\%
 PuOr-11-2,mark=+\\%
 PuOr-11-3,mark=-\\%
 PuOr-11-4,mark=|\\%
 PuOr-11-5,mark=asterisk\\%
 PuOr-11-6,mark=star\\%
 PuOr-11-7,mark=10-pointed star\\%
 PuOr-11-8,mark=Mercedes star\\%
 PuOr-11-9,mark=Mercedes star flipped\\%
 PuOr-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-3}{%
 BrBG-3-1,mark=x\\%
 BrBG-3-2,mark=+\\%
 BrBG-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-4}{%
 BrBG-4-1,mark=x\\%
 BrBG-4-2,mark=+\\%
 BrBG-4-3,mark=-\\%
 BrBG-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-5}{%
 BrBG-5-1,mark=x\\%
 BrBG-5-2,mark=+\\%
 BrBG-5-3,mark=-\\%
 BrBG-5-4,mark=|\\%
 BrBG-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-6}{%
 BrBG-6-1,mark=x\\%
 BrBG-6-2,mark=+\\%
 BrBG-6-3,mark=-\\%
 BrBG-6-4,mark=|\\%
 BrBG-6-5,mark=asterisk\\%
 BrBG-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-7}{%
 BrBG-7-1,mark=x\\%
 BrBG-7-2,mark=+\\%
 BrBG-7-3,mark=-\\%
 BrBG-7-4,mark=|\\%
 BrBG-7-5,mark=asterisk\\%
 BrBG-7-6,mark=star\\%
 BrBG-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-8}{%
 BrBG-8-1,mark=x\\%
 BrBG-8-2,mark=+\\%
 BrBG-8-3,mark=-\\%
 BrBG-8-4,mark=|\\%
 BrBG-8-5,mark=asterisk\\%
 BrBG-8-6,mark=star\\%
 BrBG-8-7,mark=10-pointed star\\%
 BrBG-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-9}{%
 BrBG-9-1,mark=x\\%
 BrBG-9-2,mark=+\\%
 BrBG-9-3,mark=-\\%
 BrBG-9-4,mark=|\\%
 BrBG-9-5,mark=asterisk\\%
 BrBG-9-6,mark=star\\%
 BrBG-9-7,mark=10-pointed star\\%
 BrBG-9-8,mark=Mercedes star\\%
 BrBG-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-10}{%
 BrBG-10-1,mark=x\\%
 BrBG-10-2,mark=+\\%
 BrBG-10-3,mark=-\\%
 BrBG-10-4,mark=|\\%
 BrBG-10-5,mark=asterisk\\%
 BrBG-10-6,mark=star\\%
 BrBG-10-7,mark=10-pointed star\\%
 BrBG-10-8,mark=Mercedes star\\%
 BrBG-10-9,mark=Mercedes star flipped\\%
 BrBG-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-11}{%
 BrBG-11-1,mark=x\\%
 BrBG-11-2,mark=+\\%
 BrBG-11-3,mark=-\\%
 BrBG-11-4,mark=|\\%
 BrBG-11-5,mark=asterisk\\%
 BrBG-11-6,mark=star\\%
 BrBG-11-7,mark=10-pointed star\\%
 BrBG-11-8,mark=Mercedes star\\%
 BrBG-11-9,mark=Mercedes star flipped\\%
 BrBG-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-3}{%
 PRGn-3-1,mark=x\\%
 PRGn-3-2,mark=+\\%
 PRGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-4}{%
 PRGn-4-1,mark=x\\%
 PRGn-4-2,mark=+\\%
 PRGn-4-3,mark=-\\%
 PRGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-5}{%
 PRGn-5-1,mark=x\\%
 PRGn-5-2,mark=+\\%
 PRGn-5-3,mark=-\\%
 PRGn-5-4,mark=|\\%
 PRGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-6}{%
 PRGn-6-1,mark=x\\%
 PRGn-6-2,mark=+\\%
 PRGn-6-3,mark=-\\%
 PRGn-6-4,mark=|\\%
 PRGn-6-5,mark=asterisk\\%
 PRGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-7}{%
 PRGn-7-1,mark=x\\%
 PRGn-7-2,mark=+\\%
 PRGn-7-3,mark=-\\%
 PRGn-7-4,mark=|\\%
 PRGn-7-5,mark=asterisk\\%
 PRGn-7-6,mark=star\\%
 PRGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-8}{%
 PRGn-8-1,mark=x\\%
 PRGn-8-2,mark=+\\%
 PRGn-8-3,mark=-\\%
 PRGn-8-4,mark=|\\%
 PRGn-8-5,mark=asterisk\\%
 PRGn-8-6,mark=star\\%
 PRGn-8-7,mark=10-pointed star\\%
 PRGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-9}{%
 PRGn-9-1,mark=x\\%
 PRGn-9-2,mark=+\\%
 PRGn-9-3,mark=-\\%
 PRGn-9-4,mark=|\\%
 PRGn-9-5,mark=asterisk\\%
 PRGn-9-6,mark=star\\%
 PRGn-9-7,mark=10-pointed star\\%
 PRGn-9-8,mark=Mercedes star\\%
 PRGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-10}{%
 PRGn-10-1,mark=x\\%
 PRGn-10-2,mark=+\\%
 PRGn-10-3,mark=-\\%
 PRGn-10-4,mark=|\\%
 PRGn-10-5,mark=asterisk\\%
 PRGn-10-6,mark=star\\%
 PRGn-10-7,mark=10-pointed star\\%
 PRGn-10-8,mark=Mercedes star\\%
 PRGn-10-9,mark=Mercedes star flipped\\%
 PRGn-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-11}{%
 PRGn-11-1,mark=x\\%
 PRGn-11-2,mark=+\\%
 PRGn-11-3,mark=-\\%
 PRGn-11-4,mark=|\\%
 PRGn-11-5,mark=asterisk\\%
 PRGn-11-6,mark=star\\%
 PRGn-11-7,mark=10-pointed star\\%
 PRGn-11-8,mark=Mercedes star\\%
 PRGn-11-9,mark=Mercedes star flipped\\%
 PRGn-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-3}{%
 PiYG-3-1,mark=x\\%
 PiYG-3-2,mark=+\\%
 PiYG-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-4}{%
 PiYG-4-1,mark=x\\%
 PiYG-4-2,mark=+\\%
 PiYG-4-3,mark=-\\%
 PiYG-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-5}{%
 PiYG-5-1,mark=x\\%
 PiYG-5-2,mark=+\\%
 PiYG-5-3,mark=-\\%
 PiYG-5-4,mark=|\\%
 PiYG-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-6}{%
 PiYG-6-1,mark=x\\%
 PiYG-6-2,mark=+\\%
 PiYG-6-3,mark=-\\%
 PiYG-6-4,mark=|\\%
 PiYG-6-5,mark=asterisk\\%
 PiYG-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-7}{%
 PiYG-7-1,mark=x\\%
 PiYG-7-2,mark=+\\%
 PiYG-7-3,mark=-\\%
 PiYG-7-4,mark=|\\%
 PiYG-7-5,mark=asterisk\\%
 PiYG-7-6,mark=star\\%
 PiYG-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-8}{%
 PiYG-8-1,mark=x\\%
 PiYG-8-2,mark=+\\%
 PiYG-8-3,mark=-\\%
 PiYG-8-4,mark=|\\%
 PiYG-8-5,mark=asterisk\\%
 PiYG-8-6,mark=star\\%
 PiYG-8-7,mark=10-pointed star\\%
 PiYG-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-9}{%
 PiYG-9-1,mark=x\\%
 PiYG-9-2,mark=+\\%
 PiYG-9-3,mark=-\\%
 PiYG-9-4,mark=|\\%
 PiYG-9-5,mark=asterisk\\%
 PiYG-9-6,mark=star\\%
 PiYG-9-7,mark=10-pointed star\\%
 PiYG-9-8,mark=Mercedes star\\%
 PiYG-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-10}{%
 PiYG-10-1,mark=x\\%
 PiYG-10-2,mark=+\\%
 PiYG-10-3,mark=-\\%
 PiYG-10-4,mark=|\\%
 PiYG-10-5,mark=asterisk\\%
 PiYG-10-6,mark=star\\%
 PiYG-10-7,mark=10-pointed star\\%
 PiYG-10-8,mark=Mercedes star\\%
 PiYG-10-9,mark=Mercedes star flipped\\%
 PiYG-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-11}{%
 PiYG-11-1,mark=x\\%
 PiYG-11-2,mark=+\\%
 PiYG-11-3,mark=-\\%
 PiYG-11-4,mark=|\\%
 PiYG-11-5,mark=asterisk\\%
 PiYG-11-6,mark=star\\%
 PiYG-11-7,mark=10-pointed star\\%
 PiYG-11-8,mark=Mercedes star\\%
 PiYG-11-9,mark=Mercedes star flipped\\%
 PiYG-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-3}{%
 RdBu-3-1,mark=x\\%
 RdBu-3-2,mark=+\\%
 RdBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-4}{%
 RdBu-4-1,mark=x\\%
 RdBu-4-2,mark=+\\%
 RdBu-4-3,mark=-\\%
 RdBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-5}{%
 RdBu-5-1,mark=x\\%
 RdBu-5-2,mark=+\\%
 RdBu-5-3,mark=-\\%
 RdBu-5-4,mark=|\\%
 RdBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-6}{%
 RdBu-6-1,mark=x\\%
 RdBu-6-2,mark=+\\%
 RdBu-6-3,mark=-\\%
 RdBu-6-4,mark=|\\%
 RdBu-6-5,mark=asterisk\\%
 RdBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-7}{%
 RdBu-7-1,mark=x\\%
 RdBu-7-2,mark=+\\%
 RdBu-7-3,mark=-\\%
 RdBu-7-4,mark=|\\%
 RdBu-7-5,mark=asterisk\\%
 RdBu-7-6,mark=star\\%
 RdBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-8}{%
 RdBu-8-1,mark=x\\%
 RdBu-8-2,mark=+\\%
 RdBu-8-3,mark=-\\%
 RdBu-8-4,mark=|\\%
 RdBu-8-5,mark=asterisk\\%
 RdBu-8-6,mark=star\\%
 RdBu-8-7,mark=10-pointed star\\%
 RdBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-9}{%
 RdBu-9-1,mark=x\\%
 RdBu-9-2,mark=+\\%
 RdBu-9-3,mark=-\\%
 RdBu-9-4,mark=|\\%
 RdBu-9-5,mark=asterisk\\%
 RdBu-9-6,mark=star\\%
 RdBu-9-7,mark=10-pointed star\\%
 RdBu-9-8,mark=Mercedes star\\%
 RdBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-10}{%
 RdBu-10-1,mark=x\\%
 RdBu-10-2,mark=+\\%
 RdBu-10-3,mark=-\\%
 RdBu-10-4,mark=|\\%
 RdBu-10-5,mark=asterisk\\%
 RdBu-10-6,mark=star\\%
 RdBu-10-7,mark=10-pointed star\\%
 RdBu-10-8,mark=Mercedes star\\%
 RdBu-10-9,mark=Mercedes star flipped\\%
 RdBu-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-11}{%
 RdBu-11-1,mark=x\\%
 RdBu-11-2,mark=+\\%
 RdBu-11-3,mark=-\\%
 RdBu-11-4,mark=|\\%
 RdBu-11-5,mark=asterisk\\%
 RdBu-11-6,mark=star\\%
 RdBu-11-7,mark=10-pointed star\\%
 RdBu-11-8,mark=Mercedes star\\%
 RdBu-11-9,mark=Mercedes star flipped\\%
 RdBu-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-3}{%
 RdGy-3-1,mark=x\\%
 RdGy-3-2,mark=+\\%
 RdGy-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-4}{%
 RdGy-4-1,mark=x\\%
 RdGy-4-2,mark=+\\%
 RdGy-4-3,mark=-\\%
 RdGy-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-5}{%
 RdGy-5-1,mark=x\\%
 RdGy-5-2,mark=+\\%
 RdGy-5-3,mark=-\\%
 RdGy-5-4,mark=|\\%
 RdGy-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-6}{%
 RdGy-6-1,mark=x\\%
 RdGy-6-2,mark=+\\%
 RdGy-6-3,mark=-\\%
 RdGy-6-4,mark=|\\%
 RdGy-6-5,mark=asterisk\\%
 RdGy-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-7}{%
 RdGy-7-1,mark=x\\%
 RdGy-7-2,mark=+\\%
 RdGy-7-3,mark=-\\%
 RdGy-7-4,mark=|\\%
 RdGy-7-5,mark=asterisk\\%
 RdGy-7-6,mark=star\\%
 RdGy-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-8}{%
 RdGy-8-1,mark=x\\%
 RdGy-8-2,mark=+\\%
 RdGy-8-3,mark=-\\%
 RdGy-8-4,mark=|\\%
 RdGy-8-5,mark=asterisk\\%
 RdGy-8-6,mark=star\\%
 RdGy-8-7,mark=10-pointed star\\%
 RdGy-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-9}{%
 RdGy-9-1,mark=x\\%
 RdGy-9-2,mark=+\\%
 RdGy-9-3,mark=-\\%
 RdGy-9-4,mark=|\\%
 RdGy-9-5,mark=asterisk\\%
 RdGy-9-6,mark=star\\%
 RdGy-9-7,mark=10-pointed star\\%
 RdGy-9-8,mark=Mercedes star\\%
 RdGy-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-10}{%
 RdGy-10-1,mark=x\\%
 RdGy-10-2,mark=+\\%
 RdGy-10-3,mark=-\\%
 RdGy-10-4,mark=|\\%
 RdGy-10-5,mark=asterisk\\%
 RdGy-10-6,mark=star\\%
 RdGy-10-7,mark=10-pointed star\\%
 RdGy-10-8,mark=Mercedes star\\%
 RdGy-10-9,mark=Mercedes star flipped\\%
 RdGy-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-11}{%
 RdGy-11-1,mark=x\\%
 RdGy-11-2,mark=+\\%
 RdGy-11-3,mark=-\\%
 RdGy-11-4,mark=|\\%
 RdGy-11-5,mark=asterisk\\%
 RdGy-11-6,mark=star\\%
 RdGy-11-7,mark=10-pointed star\\%
 RdGy-11-8,mark=Mercedes star\\%
 RdGy-11-9,mark=Mercedes star flipped\\%
 RdGy-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-3}{%
 RdYlBu-3-1,mark=x\\%
 RdYlBu-3-2,mark=+\\%
 RdYlBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-4}{%
 RdYlBu-4-1,mark=x\\%
 RdYlBu-4-2,mark=+\\%
 RdYlBu-4-3,mark=-\\%
 RdYlBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-5}{%
 RdYlBu-5-1,mark=x\\%
 RdYlBu-5-2,mark=+\\%
 RdYlBu-5-3,mark=-\\%
 RdYlBu-5-4,mark=|\\%
 RdYlBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-6}{%
 RdYlBu-6-1,mark=x\\%
 RdYlBu-6-2,mark=+\\%
 RdYlBu-6-3,mark=-\\%
 RdYlBu-6-4,mark=|\\%
 RdYlBu-6-5,mark=asterisk\\%
 RdYlBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-7}{%
 RdYlBu-7-1,mark=x\\%
 RdYlBu-7-2,mark=+\\%
 RdYlBu-7-3,mark=-\\%
 RdYlBu-7-4,mark=|\\%
 RdYlBu-7-5,mark=asterisk\\%
 RdYlBu-7-6,mark=star\\%
 RdYlBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-8}{%
 RdYlBu-8-1,mark=x\\%
 RdYlBu-8-2,mark=+\\%
 RdYlBu-8-3,mark=-\\%
 RdYlBu-8-4,mark=|\\%
 RdYlBu-8-5,mark=asterisk\\%
 RdYlBu-8-6,mark=star\\%
 RdYlBu-8-7,mark=10-pointed star\\%
 RdYlBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-9}{%
 RdYlBu-9-1,mark=x\\%
 RdYlBu-9-2,mark=+\\%
 RdYlBu-9-3,mark=-\\%
 RdYlBu-9-4,mark=|\\%
 RdYlBu-9-5,mark=asterisk\\%
 RdYlBu-9-6,mark=star\\%
 RdYlBu-9-7,mark=10-pointed star\\%
 RdYlBu-9-8,mark=Mercedes star\\%
 RdYlBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-10}{%
 RdYlBu-10-1,mark=x\\%
 RdYlBu-10-2,mark=+\\%
 RdYlBu-10-3,mark=-\\%
 RdYlBu-10-4,mark=|\\%
 RdYlBu-10-5,mark=asterisk\\%
 RdYlBu-10-6,mark=star\\%
 RdYlBu-10-7,mark=10-pointed star\\%
 RdYlBu-10-8,mark=Mercedes star\\%
 RdYlBu-10-9,mark=Mercedes star flipped\\%
 RdYlBu-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-11}{%
 RdYlBu-11-1,mark=x\\%
 RdYlBu-11-2,mark=+\\%
 RdYlBu-11-3,mark=-\\%
 RdYlBu-11-4,mark=|\\%
 RdYlBu-11-5,mark=asterisk\\%
 RdYlBu-11-6,mark=star\\%
 RdYlBu-11-7,mark=10-pointed star\\%
 RdYlBu-11-8,mark=Mercedes star\\%
 RdYlBu-11-9,mark=Mercedes star flipped\\%
 RdYlBu-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-3}{%
 Spectral-3-1,mark=x\\%
 Spectral-3-2,mark=+\\%
 Spectral-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-4}{%
 Spectral-4-1,mark=x\\%
 Spectral-4-2,mark=+\\%
 Spectral-4-3,mark=-\\%
 Spectral-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-5}{%
 Spectral-5-1,mark=x\\%
 Spectral-5-2,mark=+\\%
 Spectral-5-3,mark=-\\%
 Spectral-5-4,mark=|\\%
 Spectral-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-6}{%
 Spectral-6-1,mark=x\\%
 Spectral-6-2,mark=+\\%
 Spectral-6-3,mark=-\\%
 Spectral-6-4,mark=|\\%
 Spectral-6-5,mark=asterisk\\%
 Spectral-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-7}{%
 Spectral-7-1,mark=x\\%
 Spectral-7-2,mark=+\\%
 Spectral-7-3,mark=-\\%
 Spectral-7-4,mark=|\\%
 Spectral-7-5,mark=asterisk\\%
 Spectral-7-6,mark=star\\%
 Spectral-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-8}{%
 Spectral-8-1,mark=x\\%
 Spectral-8-2,mark=+\\%
 Spectral-8-3,mark=-\\%
 Spectral-8-4,mark=|\\%
 Spectral-8-5,mark=asterisk\\%
 Spectral-8-6,mark=star\\%
 Spectral-8-7,mark=10-pointed star\\%
 Spectral-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-9}{%
 Spectral-9-1,mark=x\\%
 Spectral-9-2,mark=+\\%
 Spectral-9-3,mark=-\\%
 Spectral-9-4,mark=|\\%
 Spectral-9-5,mark=asterisk\\%
 Spectral-9-6,mark=star\\%
 Spectral-9-7,mark=10-pointed star\\%
 Spectral-9-8,mark=Mercedes star\\%
 Spectral-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-10}{%
 Spectral-10-1,mark=x\\%
 Spectral-10-2,mark=+\\%
 Spectral-10-3,mark=-\\%
 Spectral-10-4,mark=|\\%
 Spectral-10-5,mark=asterisk\\%
 Spectral-10-6,mark=star\\%
 Spectral-10-7,mark=10-pointed star\\%
 Spectral-10-8,mark=Mercedes star\\%
 Spectral-10-9,mark=Mercedes star flipped\\%
 Spectral-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-11}{%
 Spectral-11-1,mark=x\\%
 Spectral-11-2,mark=+\\%
 Spectral-11-3,mark=-\\%
 Spectral-11-4,mark=|\\%
 Spectral-11-5,mark=asterisk\\%
 Spectral-11-6,mark=star\\%
 Spectral-11-7,mark=10-pointed star\\%
 Spectral-11-8,mark=Mercedes star\\%
 Spectral-11-9,mark=Mercedes star flipped\\%
 Spectral-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-3}{%
 RdYlGn-3-1,mark=x\\%
 RdYlGn-3-2,mark=+\\%
 RdYlGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-4}{%
 RdYlGn-4-1,mark=x\\%
 RdYlGn-4-2,mark=+\\%
 RdYlGn-4-3,mark=-\\%
 RdYlGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-5}{%
 RdYlGn-5-1,mark=x\\%
 RdYlGn-5-2,mark=+\\%
 RdYlGn-5-3,mark=-\\%
 RdYlGn-5-4,mark=|\\%
 RdYlGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-6}{%
 RdYlGn-6-1,mark=x\\%
 RdYlGn-6-2,mark=+\\%
 RdYlGn-6-3,mark=-\\%
 RdYlGn-6-4,mark=|\\%
 RdYlGn-6-5,mark=asterisk\\%
 RdYlGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-7}{%
 RdYlGn-7-1,mark=x\\%
 RdYlGn-7-2,mark=+\\%
 RdYlGn-7-3,mark=-\\%
 RdYlGn-7-4,mark=|\\%
 RdYlGn-7-5,mark=asterisk\\%
 RdYlGn-7-6,mark=star\\%
 RdYlGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-8}{%
 RdYlGn-8-1,mark=x\\%
 RdYlGn-8-2,mark=+\\%
 RdYlGn-8-3,mark=-\\%
 RdYlGn-8-4,mark=|\\%
 RdYlGn-8-5,mark=asterisk\\%
 RdYlGn-8-6,mark=star\\%
 RdYlGn-8-7,mark=10-pointed star\\%
 RdYlGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-9}{%
 RdYlGn-9-1,mark=x\\%
 RdYlGn-9-2,mark=+\\%
 RdYlGn-9-3,mark=-\\%
 RdYlGn-9-4,mark=|\\%
 RdYlGn-9-5,mark=asterisk\\%
 RdYlGn-9-6,mark=star\\%
 RdYlGn-9-7,mark=10-pointed star\\%
 RdYlGn-9-8,mark=Mercedes star\\%
 RdYlGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-10}{%
 RdYlGn-10-1,mark=x\\%
 RdYlGn-10-2,mark=+\\%
 RdYlGn-10-3,mark=-\\%
 RdYlGn-10-4,mark=|\\%
 RdYlGn-10-5,mark=asterisk\\%
 RdYlGn-10-6,mark=star\\%
 RdYlGn-10-7,mark=10-pointed star\\%
 RdYlGn-10-8,mark=Mercedes star\\%
 RdYlGn-10-9,mark=Mercedes star flipped\\%
 RdYlGn-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-11}{%
 RdYlGn-11-1,mark=x\\%
 RdYlGn-11-2,mark=+\\%
 RdYlGn-11-3,mark=-\\%
 RdYlGn-11-4,mark=|\\%
 RdYlGn-11-5,mark=asterisk\\%
 RdYlGn-11-6,mark=star\\%
 RdYlGn-11-7,mark=10-pointed star\\%
 RdYlGn-11-8,mark=Mercedes star\\%
 RdYlGn-11-9,mark=Mercedes star flipped\\%
 RdYlGn-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-3}{%
 Set3-3-1,mark=x\\%
 Set3-3-2,mark=+\\%
 Set3-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-4}{%
 Set3-4-1,mark=x\\%
 Set3-4-2,mark=+\\%
 Set3-4-3,mark=-\\%
 Set3-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-5}{%
 Set3-5-1,mark=x\\%
 Set3-5-2,mark=+\\%
 Set3-5-3,mark=-\\%
 Set3-5-4,mark=|\\%
 Set3-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-6}{%
 Set3-6-1,mark=x\\%
 Set3-6-2,mark=+\\%
 Set3-6-3,mark=-\\%
 Set3-6-4,mark=|\\%
 Set3-6-5,mark=asterisk\\%
 Set3-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-7}{%
 Set3-7-1,mark=x\\%
 Set3-7-2,mark=+\\%
 Set3-7-3,mark=-\\%
 Set3-7-4,mark=|\\%
 Set3-7-5,mark=asterisk\\%
 Set3-7-6,mark=star\\%
 Set3-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-8}{%
 Set3-8-1,mark=x\\%
 Set3-8-2,mark=+\\%
 Set3-8-3,mark=-\\%
 Set3-8-4,mark=|\\%
 Set3-8-5,mark=asterisk\\%
 Set3-8-6,mark=star\\%
 Set3-8-7,mark=10-pointed star\\%
 Set3-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-9}{%
 Set3-9-1,mark=x\\%
 Set3-9-2,mark=+\\%
 Set3-9-3,mark=-\\%
 Set3-9-4,mark=|\\%
 Set3-9-5,mark=asterisk\\%
 Set3-9-6,mark=star\\%
 Set3-9-7,mark=10-pointed star\\%
 Set3-9-8,mark=Mercedes star\\%
 Set3-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-10}{%
 Set3-10-1,mark=x\\%
 Set3-10-2,mark=+\\%
 Set3-10-3,mark=-\\%
 Set3-10-4,mark=|\\%
 Set3-10-5,mark=asterisk\\%
 Set3-10-6,mark=star\\%
 Set3-10-7,mark=10-pointed star\\%
 Set3-10-8,mark=Mercedes star\\%
 Set3-10-9,mark=Mercedes star flipped\\%
 Set3-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-11}{%
 Set3-11-1,mark=x\\%
 Set3-11-2,mark=+\\%
 Set3-11-3,mark=-\\%
 Set3-11-4,mark=|\\%
 Set3-11-5,mark=asterisk\\%
 Set3-11-6,mark=star\\%
 Set3-11-7,mark=10-pointed star\\%
 Set3-11-8,mark=Mercedes star\\%
 Set3-11-9,mark=Mercedes star flipped\\%
 Set3-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-12}{%
 Set3-12-1,mark=x\\%
 Set3-12-2,mark=+\\%
 Set3-12-3,mark=-\\%
 Set3-12-4,mark=|\\%
 Set3-12-5,mark=asterisk\\%
 Set3-12-6,mark=star\\%
 Set3-12-7,mark=10-pointed star\\%
 Set3-12-8,mark=Mercedes star\\%
 Set3-12-9,mark=Mercedes star flipped\\%
 Set3-12-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-3}{%
 Pastel1-3-1,mark=x\\%
 Pastel1-3-2,mark=+\\%
 Pastel1-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-4}{%
 Pastel1-4-1,mark=x\\%
 Pastel1-4-2,mark=+\\%
 Pastel1-4-3,mark=-\\%
 Pastel1-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-5}{%
 Pastel1-5-1,mark=x\\%
 Pastel1-5-2,mark=+\\%
 Pastel1-5-3,mark=-\\%
 Pastel1-5-4,mark=|\\%
 Pastel1-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-6}{%
 Pastel1-6-1,mark=x\\%
 Pastel1-6-2,mark=+\\%
 Pastel1-6-3,mark=-\\%
 Pastel1-6-4,mark=|\\%
 Pastel1-6-5,mark=asterisk\\%
 Pastel1-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-7}{%
 Pastel1-7-1,mark=x\\%
 Pastel1-7-2,mark=+\\%
 Pastel1-7-3,mark=-\\%
 Pastel1-7-4,mark=|\\%
 Pastel1-7-5,mark=asterisk\\%
 Pastel1-7-6,mark=star\\%
 Pastel1-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-8}{%
 Pastel1-8-1,mark=x\\%
 Pastel1-8-2,mark=+\\%
 Pastel1-8-3,mark=-\\%
 Pastel1-8-4,mark=|\\%
 Pastel1-8-5,mark=asterisk\\%
 Pastel1-8-6,mark=star\\%
 Pastel1-8-7,mark=10-pointed star\\%
 Pastel1-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-9}{%
 Pastel1-9-1,mark=x\\%
 Pastel1-9-2,mark=+\\%
 Pastel1-9-3,mark=-\\%
 Pastel1-9-4,mark=|\\%
 Pastel1-9-5,mark=asterisk\\%
 Pastel1-9-6,mark=star\\%
 Pastel1-9-7,mark=10-pointed star\\%
 Pastel1-9-8,mark=Mercedes star\\%
 Pastel1-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-3}{%
 Set1-3-1,mark=x\\%
 Set1-3-2,mark=+\\%
 Set1-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-4}{%
 Set1-4-1,mark=x\\%
 Set1-4-2,mark=+\\%
 Set1-4-3,mark=-\\%
 Set1-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-5}{%
 Set1-5-1,mark=x\\%
 Set1-5-2,mark=+\\%
 Set1-5-3,mark=-\\%
 Set1-5-4,mark=|\\%
 Set1-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-6}{%
 Set1-6-1,mark=x\\%
 Set1-6-2,mark=+\\%
 Set1-6-3,mark=-\\%
 Set1-6-4,mark=|\\%
 Set1-6-5,mark=asterisk\\%
 Set1-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-7}{%
 Set1-7-1,mark=x\\%
 Set1-7-2,mark=+\\%
 Set1-7-3,mark=-\\%
 Set1-7-4,mark=|\\%
 Set1-7-5,mark=asterisk\\%
 Set1-7-6,mark=star\\%
 Set1-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-8}{%
 Set1-8-1,mark=x\\%
 Set1-8-2,mark=+\\%
 Set1-8-3,mark=-\\%
 Set1-8-4,mark=|\\%
 Set1-8-5,mark=asterisk\\%
 Set1-8-6,mark=star\\%
 Set1-8-7,mark=10-pointed star\\%
 Set1-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-9}{%
 Set1-9-1,mark=x\\%
 Set1-9-2,mark=+\\%
 Set1-9-3,mark=-\\%
 Set1-9-4,mark=|\\%
 Set1-9-5,mark=asterisk\\%
 Set1-9-6,mark=star\\%
 Set1-9-7,mark=10-pointed star\\%
 Set1-9-8,mark=Mercedes star\\%
 Set1-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-3}{%
 Pastel2-3-1,mark=x\\%
 Pastel2-3-2,mark=+\\%
 Pastel2-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-4}{%
 Pastel2-4-1,mark=x\\%
 Pastel2-4-2,mark=+\\%
 Pastel2-4-3,mark=-\\%
 Pastel2-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-5}{%
 Pastel2-5-1,mark=x\\%
 Pastel2-5-2,mark=+\\%
 Pastel2-5-3,mark=-\\%
 Pastel2-5-4,mark=|\\%
 Pastel2-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-6}{%
 Pastel2-6-1,mark=x\\%
 Pastel2-6-2,mark=+\\%
 Pastel2-6-3,mark=-\\%
 Pastel2-6-4,mark=|\\%
 Pastel2-6-5,mark=asterisk\\%
 Pastel2-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-7}{%
 Pastel2-7-1,mark=x\\%
 Pastel2-7-2,mark=+\\%
 Pastel2-7-3,mark=-\\%
 Pastel2-7-4,mark=|\\%
 Pastel2-7-5,mark=asterisk\\%
 Pastel2-7-6,mark=star\\%
 Pastel2-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-8}{%
 Pastel2-8-1,mark=x\\%
 Pastel2-8-2,mark=+\\%
 Pastel2-8-3,mark=-\\%
 Pastel2-8-4,mark=|\\%
 Pastel2-8-5,mark=asterisk\\%
 Pastel2-8-6,mark=star\\%
 Pastel2-8-7,mark=10-pointed star\\%
 Pastel2-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-3}{%
 Set2-3-1,mark=x\\%
 Set2-3-2,mark=+\\%
 Set2-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-4}{%
 Set2-4-1,mark=x\\%
 Set2-4-2,mark=+\\%
 Set2-4-3,mark=-\\%
 Set2-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-5}{%
 Set2-5-1,mark=x\\%
 Set2-5-2,mark=+\\%
 Set2-5-3,mark=-\\%
 Set2-5-4,mark=|\\%
 Set2-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-6}{%
 Set2-6-1,mark=x\\%
 Set2-6-2,mark=+\\%
 Set2-6-3,mark=-\\%
 Set2-6-4,mark=|\\%
 Set2-6-5,mark=asterisk\\%
 Set2-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-7}{%
 Set2-7-1,mark=x\\%
 Set2-7-2,mark=+\\%
 Set2-7-3,mark=-\\%
 Set2-7-4,mark=|\\%
 Set2-7-5,mark=asterisk\\%
 Set2-7-6,mark=star\\%
 Set2-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-8}{%
 Set2-8-1,mark=x\\%
 Set2-8-2,mark=+\\%
 Set2-8-3,mark=-\\%
 Set2-8-4,mark=|\\%
 Set2-8-5,mark=asterisk\\%
 Set2-8-6,mark=star\\%
 Set2-8-7,mark=10-pointed star\\%
 Set2-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-3}{%
 Dark2-3-1,mark=x\\%
 Dark2-3-2,mark=+\\%
 Dark2-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-4}{%
 Dark2-4-1,mark=x\\%
 Dark2-4-2,mark=+\\%
 Dark2-4-3,mark=-\\%
 Dark2-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-5}{%
 Dark2-5-1,mark=x\\%
 Dark2-5-2,mark=+\\%
 Dark2-5-3,mark=-\\%
 Dark2-5-4,mark=|\\%
 Dark2-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-6}{%
 Dark2-6-1,mark=x\\%
 Dark2-6-2,mark=+\\%
 Dark2-6-3,mark=-\\%
 Dark2-6-4,mark=|\\%
 Dark2-6-5,mark=asterisk\\%
 Dark2-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-7}{%
 Dark2-7-1,mark=x\\%
 Dark2-7-2,mark=+\\%
 Dark2-7-3,mark=-\\%
 Dark2-7-4,mark=|\\%
 Dark2-7-5,mark=asterisk\\%
 Dark2-7-6,mark=star\\%
 Dark2-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-8}{%
 Dark2-8-1,mark=x\\%
 Dark2-8-2,mark=+\\%
 Dark2-8-3,mark=-\\%
 Dark2-8-4,mark=|\\%
 Dark2-8-5,mark=asterisk\\%
 Dark2-8-6,mark=star\\%
 Dark2-8-7,mark=10-pointed star\\%
 Dark2-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-3}{%
 Paired-3-1,mark=x\\%
 Paired-3-2,mark=+\\%
 Paired-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-4}{%
 Paired-4-1,mark=x\\%
 Paired-4-2,mark=+\\%
 Paired-4-3,mark=-\\%
 Paired-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-5}{%
 Paired-5-1,mark=x\\%
 Paired-5-2,mark=+\\%
 Paired-5-3,mark=-\\%
 Paired-5-4,mark=|\\%
 Paired-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-6}{%
 Paired-6-1,mark=x\\%
 Paired-6-2,mark=+\\%
 Paired-6-3,mark=-\\%
 Paired-6-4,mark=|\\%
 Paired-6-5,mark=asterisk\\%
 Paired-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-7}{%
 Paired-7-1,mark=x\\%
 Paired-7-2,mark=+\\%
 Paired-7-3,mark=-\\%
 Paired-7-4,mark=|\\%
 Paired-7-5,mark=asterisk\\%
 Paired-7-6,mark=star\\%
 Paired-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-8}{%
 Paired-8-1,mark=x\\%
 Paired-8-2,mark=+\\%
 Paired-8-3,mark=-\\%
 Paired-8-4,mark=|\\%
 Paired-8-5,mark=asterisk\\%
 Paired-8-6,mark=star\\%
 Paired-8-7,mark=10-pointed star\\%
 Paired-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-9}{%
 Paired-9-1,mark=x\\%
 Paired-9-2,mark=+\\%
 Paired-9-3,mark=-\\%
 Paired-9-4,mark=|\\%
 Paired-9-5,mark=asterisk\\%
 Paired-9-6,mark=star\\%
 Paired-9-7,mark=10-pointed star\\%
 Paired-9-8,mark=Mercedes star\\%
 Paired-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-10}{%
 Paired-10-1,mark=x\\%
 Paired-10-2,mark=+\\%
 Paired-10-3,mark=-\\%
 Paired-10-4,mark=|\\%
 Paired-10-5,mark=asterisk\\%
 Paired-10-6,mark=star\\%
 Paired-10-7,mark=10-pointed star\\%
 Paired-10-8,mark=Mercedes star\\%
 Paired-10-9,mark=Mercedes star flipped\\%
 Paired-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-11}{%
 Paired-11-1,mark=x\\%
 Paired-11-2,mark=+\\%
 Paired-11-3,mark=-\\%
 Paired-11-4,mark=|\\%
 Paired-11-5,mark=asterisk\\%
 Paired-11-6,mark=star\\%
 Paired-11-7,mark=10-pointed star\\%
 Paired-11-8,mark=Mercedes star\\%
 Paired-11-9,mark=Mercedes star flipped\\%
 Paired-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-12}{%
 Paired-12-1,mark=x\\%
 Paired-12-2,mark=+\\%
 Paired-12-3,mark=-\\%
 Paired-12-4,mark=|\\%
 Paired-12-5,mark=asterisk\\%
 Paired-12-6,mark=star\\%
 Paired-12-7,mark=10-pointed star\\%
 Paired-12-8,mark=Mercedes star\\%
 Paired-12-9,mark=Mercedes star flipped\\%
 Paired-12-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-3}{%
 Accent-3-1,mark=x\\%
 Accent-3-2,mark=+\\%
 Accent-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-4}{%
 Accent-4-1,mark=x\\%
 Accent-4-2,mark=+\\%
 Accent-4-3,mark=-\\%
 Accent-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-5}{%
 Accent-5-1,mark=x\\%
 Accent-5-2,mark=+\\%
 Accent-5-3,mark=-\\%
 Accent-5-4,mark=|\\%
 Accent-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-6}{%
 Accent-6-1,mark=x\\%
 Accent-6-2,mark=+\\%
 Accent-6-3,mark=-\\%
 Accent-6-4,mark=|\\%
 Accent-6-5,mark=asterisk\\%
 Accent-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-7}{%
 Accent-7-1,mark=x\\%
 Accent-7-2,mark=+\\%
 Accent-7-3,mark=-\\%
 Accent-7-4,mark=|\\%
 Accent-7-5,mark=asterisk\\%
 Accent-7-6,mark=star\\%
 Accent-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-8}{%
 Accent-8-1,mark=x\\%
 Accent-8-2,mark=+\\%
 Accent-8-3,mark=-\\%
 Accent-8-4,mark=|\\%
 Accent-8-5,mark=asterisk\\%
 Accent-8-6,mark=star\\%
 Accent-8-7,mark=10-pointed star\\%
 Accent-8-8,mark=Mercedes star\\%
}
\pgfplotsset{
colormap={YlGn-3}{
  color=(YlGn-3-1);
  color=(YlGn-3-2);
  color=(YlGn-3-3);
},
colormap={YlGn-4}{
  color=(YlGn-4-1);
  color=(YlGn-4-2);
  color=(YlGn-4-3);
  color=(YlGn-4-4);
},
colormap={YlGn-5}{
  color=(YlGn-5-1);
  color=(YlGn-5-2);
  color=(YlGn-5-3);
  color=(YlGn-5-4);
  color=(YlGn-5-5);
},
colormap={YlGn-6}{
  color=(YlGn-6-1);
  color=(YlGn-6-2);
  color=(YlGn-6-3);
  color=(YlGn-6-4);
  color=(YlGn-6-5);
  color=(YlGn-6-6);
},
colormap={YlGn-7}{
  color=(YlGn-7-1);
  color=(YlGn-7-2);
  color=(YlGn-7-3);
  color=(YlGn-7-4);
  color=(YlGn-7-5);
  color=(YlGn-7-6);
  color=(YlGn-7-7);
},
colormap={YlGn-8}{
  color=(YlGn-8-1);
  color=(YlGn-8-2);
  color=(YlGn-8-3);
  color=(YlGn-8-4);
  color=(YlGn-8-5);
  color=(YlGn-8-6);
  color=(YlGn-8-7);
  color=(YlGn-8-8);
},
colormap={YlGn-9}{
  color=(YlGn-9-1);
  color=(YlGn-9-2);
  color=(YlGn-9-3);
  color=(YlGn-9-4);
  color=(YlGn-9-5);
  color=(YlGn-9-6);
  color=(YlGn-9-7);
  color=(YlGn-9-8);
  color=(YlGn-9-9);
},
colormap={YlGnBu-3}{
  color=(YlGnBu-3-1);
  color=(YlGnBu-3-2);
  color=(YlGnBu-3-3);
},
colormap={YlGnBu-4}{
  color=(YlGnBu-4-1);
  color=(YlGnBu-4-2);
  color=(YlGnBu-4-3);
  color=(YlGnBu-4-4);
},
colormap={YlGnBu-5}{
  color=(YlGnBu-5-1);
  color=(YlGnBu-5-2);
  color=(YlGnBu-5-3);
  color=(YlGnBu-5-4);
  color=(YlGnBu-5-5);
},
colormap={YlGnBu-6}{
  color=(YlGnBu-6-1);
  color=(YlGnBu-6-2);
  color=(YlGnBu-6-3);
  color=(YlGnBu-6-4);
  color=(YlGnBu-6-5);
  color=(YlGnBu-6-6);
},
colormap={YlGnBu-7}{
  color=(YlGnBu-7-1);
  color=(YlGnBu-7-2);
  color=(YlGnBu-7-3);
  color=(YlGnBu-7-4);
  color=(YlGnBu-7-5);
  color=(YlGnBu-7-6);
  color=(YlGnBu-7-7);
},
colormap={YlGnBu-8}{
  color=(YlGnBu-8-1);
  color=(YlGnBu-8-2);
  color=(YlGnBu-8-3);
  color=(YlGnBu-8-4);
  color=(YlGnBu-8-5);
  color=(YlGnBu-8-6);
  color=(YlGnBu-8-7);
  color=(YlGnBu-8-8);
},
colormap={YlGnBu-9}{
  color=(YlGnBu-9-1);
  color=(YlGnBu-9-2);
  color=(YlGnBu-9-3);
  color=(YlGnBu-9-4);
  color=(YlGnBu-9-5);
  color=(YlGnBu-9-6);
  color=(YlGnBu-9-7);
  color=(YlGnBu-9-8);
  color=(YlGnBu-9-9);
},
colormap={GnBu-3}{
  color=(GnBu-3-1);
  color=(GnBu-3-2);
  color=(GnBu-3-3);
},
colormap={GnBu-4}{
  color=(GnBu-4-1);
  color=(GnBu-4-2);
  color=(GnBu-4-3);
  color=(GnBu-4-4);
},
colormap={GnBu-5}{
  color=(GnBu-5-1);
  color=(GnBu-5-2);
  color=(GnBu-5-3);
  color=(GnBu-5-4);
  color=(GnBu-5-5);
},
colormap={GnBu-6}{
  color=(GnBu-6-1);
  color=(GnBu-6-2);
  color=(GnBu-6-3);
  color=(GnBu-6-4);
  color=(GnBu-6-5);
  color=(GnBu-6-6);
},
colormap={GnBu-7}{
  color=(GnBu-7-1);
  color=(GnBu-7-2);
  color=(GnBu-7-3);
  color=(GnBu-7-4);
  color=(GnBu-7-5);
  color=(GnBu-7-6);
  color=(GnBu-7-7);
},
colormap={GnBu-8}{
  color=(GnBu-8-1);
  color=(GnBu-8-2);
  color=(GnBu-8-3);
  color=(GnBu-8-4);
  color=(GnBu-8-5);
  color=(GnBu-8-6);
  color=(GnBu-8-7);
  color=(GnBu-8-8);
},
colormap={GnBu-9}{
  color=(GnBu-9-1);
  color=(GnBu-9-2);
  color=(GnBu-9-3);
  color=(GnBu-9-4);
  color=(GnBu-9-5);
  color=(GnBu-9-6);
  color=(GnBu-9-7);
  color=(GnBu-9-8);
  color=(GnBu-9-9);
},
colormap={BuGn-3}{
  color=(BuGn-3-1);
  color=(BuGn-3-2);
  color=(BuGn-3-3);
},
colormap={BuGn-4}{
  color=(BuGn-4-1);
  color=(BuGn-4-2);
  color=(BuGn-4-3);
  color=(BuGn-4-4);
},
colormap={BuGn-5}{
  color=(BuGn-5-1);
  color=(BuGn-5-2);
  color=(BuGn-5-3);
  color=(BuGn-5-4);
  color=(BuGn-5-5);
},
colormap={BuGn-6}{
  color=(BuGn-6-1);
  color=(BuGn-6-2);
  color=(BuGn-6-3);
  color=(BuGn-6-4);
  color=(BuGn-6-5);
  color=(BuGn-6-6);
},
colormap={BuGn-7}{
  color=(BuGn-7-1);
  color=(BuGn-7-2);
  color=(BuGn-7-3);
  color=(BuGn-7-4);
  color=(BuGn-7-5);
  color=(BuGn-7-6);
  color=(BuGn-7-7);
},
colormap={BuGn-8}{
  color=(BuGn-8-1);
  color=(BuGn-8-2);
  color=(BuGn-8-3);
  color=(BuGn-8-4);
  color=(BuGn-8-5);
  color=(BuGn-8-6);
  color=(BuGn-8-7);
  color=(BuGn-8-8);
},
colormap={BuGn-9}{
  color=(BuGn-9-1);
  color=(BuGn-9-2);
  color=(BuGn-9-3);
  color=(BuGn-9-4);
  color=(BuGn-9-5);
  color=(BuGn-9-6);
  color=(BuGn-9-7);
  color=(BuGn-9-8);
  color=(BuGn-9-9);
},
colormap={PuBuGn-3}{
  color=(PuBuGn-3-1);
  color=(PuBuGn-3-2);
  color=(PuBuGn-3-3);
},
colormap={PuBuGn-4}{
  color=(PuBuGn-4-1);
  color=(PuBuGn-4-2);
  color=(PuBuGn-4-3);
  color=(PuBuGn-4-4);
},
colormap={PuBuGn-5}{
  color=(PuBuGn-5-1);
  color=(PuBuGn-5-2);
  color=(PuBuGn-5-3);
  color=(PuBuGn-5-4);
  color=(PuBuGn-5-5);
},
colormap={PuBuGn-6}{
  color=(PuBuGn-6-1);
  color=(PuBuGn-6-2);
  color=(PuBuGn-6-3);
  color=(PuBuGn-6-4);
  color=(PuBuGn-6-5);
  color=(PuBuGn-6-6);
},
colormap={PuBuGn-7}{
  color=(PuBuGn-7-1);
  color=(PuBuGn-7-2);
  color=(PuBuGn-7-3);
  color=(PuBuGn-7-4);
  color=(PuBuGn-7-5);
  color=(PuBuGn-7-6);
  color=(PuBuGn-7-7);
},
colormap={PuBuGn-8}{
  color=(PuBuGn-8-1);
  color=(PuBuGn-8-2);
  color=(PuBuGn-8-3);
  color=(PuBuGn-8-4);
  color=(PuBuGn-8-5);
  color=(PuBuGn-8-6);
  color=(PuBuGn-8-7);
  color=(PuBuGn-8-8);
},
colormap={PuBuGn-9}{
  color=(PuBuGn-9-1);
  color=(PuBuGn-9-2);
  color=(PuBuGn-9-3);
  color=(PuBuGn-9-4);
  color=(PuBuGn-9-5);
  color=(PuBuGn-9-6);
  color=(PuBuGn-9-7);
  color=(PuBuGn-9-8);
  color=(PuBuGn-9-9);
},
colormap={PuBu-3}{
  color=(PuBu-3-1);
  color=(PuBu-3-2);
  color=(PuBu-3-3);
},
colormap={PuBu-4}{
  color=(PuBu-4-1);
  color=(PuBu-4-2);
  color=(PuBu-4-3);
  color=(PuBu-4-4);
},
colormap={PuBu-5}{
  color=(PuBu-5-1);
  color=(PuBu-5-2);
  color=(PuBu-5-3);
  color=(PuBu-5-4);
  color=(PuBu-5-5);
},
colormap={PuBu-6}{
  color=(PuBu-6-1);
  color=(PuBu-6-2);
  color=(PuBu-6-3);
  color=(PuBu-6-4);
  color=(PuBu-6-5);
  color=(PuBu-6-6);
},
colormap={PuBu-7}{
  color=(PuBu-7-1);
  color=(PuBu-7-2);
  color=(PuBu-7-3);
  color=(PuBu-7-4);
  color=(PuBu-7-5);
  color=(PuBu-7-6);
  color=(PuBu-7-7);
},
colormap={PuBu-8}{
  color=(PuBu-8-1);
  color=(PuBu-8-2);
  color=(PuBu-8-3);
  color=(PuBu-8-4);
  color=(PuBu-8-5);
  color=(PuBu-8-6);
  color=(PuBu-8-7);
  color=(PuBu-8-8);
},
colormap={PuBu-9}{
  color=(PuBu-9-1);
  color=(PuBu-9-2);
  color=(PuBu-9-3);
  color=(PuBu-9-4);
  color=(PuBu-9-5);
  color=(PuBu-9-6);
  color=(PuBu-9-7);
  color=(PuBu-9-8);
  color=(PuBu-9-9);
},
colormap={BuPu-3}{
  color=(BuPu-3-1);
  color=(BuPu-3-2);
  color=(BuPu-3-3);
},
colormap={BuPu-4}{
  color=(BuPu-4-1);
  color=(BuPu-4-2);
  color=(BuPu-4-3);
  color=(BuPu-4-4);
},
colormap={BuPu-5}{
  color=(BuPu-5-1);
  color=(BuPu-5-2);
  color=(BuPu-5-3);
  color=(BuPu-5-4);
  color=(BuPu-5-5);
},
colormap={BuPu-6}{
  color=(BuPu-6-1);
  color=(BuPu-6-2);
  color=(BuPu-6-3);
  color=(BuPu-6-4);
  color=(BuPu-6-5);
  color=(BuPu-6-6);
},
colormap={BuPu-7}{
  color=(BuPu-7-1);
  color=(BuPu-7-2);
  color=(BuPu-7-3);
  color=(BuPu-7-4);
  color=(BuPu-7-5);
  color=(BuPu-7-6);
  color=(BuPu-7-7);
},
colormap={BuPu-8}{
  color=(BuPu-8-1);
  color=(BuPu-8-2);
  color=(BuPu-8-3);
  color=(BuPu-8-4);
  color=(BuPu-8-5);
  color=(BuPu-8-6);
  color=(BuPu-8-7);
  color=(BuPu-8-8);
},
colormap={BuPu-9}{
  color=(BuPu-9-1);
  color=(BuPu-9-2);
  color=(BuPu-9-3);
  color=(BuPu-9-4);
  color=(BuPu-9-5);
  color=(BuPu-9-6);
  color=(BuPu-9-7);
  color=(BuPu-9-8);
  color=(BuPu-9-9);
},
colormap={RdPu-3}{
  color=(RdPu-3-1);
  color=(RdPu-3-2);
  color=(RdPu-3-3);
},
colormap={RdPu-4}{
  color=(RdPu-4-1);
  color=(RdPu-4-2);
  color=(RdPu-4-3);
  color=(RdPu-4-4);
},
colormap={RdPu-5}{
  color=(RdPu-5-1);
  color=(RdPu-5-2);
  color=(RdPu-5-3);
  color=(RdPu-5-4);
  color=(RdPu-5-5);
},
colormap={RdPu-6}{
  color=(RdPu-6-1);
  color=(RdPu-6-2);
  color=(RdPu-6-3);
  color=(RdPu-6-4);
  color=(RdPu-6-5);
  color=(RdPu-6-6);
},
colormap={RdPu-7}{
  color=(RdPu-7-1);
  color=(RdPu-7-2);
  color=(RdPu-7-3);
  color=(RdPu-7-4);
  color=(RdPu-7-5);
  color=(RdPu-7-6);
  color=(RdPu-7-7);
},
colormap={RdPu-8}{
  color=(RdPu-8-1);
  color=(RdPu-8-2);
  color=(RdPu-8-3);
  color=(RdPu-8-4);
  color=(RdPu-8-5);
  color=(RdPu-8-6);
  color=(RdPu-8-7);
  color=(RdPu-8-8);
},
colormap={RdPu-9}{
  color=(RdPu-9-1);
  color=(RdPu-9-2);
  color=(RdPu-9-3);
  color=(RdPu-9-4);
  color=(RdPu-9-5);
  color=(RdPu-9-6);
  color=(RdPu-9-7);
  color=(RdPu-9-8);
  color=(RdPu-9-9);
},
colormap={PuRd-3}{
  color=(PuRd-3-1);
  color=(PuRd-3-2);
  color=(PuRd-3-3);
},
colormap={PuRd-4}{
  color=(PuRd-4-1);
  color=(PuRd-4-2);
  color=(PuRd-4-3);
  color=(PuRd-4-4);
},
colormap={PuRd-5}{
  color=(PuRd-5-1);
  color=(PuRd-5-2);
  color=(PuRd-5-3);
  color=(PuRd-5-4);
  color=(PuRd-5-5);
},
colormap={PuRd-6}{
  color=(PuRd-6-1);
  color=(PuRd-6-2);
  color=(PuRd-6-3);
  color=(PuRd-6-4);
  color=(PuRd-6-5);
  color=(PuRd-6-6);
},
colormap={PuRd-7}{
  color=(PuRd-7-1);
  color=(PuRd-7-2);
  color=(PuRd-7-3);
  color=(PuRd-7-4);
  color=(PuRd-7-5);
  color=(PuRd-7-6);
  color=(PuRd-7-7);
},
colormap={PuRd-8}{
  color=(PuRd-8-1);
  color=(PuRd-8-2);
  color=(PuRd-8-3);
  color=(PuRd-8-4);
  color=(PuRd-8-5);
  color=(PuRd-8-6);
  color=(PuRd-8-7);
  color=(PuRd-8-8);
},
colormap={PuRd-9}{
  color=(PuRd-9-1);
  color=(PuRd-9-2);
  color=(PuRd-9-3);
  color=(PuRd-9-4);
  color=(PuRd-9-5);
  color=(PuRd-9-6);
  color=(PuRd-9-7);
  color=(PuRd-9-8);
  color=(PuRd-9-9);
},
colormap={OrRd-3}{
  color=(OrRd-3-1);
  color=(OrRd-3-2);
  color=(OrRd-3-3);
},
colormap={OrRd-4}{
  color=(OrRd-4-1);
  color=(OrRd-4-2);
  color=(OrRd-4-3);
  color=(OrRd-4-4);
},
colormap={OrRd-5}{
  color=(OrRd-5-1);
  color=(OrRd-5-2);
  color=(OrRd-5-3);
  color=(OrRd-5-4);
  color=(OrRd-5-5);
},
colormap={OrRd-6}{
  color=(OrRd-6-1);
  color=(OrRd-6-2);
  color=(OrRd-6-3);
  color=(OrRd-6-4);
  color=(OrRd-6-5);
  color=(OrRd-6-6);
},
colormap={OrRd-7}{
  color=(OrRd-7-1);
  color=(OrRd-7-2);
  color=(OrRd-7-3);
  color=(OrRd-7-4);
  color=(OrRd-7-5);
  color=(OrRd-7-6);
  color=(OrRd-7-7);
},
colormap={OrRd-8}{
  color=(OrRd-8-1);
  color=(OrRd-8-2);
  color=(OrRd-8-3);
  color=(OrRd-8-4);
  color=(OrRd-8-5);
  color=(OrRd-8-6);
  color=(OrRd-8-7);
  color=(OrRd-8-8);
},
colormap={OrRd-9}{
  color=(OrRd-9-1);
  color=(OrRd-9-2);
  color=(OrRd-9-3);
  color=(OrRd-9-4);
  color=(OrRd-9-5);
  color=(OrRd-9-6);
  color=(OrRd-9-7);
  color=(OrRd-9-8);
  color=(OrRd-9-9);
},
colormap={YlOrRd-3}{
  color=(YlOrRd-3-1);
  color=(YlOrRd-3-2);
  color=(YlOrRd-3-3);
},
colormap={YlOrRd-4}{
  color=(YlOrRd-4-1);
  color=(YlOrRd-4-2);
  color=(YlOrRd-4-3);
  color=(YlOrRd-4-4);
},
colormap={YlOrRd-5}{
  color=(YlOrRd-5-1);
  color=(YlOrRd-5-2);
  color=(YlOrRd-5-3);
  color=(YlOrRd-5-4);
  color=(YlOrRd-5-5);
},
colormap={YlOrRd-6}{
  color=(YlOrRd-6-1);
  color=(YlOrRd-6-2);
  color=(YlOrRd-6-3);
  color=(YlOrRd-6-4);
  color=(YlOrRd-6-5);
  color=(YlOrRd-6-6);
},
colormap={YlOrRd-7}{
  color=(YlOrRd-7-1);
  color=(YlOrRd-7-2);
  color=(YlOrRd-7-3);
  color=(YlOrRd-7-4);
  color=(YlOrRd-7-5);
  color=(YlOrRd-7-6);
  color=(YlOrRd-7-7);
},
colormap={YlOrRd-8}{
  color=(YlOrRd-8-1);
  color=(YlOrRd-8-2);
  color=(YlOrRd-8-3);
  color=(YlOrRd-8-4);
  color=(YlOrRd-8-5);
  color=(YlOrRd-8-6);
  color=(YlOrRd-8-7);
  color=(YlOrRd-8-8);
},
colormap={YlOrRd-9}{
  color=(YlOrRd-9-1);
  color=(YlOrRd-9-2);
  color=(YlOrRd-9-3);
  color=(YlOrRd-9-4);
  color=(YlOrRd-9-5);
  color=(YlOrRd-9-6);
  color=(YlOrRd-9-7);
  color=(YlOrRd-9-8);
  color=(YlOrRd-9-9);
},
colormap={YlOrBr-3}{
  color=(YlOrBr-3-1);
  color=(YlOrBr-3-2);
  color=(YlOrBr-3-3);
},
colormap={YlOrBr-4}{
  color=(YlOrBr-4-1);
  color=(YlOrBr-4-2);
  color=(YlOrBr-4-3);
  color=(YlOrBr-4-4);
},
colormap={YlOrBr-5}{
  color=(YlOrBr-5-1);
  color=(YlOrBr-5-2);
  color=(YlOrBr-5-3);
  color=(YlOrBr-5-4);
  color=(YlOrBr-5-5);
},
colormap={YlOrBr-6}{
  color=(YlOrBr-6-1);
  color=(YlOrBr-6-2);
  color=(YlOrBr-6-3);
  color=(YlOrBr-6-4);
  color=(YlOrBr-6-5);
  color=(YlOrBr-6-6);
},
colormap={YlOrBr-7}{
  color=(YlOrBr-7-1);
  color=(YlOrBr-7-2);
  color=(YlOrBr-7-3);
  color=(YlOrBr-7-4);
  color=(YlOrBr-7-5);
  color=(YlOrBr-7-6);
  color=(YlOrBr-7-7);
},
colormap={YlOrBr-8}{
  color=(YlOrBr-8-1);
  color=(YlOrBr-8-2);
  color=(YlOrBr-8-3);
  color=(YlOrBr-8-4);
  color=(YlOrBr-8-5);
  color=(YlOrBr-8-6);
  color=(YlOrBr-8-7);
  color=(YlOrBr-8-8);
},
colormap={YlOrBr-9}{
  color=(YlOrBr-9-1);
  color=(YlOrBr-9-2);
  color=(YlOrBr-9-3);
  color=(YlOrBr-9-4);
  color=(YlOrBr-9-5);
  color=(YlOrBr-9-6);
  color=(YlOrBr-9-7);
  color=(YlOrBr-9-8);
  color=(YlOrBr-9-9);
},
colormap={Purples-3}{
  color=(Purples-3-1);
  color=(Purples-3-2);
  color=(Purples-3-3);
},
colormap={Purples-4}{
  color=(Purples-4-1);
  color=(Purples-4-2);
  color=(Purples-4-3);
  color=(Purples-4-4);
},
colormap={Purples-5}{
  color=(Purples-5-1);
  color=(Purples-5-2);
  color=(Purples-5-3);
  color=(Purples-5-4);
  color=(Purples-5-5);
},
colormap={Purples-6}{
  color=(Purples-6-1);
  color=(Purples-6-2);
  color=(Purples-6-3);
  color=(Purples-6-4);
  color=(Purples-6-5);
  color=(Purples-6-6);
},
colormap={Purples-7}{
  color=(Purples-7-1);
  color=(Purples-7-2);
  color=(Purples-7-3);
  color=(Purples-7-4);
  color=(Purples-7-5);
  color=(Purples-7-6);
  color=(Purples-7-7);
},
colormap={Purples-8}{
  color=(Purples-8-1);
  color=(Purples-8-2);
  color=(Purples-8-3);
  color=(Purples-8-4);
  color=(Purples-8-5);
  color=(Purples-8-6);
  color=(Purples-8-7);
  color=(Purples-8-8);
},
colormap={Purples-9}{
  color=(Purples-9-1);
  color=(Purples-9-2);
  color=(Purples-9-3);
  color=(Purples-9-4);
  color=(Purples-9-5);
  color=(Purples-9-6);
  color=(Purples-9-7);
  color=(Purples-9-8);
  color=(Purples-9-9);
},
colormap={Blues-3}{
  color=(Blues-3-1);
  color=(Blues-3-2);
  color=(Blues-3-3);
},
colormap={Blues-4}{
  color=(Blues-4-1);
  color=(Blues-4-2);
  color=(Blues-4-3);
  color=(Blues-4-4);
},
colormap={Blues-5}{
  color=(Blues-5-1);
  color=(Blues-5-2);
  color=(Blues-5-3);
  color=(Blues-5-4);
  color=(Blues-5-5);
},
colormap={Blues-6}{
  color=(Blues-6-1);
  color=(Blues-6-2);
  color=(Blues-6-3);
  color=(Blues-6-4);
  color=(Blues-6-5);
  color=(Blues-6-6);
},
colormap={Blues-7}{
  color=(Blues-7-1);
  color=(Blues-7-2);
  color=(Blues-7-3);
  color=(Blues-7-4);
  color=(Blues-7-5);
  color=(Blues-7-6);
  color=(Blues-7-7);
},
colormap={Blues-8}{
  color=(Blues-8-1);
  color=(Blues-8-2);
  color=(Blues-8-3);
  color=(Blues-8-4);
  color=(Blues-8-5);
  color=(Blues-8-6);
  color=(Blues-8-7);
  color=(Blues-8-8);
},
colormap={Blues-9}{
  color=(Blues-9-1);
  color=(Blues-9-2);
  color=(Blues-9-3);
  color=(Blues-9-4);
  color=(Blues-9-5);
  color=(Blues-9-6);
  color=(Blues-9-7);
  color=(Blues-9-8);
  color=(Blues-9-9);
},
colormap={Greens-3}{
  color=(Greens-3-1);
  color=(Greens-3-2);
  color=(Greens-3-3);
},
colormap={Greens-4}{
  color=(Greens-4-1);
  color=(Greens-4-2);
  color=(Greens-4-3);
  color=(Greens-4-4);
},
colormap={Greens-5}{
  color=(Greens-5-1);
  color=(Greens-5-2);
  color=(Greens-5-3);
  color=(Greens-5-4);
  color=(Greens-5-5);
},
colormap={Greens-6}{
  color=(Greens-6-1);
  color=(Greens-6-2);
  color=(Greens-6-3);
  color=(Greens-6-4);
  color=(Greens-6-5);
  color=(Greens-6-6);
},
colormap={Greens-7}{
  color=(Greens-7-1);
  color=(Greens-7-2);
  color=(Greens-7-3);
  color=(Greens-7-4);
  color=(Greens-7-5);
  color=(Greens-7-6);
  color=(Greens-7-7);
},
colormap={Greens-8}{
  color=(Greens-8-1);
  color=(Greens-8-2);
  color=(Greens-8-3);
  color=(Greens-8-4);
  color=(Greens-8-5);
  color=(Greens-8-6);
  color=(Greens-8-7);
  color=(Greens-8-8);
},
colormap={Greens-9}{
  color=(Greens-9-1);
  color=(Greens-9-2);
  color=(Greens-9-3);
  color=(Greens-9-4);
  color=(Greens-9-5);
  color=(Greens-9-6);
  color=(Greens-9-7);
  color=(Greens-9-8);
  color=(Greens-9-9);
},
colormap={Oranges-3}{
  color=(Oranges-3-1);
  color=(Oranges-3-2);
  color=(Oranges-3-3);
},
colormap={Oranges-4}{
  color=(Oranges-4-1);
  color=(Oranges-4-2);
  color=(Oranges-4-3);
  color=(Oranges-4-4);
},
colormap={Oranges-5}{
  color=(Oranges-5-1);
  color=(Oranges-5-2);
  color=(Oranges-5-3);
  color=(Oranges-5-4);
  color=(Oranges-5-5);
},
colormap={Oranges-6}{
  color=(Oranges-6-1);
  color=(Oranges-6-2);
  color=(Oranges-6-3);
  color=(Oranges-6-4);
  color=(Oranges-6-5);
  color=(Oranges-6-6);
},
colormap={Oranges-7}{
  color=(Oranges-7-1);
  color=(Oranges-7-2);
  color=(Oranges-7-3);
  color=(Oranges-7-4);
  color=(Oranges-7-5);
  color=(Oranges-7-6);
  color=(Oranges-7-7);
},
colormap={Oranges-8}{
  color=(Oranges-8-1);
  color=(Oranges-8-2);
  color=(Oranges-8-3);
  color=(Oranges-8-4);
  color=(Oranges-8-5);
  color=(Oranges-8-6);
  color=(Oranges-8-7);
  color=(Oranges-8-8);
},
colormap={Oranges-9}{
  color=(Oranges-9-1);
  color=(Oranges-9-2);
  color=(Oranges-9-3);
  color=(Oranges-9-4);
  color=(Oranges-9-5);
  color=(Oranges-9-6);
  color=(Oranges-9-7);
  color=(Oranges-9-8);
  color=(Oranges-9-9);
},
colormap={Reds-3}{
  color=(Reds-3-1);
  color=(Reds-3-2);
  color=(Reds-3-3);
},
colormap={Reds-4}{
  color=(Reds-4-1);
  color=(Reds-4-2);
  color=(Reds-4-3);
  color=(Reds-4-4);
},
colormap={Reds-5}{
  color=(Reds-5-1);
  color=(Reds-5-2);
  color=(Reds-5-3);
  color=(Reds-5-4);
  color=(Reds-5-5);
},
colormap={Reds-6}{
  color=(Reds-6-1);
  color=(Reds-6-2);
  color=(Reds-6-3);
  color=(Reds-6-4);
  color=(Reds-6-5);
  color=(Reds-6-6);
},
colormap={Reds-7}{
  color=(Reds-7-1);
  color=(Reds-7-2);
  color=(Reds-7-3);
  color=(Reds-7-4);
  color=(Reds-7-5);
  color=(Reds-7-6);
  color=(Reds-7-7);
},
colormap={Reds-8}{
  color=(Reds-8-1);
  color=(Reds-8-2);
  color=(Reds-8-3);
  color=(Reds-8-4);
  color=(Reds-8-5);
  color=(Reds-8-6);
  color=(Reds-8-7);
  color=(Reds-8-8);
},
colormap={Reds-9}{
  color=(Reds-9-1);
  color=(Reds-9-2);
  color=(Reds-9-3);
  color=(Reds-9-4);
  color=(Reds-9-5);
  color=(Reds-9-6);
  color=(Reds-9-7);
  color=(Reds-9-8);
  color=(Reds-9-9);
},
colormap={Greys-3}{
  color=(Greys-3-1);
  color=(Greys-3-2);
  color=(Greys-3-3);
},
colormap={Greys-4}{
  color=(Greys-4-1);
  color=(Greys-4-2);
  color=(Greys-4-3);
  color=(Greys-4-4);
},
colormap={Greys-5}{
  color=(Greys-5-1);
  color=(Greys-5-2);
  color=(Greys-5-3);
  color=(Greys-5-4);
  color=(Greys-5-5);
},
colormap={Greys-6}{
  color=(Greys-6-1);
  color=(Greys-6-2);
  color=(Greys-6-3);
  color=(Greys-6-4);
  color=(Greys-6-5);
  color=(Greys-6-6);
},
colormap={Greys-7}{
  color=(Greys-7-1);
  color=(Greys-7-2);
  color=(Greys-7-3);
  color=(Greys-7-4);
  color=(Greys-7-5);
  color=(Greys-7-6);
  color=(Greys-7-7);
},
colormap={Greys-8}{
  color=(Greys-8-1);
  color=(Greys-8-2);
  color=(Greys-8-3);
  color=(Greys-8-4);
  color=(Greys-8-5);
  color=(Greys-8-6);
  color=(Greys-8-7);
  color=(Greys-8-8);
},
colormap={Greys-9}{
  color=(Greys-9-1);
  color=(Greys-9-2);
  color=(Greys-9-3);
  color=(Greys-9-4);
  color=(Greys-9-5);
  color=(Greys-9-6);
  color=(Greys-9-7);
  color=(Greys-9-8);
  color=(Greys-9-9);
},
colormap={PuOr-3}{
  color=(PuOr-3-1);
  color=(PuOr-3-2);
  color=(PuOr-3-3);
},
colormap={PuOr-4}{
  color=(PuOr-4-1);
  color=(PuOr-4-2);
  color=(PuOr-4-3);
  color=(PuOr-4-4);
},
colormap={PuOr-5}{
  color=(PuOr-5-1);
  color=(PuOr-5-2);
  color=(PuOr-5-3);
  color=(PuOr-5-4);
  color=(PuOr-5-5);
},
colormap={PuOr-6}{
  color=(PuOr-6-1);
  color=(PuOr-6-2);
  color=(PuOr-6-3);
  color=(PuOr-6-4);
  color=(PuOr-6-5);
  color=(PuOr-6-6);
},
colormap={PuOr-7}{
  color=(PuOr-7-1);
  color=(PuOr-7-2);
  color=(PuOr-7-3);
  color=(PuOr-7-4);
  color=(PuOr-7-5);
  color=(PuOr-7-6);
  color=(PuOr-7-7);
},
colormap={PuOr-8}{
  color=(PuOr-8-1);
  color=(PuOr-8-2);
  color=(PuOr-8-3);
  color=(PuOr-8-4);
  color=(PuOr-8-5);
  color=(PuOr-8-6);
  color=(PuOr-8-7);
  color=(PuOr-8-8);
},
colormap={PuOr-9}{
  color=(PuOr-9-1);
  color=(PuOr-9-2);
  color=(PuOr-9-3);
  color=(PuOr-9-4);
  color=(PuOr-9-5);
  color=(PuOr-9-6);
  color=(PuOr-9-7);
  color=(PuOr-9-8);
  color=(PuOr-9-9);
},
colormap={PuOr-10}{
  color=(PuOr-10-1);
  color=(PuOr-10-2);
  color=(PuOr-10-3);
  color=(PuOr-10-4);
  color=(PuOr-10-5);
  color=(PuOr-10-6);
  color=(PuOr-10-7);
  color=(PuOr-10-8);
  color=(PuOr-10-9);
  color=(PuOr-10-10);
},
colormap={PuOr-11}{
  color=(PuOr-11-1);
  color=(PuOr-11-2);
  color=(PuOr-11-3);
  color=(PuOr-11-4);
  color=(PuOr-11-5);
  color=(PuOr-11-6);
  color=(PuOr-11-7);
  color=(PuOr-11-8);
  color=(PuOr-11-9);
  color=(PuOr-11-10);
  color=(PuOr-11-11);
},
colormap={BrBG-3}{
  color=(BrBG-3-1);
  color=(BrBG-3-2);
  color=(BrBG-3-3);
},
colormap={BrBG-4}{
  color=(BrBG-4-1);
  color=(BrBG-4-2);
  color=(BrBG-4-3);
  color=(BrBG-4-4);
},
colormap={BrBG-5}{
  color=(BrBG-5-1);
  color=(BrBG-5-2);
  color=(BrBG-5-3);
  color=(BrBG-5-4);
  color=(BrBG-5-5);
},
colormap={BrBG-6}{
  color=(BrBG-6-1);
  color=(BrBG-6-2);
  color=(BrBG-6-3);
  color=(BrBG-6-4);
  color=(BrBG-6-5);
  color=(BrBG-6-6);
},
colormap={BrBG-7}{
  color=(BrBG-7-1);
  color=(BrBG-7-2);
  color=(BrBG-7-3);
  color=(BrBG-7-4);
  color=(BrBG-7-5);
  color=(BrBG-7-6);
  color=(BrBG-7-7);
},
colormap={BrBG-8}{
  color=(BrBG-8-1);
  color=(BrBG-8-2);
  color=(BrBG-8-3);
  color=(BrBG-8-4);
  color=(BrBG-8-5);
  color=(BrBG-8-6);
  color=(BrBG-8-7);
  color=(BrBG-8-8);
},
colormap={BrBG-9}{
  color=(BrBG-9-1);
  color=(BrBG-9-2);
  color=(BrBG-9-3);
  color=(BrBG-9-4);
  color=(BrBG-9-5);
  color=(BrBG-9-6);
  color=(BrBG-9-7);
  color=(BrBG-9-8);
  color=(BrBG-9-9);
},
colormap={BrBG-10}{
  color=(BrBG-10-1);
  color=(BrBG-10-2);
  color=(BrBG-10-3);
  color=(BrBG-10-4);
  color=(BrBG-10-5);
  color=(BrBG-10-6);
  color=(BrBG-10-7);
  color=(BrBG-10-8);
  color=(BrBG-10-9);
  color=(BrBG-10-10);
},
colormap={BrBG-11}{
  color=(BrBG-11-1);
  color=(BrBG-11-2);
  color=(BrBG-11-3);
  color=(BrBG-11-4);
  color=(BrBG-11-5);
  color=(BrBG-11-6);
  color=(BrBG-11-7);
  color=(BrBG-11-8);
  color=(BrBG-11-9);
  color=(BrBG-11-10);
  color=(BrBG-11-11);
},
colormap={PRGn-3}{
  color=(PRGn-3-1);
  color=(PRGn-3-2);
  color=(PRGn-3-3);
},
colormap={PRGn-4}{
  color=(PRGn-4-1);
  color=(PRGn-4-2);
  color=(PRGn-4-3);
  color=(PRGn-4-4);
},
colormap={PRGn-5}{
  color=(PRGn-5-1);
  color=(PRGn-5-2);
  color=(PRGn-5-3);
  color=(PRGn-5-4);
  color=(PRGn-5-5);
},
colormap={PRGn-6}{
  color=(PRGn-6-1);
  color=(PRGn-6-2);
  color=(PRGn-6-3);
  color=(PRGn-6-4);
  color=(PRGn-6-5);
  color=(PRGn-6-6);
},
colormap={PRGn-7}{
  color=(PRGn-7-1);
  color=(PRGn-7-2);
  color=(PRGn-7-3);
  color=(PRGn-7-4);
  color=(PRGn-7-5);
  color=(PRGn-7-6);
  color=(PRGn-7-7);
},
colormap={PRGn-8}{
  color=(PRGn-8-1);
  color=(PRGn-8-2);
  color=(PRGn-8-3);
  color=(PRGn-8-4);
  color=(PRGn-8-5);
  color=(PRGn-8-6);
  color=(PRGn-8-7);
  color=(PRGn-8-8);
},
colormap={PRGn-9}{
  color=(PRGn-9-1);
  color=(PRGn-9-2);
  color=(PRGn-9-3);
  color=(PRGn-9-4);
  color=(PRGn-9-5);
  color=(PRGn-9-6);
  color=(PRGn-9-7);
  color=(PRGn-9-8);
  color=(PRGn-9-9);
},
colormap={PRGn-10}{
  color=(PRGn-10-1);
  color=(PRGn-10-2);
  color=(PRGn-10-3);
  color=(PRGn-10-4);
  color=(PRGn-10-5);
  color=(PRGn-10-6);
  color=(PRGn-10-7);
  color=(PRGn-10-8);
  color=(PRGn-10-9);
  color=(PRGn-10-10);
},
colormap={PRGn-11}{
  color=(PRGn-11-1);
  color=(PRGn-11-2);
  color=(PRGn-11-3);
  color=(PRGn-11-4);
  color=(PRGn-11-5);
  color=(PRGn-11-6);
  color=(PRGn-11-7);
  color=(PRGn-11-8);
  color=(PRGn-11-9);
  color=(PRGn-11-10);
  color=(PRGn-11-11);
},
colormap={PiYG-3}{
  color=(PiYG-3-1);
  color=(PiYG-3-2);
  color=(PiYG-3-3);
},
colormap={PiYG-4}{
  color=(PiYG-4-1);
  color=(PiYG-4-2);
  color=(PiYG-4-3);
  color=(PiYG-4-4);
},
colormap={PiYG-5}{
  color=(PiYG-5-1);
  color=(PiYG-5-2);
  color=(PiYG-5-3);
  color=(PiYG-5-4);
  color=(PiYG-5-5);
},
colormap={PiYG-6}{
  color=(PiYG-6-1);
  color=(PiYG-6-2);
  color=(PiYG-6-3);
  color=(PiYG-6-4);
  color=(PiYG-6-5);
  color=(PiYG-6-6);
},
colormap={PiYG-7}{
  color=(PiYG-7-1);
  color=(PiYG-7-2);
  color=(PiYG-7-3);
  color=(PiYG-7-4);
  color=(PiYG-7-5);
  color=(PiYG-7-6);
  color=(PiYG-7-7);
},
colormap={PiYG-8}{
  color=(PiYG-8-1);
  color=(PiYG-8-2);
  color=(PiYG-8-3);
  color=(PiYG-8-4);
  color=(PiYG-8-5);
  color=(PiYG-8-6);
  color=(PiYG-8-7);
  color=(PiYG-8-8);
},
colormap={PiYG-9}{
  color=(PiYG-9-1);
  color=(PiYG-9-2);
  color=(PiYG-9-3);
  color=(PiYG-9-4);
  color=(PiYG-9-5);
  color=(PiYG-9-6);
  color=(PiYG-9-7);
  color=(PiYG-9-8);
  color=(PiYG-9-9);
},
colormap={PiYG-10}{
  color=(PiYG-10-1);
  color=(PiYG-10-2);
  color=(PiYG-10-3);
  color=(PiYG-10-4);
  color=(PiYG-10-5);
  color=(PiYG-10-6);
  color=(PiYG-10-7);
  color=(PiYG-10-8);
  color=(PiYG-10-9);
  color=(PiYG-10-10);
},
colormap={PiYG-11}{
  color=(PiYG-11-1);
  color=(PiYG-11-2);
  color=(PiYG-11-3);
  color=(PiYG-11-4);
  color=(PiYG-11-5);
  color=(PiYG-11-6);
  color=(PiYG-11-7);
  color=(PiYG-11-8);
  color=(PiYG-11-9);
  color=(PiYG-11-10);
  color=(PiYG-11-11);
},
colormap={RdBu-3}{
  color=(RdBu-3-1);
  color=(RdBu-3-2);
  color=(RdBu-3-3);
},
colormap={RdBu-4}{
  color=(RdBu-4-1);
  color=(RdBu-4-2);
  color=(RdBu-4-3);
  color=(RdBu-4-4);
},
colormap={RdBu-5}{
  color=(RdBu-5-1);
  color=(RdBu-5-2);
  color=(RdBu-5-3);
  color=(RdBu-5-4);
  color=(RdBu-5-5);
},
colormap={RdBu-6}{
  color=(RdBu-6-1);
  color=(RdBu-6-2);
  color=(RdBu-6-3);
  color=(RdBu-6-4);
  color=(RdBu-6-5);
  color=(RdBu-6-6);
},
colormap={RdBu-7}{
  color=(RdBu-7-1);
  color=(RdBu-7-2);
  color=(RdBu-7-3);
  color=(RdBu-7-4);
  color=(RdBu-7-5);
  color=(RdBu-7-6);
  color=(RdBu-7-7);
},
colormap={RdBu-8}{
  color=(RdBu-8-1);
  color=(RdBu-8-2);
  color=(RdBu-8-3);
  color=(RdBu-8-4);
  color=(RdBu-8-5);
  color=(RdBu-8-6);
  color=(RdBu-8-7);
  color=(RdBu-8-8);
},
colormap={RdBu-9}{
  color=(RdBu-9-1);
  color=(RdBu-9-2);
  color=(RdBu-9-3);
  color=(RdBu-9-4);
  color=(RdBu-9-5);
  color=(RdBu-9-6);
  color=(RdBu-9-7);
  color=(RdBu-9-8);
  color=(RdBu-9-9);
},
colormap={RdBu-10}{
  color=(RdBu-10-1);
  color=(RdBu-10-2);
  color=(RdBu-10-3);
  color=(RdBu-10-4);
  color=(RdBu-10-5);
  color=(RdBu-10-6);
  color=(RdBu-10-7);
  color=(RdBu-10-8);
  color=(RdBu-10-9);
  color=(RdBu-10-10);
},
colormap={RdBu-11}{
  color=(RdBu-11-1);
  color=(RdBu-11-2);
  color=(RdBu-11-3);
  color=(RdBu-11-4);
  color=(RdBu-11-5);
  color=(RdBu-11-6);
  color=(RdBu-11-7);
  color=(RdBu-11-8);
  color=(RdBu-11-9);
  color=(RdBu-11-10);
  color=(RdBu-11-11);
},
colormap={RdGy-3}{
  color=(RdGy-3-1);
  color=(RdGy-3-2);
  color=(RdGy-3-3);
},
colormap={RdGy-4}{
  color=(RdGy-4-1);
  color=(RdGy-4-2);
  color=(RdGy-4-3);
  color=(RdGy-4-4);
},
colormap={RdGy-5}{
  color=(RdGy-5-1);
  color=(RdGy-5-2);
  color=(RdGy-5-3);
  color=(RdGy-5-4);
  color=(RdGy-5-5);
},
colormap={RdGy-6}{
  color=(RdGy-6-1);
  color=(RdGy-6-2);
  color=(RdGy-6-3);
  color=(RdGy-6-4);
  color=(RdGy-6-5);
  color=(RdGy-6-6);
},
colormap={RdGy-7}{
  color=(RdGy-7-1);
  color=(RdGy-7-2);
  color=(RdGy-7-3);
  color=(RdGy-7-4);
  color=(RdGy-7-5);
  color=(RdGy-7-6);
  color=(RdGy-7-7);
},
colormap={RdGy-8}{
  color=(RdGy-8-1);
  color=(RdGy-8-2);
  color=(RdGy-8-3);
  color=(RdGy-8-4);
  color=(RdGy-8-5);
  color=(RdGy-8-6);
  color=(RdGy-8-7);
  color=(RdGy-8-8);
},
colormap={RdGy-9}{
  color=(RdGy-9-1);
  color=(RdGy-9-2);
  color=(RdGy-9-3);
  color=(RdGy-9-4);
  color=(RdGy-9-5);
  color=(RdGy-9-6);
  color=(RdGy-9-7);
  color=(RdGy-9-8);
  color=(RdGy-9-9);
},
colormap={RdGy-10}{
  color=(RdGy-10-1);
  color=(RdGy-10-2);
  color=(RdGy-10-3);
  color=(RdGy-10-4);
  color=(RdGy-10-5);
  color=(RdGy-10-6);
  color=(RdGy-10-7);
  color=(RdGy-10-8);
  color=(RdGy-10-9);
  color=(RdGy-10-10);
},
colormap={RdGy-11}{
  color=(RdGy-11-1);
  color=(RdGy-11-2);
  color=(RdGy-11-3);
  color=(RdGy-11-4);
  color=(RdGy-11-5);
  color=(RdGy-11-6);
  color=(RdGy-11-7);
  color=(RdGy-11-8);
  color=(RdGy-11-9);
  color=(RdGy-11-10);
  color=(RdGy-11-11);
},
colormap={RdYlBu-3}{
  color=(RdYlBu-3-1);
  color=(RdYlBu-3-2);
  color=(RdYlBu-3-3);
},
colormap={RdYlBu-4}{
  color=(RdYlBu-4-1);
  color=(RdYlBu-4-2);
  color=(RdYlBu-4-3);
  color=(RdYlBu-4-4);
},
colormap={RdYlBu-5}{
  color=(RdYlBu-5-1);
  color=(RdYlBu-5-2);
  color=(RdYlBu-5-3);
  color=(RdYlBu-5-4);
  color=(RdYlBu-5-5);
},
colormap={RdYlBu-6}{
  color=(RdYlBu-6-1);
  color=(RdYlBu-6-2);
  color=(RdYlBu-6-3);
  color=(RdYlBu-6-4);
  color=(RdYlBu-6-5);
  color=(RdYlBu-6-6);
},
colormap={RdYlBu-7}{
  color=(RdYlBu-7-1);
  color=(RdYlBu-7-2);
  color=(RdYlBu-7-3);
  color=(RdYlBu-7-4);
  color=(RdYlBu-7-5);
  color=(RdYlBu-7-6);
  color=(RdYlBu-7-7);
},
colormap={RdYlBu-8}{
  color=(RdYlBu-8-1);
  color=(RdYlBu-8-2);
  color=(RdYlBu-8-3);
  color=(RdYlBu-8-4);
  color=(RdYlBu-8-5);
  color=(RdYlBu-8-6);
  color=(RdYlBu-8-7);
  color=(RdYlBu-8-8);
},
colormap={RdYlBu-9}{
  color=(RdYlBu-9-1);
  color=(RdYlBu-9-2);
  color=(RdYlBu-9-3);
  color=(RdYlBu-9-4);
  color=(RdYlBu-9-5);
  color=(RdYlBu-9-6);
  color=(RdYlBu-9-7);
  color=(RdYlBu-9-8);
  color=(RdYlBu-9-9);
},
colormap={RdYlBu-10}{
  color=(RdYlBu-10-1);
  color=(RdYlBu-10-2);
  color=(RdYlBu-10-3);
  color=(RdYlBu-10-4);
  color=(RdYlBu-10-5);
  color=(RdYlBu-10-6);
  color=(RdYlBu-10-7);
  color=(RdYlBu-10-8);
  color=(RdYlBu-10-9);
  color=(RdYlBu-10-10);
},
colormap={RdYlBu-11}{
  color=(RdYlBu-11-1);
  color=(RdYlBu-11-2);
  color=(RdYlBu-11-3);
  color=(RdYlBu-11-4);
  color=(RdYlBu-11-5);
  color=(RdYlBu-11-6);
  color=(RdYlBu-11-7);
  color=(RdYlBu-11-8);
  color=(RdYlBu-11-9);
  color=(RdYlBu-11-10);
  color=(RdYlBu-11-11);
},
colormap={Spectral-3}{
  color=(Spectral-3-1);
  color=(Spectral-3-2);
  color=(Spectral-3-3);
},
colormap={Spectral-4}{
  color=(Spectral-4-1);
  color=(Spectral-4-2);
  color=(Spectral-4-3);
  color=(Spectral-4-4);
},
colormap={Spectral-5}{
  color=(Spectral-5-1);
  color=(Spectral-5-2);
  color=(Spectral-5-3);
  color=(Spectral-5-4);
  color=(Spectral-5-5);
},
colormap={Spectral-6}{
  color=(Spectral-6-1);
  color=(Spectral-6-2);
  color=(Spectral-6-3);
  color=(Spectral-6-4);
  color=(Spectral-6-5);
  color=(Spectral-6-6);
},
colormap={Spectral-7}{
  color=(Spectral-7-1);
  color=(Spectral-7-2);
  color=(Spectral-7-3);
  color=(Spectral-7-4);
  color=(Spectral-7-5);
  color=(Spectral-7-6);
  color=(Spectral-7-7);
},
colormap={Spectral-8}{
  color=(Spectral-8-1);
  color=(Spectral-8-2);
  color=(Spectral-8-3);
  color=(Spectral-8-4);
  color=(Spectral-8-5);
  color=(Spectral-8-6);
  color=(Spectral-8-7);
  color=(Spectral-8-8);
},
colormap={Spectral-9}{
  color=(Spectral-9-1);
  color=(Spectral-9-2);
  color=(Spectral-9-3);
  color=(Spectral-9-4);
  color=(Spectral-9-5);
  color=(Spectral-9-6);
  color=(Spectral-9-7);
  color=(Spectral-9-8);
  color=(Spectral-9-9);
},
colormap={Spectral-10}{
  color=(Spectral-10-1);
  color=(Spectral-10-2);
  color=(Spectral-10-3);
  color=(Spectral-10-4);
  color=(Spectral-10-5);
  color=(Spectral-10-6);
  color=(Spectral-10-7);
  color=(Spectral-10-8);
  color=(Spectral-10-9);
  color=(Spectral-10-10);
},
colormap={Spectral-11}{
  color=(Spectral-11-1);
  color=(Spectral-11-2);
  color=(Spectral-11-3);
  color=(Spectral-11-4);
  color=(Spectral-11-5);
  color=(Spectral-11-6);
  color=(Spectral-11-7);
  color=(Spectral-11-8);
  color=(Spectral-11-9);
  color=(Spectral-11-10);
  color=(Spectral-11-11);
},
colormap={RdYlGn-3}{
  color=(RdYlGn-3-1);
  color=(RdYlGn-3-2);
  color=(RdYlGn-3-3);
},
colormap={RdYlGn-4}{
  color=(RdYlGn-4-1);
  color=(RdYlGn-4-2);
  color=(RdYlGn-4-3);
  color=(RdYlGn-4-4);
},
colormap={RdYlGn-5}{
  color=(RdYlGn-5-1);
  color=(RdYlGn-5-2);
  color=(RdYlGn-5-3);
  color=(RdYlGn-5-4);
  color=(RdYlGn-5-5);
},
colormap={RdYlGn-6}{
  color=(RdYlGn-6-1);
  color=(RdYlGn-6-2);
  color=(RdYlGn-6-3);
  color=(RdYlGn-6-4);
  color=(RdYlGn-6-5);
  color=(RdYlGn-6-6);
},
colormap={RdYlGn-7}{
  color=(RdYlGn-7-1);
  color=(RdYlGn-7-2);
  color=(RdYlGn-7-3);
  color=(RdYlGn-7-4);
  color=(RdYlGn-7-5);
  color=(RdYlGn-7-6);
  color=(RdYlGn-7-7);
},
colormap={RdYlGn-8}{
  color=(RdYlGn-8-1);
  color=(RdYlGn-8-2);
  color=(RdYlGn-8-3);
  color=(RdYlGn-8-4);
  color=(RdYlGn-8-5);
  color=(RdYlGn-8-6);
  color=(RdYlGn-8-7);
  color=(RdYlGn-8-8);
},
colormap={RdYlGn-9}{
  color=(RdYlGn-9-1);
  color=(RdYlGn-9-2);
  color=(RdYlGn-9-3);
  color=(RdYlGn-9-4);
  color=(RdYlGn-9-5);
  color=(RdYlGn-9-6);
  color=(RdYlGn-9-7);
  color=(RdYlGn-9-8);
  color=(RdYlGn-9-9);
},
colormap={RdYlGn-10}{
  color=(RdYlGn-10-1);
  color=(RdYlGn-10-2);
  color=(RdYlGn-10-3);
  color=(RdYlGn-10-4);
  color=(RdYlGn-10-5);
  color=(RdYlGn-10-6);
  color=(RdYlGn-10-7);
  color=(RdYlGn-10-8);
  color=(RdYlGn-10-9);
  color=(RdYlGn-10-10);
},
colormap={RdYlGn-11}{
  color=(RdYlGn-11-1);
  color=(RdYlGn-11-2);
  color=(RdYlGn-11-3);
  color=(RdYlGn-11-4);
  color=(RdYlGn-11-5);
  color=(RdYlGn-11-6);
  color=(RdYlGn-11-7);
  color=(RdYlGn-11-8);
  color=(RdYlGn-11-9);
  color=(RdYlGn-11-10);
  color=(RdYlGn-11-11);
},
colormap={Set3-3}{
  color=(Set3-3-1);
  color=(Set3-3-2);
  color=(Set3-3-3);
},
colormap={Set3-4}{
  color=(Set3-4-1);
  color=(Set3-4-2);
  color=(Set3-4-3);
  color=(Set3-4-4);
},
colormap={Set3-5}{
  color=(Set3-5-1);
  color=(Set3-5-2);
  color=(Set3-5-3);
  color=(Set3-5-4);
  color=(Set3-5-5);
},
colormap={Set3-6}{
  color=(Set3-6-1);
  color=(Set3-6-2);
  color=(Set3-6-3);
  color=(Set3-6-4);
  color=(Set3-6-5);
  color=(Set3-6-6);
},
colormap={Set3-7}{
  color=(Set3-7-1);
  color=(Set3-7-2);
  color=(Set3-7-3);
  color=(Set3-7-4);
  color=(Set3-7-5);
  color=(Set3-7-6);
  color=(Set3-7-7);
},
colormap={Set3-8}{
  color=(Set3-8-1);
  color=(Set3-8-2);
  color=(Set3-8-3);
  color=(Set3-8-4);
  color=(Set3-8-5);
  color=(Set3-8-6);
  color=(Set3-8-7);
  color=(Set3-8-8);
},
colormap={Set3-9}{
  color=(Set3-9-1);
  color=(Set3-9-2);
  color=(Set3-9-3);
  color=(Set3-9-4);
  color=(Set3-9-5);
  color=(Set3-9-6);
  color=(Set3-9-7);
  color=(Set3-9-8);
  color=(Set3-9-9);
},
colormap={Set3-10}{
  color=(Set3-10-1);
  color=(Set3-10-2);
  color=(Set3-10-3);
  color=(Set3-10-4);
  color=(Set3-10-5);
  color=(Set3-10-6);
  color=(Set3-10-7);
  color=(Set3-10-8);
  color=(Set3-10-9);
  color=(Set3-10-10);
},
colormap={Set3-11}{
  color=(Set3-11-1);
  color=(Set3-11-2);
  color=(Set3-11-3);
  color=(Set3-11-4);
  color=(Set3-11-5);
  color=(Set3-11-6);
  color=(Set3-11-7);
  color=(Set3-11-8);
  color=(Set3-11-9);
  color=(Set3-11-10);
  color=(Set3-11-11);
},
colormap={Set3-12}{
  color=(Set3-12-1);
  color=(Set3-12-2);
  color=(Set3-12-3);
  color=(Set3-12-4);
  color=(Set3-12-5);
  color=(Set3-12-6);
  color=(Set3-12-7);
  color=(Set3-12-8);
  color=(Set3-12-9);
  color=(Set3-12-10);
  color=(Set3-12-11);
  color=(Set3-12-12);
},
colormap={Pastel1-3}{
  color=(Pastel1-3-1);
  color=(Pastel1-3-2);
  color=(Pastel1-3-3);
},
colormap={Pastel1-4}{
  color=(Pastel1-4-1);
  color=(Pastel1-4-2);
  color=(Pastel1-4-3);
  color=(Pastel1-4-4);
},
colormap={Pastel1-5}{
  color=(Pastel1-5-1);
  color=(Pastel1-5-2);
  color=(Pastel1-5-3);
  color=(Pastel1-5-4);
  color=(Pastel1-5-5);
},
colormap={Pastel1-6}{
  color=(Pastel1-6-1);
  color=(Pastel1-6-2);
  color=(Pastel1-6-3);
  color=(Pastel1-6-4);
  color=(Pastel1-6-5);
  color=(Pastel1-6-6);
},
colormap={Pastel1-7}{
  color=(Pastel1-7-1);
  color=(Pastel1-7-2);
  color=(Pastel1-7-3);
  color=(Pastel1-7-4);
  color=(Pastel1-7-5);
  color=(Pastel1-7-6);
  color=(Pastel1-7-7);
},
colormap={Pastel1-8}{
  color=(Pastel1-8-1);
  color=(Pastel1-8-2);
  color=(Pastel1-8-3);
  color=(Pastel1-8-4);
  color=(Pastel1-8-5);
  color=(Pastel1-8-6);
  color=(Pastel1-8-7);
  color=(Pastel1-8-8);
},
colormap={Pastel1-9}{
  color=(Pastel1-9-1);
  color=(Pastel1-9-2);
  color=(Pastel1-9-3);
  color=(Pastel1-9-4);
  color=(Pastel1-9-5);
  color=(Pastel1-9-6);
  color=(Pastel1-9-7);
  color=(Pastel1-9-8);
  color=(Pastel1-9-9);
},
colormap={Set1-3}{
  color=(Set1-3-1);
  color=(Set1-3-2);
  color=(Set1-3-3);
},
colormap={Set1-4}{
  color=(Set1-4-1);
  color=(Set1-4-2);
  color=(Set1-4-3);
  color=(Set1-4-4);
},
colormap={Set1-5}{
  color=(Set1-5-1);
  color=(Set1-5-2);
  color=(Set1-5-3);
  color=(Set1-5-4);
  color=(Set1-5-5);
},
colormap={Set1-6}{
  color=(Set1-6-1);
  color=(Set1-6-2);
  color=(Set1-6-3);
  color=(Set1-6-4);
  color=(Set1-6-5);
  color=(Set1-6-6);
},
colormap={Set1-7}{
  color=(Set1-7-1);
  color=(Set1-7-2);
  color=(Set1-7-3);
  color=(Set1-7-4);
  color=(Set1-7-5);
  color=(Set1-7-6);
  color=(Set1-7-7);
},
colormap={Set1-8}{
  color=(Set1-8-1);
  color=(Set1-8-2);
  color=(Set1-8-3);
  color=(Set1-8-4);
  color=(Set1-8-5);
  color=(Set1-8-6);
  color=(Set1-8-7);
  color=(Set1-8-8);
},
colormap={Set1-9}{
  color=(Set1-9-1);
  color=(Set1-9-2);
  color=(Set1-9-3);
  color=(Set1-9-4);
  color=(Set1-9-5);
  color=(Set1-9-6);
  color=(Set1-9-7);
  color=(Set1-9-8);
  color=(Set1-9-9);
},
colormap={Pastel2-3}{
  color=(Pastel2-3-1);
  color=(Pastel2-3-2);
  color=(Pastel2-3-3);
},
colormap={Pastel2-4}{
  color=(Pastel2-4-1);
  color=(Pastel2-4-2);
  color=(Pastel2-4-3);
  color=(Pastel2-4-4);
},
colormap={Pastel2-5}{
  color=(Pastel2-5-1);
  color=(Pastel2-5-2);
  color=(Pastel2-5-3);
  color=(Pastel2-5-4);
  color=(Pastel2-5-5);
},
colormap={Pastel2-6}{
  color=(Pastel2-6-1);
  color=(Pastel2-6-2);
  color=(Pastel2-6-3);
  color=(Pastel2-6-4);
  color=(Pastel2-6-5);
  color=(Pastel2-6-6);
},
colormap={Pastel2-7}{
  color=(Pastel2-7-1);
  color=(Pastel2-7-2);
  color=(Pastel2-7-3);
  color=(Pastel2-7-4);
  color=(Pastel2-7-5);
  color=(Pastel2-7-6);
  color=(Pastel2-7-7);
},
colormap={Pastel2-8}{
  color=(Pastel2-8-1);
  color=(Pastel2-8-2);
  color=(Pastel2-8-3);
  color=(Pastel2-8-4);
  color=(Pastel2-8-5);
  color=(Pastel2-8-6);
  color=(Pastel2-8-7);
  color=(Pastel2-8-8);
},
colormap={Set2-3}{
  color=(Set2-3-1);
  color=(Set2-3-2);
  color=(Set2-3-3);
},
colormap={Set2-4}{
  color=(Set2-4-1);
  color=(Set2-4-2);
  color=(Set2-4-3);
  color=(Set2-4-4);
},
colormap={Set2-5}{
  color=(Set2-5-1);
  color=(Set2-5-2);
  color=(Set2-5-3);
  color=(Set2-5-4);
  color=(Set2-5-5);
},
colormap={Set2-6}{
  color=(Set2-6-1);
  color=(Set2-6-2);
  color=(Set2-6-3);
  color=(Set2-6-4);
  color=(Set2-6-5);
  color=(Set2-6-6);
},
colormap={Set2-7}{
  color=(Set2-7-1);
  color=(Set2-7-2);
  color=(Set2-7-3);
  color=(Set2-7-4);
  color=(Set2-7-5);
  color=(Set2-7-6);
  color=(Set2-7-7);
},
colormap={Set2-8}{
  color=(Set2-8-1);
  color=(Set2-8-2);
  color=(Set2-8-3);
  color=(Set2-8-4);
  color=(Set2-8-5);
  color=(Set2-8-6);
  color=(Set2-8-7);
  color=(Set2-8-8);
},
colormap={Dark2-3}{
  color=(Dark2-3-1);
  color=(Dark2-3-2);
  color=(Dark2-3-3);
},
colormap={Dark2-4}{
  color=(Dark2-4-1);
  color=(Dark2-4-2);
  color=(Dark2-4-3);
  color=(Dark2-4-4);
},
colormap={Dark2-5}{
  color=(Dark2-5-1);
  color=(Dark2-5-2);
  color=(Dark2-5-3);
  color=(Dark2-5-4);
  color=(Dark2-5-5);
},
colormap={Dark2-6}{
  color=(Dark2-6-1);
  color=(Dark2-6-2);
  color=(Dark2-6-3);
  color=(Dark2-6-4);
  color=(Dark2-6-5);
  color=(Dark2-6-6);
},
colormap={Dark2-7}{
  color=(Dark2-7-1);
  color=(Dark2-7-2);
  color=(Dark2-7-3);
  color=(Dark2-7-4);
  color=(Dark2-7-5);
  color=(Dark2-7-6);
  color=(Dark2-7-7);
},
colormap={Dark2-8}{
  color=(Dark2-8-1);
  color=(Dark2-8-2);
  color=(Dark2-8-3);
  color=(Dark2-8-4);
  color=(Dark2-8-5);
  color=(Dark2-8-6);
  color=(Dark2-8-7);
  color=(Dark2-8-8);
},
colormap={Paired-3}{
  color=(Paired-3-1);
  color=(Paired-3-2);
  color=(Paired-3-3);
},
colormap={Paired-4}{
  color=(Paired-4-1);
  color=(Paired-4-2);
  color=(Paired-4-3);
  color=(Paired-4-4);
},
colormap={Paired-5}{
  color=(Paired-5-1);
  color=(Paired-5-2);
  color=(Paired-5-3);
  color=(Paired-5-4);
  color=(Paired-5-5);
},
colormap={Paired-6}{
  color=(Paired-6-1);
  color=(Paired-6-2);
  color=(Paired-6-3);
  color=(Paired-6-4);
  color=(Paired-6-5);
  color=(Paired-6-6);
},
colormap={Paired-7}{
  color=(Paired-7-1);
  color=(Paired-7-2);
  color=(Paired-7-3);
  color=(Paired-7-4);
  color=(Paired-7-5);
  color=(Paired-7-6);
  color=(Paired-7-7);
},
colormap={Paired-8}{
  color=(Paired-8-1);
  color=(Paired-8-2);
  color=(Paired-8-3);
  color=(Paired-8-4);
  color=(Paired-8-5);
  color=(Paired-8-6);
  color=(Paired-8-7);
  color=(Paired-8-8);
},
colormap={Paired-9}{
  color=(Paired-9-1);
  color=(Paired-9-2);
  color=(Paired-9-3);
  color=(Paired-9-4);
  color=(Paired-9-5);
  color=(Paired-9-6);
  color=(Paired-9-7);
  color=(Paired-9-8);
  color=(Paired-9-9);
},
colormap={Paired-10}{
  color=(Paired-10-1);
  color=(Paired-10-2);
  color=(Paired-10-3);
  color=(Paired-10-4);
  color=(Paired-10-5);
  color=(Paired-10-6);
  color=(Paired-10-7);
  color=(Paired-10-8);
  color=(Paired-10-9);
  color=(Paired-10-10);
},
colormap={Paired-11}{
  color=(Paired-11-1);
  color=(Paired-11-2);
  color=(Paired-11-3);
  color=(Paired-11-4);
  color=(Paired-11-5);
  color=(Paired-11-6);
  color=(Paired-11-7);
  color=(Paired-11-8);
  color=(Paired-11-9);
  color=(Paired-11-10);
  color=(Paired-11-11);
},
colormap={Paired-12}{
  color=(Paired-12-1);
  color=(Paired-12-2);
  color=(Paired-12-3);
  color=(Paired-12-4);
  color=(Paired-12-5);
  color=(Paired-12-6);
  color=(Paired-12-7);
  color=(Paired-12-8);
  color=(Paired-12-9);
  color=(Paired-12-10);
  color=(Paired-12-11);
  color=(Paired-12-12);
},
colormap={Accent-3}{
  color=(Accent-3-1);
  color=(Accent-3-2);
  color=(Accent-3-3);
},
colormap={Accent-4}{
  color=(Accent-4-1);
  color=(Accent-4-2);
  color=(Accent-4-3);
  color=(Accent-4-4);
},
colormap={Accent-5}{
  color=(Accent-5-1);
  color=(Accent-5-2);
  color=(Accent-5-3);
  color=(Accent-5-4);
  color=(Accent-5-5);
},
colormap={Accent-6}{
  color=(Accent-6-1);
  color=(Accent-6-2);
  color=(Accent-6-3);
  color=(Accent-6-4);
  color=(Accent-6-5);
  color=(Accent-6-6);
},
colormap={Accent-7}{
  color=(Accent-7-1);
  color=(Accent-7-2);
  color=(Accent-7-3);
  color=(Accent-7-4);
  color=(Accent-7-5);
  color=(Accent-7-6);
  color=(Accent-7-7);
},
colormap={Accent-8}{
  color=(Accent-8-1);
  color=(Accent-8-2);
  color=(Accent-8-3);
  color=(Accent-8-4);
  color=(Accent-8-5);
  color=(Accent-8-6);
  color=(Accent-8-7);
  color=(Accent-8-8);
}
}


==> tikzlibrarycolorbrewer.code.tex <==
% Color schemes as obtained from http://colorbrewer2.org/
%
% Apache-Style Software License for ColorBrewer software and ColorBrewer Color
% Schemes
% 
% Copyright (c) 2002 Cynthia Brewer, Mark Harrower, and The Pennsylvania State
% University.
% 
% Licensed under the Apache License, Version 2.0 (the "License"); you may not
% use this file except in compliance with the License.  You may obtain a copy of
% the License at
% 
%        http://www.apache.org/licenses/LICENSE-2.0
% 
% Unless required by applicable law or agreed to in writing, software
% distributed under the License is distributed on an "AS IS" BASIS, WITHOUT
% WARRANTIES OR CONDITIONS OF ANY KIND, either express or implied.  See the
% License for the specific language governing permissions and limitations under
% the License.
% 
% Redistribution and use in source and binary forms, with or without
% modification, are permitted provided that the following conditions are met:
% 1. Redistributions as source code must retain the above copyright notice, this
%    list of conditions and the following disclaimer.
% 2. The end-user documentation included with the redistribution, if any, must
%    include the following acknowledgment: This product includes color
%    specifications and designs developed by Cynthia Brewer
%    (http://colorbrewer.org/).  Alternately, this acknowledgment may appear in the
%    software itself, if and wherever such third-party acknowledgments normally
%    appear.
% 3. The name "ColorBrewer" must not be used to endorse or promote products
%    derived from this software without prior written permission.  For written
%    permission, please contact Cynthia Brewer at cbrewer@psu.edu.
% 4. Products derived from this software may not be called "ColorBrewer", nor
%    may "ColorBrewer" appear in their name, without prior written permission of
%    Cynthia Brewer.
\definecolor{YlGn-3-1}{RGB}{247,252,185}
\definecolor{YlGn-3-C}{RGB}{247,252,185}
\definecolor{YlGn-3-2}{RGB}{173,221,142}
\definecolor{YlGn-3-F}{RGB}{173,221,142}
\definecolor{YlGn-3-3}{RGB}{49,163,84}
\definecolor{YlGn-3-I}{RGB}{49,163,84}
\definecolor{YlGn-4-1}{RGB}{255,255,204}
\definecolor{YlGn-4-B}{RGB}{255,255,204}
\definecolor{YlGn-4-2}{RGB}{194,230,153}
\definecolor{YlGn-4-E}{RGB}{194,230,153}
\definecolor{YlGn-4-3}{RGB}{120,198,121}
\definecolor{YlGn-4-G}{RGB}{120,198,121}
\definecolor{YlGn-4-4}{RGB}{35,132,67}
\definecolor{YlGn-4-J}{RGB}{35,132,67}
\definecolor{YlGn-5-1}{RGB}{255,255,204}
\definecolor{YlGn-5-B}{RGB}{255,255,204}
\definecolor{YlGn-5-2}{RGB}{194,230,153}
\definecolor{YlGn-5-E}{RGB}{194,230,153}
\definecolor{YlGn-5-3}{RGB}{120,198,121}
\definecolor{YlGn-5-G}{RGB}{120,198,121}
\definecolor{YlGn-5-4}{RGB}{49,163,84}
\definecolor{YlGn-5-I}{RGB}{49,163,84}
\definecolor{YlGn-5-5}{RGB}{0,104,55}
\definecolor{YlGn-5-K}{RGB}{0,104,55}
\definecolor{YlGn-6-1}{RGB}{255,255,204}
\definecolor{YlGn-6-B}{RGB}{255,255,204}
\definecolor{YlGn-6-2}{RGB}{217,240,163}
\definecolor{YlGn-6-D}{RGB}{217,240,163}
\definecolor{YlGn-6-3}{RGB}{173,221,142}
\definecolor{YlGn-6-F}{RGB}{173,221,142}
\definecolor{YlGn-6-4}{RGB}{120,198,121}
\definecolor{YlGn-6-G}{RGB}{120,198,121}
\definecolor{YlGn-6-5}{RGB}{49,163,84}
\definecolor{YlGn-6-I}{RGB}{49,163,84}
\definecolor{YlGn-6-6}{RGB}{0,104,55}
\definecolor{YlGn-6-K}{RGB}{0,104,55}
\definecolor{YlGn-7-1}{RGB}{255,255,204}
\definecolor{YlGn-7-B}{RGB}{255,255,204}
\definecolor{YlGn-7-2}{RGB}{217,240,163}
\definecolor{YlGn-7-D}{RGB}{217,240,163}
\definecolor{YlGn-7-3}{RGB}{173,221,142}
\definecolor{YlGn-7-F}{RGB}{173,221,142}
\definecolor{YlGn-7-4}{RGB}{120,198,121}
\definecolor{YlGn-7-G}{RGB}{120,198,121}
\definecolor{YlGn-7-5}{RGB}{65,171,93}
\definecolor{YlGn-7-H}{RGB}{65,171,93}
\definecolor{YlGn-7-6}{RGB}{35,132,67}
\definecolor{YlGn-7-J}{RGB}{35,132,67}
\definecolor{YlGn-7-7}{RGB}{0,90,50}
\definecolor{YlGn-7-L}{RGB}{0,90,50}
\definecolor{YlGn-8-1}{RGB}{255,255,229}
\definecolor{YlGn-8-A}{RGB}{255,255,229}
\definecolor{YlGn-8-2}{RGB}{247,252,185}
\definecolor{YlGn-8-C}{RGB}{247,252,185}
\definecolor{YlGn-8-3}{RGB}{217,240,163}
\definecolor{YlGn-8-D}{RGB}{217,240,163}
\definecolor{YlGn-8-4}{RGB}{173,221,142}
\definecolor{YlGn-8-F}{RGB}{173,221,142}
\definecolor{YlGn-8-5}{RGB}{120,198,121}
\definecolor{YlGn-8-G}{RGB}{120,198,121}
\definecolor{YlGn-8-6}{RGB}{65,171,93}
\definecolor{YlGn-8-H}{RGB}{65,171,93}
\definecolor{YlGn-8-7}{RGB}{35,132,67}
\definecolor{YlGn-8-J}{RGB}{35,132,67}
\definecolor{YlGn-8-8}{RGB}{0,90,50}
\definecolor{YlGn-8-L}{RGB}{0,90,50}
\definecolor{YlGn-9-1}{RGB}{255,255,229}
\definecolor{YlGn-9-A}{RGB}{255,255,229}
\definecolor{YlGn-9-2}{RGB}{247,252,185}
\definecolor{YlGn-9-C}{RGB}{247,252,185}
\definecolor{YlGn-9-3}{RGB}{217,240,163}
\definecolor{YlGn-9-D}{RGB}{217,240,163}
\definecolor{YlGn-9-4}{RGB}{173,221,142}
\definecolor{YlGn-9-F}{RGB}{173,221,142}
\definecolor{YlGn-9-5}{RGB}{120,198,121}
\definecolor{YlGn-9-G}{RGB}{120,198,121}
\definecolor{YlGn-9-6}{RGB}{65,171,93}
\definecolor{YlGn-9-H}{RGB}{65,171,93}
\definecolor{YlGn-9-7}{RGB}{35,132,67}
\definecolor{YlGn-9-J}{RGB}{35,132,67}
\definecolor{YlGn-9-8}{RGB}{0,104,55}
\definecolor{YlGn-9-K}{RGB}{0,104,55}
\definecolor{YlGn-9-9}{RGB}{0,69,41}
\definecolor{YlGn-9-M}{RGB}{0,69,41}
\definecolor{YlGnBu-3-1}{RGB}{237,248,177}
\definecolor{YlGnBu-3-C}{RGB}{237,248,177}
\definecolor{YlGnBu-3-2}{RGB}{127,205,187}
\definecolor{YlGnBu-3-F}{RGB}{127,205,187}
\definecolor{YlGnBu-3-3}{RGB}{44,127,184}
\definecolor{YlGnBu-3-I}{RGB}{44,127,184}
\definecolor{YlGnBu-4-1}{RGB}{255,255,204}
\definecolor{YlGnBu-4-B}{RGB}{255,255,204}
\definecolor{YlGnBu-4-2}{RGB}{161,218,180}
\definecolor{YlGnBu-4-E}{RGB}{161,218,180}
\definecolor{YlGnBu-4-3}{RGB}{65,182,196}
\definecolor{YlGnBu-4-G}{RGB}{65,182,196}
\definecolor{YlGnBu-4-4}{RGB}{34,94,168}
\definecolor{YlGnBu-4-J}{RGB}{34,94,168}
\definecolor{YlGnBu-5-1}{RGB}{255,255,204}
\definecolor{YlGnBu-5-B}{RGB}{255,255,204}
\definecolor{YlGnBu-5-2}{RGB}{161,218,180}
\definecolor{YlGnBu-5-E}{RGB}{161,218,180}
\definecolor{YlGnBu-5-3}{RGB}{65,182,196}
\definecolor{YlGnBu-5-G}{RGB}{65,182,196}
\definecolor{YlGnBu-5-4}{RGB}{44,127,184}
\definecolor{YlGnBu-5-I}{RGB}{44,127,184}
\definecolor{YlGnBu-5-5}{RGB}{37,52,148}
\definecolor{YlGnBu-5-K}{RGB}{37,52,148}
\definecolor{YlGnBu-6-1}{RGB}{255,255,204}
\definecolor{YlGnBu-6-B}{RGB}{255,255,204}
\definecolor{YlGnBu-6-2}{RGB}{199,233,180}
\definecolor{YlGnBu-6-D}{RGB}{199,233,180}
\definecolor{YlGnBu-6-3}{RGB}{127,205,187}
\definecolor{YlGnBu-6-F}{RGB}{127,205,187}
\definecolor{YlGnBu-6-4}{RGB}{65,182,196}
\definecolor{YlGnBu-6-G}{RGB}{65,182,196}
\definecolor{YlGnBu-6-5}{RGB}{44,127,184}
\definecolor{YlGnBu-6-I}{RGB}{44,127,184}
\definecolor{YlGnBu-6-6}{RGB}{37,52,148}
\definecolor{YlGnBu-6-K}{RGB}{37,52,148}
\definecolor{YlGnBu-7-1}{RGB}{255,255,204}
\definecolor{YlGnBu-7-B}{RGB}{255,255,204}
\definecolor{YlGnBu-7-2}{RGB}{199,233,180}
\definecolor{YlGnBu-7-D}{RGB}{199,233,180}
\definecolor{YlGnBu-7-3}{RGB}{127,205,187}
\definecolor{YlGnBu-7-F}{RGB}{127,205,187}
\definecolor{YlGnBu-7-4}{RGB}{65,182,196}
\definecolor{YlGnBu-7-G}{RGB}{65,182,196}
\definecolor{YlGnBu-7-5}{RGB}{29,145,192}
\definecolor{YlGnBu-7-H}{RGB}{29,145,192}
\definecolor{YlGnBu-7-6}{RGB}{34,94,168}
\definecolor{YlGnBu-7-J}{RGB}{34,94,168}
\definecolor{YlGnBu-7-7}{RGB}{12,44,132}
\definecolor{YlGnBu-7-L}{RGB}{12,44,132}
\definecolor{YlGnBu-8-1}{RGB}{255,255,217}
\definecolor{YlGnBu-8-A}{RGB}{255,255,217}
\definecolor{YlGnBu-8-2}{RGB}{237,248,177}
\definecolor{YlGnBu-8-C}{RGB}{237,248,177}
\definecolor{YlGnBu-8-3}{RGB}{199,233,180}
\definecolor{YlGnBu-8-D}{RGB}{199,233,180}
\definecolor{YlGnBu-8-4}{RGB}{127,205,187}
\definecolor{YlGnBu-8-F}{RGB}{127,205,187}
\definecolor{YlGnBu-8-5}{RGB}{65,182,196}
\definecolor{YlGnBu-8-G}{RGB}{65,182,196}
\definecolor{YlGnBu-8-6}{RGB}{29,145,192}
\definecolor{YlGnBu-8-H}{RGB}{29,145,192}
\definecolor{YlGnBu-8-7}{RGB}{34,94,168}
\definecolor{YlGnBu-8-J}{RGB}{34,94,168}
\definecolor{YlGnBu-8-8}{RGB}{12,44,132}
\definecolor{YlGnBu-8-L}{RGB}{12,44,132}
\definecolor{YlGnBu-9-1}{RGB}{255,255,217}
\definecolor{YlGnBu-9-A}{RGB}{255,255,217}
\definecolor{YlGnBu-9-2}{RGB}{237,248,177}
\definecolor{YlGnBu-9-C}{RGB}{237,248,177}
\definecolor{YlGnBu-9-3}{RGB}{199,233,180}
\definecolor{YlGnBu-9-D}{RGB}{199,233,180}
\definecolor{YlGnBu-9-4}{RGB}{127,205,187}
\definecolor{YlGnBu-9-F}{RGB}{127,205,187}
\definecolor{YlGnBu-9-5}{RGB}{65,182,196}
\definecolor{YlGnBu-9-G}{RGB}{65,182,196}
\definecolor{YlGnBu-9-6}{RGB}{29,145,192}
\definecolor{YlGnBu-9-H}{RGB}{29,145,192}
\definecolor{YlGnBu-9-7}{RGB}{34,94,168}
\definecolor{YlGnBu-9-J}{RGB}{34,94,168}
\definecolor{YlGnBu-9-8}{RGB}{37,52,148}
\definecolor{YlGnBu-9-K}{RGB}{37,52,148}
\definecolor{YlGnBu-9-9}{RGB}{8,29,88}
\definecolor{YlGnBu-9-M}{RGB}{8,29,88}
\definecolor{GnBu-3-1}{RGB}{224,243,219}
\definecolor{GnBu-3-C}{RGB}{224,243,219}
\definecolor{GnBu-3-2}{RGB}{168,221,181}
\definecolor{GnBu-3-F}{RGB}{168,221,181}
\definecolor{GnBu-3-3}{RGB}{67,162,202}
\definecolor{GnBu-3-I}{RGB}{67,162,202}
\definecolor{GnBu-4-1}{RGB}{240,249,232}
\definecolor{GnBu-4-B}{RGB}{240,249,232}
\definecolor{GnBu-4-2}{RGB}{186,228,188}
\definecolor{GnBu-4-E}{RGB}{186,228,188}
\definecolor{GnBu-4-3}{RGB}{123,204,196}
\definecolor{GnBu-4-G}{RGB}{123,204,196}
\definecolor{GnBu-4-4}{RGB}{43,140,190}
\definecolor{GnBu-4-J}{RGB}{43,140,190}
\definecolor{GnBu-5-1}{RGB}{240,249,232}
\definecolor{GnBu-5-B}{RGB}{240,249,232}
\definecolor{GnBu-5-2}{RGB}{186,228,188}
\definecolor{GnBu-5-E}{RGB}{186,228,188}
\definecolor{GnBu-5-3}{RGB}{123,204,196}
\definecolor{GnBu-5-G}{RGB}{123,204,196}
\definecolor{GnBu-5-4}{RGB}{67,162,202}
\definecolor{GnBu-5-I}{RGB}{67,162,202}
\definecolor{GnBu-5-5}{RGB}{8,104,172}
\definecolor{GnBu-5-K}{RGB}{8,104,172}
\definecolor{GnBu-6-1}{RGB}{240,249,232}
\definecolor{GnBu-6-B}{RGB}{240,249,232}
\definecolor{GnBu-6-2}{RGB}{204,235,197}
\definecolor{GnBu-6-D}{RGB}{204,235,197}
\definecolor{GnBu-6-3}{RGB}{168,221,181}
\definecolor{GnBu-6-F}{RGB}{168,221,181}
\definecolor{GnBu-6-4}{RGB}{123,204,196}
\definecolor{GnBu-6-G}{RGB}{123,204,196}
\definecolor{GnBu-6-5}{RGB}{67,162,202}
\definecolor{GnBu-6-I}{RGB}{67,162,202}
\definecolor{GnBu-6-6}{RGB}{8,104,172}
\definecolor{GnBu-6-K}{RGB}{8,104,172}
\definecolor{GnBu-7-1}{RGB}{240,249,232}
\definecolor{GnBu-7-B}{RGB}{240,249,232}
\definecolor{GnBu-7-2}{RGB}{204,235,197}
\definecolor{GnBu-7-D}{RGB}{204,235,197}
\definecolor{GnBu-7-3}{RGB}{168,221,181}
\definecolor{GnBu-7-F}{RGB}{168,221,181}
\definecolor{GnBu-7-4}{RGB}{123,204,196}
\definecolor{GnBu-7-G}{RGB}{123,204,196}
\definecolor{GnBu-7-5}{RGB}{78,179,211}
\definecolor{GnBu-7-H}{RGB}{78,179,211}
\definecolor{GnBu-7-6}{RGB}{43,140,190}
\definecolor{GnBu-7-J}{RGB}{43,140,190}
\definecolor{GnBu-7-7}{RGB}{8,88,158}
\definecolor{GnBu-7-L}{RGB}{8,88,158}
\definecolor{GnBu-8-1}{RGB}{247,252,240}
\definecolor{GnBu-8-A}{RGB}{247,252,240}
\definecolor{GnBu-8-2}{RGB}{224,243,219}
\definecolor{GnBu-8-C}{RGB}{224,243,219}
\definecolor{GnBu-8-3}{RGB}{204,235,197}
\definecolor{GnBu-8-D}{RGB}{204,235,197}
\definecolor{GnBu-8-4}{RGB}{168,221,181}
\definecolor{GnBu-8-F}{RGB}{168,221,181}
\definecolor{GnBu-8-5}{RGB}{123,204,196}
\definecolor{GnBu-8-G}{RGB}{123,204,196}
\definecolor{GnBu-8-6}{RGB}{78,179,211}
\definecolor{GnBu-8-H}{RGB}{78,179,211}
\definecolor{GnBu-8-7}{RGB}{43,140,190}
\definecolor{GnBu-8-J}{RGB}{43,140,190}
\definecolor{GnBu-8-8}{RGB}{8,88,158}
\definecolor{GnBu-8-L}{RGB}{8,88,158}
\definecolor{GnBu-9-1}{RGB}{247,252,240}
\definecolor{GnBu-9-A}{RGB}{247,252,240}
\definecolor{GnBu-9-2}{RGB}{224,243,219}
\definecolor{GnBu-9-C}{RGB}{224,243,219}
\definecolor{GnBu-9-3}{RGB}{204,235,197}
\definecolor{GnBu-9-D}{RGB}{204,235,197}
\definecolor{GnBu-9-4}{RGB}{168,221,181}
\definecolor{GnBu-9-F}{RGB}{168,221,181}
\definecolor{GnBu-9-5}{RGB}{123,204,196}
\definecolor{GnBu-9-G}{RGB}{123,204,196}
\definecolor{GnBu-9-6}{RGB}{78,179,211}
\definecolor{GnBu-9-H}{RGB}{78,179,211}
\definecolor{GnBu-9-7}{RGB}{43,140,190}
\definecolor{GnBu-9-J}{RGB}{43,140,190}
\definecolor{GnBu-9-8}{RGB}{8,104,172}
\definecolor{GnBu-9-K}{RGB}{8,104,172}
\definecolor{GnBu-9-9}{RGB}{8,64,129}
\definecolor{GnBu-9-M}{RGB}{8,64,129}
\definecolor{BuGn-3-1}{RGB}{229,245,249}
\definecolor{BuGn-3-C}{RGB}{229,245,249}
\definecolor{BuGn-3-2}{RGB}{153,216,201}
\definecolor{BuGn-3-F}{RGB}{153,216,201}
\definecolor{BuGn-3-3}{RGB}{44,162,95}
\definecolor{BuGn-3-I}{RGB}{44,162,95}
\definecolor{BuGn-4-1}{RGB}{237,248,251}
\definecolor{BuGn-4-B}{RGB}{237,248,251}
\definecolor{BuGn-4-2}{RGB}{178,226,226}
\definecolor{BuGn-4-E}{RGB}{178,226,226}
\definecolor{BuGn-4-3}{RGB}{102,194,164}
\definecolor{BuGn-4-G}{RGB}{102,194,164}
\definecolor{BuGn-4-4}{RGB}{35,139,69}
\definecolor{BuGn-4-J}{RGB}{35,139,69}
\definecolor{BuGn-5-1}{RGB}{237,248,251}
\definecolor{BuGn-5-B}{RGB}{237,248,251}
\definecolor{BuGn-5-2}{RGB}{178,226,226}
\definecolor{BuGn-5-E}{RGB}{178,226,226}
\definecolor{BuGn-5-3}{RGB}{102,194,164}
\definecolor{BuGn-5-G}{RGB}{102,194,164}
\definecolor{BuGn-5-4}{RGB}{44,162,95}
\definecolor{BuGn-5-I}{RGB}{44,162,95}
\definecolor{BuGn-5-5}{RGB}{0,109,44}
\definecolor{BuGn-5-K}{RGB}{0,109,44}
\definecolor{BuGn-6-1}{RGB}{237,248,251}
\definecolor{BuGn-6-B}{RGB}{237,248,251}
\definecolor{BuGn-6-2}{RGB}{204,236,230}
\definecolor{BuGn-6-D}{RGB}{204,236,230}
\definecolor{BuGn-6-3}{RGB}{153,216,201}
\definecolor{BuGn-6-F}{RGB}{153,216,201}
\definecolor{BuGn-6-4}{RGB}{102,194,164}
\definecolor{BuGn-6-G}{RGB}{102,194,164}
\definecolor{BuGn-6-5}{RGB}{44,162,95}
\definecolor{BuGn-6-I}{RGB}{44,162,95}
\definecolor{BuGn-6-6}{RGB}{0,109,44}
\definecolor{BuGn-6-K}{RGB}{0,109,44}
\definecolor{BuGn-7-1}{RGB}{237,248,251}
\definecolor{BuGn-7-B}{RGB}{237,248,251}
\definecolor{BuGn-7-2}{RGB}{204,236,230}
\definecolor{BuGn-7-D}{RGB}{204,236,230}
\definecolor{BuGn-7-3}{RGB}{153,216,201}
\definecolor{BuGn-7-F}{RGB}{153,216,201}
\definecolor{BuGn-7-4}{RGB}{102,194,164}
\definecolor{BuGn-7-G}{RGB}{102,194,164}
\definecolor{BuGn-7-5}{RGB}{65,174,118}
\definecolor{BuGn-7-H}{RGB}{65,174,118}
\definecolor{BuGn-7-6}{RGB}{35,139,69}
\definecolor{BuGn-7-J}{RGB}{35,139,69}
\definecolor{BuGn-7-7}{RGB}{0,88,36}
\definecolor{BuGn-7-L}{RGB}{0,88,36}
\definecolor{BuGn-8-1}{RGB}{247,252,253}
\definecolor{BuGn-8-A}{RGB}{247,252,253}
\definecolor{BuGn-8-2}{RGB}{229,245,249}
\definecolor{BuGn-8-C}{RGB}{229,245,249}
\definecolor{BuGn-8-3}{RGB}{204,236,230}
\definecolor{BuGn-8-D}{RGB}{204,236,230}
\definecolor{BuGn-8-4}{RGB}{153,216,201}
\definecolor{BuGn-8-F}{RGB}{153,216,201}
\definecolor{BuGn-8-5}{RGB}{102,194,164}
\definecolor{BuGn-8-G}{RGB}{102,194,164}
\definecolor{BuGn-8-6}{RGB}{65,174,118}
\definecolor{BuGn-8-H}{RGB}{65,174,118}
\definecolor{BuGn-8-7}{RGB}{35,139,69}
\definecolor{BuGn-8-J}{RGB}{35,139,69}
\definecolor{BuGn-8-8}{RGB}{0,88,36}
\definecolor{BuGn-8-L}{RGB}{0,88,36}
\definecolor{BuGn-9-1}{RGB}{247,252,253}
\definecolor{BuGn-9-A}{RGB}{247,252,253}
\definecolor{BuGn-9-2}{RGB}{229,245,249}
\definecolor{BuGn-9-C}{RGB}{229,245,249}
\definecolor{BuGn-9-3}{RGB}{204,236,230}
\definecolor{BuGn-9-D}{RGB}{204,236,230}
\definecolor{BuGn-9-4}{RGB}{153,216,201}
\definecolor{BuGn-9-F}{RGB}{153,216,201}
\definecolor{BuGn-9-5}{RGB}{102,194,164}
\definecolor{BuGn-9-G}{RGB}{102,194,164}
\definecolor{BuGn-9-6}{RGB}{65,174,118}
\definecolor{BuGn-9-H}{RGB}{65,174,118}
\definecolor{BuGn-9-7}{RGB}{35,139,69}
\definecolor{BuGn-9-J}{RGB}{35,139,69}
\definecolor{BuGn-9-8}{RGB}{0,109,44}
\definecolor{BuGn-9-K}{RGB}{0,109,44}
\definecolor{BuGn-9-9}{RGB}{0,68,27}
\definecolor{BuGn-9-M}{RGB}{0,68,27}
\definecolor{PuBuGn-3-1}{RGB}{236,226,240}
\definecolor{PuBuGn-3-C}{RGB}{236,226,240}
\definecolor{PuBuGn-3-2}{RGB}{166,189,219}
\definecolor{PuBuGn-3-F}{RGB}{166,189,219}
\definecolor{PuBuGn-3-3}{RGB}{28,144,153}
\definecolor{PuBuGn-3-I}{RGB}{28,144,153}
\definecolor{PuBuGn-4-1}{RGB}{246,239,247}
\definecolor{PuBuGn-4-B}{RGB}{246,239,247}
\definecolor{PuBuGn-4-2}{RGB}{189,201,225}
\definecolor{PuBuGn-4-E}{RGB}{189,201,225}
\definecolor{PuBuGn-4-3}{RGB}{103,169,207}
\definecolor{PuBuGn-4-G}{RGB}{103,169,207}
\definecolor{PuBuGn-4-4}{RGB}{2,129,138}
\definecolor{PuBuGn-4-J}{RGB}{2,129,138}
\definecolor{PuBuGn-5-1}{RGB}{246,239,247}
\definecolor{PuBuGn-5-B}{RGB}{246,239,247}
\definecolor{PuBuGn-5-2}{RGB}{189,201,225}
\definecolor{PuBuGn-5-E}{RGB}{189,201,225}
\definecolor{PuBuGn-5-3}{RGB}{103,169,207}
\definecolor{PuBuGn-5-G}{RGB}{103,169,207}
\definecolor{PuBuGn-5-4}{RGB}{28,144,153}
\definecolor{PuBuGn-5-I}{RGB}{28,144,153}
\definecolor{PuBuGn-5-5}{RGB}{1,108,89}
\definecolor{PuBuGn-5-K}{RGB}{1,108,89}
\definecolor{PuBuGn-6-1}{RGB}{246,239,247}
\definecolor{PuBuGn-6-B}{RGB}{246,239,247}
\definecolor{PuBuGn-6-2}{RGB}{208,209,230}
\definecolor{PuBuGn-6-D}{RGB}{208,209,230}
\definecolor{PuBuGn-6-3}{RGB}{166,189,219}
\definecolor{PuBuGn-6-F}{RGB}{166,189,219}
\definecolor{PuBuGn-6-4}{RGB}{103,169,207}
\definecolor{PuBuGn-6-G}{RGB}{103,169,207}
\definecolor{PuBuGn-6-5}{RGB}{28,144,153}
\definecolor{PuBuGn-6-I}{RGB}{28,144,153}
\definecolor{PuBuGn-6-6}{RGB}{1,108,89}
\definecolor{PuBuGn-6-K}{RGB}{1,108,89}
\definecolor{PuBuGn-7-1}{RGB}{246,239,247}
\definecolor{PuBuGn-7-B}{RGB}{246,239,247}
\definecolor{PuBuGn-7-2}{RGB}{208,209,230}
\definecolor{PuBuGn-7-D}{RGB}{208,209,230}
\definecolor{PuBuGn-7-3}{RGB}{166,189,219}
\definecolor{PuBuGn-7-F}{RGB}{166,189,219}
\definecolor{PuBuGn-7-4}{RGB}{103,169,207}
\definecolor{PuBuGn-7-G}{RGB}{103,169,207}
\definecolor{PuBuGn-7-5}{RGB}{54,144,192}
\definecolor{PuBuGn-7-H}{RGB}{54,144,192}
\definecolor{PuBuGn-7-6}{RGB}{2,129,138}
\definecolor{PuBuGn-7-J}{RGB}{2,129,138}
\definecolor{PuBuGn-7-7}{RGB}{1,100,80}
\definecolor{PuBuGn-7-L}{RGB}{1,100,80}
\definecolor{PuBuGn-8-1}{RGB}{255,247,251}
\definecolor{PuBuGn-8-A}{RGB}{255,247,251}
\definecolor{PuBuGn-8-2}{RGB}{236,226,240}
\definecolor{PuBuGn-8-C}{RGB}{236,226,240}
\definecolor{PuBuGn-8-3}{RGB}{208,209,230}
\definecolor{PuBuGn-8-D}{RGB}{208,209,230}
\definecolor{PuBuGn-8-4}{RGB}{166,189,219}
\definecolor{PuBuGn-8-F}{RGB}{166,189,219}
\definecolor{PuBuGn-8-5}{RGB}{103,169,207}
\definecolor{PuBuGn-8-G}{RGB}{103,169,207}
\definecolor{PuBuGn-8-6}{RGB}{54,144,192}
\definecolor{PuBuGn-8-H}{RGB}{54,144,192}
\definecolor{PuBuGn-8-7}{RGB}{2,129,138}
\definecolor{PuBuGn-8-J}{RGB}{2,129,138}
\definecolor{PuBuGn-8-8}{RGB}{1,100,80}
\definecolor{PuBuGn-8-L}{RGB}{1,100,80}
\definecolor{PuBuGn-9-1}{RGB}{255,247,251}
\definecolor{PuBuGn-9-A}{RGB}{255,247,251}
\definecolor{PuBuGn-9-2}{RGB}{236,226,240}
\definecolor{PuBuGn-9-C}{RGB}{236,226,240}
\definecolor{PuBuGn-9-3}{RGB}{208,209,230}
\definecolor{PuBuGn-9-D}{RGB}{208,209,230}
\definecolor{PuBuGn-9-4}{RGB}{166,189,219}
\definecolor{PuBuGn-9-F}{RGB}{166,189,219}
\definecolor{PuBuGn-9-5}{RGB}{103,169,207}
\definecolor{PuBuGn-9-G}{RGB}{103,169,207}
\definecolor{PuBuGn-9-6}{RGB}{54,144,192}
\definecolor{PuBuGn-9-H}{RGB}{54,144,192}
\definecolor{PuBuGn-9-7}{RGB}{2,129,138}
\definecolor{PuBuGn-9-J}{RGB}{2,129,138}
\definecolor{PuBuGn-9-8}{RGB}{1,108,89}
\definecolor{PuBuGn-9-K}{RGB}{1,108,89}
\definecolor{PuBuGn-9-9}{RGB}{1,70,54}
\definecolor{PuBuGn-9-M}{RGB}{1,70,54}
\definecolor{PuBu-3-1}{RGB}{236,231,242}
\definecolor{PuBu-3-C}{RGB}{236,231,242}
\definecolor{PuBu-3-2}{RGB}{166,189,219}
\definecolor{PuBu-3-F}{RGB}{166,189,219}
\definecolor{PuBu-3-3}{RGB}{43,140,190}
\definecolor{PuBu-3-I}{RGB}{43,140,190}
\definecolor{PuBu-4-1}{RGB}{241,238,246}
\definecolor{PuBu-4-B}{RGB}{241,238,246}
\definecolor{PuBu-4-2}{RGB}{189,201,225}
\definecolor{PuBu-4-E}{RGB}{189,201,225}
\definecolor{PuBu-4-3}{RGB}{116,169,207}
\definecolor{PuBu-4-G}{RGB}{116,169,207}
\definecolor{PuBu-4-4}{RGB}{5,112,176}
\definecolor{PuBu-4-J}{RGB}{5,112,176}
\definecolor{PuBu-5-1}{RGB}{241,238,246}
\definecolor{PuBu-5-B}{RGB}{241,238,246}
\definecolor{PuBu-5-2}{RGB}{189,201,225}
\definecolor{PuBu-5-E}{RGB}{189,201,225}
\definecolor{PuBu-5-3}{RGB}{116,169,207}
\definecolor{PuBu-5-G}{RGB}{116,169,207}
\definecolor{PuBu-5-4}{RGB}{43,140,190}
\definecolor{PuBu-5-I}{RGB}{43,140,190}
\definecolor{PuBu-5-5}{RGB}{4,90,141}
\definecolor{PuBu-5-K}{RGB}{4,90,141}
\definecolor{PuBu-6-1}{RGB}{241,238,246}
\definecolor{PuBu-6-B}{RGB}{241,238,246}
\definecolor{PuBu-6-2}{RGB}{208,209,230}
\definecolor{PuBu-6-D}{RGB}{208,209,230}
\definecolor{PuBu-6-3}{RGB}{166,189,219}
\definecolor{PuBu-6-F}{RGB}{166,189,219}
\definecolor{PuBu-6-4}{RGB}{116,169,207}
\definecolor{PuBu-6-G}{RGB}{116,169,207}
\definecolor{PuBu-6-5}{RGB}{43,140,190}
\definecolor{PuBu-6-I}{RGB}{43,140,190}
\definecolor{PuBu-6-6}{RGB}{4,90,141}
\definecolor{PuBu-6-K}{RGB}{4,90,141}
\definecolor{PuBu-7-1}{RGB}{241,238,246}
\definecolor{PuBu-7-B}{RGB}{241,238,246}
\definecolor{PuBu-7-2}{RGB}{208,209,230}
\definecolor{PuBu-7-D}{RGB}{208,209,230}
\definecolor{PuBu-7-3}{RGB}{166,189,219}
\definecolor{PuBu-7-F}{RGB}{166,189,219}
\definecolor{PuBu-7-4}{RGB}{116,169,207}
\definecolor{PuBu-7-G}{RGB}{116,169,207}
\definecolor{PuBu-7-5}{RGB}{54,144,192}
\definecolor{PuBu-7-H}{RGB}{54,144,192}
\definecolor{PuBu-7-6}{RGB}{5,112,176}
\definecolor{PuBu-7-J}{RGB}{5,112,176}
\definecolor{PuBu-7-7}{RGB}{3,78,123}
\definecolor{PuBu-7-L}{RGB}{3,78,123}
\definecolor{PuBu-8-1}{RGB}{255,247,251}
\definecolor{PuBu-8-A}{RGB}{255,247,251}
\definecolor{PuBu-8-2}{RGB}{236,231,242}
\definecolor{PuBu-8-C}{RGB}{236,231,242}
\definecolor{PuBu-8-3}{RGB}{208,209,230}
\definecolor{PuBu-8-D}{RGB}{208,209,230}
\definecolor{PuBu-8-4}{RGB}{166,189,219}
\definecolor{PuBu-8-F}{RGB}{166,189,219}
\definecolor{PuBu-8-5}{RGB}{116,169,207}
\definecolor{PuBu-8-G}{RGB}{116,169,207}
\definecolor{PuBu-8-6}{RGB}{54,144,192}
\definecolor{PuBu-8-H}{RGB}{54,144,192}
\definecolor{PuBu-8-7}{RGB}{5,112,176}
\definecolor{PuBu-8-J}{RGB}{5,112,176}
\definecolor{PuBu-8-8}{RGB}{3,78,123}
\definecolor{PuBu-8-L}{RGB}{3,78,123}
\definecolor{PuBu-9-1}{RGB}{255,247,251}
\definecolor{PuBu-9-A}{RGB}{255,247,251}
\definecolor{PuBu-9-2}{RGB}{236,231,242}
\definecolor{PuBu-9-C}{RGB}{236,231,242}
\definecolor{PuBu-9-3}{RGB}{208,209,230}
\definecolor{PuBu-9-D}{RGB}{208,209,230}
\definecolor{PuBu-9-4}{RGB}{166,189,219}
\definecolor{PuBu-9-F}{RGB}{166,189,219}
\definecolor{PuBu-9-5}{RGB}{116,169,207}
\definecolor{PuBu-9-G}{RGB}{116,169,207}
\definecolor{PuBu-9-6}{RGB}{54,144,192}
\definecolor{PuBu-9-H}{RGB}{54,144,192}
\definecolor{PuBu-9-7}{RGB}{5,112,176}
\definecolor{PuBu-9-J}{RGB}{5,112,176}
\definecolor{PuBu-9-8}{RGB}{4,90,141}
\definecolor{PuBu-9-K}{RGB}{4,90,141}
\definecolor{PuBu-9-9}{RGB}{2,56,88}
\definecolor{PuBu-9-M}{RGB}{2,56,88}
\definecolor{BuPu-3-1}{RGB}{224,236,244}
\definecolor{BuPu-3-C}{RGB}{224,236,244}
\definecolor{BuPu-3-2}{RGB}{158,188,218}
\definecolor{BuPu-3-F}{RGB}{158,188,218}
\definecolor{BuPu-3-3}{RGB}{136,86,167}
\definecolor{BuPu-3-I}{RGB}{136,86,167}
\definecolor{BuPu-4-1}{RGB}{237,248,251}
\definecolor{BuPu-4-B}{RGB}{237,248,251}
\definecolor{BuPu-4-2}{RGB}{179,205,227}
\definecolor{BuPu-4-E}{RGB}{179,205,227}
\definecolor{BuPu-4-3}{RGB}{140,150,198}
\definecolor{BuPu-4-G}{RGB}{140,150,198}
\definecolor{BuPu-4-4}{RGB}{136,65,157}
\definecolor{BuPu-4-J}{RGB}{136,65,157}
\definecolor{BuPu-5-1}{RGB}{237,248,251}
\definecolor{BuPu-5-B}{RGB}{237,248,251}
\definecolor{BuPu-5-2}{RGB}{179,205,227}
\definecolor{BuPu-5-E}{RGB}{179,205,227}
\definecolor{BuPu-5-3}{RGB}{140,150,198}
\definecolor{BuPu-5-G}{RGB}{140,150,198}
\definecolor{BuPu-5-4}{RGB}{136,86,167}
\definecolor{BuPu-5-I}{RGB}{136,86,167}
\definecolor{BuPu-5-5}{RGB}{129,15,124}
\definecolor{BuPu-5-K}{RGB}{129,15,124}
\definecolor{BuPu-6-1}{RGB}{237,248,251}
\definecolor{BuPu-6-B}{RGB}{237,248,251}
\definecolor{BuPu-6-2}{RGB}{191,211,230}
\definecolor{BuPu-6-D}{RGB}{191,211,230}
\definecolor{BuPu-6-3}{RGB}{158,188,218}
\definecolor{BuPu-6-F}{RGB}{158,188,218}
\definecolor{BuPu-6-4}{RGB}{140,150,198}
\definecolor{BuPu-6-G}{RGB}{140,150,198}
\definecolor{BuPu-6-5}{RGB}{136,86,167}
\definecolor{BuPu-6-I}{RGB}{136,86,167}
\definecolor{BuPu-6-6}{RGB}{129,15,124}
\definecolor{BuPu-6-K}{RGB}{129,15,124}
\definecolor{BuPu-7-1}{RGB}{237,248,251}
\definecolor{BuPu-7-B}{RGB}{237,248,251}
\definecolor{BuPu-7-2}{RGB}{191,211,230}
\definecolor{BuPu-7-D}{RGB}{191,211,230}
\definecolor{BuPu-7-3}{RGB}{158,188,218}
\definecolor{BuPu-7-F}{RGB}{158,188,218}
\definecolor{BuPu-7-4}{RGB}{140,150,198}
\definecolor{BuPu-7-G}{RGB}{140,150,198}
\definecolor{BuPu-7-5}{RGB}{140,107,177}
\definecolor{BuPu-7-H}{RGB}{140,107,177}
\definecolor{BuPu-7-6}{RGB}{136,65,157}
\definecolor{BuPu-7-J}{RGB}{136,65,157}
\definecolor{BuPu-7-7}{RGB}{110,1,107}
\definecolor{BuPu-7-L}{RGB}{110,1,107}
\definecolor{BuPu-8-1}{RGB}{247,252,253}
\definecolor{BuPu-8-A}{RGB}{247,252,253}
\definecolor{BuPu-8-2}{RGB}{224,236,244}
\definecolor{BuPu-8-C}{RGB}{224,236,244}
\definecolor{BuPu-8-3}{RGB}{191,211,230}
\definecolor{BuPu-8-D}{RGB}{191,211,230}
\definecolor{BuPu-8-4}{RGB}{158,188,218}
\definecolor{BuPu-8-F}{RGB}{158,188,218}
\definecolor{BuPu-8-5}{RGB}{140,150,198}
\definecolor{BuPu-8-G}{RGB}{140,150,198}
\definecolor{BuPu-8-6}{RGB}{140,107,177}
\definecolor{BuPu-8-H}{RGB}{140,107,177}
\definecolor{BuPu-8-7}{RGB}{136,65,157}
\definecolor{BuPu-8-J}{RGB}{136,65,157}
\definecolor{BuPu-8-8}{RGB}{110,1,107}
\definecolor{BuPu-8-L}{RGB}{110,1,107}
\definecolor{BuPu-9-1}{RGB}{247,252,253}
\definecolor{BuPu-9-A}{RGB}{247,252,253}
\definecolor{BuPu-9-2}{RGB}{224,236,244}
\definecolor{BuPu-9-C}{RGB}{224,236,244}
\definecolor{BuPu-9-3}{RGB}{191,211,230}
\definecolor{BuPu-9-D}{RGB}{191,211,230}
\definecolor{BuPu-9-4}{RGB}{158,188,218}
\definecolor{BuPu-9-F}{RGB}{158,188,218}
\definecolor{BuPu-9-5}{RGB}{140,150,198}
\definecolor{BuPu-9-G}{RGB}{140,150,198}
\definecolor{BuPu-9-6}{RGB}{140,107,177}
\definecolor{BuPu-9-H}{RGB}{140,107,177}
\definecolor{BuPu-9-7}{RGB}{136,65,157}
\definecolor{BuPu-9-J}{RGB}{136,65,157}
\definecolor{BuPu-9-8}{RGB}{129,15,124}
\definecolor{BuPu-9-K}{RGB}{129,15,124}
\definecolor{BuPu-9-9}{RGB}{77,0,75}
\definecolor{BuPu-9-M}{RGB}{77,0,75}
\definecolor{RdPu-3-1}{RGB}{253,224,221}
\definecolor{RdPu-3-C}{RGB}{253,224,221}
\definecolor{RdPu-3-2}{RGB}{250,159,181}
\definecolor{RdPu-3-F}{RGB}{250,159,181}
\definecolor{RdPu-3-3}{RGB}{197,27,138}
\definecolor{RdPu-3-I}{RGB}{197,27,138}
\definecolor{RdPu-4-1}{RGB}{254,235,226}
\definecolor{RdPu-4-B}{RGB}{254,235,226}
\definecolor{RdPu-4-2}{RGB}{251,180,185}
\definecolor{RdPu-4-E}{RGB}{251,180,185}
\definecolor{RdPu-4-3}{RGB}{247,104,161}
\definecolor{RdPu-4-G}{RGB}{247,104,161}
\definecolor{RdPu-4-4}{RGB}{174,1,126}
\definecolor{RdPu-4-J}{RGB}{174,1,126}
\definecolor{RdPu-5-1}{RGB}{254,235,226}
\definecolor{RdPu-5-B}{RGB}{254,235,226}
\definecolor{RdPu-5-2}{RGB}{251,180,185}
\definecolor{RdPu-5-E}{RGB}{251,180,185}
\definecolor{RdPu-5-3}{RGB}{247,104,161}
\definecolor{RdPu-5-G}{RGB}{247,104,161}
\definecolor{RdPu-5-4}{RGB}{197,27,138}
\definecolor{RdPu-5-I}{RGB}{197,27,138}
\definecolor{RdPu-5-5}{RGB}{122,1,119}
\definecolor{RdPu-5-K}{RGB}{122,1,119}
\definecolor{RdPu-6-1}{RGB}{254,235,226}
\definecolor{RdPu-6-B}{RGB}{254,235,226}
\definecolor{RdPu-6-2}{RGB}{252,197,192}
\definecolor{RdPu-6-D}{RGB}{252,197,192}
\definecolor{RdPu-6-3}{RGB}{250,159,181}
\definecolor{RdPu-6-F}{RGB}{250,159,181}
\definecolor{RdPu-6-4}{RGB}{247,104,161}
\definecolor{RdPu-6-G}{RGB}{247,104,161}
\definecolor{RdPu-6-5}{RGB}{197,27,138}
\definecolor{RdPu-6-I}{RGB}{197,27,138}
\definecolor{RdPu-6-6}{RGB}{122,1,119}
\definecolor{RdPu-6-K}{RGB}{122,1,119}
\definecolor{RdPu-7-1}{RGB}{254,235,226}
\definecolor{RdPu-7-B}{RGB}{254,235,226}
\definecolor{RdPu-7-2}{RGB}{252,197,192}
\definecolor{RdPu-7-D}{RGB}{252,197,192}
\definecolor{RdPu-7-3}{RGB}{250,159,181}
\definecolor{RdPu-7-F}{RGB}{250,159,181}
\definecolor{RdPu-7-4}{RGB}{247,104,161}
\definecolor{RdPu-7-G}{RGB}{247,104,161}
\definecolor{RdPu-7-5}{RGB}{221,52,151}
\definecolor{RdPu-7-H}{RGB}{221,52,151}
\definecolor{RdPu-7-6}{RGB}{174,1,126}
\definecolor{RdPu-7-J}{RGB}{174,1,126}
\definecolor{RdPu-7-7}{RGB}{122,1,119}
\definecolor{RdPu-7-L}{RGB}{122,1,119}
\definecolor{RdPu-8-1}{RGB}{255,247,243}
\definecolor{RdPu-8-A}{RGB}{255,247,243}
\definecolor{RdPu-8-2}{RGB}{253,224,221}
\definecolor{RdPu-8-C}{RGB}{253,224,221}
\definecolor{RdPu-8-3}{RGB}{252,197,192}
\definecolor{RdPu-8-D}{RGB}{252,197,192}
\definecolor{RdPu-8-4}{RGB}{250,159,181}
\definecolor{RdPu-8-F}{RGB}{250,159,181}
\definecolor{RdPu-8-5}{RGB}{247,104,161}
\definecolor{RdPu-8-G}{RGB}{247,104,161}
\definecolor{RdPu-8-6}{RGB}{221,52,151}
\definecolor{RdPu-8-H}{RGB}{221,52,151}
\definecolor{RdPu-8-7}{RGB}{174,1,126}
\definecolor{RdPu-8-J}{RGB}{174,1,126}
\definecolor{RdPu-8-8}{RGB}{122,1,119}
\definecolor{RdPu-8-L}{RGB}{122,1,119}
\definecolor{RdPu-9-1}{RGB}{255,247,243}
\definecolor{RdPu-9-A}{RGB}{255,247,243}
\definecolor{RdPu-9-2}{RGB}{253,224,221}
\definecolor{RdPu-9-C}{RGB}{253,224,221}
\definecolor{RdPu-9-3}{RGB}{252,197,192}
\definecolor{RdPu-9-D}{RGB}{252,197,192}
\definecolor{RdPu-9-4}{RGB}{250,159,181}
\definecolor{RdPu-9-F}{RGB}{250,159,181}
\definecolor{RdPu-9-5}{RGB}{247,104,161}
\definecolor{RdPu-9-G}{RGB}{247,104,161}
\definecolor{RdPu-9-6}{RGB}{221,52,151}
\definecolor{RdPu-9-H}{RGB}{221,52,151}
\definecolor{RdPu-9-7}{RGB}{174,1,126}
\definecolor{RdPu-9-J}{RGB}{174,1,126}
\definecolor{RdPu-9-8}{RGB}{122,1,119}
\definecolor{RdPu-9-K}{RGB}{122,1,119}
\definecolor{RdPu-9-9}{RGB}{73,0,106}
\definecolor{RdPu-9-M}{RGB}{73,0,106}
\definecolor{PuRd-3-1}{RGB}{231,225,239}
\definecolor{PuRd-3-C}{RGB}{231,225,239}
\definecolor{PuRd-3-2}{RGB}{201,148,199}
\definecolor{PuRd-3-F}{RGB}{201,148,199}
\definecolor{PuRd-3-3}{RGB}{221,28,119}
\definecolor{PuRd-3-I}{RGB}{221,28,119}
\definecolor{PuRd-4-1}{RGB}{241,238,246}
\definecolor{PuRd-4-B}{RGB}{241,238,246}
\definecolor{PuRd-4-2}{RGB}{215,181,216}
\definecolor{PuRd-4-E}{RGB}{215,181,216}
\definecolor{PuRd-4-3}{RGB}{223,101,176}
\definecolor{PuRd-4-G}{RGB}{223,101,176}
\definecolor{PuRd-4-4}{RGB}{206,18,86}
\definecolor{PuRd-4-J}{RGB}{206,18,86}
\definecolor{PuRd-5-1}{RGB}{241,238,246}
\definecolor{PuRd-5-B}{RGB}{241,238,246}
\definecolor{PuRd-5-2}{RGB}{215,181,216}
\definecolor{PuRd-5-E}{RGB}{215,181,216}
\definecolor{PuRd-5-3}{RGB}{223,101,176}
\definecolor{PuRd-5-G}{RGB}{223,101,176}
\definecolor{PuRd-5-4}{RGB}{221,28,119}
\definecolor{PuRd-5-I}{RGB}{221,28,119}
\definecolor{PuRd-5-5}{RGB}{152,0,67}
\definecolor{PuRd-5-K}{RGB}{152,0,67}
\definecolor{PuRd-6-1}{RGB}{241,238,246}
\definecolor{PuRd-6-B}{RGB}{241,238,246}
\definecolor{PuRd-6-2}{RGB}{212,185,218}
\definecolor{PuRd-6-D}{RGB}{212,185,218}
\definecolor{PuRd-6-3}{RGB}{201,148,199}
\definecolor{PuRd-6-F}{RGB}{201,148,199}
\definecolor{PuRd-6-4}{RGB}{223,101,176}
\definecolor{PuRd-6-G}{RGB}{223,101,176}
\definecolor{PuRd-6-5}{RGB}{221,28,119}
\definecolor{PuRd-6-I}{RGB}{221,28,119}
\definecolor{PuRd-6-6}{RGB}{152,0,67}
\definecolor{PuRd-6-K}{RGB}{152,0,67}
\definecolor{PuRd-7-1}{RGB}{241,238,246}
\definecolor{PuRd-7-B}{RGB}{241,238,246}
\definecolor{PuRd-7-2}{RGB}{212,185,218}
\definecolor{PuRd-7-D}{RGB}{212,185,218}
\definecolor{PuRd-7-3}{RGB}{201,148,199}
\definecolor{PuRd-7-F}{RGB}{201,148,199}
\definecolor{PuRd-7-4}{RGB}{223,101,176}
\definecolor{PuRd-7-G}{RGB}{223,101,176}
\definecolor{PuRd-7-5}{RGB}{231,41,138}
\definecolor{PuRd-7-H}{RGB}{231,41,138}
\definecolor{PuRd-7-6}{RGB}{206,18,86}
\definecolor{PuRd-7-J}{RGB}{206,18,86}
\definecolor{PuRd-7-7}{RGB}{145,0,63}
\definecolor{PuRd-7-L}{RGB}{145,0,63}
\definecolor{PuRd-8-1}{RGB}{247,244,249}
\definecolor{PuRd-8-A}{RGB}{247,244,249}
\definecolor{PuRd-8-2}{RGB}{231,225,239}
\definecolor{PuRd-8-C}{RGB}{231,225,239}
\definecolor{PuRd-8-3}{RGB}{212,185,218}
\definecolor{PuRd-8-D}{RGB}{212,185,218}
\definecolor{PuRd-8-4}{RGB}{201,148,199}
\definecolor{PuRd-8-F}{RGB}{201,148,199}
\definecolor{PuRd-8-5}{RGB}{223,101,176}
\definecolor{PuRd-8-G}{RGB}{223,101,176}
\definecolor{PuRd-8-6}{RGB}{231,41,138}
\definecolor{PuRd-8-H}{RGB}{231,41,138}
\definecolor{PuRd-8-7}{RGB}{206,18,86}
\definecolor{PuRd-8-J}{RGB}{206,18,86}
\definecolor{PuRd-8-8}{RGB}{145,0,63}
\definecolor{PuRd-8-L}{RGB}{145,0,63}
\definecolor{PuRd-9-1}{RGB}{247,244,249}
\definecolor{PuRd-9-A}{RGB}{247,244,249}
\definecolor{PuRd-9-2}{RGB}{231,225,239}
\definecolor{PuRd-9-C}{RGB}{231,225,239}
\definecolor{PuRd-9-3}{RGB}{212,185,218}
\definecolor{PuRd-9-D}{RGB}{212,185,218}
\definecolor{PuRd-9-4}{RGB}{201,148,199}
\definecolor{PuRd-9-F}{RGB}{201,148,199}
\definecolor{PuRd-9-5}{RGB}{223,101,176}
\definecolor{PuRd-9-G}{RGB}{223,101,176}
\definecolor{PuRd-9-6}{RGB}{231,41,138}
\definecolor{PuRd-9-H}{RGB}{231,41,138}
\definecolor{PuRd-9-7}{RGB}{206,18,86}
\definecolor{PuRd-9-J}{RGB}{206,18,86}
\definecolor{PuRd-9-8}{RGB}{152,0,67}
\definecolor{PuRd-9-K}{RGB}{152,0,67}
\definecolor{PuRd-9-9}{RGB}{103,0,31}
\definecolor{PuRd-9-M}{RGB}{103,0,31}
\definecolor{OrRd-3-1}{RGB}{254,232,200}
\definecolor{OrRd-3-C}{RGB}{254,232,200}
\definecolor{OrRd-3-2}{RGB}{253,187,132}
\definecolor{OrRd-3-F}{RGB}{253,187,132}
\definecolor{OrRd-3-3}{RGB}{227,74,51}
\definecolor{OrRd-3-I}{RGB}{227,74,51}
\definecolor{OrRd-4-1}{RGB}{254,240,217}
\definecolor{OrRd-4-B}{RGB}{254,240,217}
\definecolor{OrRd-4-2}{RGB}{253,204,138}
\definecolor{OrRd-4-E}{RGB}{253,204,138}
\definecolor{OrRd-4-3}{RGB}{252,141,89}
\definecolor{OrRd-4-G}{RGB}{252,141,89}
\definecolor{OrRd-4-4}{RGB}{215,48,31}
\definecolor{OrRd-4-J}{RGB}{215,48,31}
\definecolor{OrRd-5-1}{RGB}{254,240,217}
\definecolor{OrRd-5-B}{RGB}{254,240,217}
\definecolor{OrRd-5-2}{RGB}{253,204,138}
\definecolor{OrRd-5-E}{RGB}{253,204,138}
\definecolor{OrRd-5-3}{RGB}{252,141,89}
\definecolor{OrRd-5-G}{RGB}{252,141,89}
\definecolor{OrRd-5-4}{RGB}{227,74,51}
\definecolor{OrRd-5-I}{RGB}{227,74,51}
\definecolor{OrRd-5-5}{RGB}{179,0,0}
\definecolor{OrRd-5-K}{RGB}{179,0,0}
\definecolor{OrRd-6-1}{RGB}{254,240,217}
\definecolor{OrRd-6-B}{RGB}{254,240,217}
\definecolor{OrRd-6-2}{RGB}{253,212,158}
\definecolor{OrRd-6-D}{RGB}{253,212,158}
\definecolor{OrRd-6-3}{RGB}{253,187,132}
\definecolor{OrRd-6-F}{RGB}{253,187,132}
\definecolor{OrRd-6-4}{RGB}{252,141,89}
\definecolor{OrRd-6-G}{RGB}{252,141,89}
\definecolor{OrRd-6-5}{RGB}{227,74,51}
\definecolor{OrRd-6-I}{RGB}{227,74,51}
\definecolor{OrRd-6-6}{RGB}{179,0,0}
\definecolor{OrRd-6-K}{RGB}{179,0,0}
\definecolor{OrRd-7-1}{RGB}{254,240,217}
\definecolor{OrRd-7-B}{RGB}{254,240,217}
\definecolor{OrRd-7-2}{RGB}{253,212,158}
\definecolor{OrRd-7-D}{RGB}{253,212,158}
\definecolor{OrRd-7-3}{RGB}{253,187,132}
\definecolor{OrRd-7-F}{RGB}{253,187,132}
\definecolor{OrRd-7-4}{RGB}{252,141,89}
\definecolor{OrRd-7-G}{RGB}{252,141,89}
\definecolor{OrRd-7-5}{RGB}{239,101,72}
\definecolor{OrRd-7-H}{RGB}{239,101,72}
\definecolor{OrRd-7-6}{RGB}{215,48,31}
\definecolor{OrRd-7-J}{RGB}{215,48,31}
\definecolor{OrRd-7-7}{RGB}{153,0,0}
\definecolor{OrRd-7-L}{RGB}{153,0,0}
\definecolor{OrRd-8-1}{RGB}{255,247,236}
\definecolor{OrRd-8-A}{RGB}{255,247,236}
\definecolor{OrRd-8-2}{RGB}{254,232,200}
\definecolor{OrRd-8-C}{RGB}{254,232,200}
\definecolor{OrRd-8-3}{RGB}{253,212,158}
\definecolor{OrRd-8-D}{RGB}{253,212,158}
\definecolor{OrRd-8-4}{RGB}{253,187,132}
\definecolor{OrRd-8-F}{RGB}{253,187,132}
\definecolor{OrRd-8-5}{RGB}{252,141,89}
\definecolor{OrRd-8-G}{RGB}{252,141,89}
\definecolor{OrRd-8-6}{RGB}{239,101,72}
\definecolor{OrRd-8-H}{RGB}{239,101,72}
\definecolor{OrRd-8-7}{RGB}{215,48,31}
\definecolor{OrRd-8-J}{RGB}{215,48,31}
\definecolor{OrRd-8-8}{RGB}{153,0,0}
\definecolor{OrRd-8-L}{RGB}{153,0,0}
\definecolor{OrRd-9-1}{RGB}{255,247,236}
\definecolor{OrRd-9-A}{RGB}{255,247,236}
\definecolor{OrRd-9-2}{RGB}{254,232,200}
\definecolor{OrRd-9-C}{RGB}{254,232,200}
\definecolor{OrRd-9-3}{RGB}{253,212,158}
\definecolor{OrRd-9-D}{RGB}{253,212,158}
\definecolor{OrRd-9-4}{RGB}{253,187,132}
\definecolor{OrRd-9-F}{RGB}{253,187,132}
\definecolor{OrRd-9-5}{RGB}{252,141,89}
\definecolor{OrRd-9-G}{RGB}{252,141,89}
\definecolor{OrRd-9-6}{RGB}{239,101,72}
\definecolor{OrRd-9-H}{RGB}{239,101,72}
\definecolor{OrRd-9-7}{RGB}{215,48,31}
\definecolor{OrRd-9-J}{RGB}{215,48,31}
\definecolor{OrRd-9-8}{RGB}{179,0,0}
\definecolor{OrRd-9-K}{RGB}{179,0,0}
\definecolor{OrRd-9-9}{RGB}{127,0,0}
\definecolor{OrRd-9-M}{RGB}{127,0,0}
\definecolor{YlOrRd-3-1}{RGB}{255,237,160}
\definecolor{YlOrRd-3-C}{RGB}{255,237,160}
\definecolor{YlOrRd-3-2}{RGB}{254,178,76}
\definecolor{YlOrRd-3-F}{RGB}{254,178,76}
\definecolor{YlOrRd-3-3}{RGB}{240,59,32}
\definecolor{YlOrRd-3-I}{RGB}{240,59,32}
\definecolor{YlOrRd-4-1}{RGB}{255,255,178}
\definecolor{YlOrRd-4-B}{RGB}{255,255,178}
\definecolor{YlOrRd-4-2}{RGB}{254,204,92}
\definecolor{YlOrRd-4-E}{RGB}{254,204,92}
\definecolor{YlOrRd-4-3}{RGB}{253,141,60}
\definecolor{YlOrRd-4-G}{RGB}{253,141,60}
\definecolor{YlOrRd-4-4}{RGB}{227,26,28}
\definecolor{YlOrRd-4-J}{RGB}{227,26,28}
\definecolor{YlOrRd-5-1}{RGB}{255,255,178}
\definecolor{YlOrRd-5-B}{RGB}{255,255,178}
\definecolor{YlOrRd-5-2}{RGB}{254,204,92}
\definecolor{YlOrRd-5-E}{RGB}{254,204,92}
\definecolor{YlOrRd-5-3}{RGB}{253,141,60}
\definecolor{YlOrRd-5-G}{RGB}{253,141,60}
\definecolor{YlOrRd-5-4}{RGB}{240,59,32}
\definecolor{YlOrRd-5-I}{RGB}{240,59,32}
\definecolor{YlOrRd-5-5}{RGB}{189,0,38}
\definecolor{YlOrRd-5-K}{RGB}{189,0,38}
\definecolor{YlOrRd-6-1}{RGB}{255,255,178}
\definecolor{YlOrRd-6-B}{RGB}{255,255,178}
\definecolor{YlOrRd-6-2}{RGB}{254,217,118}
\definecolor{YlOrRd-6-D}{RGB}{254,217,118}
\definecolor{YlOrRd-6-3}{RGB}{254,178,76}
\definecolor{YlOrRd-6-F}{RGB}{254,178,76}
\definecolor{YlOrRd-6-4}{RGB}{253,141,60}
\definecolor{YlOrRd-6-G}{RGB}{253,141,60}
\definecolor{YlOrRd-6-5}{RGB}{240,59,32}
\definecolor{YlOrRd-6-I}{RGB}{240,59,32}
\definecolor{YlOrRd-6-6}{RGB}{189,0,38}
\definecolor{YlOrRd-6-K}{RGB}{189,0,38}
\definecolor{YlOrRd-7-1}{RGB}{255,255,178}
\definecolor{YlOrRd-7-B}{RGB}{255,255,178}
\definecolor{YlOrRd-7-2}{RGB}{254,217,118}
\definecolor{YlOrRd-7-D}{RGB}{254,217,118}
\definecolor{YlOrRd-7-3}{RGB}{254,178,76}
\definecolor{YlOrRd-7-F}{RGB}{254,178,76}
\definecolor{YlOrRd-7-4}{RGB}{253,141,60}
\definecolor{YlOrRd-7-G}{RGB}{253,141,60}
\definecolor{YlOrRd-7-5}{RGB}{252,78,42}
\definecolor{YlOrRd-7-H}{RGB}{252,78,42}
\definecolor{YlOrRd-7-6}{RGB}{227,26,28}
\definecolor{YlOrRd-7-J}{RGB}{227,26,28}
\definecolor{YlOrRd-7-7}{RGB}{177,0,38}
\definecolor{YlOrRd-7-L}{RGB}{177,0,38}
\definecolor{YlOrRd-8-1}{RGB}{255,255,204}
\definecolor{YlOrRd-8-A}{RGB}{255,255,204}
\definecolor{YlOrRd-8-2}{RGB}{255,237,160}
\definecolor{YlOrRd-8-C}{RGB}{255,237,160}
\definecolor{YlOrRd-8-3}{RGB}{254,217,118}
\definecolor{YlOrRd-8-D}{RGB}{254,217,118}
\definecolor{YlOrRd-8-4}{RGB}{254,178,76}
\definecolor{YlOrRd-8-F}{RGB}{254,178,76}
\definecolor{YlOrRd-8-5}{RGB}{253,141,60}
\definecolor{YlOrRd-8-G}{RGB}{253,141,60}
\definecolor{YlOrRd-8-6}{RGB}{252,78,42}
\definecolor{YlOrRd-8-H}{RGB}{252,78,42}
\definecolor{YlOrRd-8-7}{RGB}{227,26,28}
\definecolor{YlOrRd-8-J}{RGB}{227,26,28}
\definecolor{YlOrRd-8-8}{RGB}{177,0,38}
\definecolor{YlOrRd-8-L}{RGB}{177,0,38}
\definecolor{YlOrRd-9-1}{RGB}{255,255,204}
\definecolor{YlOrRd-9-A}{RGB}{255,255,204}
\definecolor{YlOrRd-9-2}{RGB}{255,237,160}
\definecolor{YlOrRd-9-C}{RGB}{255,237,160}
\definecolor{YlOrRd-9-3}{RGB}{254,217,118}
\definecolor{YlOrRd-9-D}{RGB}{254,217,118}
\definecolor{YlOrRd-9-4}{RGB}{254,178,76}
\definecolor{YlOrRd-9-F}{RGB}{254,178,76}
\definecolor{YlOrRd-9-5}{RGB}{253,141,60}
\definecolor{YlOrRd-9-G}{RGB}{253,141,60}
\definecolor{YlOrRd-9-6}{RGB}{252,78,42}
\definecolor{YlOrRd-9-H}{RGB}{252,78,42}
\definecolor{YlOrRd-9-7}{RGB}{227,26,28}
\definecolor{YlOrRd-9-J}{RGB}{227,26,28}
\definecolor{YlOrRd-9-8}{RGB}{189,0,38}
\definecolor{YlOrRd-9-K}{RGB}{189,0,38}
\definecolor{YlOrRd-9-9}{RGB}{128,0,38}
\definecolor{YlOrRd-9-M}{RGB}{128,0,38}
\definecolor{YlOrBr-3-1}{RGB}{255,247,188}
\definecolor{YlOrBr-3-C}{RGB}{255,247,188}
\definecolor{YlOrBr-3-2}{RGB}{254,196,79}
\definecolor{YlOrBr-3-F}{RGB}{254,196,79}
\definecolor{YlOrBr-3-3}{RGB}{217,95,14}
\definecolor{YlOrBr-3-I}{RGB}{217,95,14}
\definecolor{YlOrBr-4-1}{RGB}{255,255,212}
\definecolor{YlOrBr-4-B}{RGB}{255,255,212}
\definecolor{YlOrBr-4-2}{RGB}{254,217,142}
\definecolor{YlOrBr-4-E}{RGB}{254,217,142}
\definecolor{YlOrBr-4-3}{RGB}{254,153,41}
\definecolor{YlOrBr-4-G}{RGB}{254,153,41}
\definecolor{YlOrBr-4-4}{RGB}{204,76,2}
\definecolor{YlOrBr-4-J}{RGB}{204,76,2}
\definecolor{YlOrBr-5-1}{RGB}{255,255,212}
\definecolor{YlOrBr-5-B}{RGB}{255,255,212}
\definecolor{YlOrBr-5-2}{RGB}{254,217,142}
\definecolor{YlOrBr-5-E}{RGB}{254,217,142}
\definecolor{YlOrBr-5-3}{RGB}{254,153,41}
\definecolor{YlOrBr-5-G}{RGB}{254,153,41}
\definecolor{YlOrBr-5-4}{RGB}{217,95,14}
\definecolor{YlOrBr-5-I}{RGB}{217,95,14}
\definecolor{YlOrBr-5-5}{RGB}{153,52,4}
\definecolor{YlOrBr-5-K}{RGB}{153,52,4}
\definecolor{YlOrBr-6-1}{RGB}{255,255,212}
\definecolor{YlOrBr-6-B}{RGB}{255,255,212}
\definecolor{YlOrBr-6-2}{RGB}{254,227,145}
\definecolor{YlOrBr-6-D}{RGB}{254,227,145}
\definecolor{YlOrBr-6-3}{RGB}{254,196,79}
\definecolor{YlOrBr-6-F}{RGB}{254,196,79}
\definecolor{YlOrBr-6-4}{RGB}{254,153,41}
\definecolor{YlOrBr-6-G}{RGB}{254,153,41}
\definecolor{YlOrBr-6-5}{RGB}{217,95,14}
\definecolor{YlOrBr-6-I}{RGB}{217,95,14}
\definecolor{YlOrBr-6-6}{RGB}{153,52,4}
\definecolor{YlOrBr-6-K}{RGB}{153,52,4}
\definecolor{YlOrBr-7-1}{RGB}{255,255,212}
\definecolor{YlOrBr-7-B}{RGB}{255,255,212}
\definecolor{YlOrBr-7-2}{RGB}{254,227,145}
\definecolor{YlOrBr-7-D}{RGB}{254,227,145}
\definecolor{YlOrBr-7-3}{RGB}{254,196,79}
\definecolor{YlOrBr-7-F}{RGB}{254,196,79}
\definecolor{YlOrBr-7-4}{RGB}{254,153,41}
\definecolor{YlOrBr-7-G}{RGB}{254,153,41}
\definecolor{YlOrBr-7-5}{RGB}{236,112,20}
\definecolor{YlOrBr-7-H}{RGB}{236,112,20}
\definecolor{YlOrBr-7-6}{RGB}{204,76,2}
\definecolor{YlOrBr-7-J}{RGB}{204,76,2}
\definecolor{YlOrBr-7-7}{RGB}{140,45,4}
\definecolor{YlOrBr-7-L}{RGB}{140,45,4}
\definecolor{YlOrBr-8-1}{RGB}{255,255,229}
\definecolor{YlOrBr-8-A}{RGB}{255,255,229}
\definecolor{YlOrBr-8-2}{RGB}{255,247,188}
\definecolor{YlOrBr-8-C}{RGB}{255,247,188}
\definecolor{YlOrBr-8-3}{RGB}{254,227,145}
\definecolor{YlOrBr-8-D}{RGB}{254,227,145}
\definecolor{YlOrBr-8-4}{RGB}{254,196,79}
\definecolor{YlOrBr-8-F}{RGB}{254,196,79}
\definecolor{YlOrBr-8-5}{RGB}{254,153,41}
\definecolor{YlOrBr-8-G}{RGB}{254,153,41}
\definecolor{YlOrBr-8-6}{RGB}{236,112,20}
\definecolor{YlOrBr-8-H}{RGB}{236,112,20}
\definecolor{YlOrBr-8-7}{RGB}{204,76,2}
\definecolor{YlOrBr-8-J}{RGB}{204,76,2}
\definecolor{YlOrBr-8-8}{RGB}{140,45,4}
\definecolor{YlOrBr-8-L}{RGB}{140,45,4}
\definecolor{YlOrBr-9-1}{RGB}{255,255,229}
\definecolor{YlOrBr-9-A}{RGB}{255,255,229}
\definecolor{YlOrBr-9-2}{RGB}{255,247,188}
\definecolor{YlOrBr-9-C}{RGB}{255,247,188}
\definecolor{YlOrBr-9-3}{RGB}{254,227,145}
\definecolor{YlOrBr-9-D}{RGB}{254,227,145}
\definecolor{YlOrBr-9-4}{RGB}{254,196,79}
\definecolor{YlOrBr-9-F}{RGB}{254,196,79}
\definecolor{YlOrBr-9-5}{RGB}{254,153,41}
\definecolor{YlOrBr-9-G}{RGB}{254,153,41}
\definecolor{YlOrBr-9-6}{RGB}{236,112,20}
\definecolor{YlOrBr-9-H}{RGB}{236,112,20}
\definecolor{YlOrBr-9-7}{RGB}{204,76,2}
\definecolor{YlOrBr-9-J}{RGB}{204,76,2}
\definecolor{YlOrBr-9-8}{RGB}{153,52,4}
\definecolor{YlOrBr-9-K}{RGB}{153,52,4}
\definecolor{YlOrBr-9-9}{RGB}{102,37,6}
\definecolor{YlOrBr-9-M}{RGB}{102,37,6}
\definecolor{Purples-3-1}{RGB}{239,237,245}
\definecolor{Purples-3-C}{RGB}{239,237,245}
\definecolor{Purples-3-2}{RGB}{188,189,220}
\definecolor{Purples-3-F}{RGB}{188,189,220}
\definecolor{Purples-3-3}{RGB}{117,107,177}
\definecolor{Purples-3-I}{RGB}{117,107,177}
\definecolor{Purples-4-1}{RGB}{242,240,247}
\definecolor{Purples-4-B}{RGB}{242,240,247}
\definecolor{Purples-4-2}{RGB}{203,201,226}
\definecolor{Purples-4-E}{RGB}{203,201,226}
\definecolor{Purples-4-3}{RGB}{158,154,200}
\definecolor{Purples-4-G}{RGB}{158,154,200}
\definecolor{Purples-4-4}{RGB}{106,81,163}
\definecolor{Purples-4-J}{RGB}{106,81,163}
\definecolor{Purples-5-1}{RGB}{242,240,247}
\definecolor{Purples-5-B}{RGB}{242,240,247}
\definecolor{Purples-5-2}{RGB}{203,201,226}
\definecolor{Purples-5-E}{RGB}{203,201,226}
\definecolor{Purples-5-3}{RGB}{158,154,200}
\definecolor{Purples-5-G}{RGB}{158,154,200}
\definecolor{Purples-5-4}{RGB}{117,107,177}
\definecolor{Purples-5-I}{RGB}{117,107,177}
\definecolor{Purples-5-5}{RGB}{84,39,143}
\definecolor{Purples-5-K}{RGB}{84,39,143}
\definecolor{Purples-6-1}{RGB}{242,240,247}
\definecolor{Purples-6-B}{RGB}{242,240,247}
\definecolor{Purples-6-2}{RGB}{218,218,235}
\definecolor{Purples-6-D}{RGB}{218,218,235}
\definecolor{Purples-6-3}{RGB}{188,189,220}
\definecolor{Purples-6-F}{RGB}{188,189,220}
\definecolor{Purples-6-4}{RGB}{158,154,200}
\definecolor{Purples-6-G}{RGB}{158,154,200}
\definecolor{Purples-6-5}{RGB}{117,107,177}
\definecolor{Purples-6-I}{RGB}{117,107,177}
\definecolor{Purples-6-6}{RGB}{84,39,143}
\definecolor{Purples-6-K}{RGB}{84,39,143}
\definecolor{Purples-7-1}{RGB}{242,240,247}
\definecolor{Purples-7-B}{RGB}{242,240,247}
\definecolor{Purples-7-2}{RGB}{218,218,235}
\definecolor{Purples-7-D}{RGB}{218,218,235}
\definecolor{Purples-7-3}{RGB}{188,189,220}
\definecolor{Purples-7-F}{RGB}{188,189,220}
\definecolor{Purples-7-4}{RGB}{158,154,200}
\definecolor{Purples-7-G}{RGB}{158,154,200}
\definecolor{Purples-7-5}{RGB}{128,125,186}
\definecolor{Purples-7-H}{RGB}{128,125,186}
\definecolor{Purples-7-6}{RGB}{106,81,163}
\definecolor{Purples-7-J}{RGB}{106,81,163}
\definecolor{Purples-7-7}{RGB}{74,20,134}
\definecolor{Purples-7-L}{RGB}{74,20,134}
\definecolor{Purples-8-1}{RGB}{252,251,253}
\definecolor{Purples-8-A}{RGB}{252,251,253}
\definecolor{Purples-8-2}{RGB}{239,237,245}
\definecolor{Purples-8-C}{RGB}{239,237,245}
\definecolor{Purples-8-3}{RGB}{218,218,235}
\definecolor{Purples-8-D}{RGB}{218,218,235}
\definecolor{Purples-8-4}{RGB}{188,189,220}
\definecolor{Purples-8-F}{RGB}{188,189,220}
\definecolor{Purples-8-5}{RGB}{158,154,200}
\definecolor{Purples-8-G}{RGB}{158,154,200}
\definecolor{Purples-8-6}{RGB}{128,125,186}
\definecolor{Purples-8-H}{RGB}{128,125,186}
\definecolor{Purples-8-7}{RGB}{106,81,163}
\definecolor{Purples-8-J}{RGB}{106,81,163}
\definecolor{Purples-8-8}{RGB}{74,20,134}
\definecolor{Purples-8-L}{RGB}{74,20,134}
\definecolor{Purples-9-1}{RGB}{252,251,253}
\definecolor{Purples-9-A}{RGB}{252,251,253}
\definecolor{Purples-9-2}{RGB}{239,237,245}
\definecolor{Purples-9-C}{RGB}{239,237,245}
\definecolor{Purples-9-3}{RGB}{218,218,235}
\definecolor{Purples-9-D}{RGB}{218,218,235}
\definecolor{Purples-9-4}{RGB}{188,189,220}
\definecolor{Purples-9-F}{RGB}{188,189,220}
\definecolor{Purples-9-5}{RGB}{158,154,200}
\definecolor{Purples-9-G}{RGB}{158,154,200}
\definecolor{Purples-9-6}{RGB}{128,125,186}
\definecolor{Purples-9-H}{RGB}{128,125,186}
\definecolor{Purples-9-7}{RGB}{106,81,163}
\definecolor{Purples-9-J}{RGB}{106,81,163}
\definecolor{Purples-9-8}{RGB}{84,39,143}
\definecolor{Purples-9-K}{RGB}{84,39,143}
\definecolor{Purples-9-9}{RGB}{63,0,125}
\definecolor{Purples-9-M}{RGB}{63,0,125}
\definecolor{Blues-3-1}{RGB}{222,235,247}
\definecolor{Blues-3-C}{RGB}{222,235,247}
\definecolor{Blues-3-2}{RGB}{158,202,225}
\definecolor{Blues-3-F}{RGB}{158,202,225}
\definecolor{Blues-3-3}{RGB}{49,130,189}
\definecolor{Blues-3-I}{RGB}{49,130,189}
\definecolor{Blues-4-1}{RGB}{239,243,255}
\definecolor{Blues-4-B}{RGB}{239,243,255}
\definecolor{Blues-4-2}{RGB}{189,215,231}
\definecolor{Blues-4-E}{RGB}{189,215,231}
\definecolor{Blues-4-3}{RGB}{107,174,214}
\definecolor{Blues-4-G}{RGB}{107,174,214}
\definecolor{Blues-4-4}{RGB}{33,113,181}
\definecolor{Blues-4-J}{RGB}{33,113,181}
\definecolor{Blues-5-1}{RGB}{239,243,255}
\definecolor{Blues-5-B}{RGB}{239,243,255}
\definecolor{Blues-5-2}{RGB}{189,215,231}
\definecolor{Blues-5-E}{RGB}{189,215,231}
\definecolor{Blues-5-3}{RGB}{107,174,214}
\definecolor{Blues-5-G}{RGB}{107,174,214}
\definecolor{Blues-5-4}{RGB}{49,130,189}
\definecolor{Blues-5-I}{RGB}{49,130,189}
\definecolor{Blues-5-5}{RGB}{8,81,156}
\definecolor{Blues-5-K}{RGB}{8,81,156}
\definecolor{Blues-6-1}{RGB}{239,243,255}
\definecolor{Blues-6-B}{RGB}{239,243,255}
\definecolor{Blues-6-2}{RGB}{198,219,239}
\definecolor{Blues-6-D}{RGB}{198,219,239}
\definecolor{Blues-6-3}{RGB}{158,202,225}
\definecolor{Blues-6-F}{RGB}{158,202,225}
\definecolor{Blues-6-4}{RGB}{107,174,214}
\definecolor{Blues-6-G}{RGB}{107,174,214}
\definecolor{Blues-6-5}{RGB}{49,130,189}
\definecolor{Blues-6-I}{RGB}{49,130,189}
\definecolor{Blues-6-6}{RGB}{8,81,156}
\definecolor{Blues-6-K}{RGB}{8,81,156}
\definecolor{Blues-7-1}{RGB}{239,243,255}
\definecolor{Blues-7-B}{RGB}{239,243,255}
\definecolor{Blues-7-2}{RGB}{198,219,239}
\definecolor{Blues-7-D}{RGB}{198,219,239}
\definecolor{Blues-7-3}{RGB}{158,202,225}
\definecolor{Blues-7-F}{RGB}{158,202,225}
\definecolor{Blues-7-4}{RGB}{107,174,214}
\definecolor{Blues-7-G}{RGB}{107,174,214}
\definecolor{Blues-7-5}{RGB}{66,146,198}
\definecolor{Blues-7-H}{RGB}{66,146,198}
\definecolor{Blues-7-6}{RGB}{33,113,181}
\definecolor{Blues-7-J}{RGB}{33,113,181}
\definecolor{Blues-7-7}{RGB}{8,69,148}
\definecolor{Blues-7-L}{RGB}{8,69,148}
\definecolor{Blues-8-1}{RGB}{247,251,255}
\definecolor{Blues-8-A}{RGB}{247,251,255}
\definecolor{Blues-8-2}{RGB}{222,235,247}
\definecolor{Blues-8-C}{RGB}{222,235,247}
\definecolor{Blues-8-3}{RGB}{198,219,239}
\definecolor{Blues-8-D}{RGB}{198,219,239}
\definecolor{Blues-8-4}{RGB}{158,202,225}
\definecolor{Blues-8-F}{RGB}{158,202,225}
\definecolor{Blues-8-5}{RGB}{107,174,214}
\definecolor{Blues-8-G}{RGB}{107,174,214}
\definecolor{Blues-8-6}{RGB}{66,146,198}
\definecolor{Blues-8-H}{RGB}{66,146,198}
\definecolor{Blues-8-7}{RGB}{33,113,181}
\definecolor{Blues-8-J}{RGB}{33,113,181}
\definecolor{Blues-8-8}{RGB}{8,69,148}
\definecolor{Blues-8-L}{RGB}{8,69,148}
\definecolor{Blues-9-1}{RGB}{247,251,255}
\definecolor{Blues-9-A}{RGB}{247,251,255}
\definecolor{Blues-9-2}{RGB}{222,235,247}
\definecolor{Blues-9-C}{RGB}{222,235,247}
\definecolor{Blues-9-3}{RGB}{198,219,239}
\definecolor{Blues-9-D}{RGB}{198,219,239}
\definecolor{Blues-9-4}{RGB}{158,202,225}
\definecolor{Blues-9-F}{RGB}{158,202,225}
\definecolor{Blues-9-5}{RGB}{107,174,214}
\definecolor{Blues-9-G}{RGB}{107,174,214}
\definecolor{Blues-9-6}{RGB}{66,146,198}
\definecolor{Blues-9-H}{RGB}{66,146,198}
\definecolor{Blues-9-7}{RGB}{33,113,181}
\definecolor{Blues-9-J}{RGB}{33,113,181}
\definecolor{Blues-9-8}{RGB}{8,81,156}
\definecolor{Blues-9-K}{RGB}{8,81,156}
\definecolor{Blues-9-9}{RGB}{8,48,107}
\definecolor{Blues-9-M}{RGB}{8,48,107}
\definecolor{Greens-3-1}{RGB}{229,245,224}
\definecolor{Greens-3-C}{RGB}{229,245,224}
\definecolor{Greens-3-2}{RGB}{161,217,155}
\definecolor{Greens-3-F}{RGB}{161,217,155}
\definecolor{Greens-3-3}{RGB}{49,163,84}
\definecolor{Greens-3-I}{RGB}{49,163,84}
\definecolor{Greens-4-1}{RGB}{237,248,233}
\definecolor{Greens-4-B}{RGB}{237,248,233}
\definecolor{Greens-4-2}{RGB}{186,228,179}
\definecolor{Greens-4-E}{RGB}{186,228,179}
\definecolor{Greens-4-3}{RGB}{116,196,118}
\definecolor{Greens-4-G}{RGB}{116,196,118}
\definecolor{Greens-4-4}{RGB}{35,139,69}
\definecolor{Greens-4-J}{RGB}{35,139,69}
\definecolor{Greens-5-1}{RGB}{237,248,233}
\definecolor{Greens-5-B}{RGB}{237,248,233}
\definecolor{Greens-5-2}{RGB}{186,228,179}
\definecolor{Greens-5-E}{RGB}{186,228,179}
\definecolor{Greens-5-3}{RGB}{116,196,118}
\definecolor{Greens-5-G}{RGB}{116,196,118}
\definecolor{Greens-5-4}{RGB}{49,163,84}
\definecolor{Greens-5-I}{RGB}{49,163,84}
\definecolor{Greens-5-5}{RGB}{0,109,44}
\definecolor{Greens-5-K}{RGB}{0,109,44}
\definecolor{Greens-6-1}{RGB}{237,248,233}
\definecolor{Greens-6-B}{RGB}{237,248,233}
\definecolor{Greens-6-2}{RGB}{199,233,192}
\definecolor{Greens-6-D}{RGB}{199,233,192}
\definecolor{Greens-6-3}{RGB}{161,217,155}
\definecolor{Greens-6-F}{RGB}{161,217,155}
\definecolor{Greens-6-4}{RGB}{116,196,118}
\definecolor{Greens-6-G}{RGB}{116,196,118}
\definecolor{Greens-6-5}{RGB}{49,163,84}
\definecolor{Greens-6-I}{RGB}{49,163,84}
\definecolor{Greens-6-6}{RGB}{0,109,44}
\definecolor{Greens-6-K}{RGB}{0,109,44}
\definecolor{Greens-7-1}{RGB}{237,248,233}
\definecolor{Greens-7-B}{RGB}{237,248,233}
\definecolor{Greens-7-2}{RGB}{199,233,192}
\definecolor{Greens-7-D}{RGB}{199,233,192}
\definecolor{Greens-7-3}{RGB}{161,217,155}
\definecolor{Greens-7-F}{RGB}{161,217,155}
\definecolor{Greens-7-4}{RGB}{116,196,118}
\definecolor{Greens-7-G}{RGB}{116,196,118}
\definecolor{Greens-7-5}{RGB}{65,171,93}
\definecolor{Greens-7-H}{RGB}{65,171,93}
\definecolor{Greens-7-6}{RGB}{35,139,69}
\definecolor{Greens-7-J}{RGB}{35,139,69}
\definecolor{Greens-7-7}{RGB}{0,90,50}
\definecolor{Greens-7-L}{RGB}{0,90,50}
\definecolor{Greens-8-1}{RGB}{247,252,245}
\definecolor{Greens-8-A}{RGB}{247,252,245}
\definecolor{Greens-8-2}{RGB}{229,245,224}
\definecolor{Greens-8-C}{RGB}{229,245,224}
\definecolor{Greens-8-3}{RGB}{199,233,192}
\definecolor{Greens-8-D}{RGB}{199,233,192}
\definecolor{Greens-8-4}{RGB}{161,217,155}
\definecolor{Greens-8-F}{RGB}{161,217,155}
\definecolor{Greens-8-5}{RGB}{116,196,118}
\definecolor{Greens-8-G}{RGB}{116,196,118}
\definecolor{Greens-8-6}{RGB}{65,171,93}
\definecolor{Greens-8-H}{RGB}{65,171,93}
\definecolor{Greens-8-7}{RGB}{35,139,69}
\definecolor{Greens-8-J}{RGB}{35,139,69}
\definecolor{Greens-8-8}{RGB}{0,90,50}
\definecolor{Greens-8-L}{RGB}{0,90,50}
\definecolor{Greens-9-1}{RGB}{247,252,245}
\definecolor{Greens-9-A}{RGB}{247,252,245}
\definecolor{Greens-9-2}{RGB}{229,245,224}
\definecolor{Greens-9-C}{RGB}{229,245,224}
\definecolor{Greens-9-3}{RGB}{199,233,192}
\definecolor{Greens-9-D}{RGB}{199,233,192}
\definecolor{Greens-9-4}{RGB}{161,217,155}
\definecolor{Greens-9-F}{RGB}{161,217,155}
\definecolor{Greens-9-5}{RGB}{116,196,118}
\definecolor{Greens-9-G}{RGB}{116,196,118}
\definecolor{Greens-9-6}{RGB}{65,171,93}
\definecolor{Greens-9-H}{RGB}{65,171,93}
\definecolor{Greens-9-7}{RGB}{35,139,69}
\definecolor{Greens-9-J}{RGB}{35,139,69}
\definecolor{Greens-9-8}{RGB}{0,109,44}
\definecolor{Greens-9-K}{RGB}{0,109,44}
\definecolor{Greens-9-9}{RGB}{0,68,27}
\definecolor{Greens-9-M}{RGB}{0,68,27}
\definecolor{Oranges-3-1}{RGB}{254,230,206}
\definecolor{Oranges-3-C}{RGB}{254,230,206}
\definecolor{Oranges-3-2}{RGB}{253,174,107}
\definecolor{Oranges-3-F}{RGB}{253,174,107}
\definecolor{Oranges-3-3}{RGB}{230,85,13}
\definecolor{Oranges-3-I}{RGB}{230,85,13}
\definecolor{Oranges-4-1}{RGB}{254,237,222}
\definecolor{Oranges-4-B}{RGB}{254,237,222}
\definecolor{Oranges-4-2}{RGB}{253,190,133}
\definecolor{Oranges-4-E}{RGB}{253,190,133}
\definecolor{Oranges-4-3}{RGB}{253,141,60}
\definecolor{Oranges-4-G}{RGB}{253,141,60}
\definecolor{Oranges-4-4}{RGB}{217,71,1}
\definecolor{Oranges-4-J}{RGB}{217,71,1}
\definecolor{Oranges-5-1}{RGB}{254,237,222}
\definecolor{Oranges-5-B}{RGB}{254,237,222}
\definecolor{Oranges-5-2}{RGB}{253,190,133}
\definecolor{Oranges-5-E}{RGB}{253,190,133}
\definecolor{Oranges-5-3}{RGB}{253,141,60}
\definecolor{Oranges-5-G}{RGB}{253,141,60}
\definecolor{Oranges-5-4}{RGB}{230,85,13}
\definecolor{Oranges-5-I}{RGB}{230,85,13}
\definecolor{Oranges-5-5}{RGB}{166,54,3}
\definecolor{Oranges-5-K}{RGB}{166,54,3}
\definecolor{Oranges-6-1}{RGB}{254,237,222}
\definecolor{Oranges-6-B}{RGB}{254,237,222}
\definecolor{Oranges-6-2}{RGB}{253,208,162}
\definecolor{Oranges-6-D}{RGB}{253,208,162}
\definecolor{Oranges-6-3}{RGB}{253,174,107}
\definecolor{Oranges-6-F}{RGB}{253,174,107}
\definecolor{Oranges-6-4}{RGB}{253,141,60}
\definecolor{Oranges-6-G}{RGB}{253,141,60}
\definecolor{Oranges-6-5}{RGB}{230,85,13}
\definecolor{Oranges-6-I}{RGB}{230,85,13}
\definecolor{Oranges-6-6}{RGB}{166,54,3}
\definecolor{Oranges-6-K}{RGB}{166,54,3}
\definecolor{Oranges-7-1}{RGB}{254,237,222}
\definecolor{Oranges-7-B}{RGB}{254,237,222}
\definecolor{Oranges-7-2}{RGB}{253,208,162}
\definecolor{Oranges-7-D}{RGB}{253,208,162}
\definecolor{Oranges-7-3}{RGB}{253,174,107}
\definecolor{Oranges-7-F}{RGB}{253,174,107}
\definecolor{Oranges-7-4}{RGB}{253,141,60}
\definecolor{Oranges-7-G}{RGB}{253,141,60}
\definecolor{Oranges-7-5}{RGB}{241,105,19}
\definecolor{Oranges-7-H}{RGB}{241,105,19}
\definecolor{Oranges-7-6}{RGB}{217,72,1}
\definecolor{Oranges-7-J}{RGB}{217,72,1}
\definecolor{Oranges-7-7}{RGB}{140,45,4}
\definecolor{Oranges-7-L}{RGB}{140,45,4}
\definecolor{Oranges-8-1}{RGB}{255,245,235}
\definecolor{Oranges-8-A}{RGB}{255,245,235}
\definecolor{Oranges-8-2}{RGB}{254,230,206}
\definecolor{Oranges-8-C}{RGB}{254,230,206}
\definecolor{Oranges-8-3}{RGB}{253,208,162}
\definecolor{Oranges-8-D}{RGB}{253,208,162}
\definecolor{Oranges-8-4}{RGB}{253,174,107}
\definecolor{Oranges-8-F}{RGB}{253,174,107}
\definecolor{Oranges-8-5}{RGB}{253,141,60}
\definecolor{Oranges-8-G}{RGB}{253,141,60}
\definecolor{Oranges-8-6}{RGB}{241,105,19}
\definecolor{Oranges-8-H}{RGB}{241,105,19}
\definecolor{Oranges-8-7}{RGB}{217,72,1}
\definecolor{Oranges-8-J}{RGB}{217,72,1}
\definecolor{Oranges-8-8}{RGB}{140,45,4}
\definecolor{Oranges-8-L}{RGB}{140,45,4}
\definecolor{Oranges-9-1}{RGB}{255,245,235}
\definecolor{Oranges-9-A}{RGB}{255,245,235}
\definecolor{Oranges-9-2}{RGB}{254,230,206}
\definecolor{Oranges-9-C}{RGB}{254,230,206}
\definecolor{Oranges-9-3}{RGB}{253,208,162}
\definecolor{Oranges-9-D}{RGB}{253,208,162}
\definecolor{Oranges-9-4}{RGB}{253,174,107}
\definecolor{Oranges-9-F}{RGB}{253,174,107}
\definecolor{Oranges-9-5}{RGB}{253,141,60}
\definecolor{Oranges-9-G}{RGB}{253,141,60}
\definecolor{Oranges-9-6}{RGB}{241,105,19}
\definecolor{Oranges-9-H}{RGB}{241,105,19}
\definecolor{Oranges-9-7}{RGB}{217,72,1}
\definecolor{Oranges-9-J}{RGB}{217,72,1}
\definecolor{Oranges-9-8}{RGB}{166,54,3}
\definecolor{Oranges-9-K}{RGB}{166,54,3}
\definecolor{Oranges-9-9}{RGB}{127,39,4}
\definecolor{Oranges-9-M}{RGB}{127,39,4}
\definecolor{Reds-3-1}{RGB}{254,224,210}
\definecolor{Reds-3-C}{RGB}{254,224,210}
\definecolor{Reds-3-2}{RGB}{252,146,114}
\definecolor{Reds-3-F}{RGB}{252,146,114}
\definecolor{Reds-3-3}{RGB}{222,45,38}
\definecolor{Reds-3-I}{RGB}{222,45,38}
\definecolor{Reds-4-1}{RGB}{254,229,217}
\definecolor{Reds-4-B}{RGB}{254,229,217}
\definecolor{Reds-4-2}{RGB}{252,174,145}
\definecolor{Reds-4-E}{RGB}{252,174,145}
\definecolor{Reds-4-3}{RGB}{251,106,74}
\definecolor{Reds-4-G}{RGB}{251,106,74}
\definecolor{Reds-4-4}{RGB}{203,24,29}
\definecolor{Reds-4-J}{RGB}{203,24,29}
\definecolor{Reds-5-1}{RGB}{254,229,217}
\definecolor{Reds-5-B}{RGB}{254,229,217}
\definecolor{Reds-5-2}{RGB}{252,174,145}
\definecolor{Reds-5-E}{RGB}{252,174,145}
\definecolor{Reds-5-3}{RGB}{251,106,74}
\definecolor{Reds-5-G}{RGB}{251,106,74}
\definecolor{Reds-5-4}{RGB}{222,45,38}
\definecolor{Reds-5-I}{RGB}{222,45,38}
\definecolor{Reds-5-5}{RGB}{165,15,21}
\definecolor{Reds-5-K}{RGB}{165,15,21}
\definecolor{Reds-6-1}{RGB}{254,229,217}
\definecolor{Reds-6-B}{RGB}{254,229,217}
\definecolor{Reds-6-2}{RGB}{252,187,161}
\definecolor{Reds-6-D}{RGB}{252,187,161}
\definecolor{Reds-6-3}{RGB}{252,146,114}
\definecolor{Reds-6-F}{RGB}{252,146,114}
\definecolor{Reds-6-4}{RGB}{251,106,74}
\definecolor{Reds-6-G}{RGB}{251,106,74}
\definecolor{Reds-6-5}{RGB}{222,45,38}
\definecolor{Reds-6-I}{RGB}{222,45,38}
\definecolor{Reds-6-6}{RGB}{165,15,21}
\definecolor{Reds-6-K}{RGB}{165,15,21}
\definecolor{Reds-7-1}{RGB}{254,229,217}
\definecolor{Reds-7-B}{RGB}{254,229,217}
\definecolor{Reds-7-2}{RGB}{252,187,161}
\definecolor{Reds-7-D}{RGB}{252,187,161}
\definecolor{Reds-7-3}{RGB}{252,146,114}
\definecolor{Reds-7-F}{RGB}{252,146,114}
\definecolor{Reds-7-4}{RGB}{251,106,74}
\definecolor{Reds-7-G}{RGB}{251,106,74}
\definecolor{Reds-7-5}{RGB}{239,59,44}
\definecolor{Reds-7-H}{RGB}{239,59,44}
\definecolor{Reds-7-6}{RGB}{203,24,29}
\definecolor{Reds-7-J}{RGB}{203,24,29}
\definecolor{Reds-7-7}{RGB}{153,0,13}
\definecolor{Reds-7-L}{RGB}{153,0,13}
\definecolor{Reds-8-1}{RGB}{255,245,240}
\definecolor{Reds-8-A}{RGB}{255,245,240}
\definecolor{Reds-8-2}{RGB}{254,224,210}
\definecolor{Reds-8-C}{RGB}{254,224,210}
\definecolor{Reds-8-3}{RGB}{252,187,161}
\definecolor{Reds-8-D}{RGB}{252,187,161}
\definecolor{Reds-8-4}{RGB}{252,146,114}
\definecolor{Reds-8-F}{RGB}{252,146,114}
\definecolor{Reds-8-5}{RGB}{251,106,74}
\definecolor{Reds-8-G}{RGB}{251,106,74}
\definecolor{Reds-8-6}{RGB}{239,59,44}
\definecolor{Reds-8-H}{RGB}{239,59,44}
\definecolor{Reds-8-7}{RGB}{203,24,29}
\definecolor{Reds-8-J}{RGB}{203,24,29}
\definecolor{Reds-8-8}{RGB}{153,0,13}
\definecolor{Reds-8-L}{RGB}{153,0,13}
\definecolor{Reds-9-1}{RGB}{255,245,240}
\definecolor{Reds-9-A}{RGB}{255,245,240}
\definecolor{Reds-9-2}{RGB}{254,224,210}
\definecolor{Reds-9-C}{RGB}{254,224,210}
\definecolor{Reds-9-3}{RGB}{252,187,161}
\definecolor{Reds-9-D}{RGB}{252,187,161}
\definecolor{Reds-9-4}{RGB}{252,146,114}
\definecolor{Reds-9-F}{RGB}{252,146,114}
\definecolor{Reds-9-5}{RGB}{251,106,74}
\definecolor{Reds-9-G}{RGB}{251,106,74}
\definecolor{Reds-9-6}{RGB}{239,59,44}
\definecolor{Reds-9-H}{RGB}{239,59,44}
\definecolor{Reds-9-7}{RGB}{203,24,29}
\definecolor{Reds-9-J}{RGB}{203,24,29}
\definecolor{Reds-9-8}{RGB}{165,15,21}
\definecolor{Reds-9-K}{RGB}{165,15,21}
\definecolor{Reds-9-9}{RGB}{103,0,13}
\definecolor{Reds-9-M}{RGB}{103,0,13}
\definecolor{Greys-3-1}{RGB}{240,240,240}
\definecolor{Greys-3-C}{RGB}{240,240,240}
\definecolor{Greys-3-2}{RGB}{189,189,189}
\definecolor{Greys-3-F}{RGB}{189,189,189}
\definecolor{Greys-3-3}{RGB}{99,99,99}
\definecolor{Greys-3-I}{RGB}{99,99,99}
\definecolor{Greys-4-1}{RGB}{247,247,247}
\definecolor{Greys-4-B}{RGB}{247,247,247}
\definecolor{Greys-4-2}{RGB}{204,204,204}
\definecolor{Greys-4-E}{RGB}{204,204,204}
\definecolor{Greys-4-3}{RGB}{150,150,150}
\definecolor{Greys-4-G}{RGB}{150,150,150}
\definecolor{Greys-4-4}{RGB}{82,82,82}
\definecolor{Greys-4-J}{RGB}{82,82,82}
\definecolor{Greys-5-1}{RGB}{247,247,247}
\definecolor{Greys-5-B}{RGB}{247,247,247}
\definecolor{Greys-5-2}{RGB}{204,204,204}
\definecolor{Greys-5-E}{RGB}{204,204,204}
\definecolor{Greys-5-3}{RGB}{150,150,150}
\definecolor{Greys-5-G}{RGB}{150,150,150}
\definecolor{Greys-5-4}{RGB}{99,99,99}
\definecolor{Greys-5-I}{RGB}{99,99,99}
\definecolor{Greys-5-5}{RGB}{37,37,37}
\definecolor{Greys-5-K}{RGB}{37,37,37}
\definecolor{Greys-6-1}{RGB}{247,247,247}
\definecolor{Greys-6-B}{RGB}{247,247,247}
\definecolor{Greys-6-2}{RGB}{217,217,217}
\definecolor{Greys-6-D}{RGB}{217,217,217}
\definecolor{Greys-6-3}{RGB}{189,189,189}
\definecolor{Greys-6-F}{RGB}{189,189,189}
\definecolor{Greys-6-4}{RGB}{150,150,150}
\definecolor{Greys-6-G}{RGB}{150,150,150}
\definecolor{Greys-6-5}{RGB}{99,99,99}
\definecolor{Greys-6-I}{RGB}{99,99,99}
\definecolor{Greys-6-6}{RGB}{37,37,37}
\definecolor{Greys-6-K}{RGB}{37,37,37}
\definecolor{Greys-7-1}{RGB}{247,247,247}
\definecolor{Greys-7-B}{RGB}{247,247,247}
\definecolor{Greys-7-2}{RGB}{217,217,217}
\definecolor{Greys-7-D}{RGB}{217,217,217}
\definecolor{Greys-7-3}{RGB}{189,189,189}
\definecolor{Greys-7-F}{RGB}{189,189,189}
\definecolor{Greys-7-4}{RGB}{150,150,150}
\definecolor{Greys-7-G}{RGB}{150,150,150}
\definecolor{Greys-7-5}{RGB}{115,115,115}
\definecolor{Greys-7-H}{RGB}{115,115,115}
\definecolor{Greys-7-6}{RGB}{82,82,82}
\definecolor{Greys-7-J}{RGB}{82,82,82}
\definecolor{Greys-7-7}{RGB}{37,37,37}
\definecolor{Greys-7-L}{RGB}{37,37,37}
\definecolor{Greys-8-1}{RGB}{255,255,255}
\definecolor{Greys-8-A}{RGB}{255,255,255}
\definecolor{Greys-8-2}{RGB}{240,240,240}
\definecolor{Greys-8-C}{RGB}{240,240,240}
\definecolor{Greys-8-3}{RGB}{217,217,217}
\definecolor{Greys-8-D}{RGB}{217,217,217}
\definecolor{Greys-8-4}{RGB}{189,189,189}
\definecolor{Greys-8-F}{RGB}{189,189,189}
\definecolor{Greys-8-5}{RGB}{150,150,150}
\definecolor{Greys-8-G}{RGB}{150,150,150}
\definecolor{Greys-8-6}{RGB}{115,115,115}
\definecolor{Greys-8-H}{RGB}{115,115,115}
\definecolor{Greys-8-7}{RGB}{82,82,82}
\definecolor{Greys-8-J}{RGB}{82,82,82}
\definecolor{Greys-8-8}{RGB}{37,37,37}
\definecolor{Greys-8-L}{RGB}{37,37,37}
\definecolor{Greys-9-1}{RGB}{255,255,255}
\definecolor{Greys-9-A}{RGB}{255,255,255}
\definecolor{Greys-9-2}{RGB}{240,240,240}
\definecolor{Greys-9-C}{RGB}{240,240,240}
\definecolor{Greys-9-3}{RGB}{217,217,217}
\definecolor{Greys-9-D}{RGB}{217,217,217}
\definecolor{Greys-9-4}{RGB}{189,189,189}
\definecolor{Greys-9-F}{RGB}{189,189,189}
\definecolor{Greys-9-5}{RGB}{150,150,150}
\definecolor{Greys-9-G}{RGB}{150,150,150}
\definecolor{Greys-9-6}{RGB}{115,115,115}
\definecolor{Greys-9-H}{RGB}{115,115,115}
\definecolor{Greys-9-7}{RGB}{82,82,82}
\definecolor{Greys-9-J}{RGB}{82,82,82}
\definecolor{Greys-9-8}{RGB}{37,37,37}
\definecolor{Greys-9-K}{RGB}{37,37,37}
\definecolor{Greys-9-9}{RGB}{0,0,0}
\definecolor{Greys-9-M}{RGB}{0,0,0}
\definecolor{PuOr-3-1}{RGB}{241,163,64}
\definecolor{PuOr-3-E}{RGB}{241,163,64}
\definecolor{PuOr-3-2}{RGB}{247,247,247}
\definecolor{PuOr-3-H}{RGB}{247,247,247}
\definecolor{PuOr-3-3}{RGB}{153,142,195}
\definecolor{PuOr-3-K}{RGB}{153,142,195}
\definecolor{PuOr-4-1}{RGB}{230,97,1}
\definecolor{PuOr-4-C}{RGB}{230,97,1}
\definecolor{PuOr-4-2}{RGB}{253,184,99}
\definecolor{PuOr-4-F}{RGB}{253,184,99}
\definecolor{PuOr-4-3}{RGB}{178,171,210}
\definecolor{PuOr-4-J}{RGB}{178,171,210}
\definecolor{PuOr-4-4}{RGB}{94,60,153}
\definecolor{PuOr-4-M}{RGB}{94,60,153}
\definecolor{PuOr-5-1}{RGB}{230,97,1}
\definecolor{PuOr-5-C}{RGB}{230,97,1}
\definecolor{PuOr-5-2}{RGB}{253,184,99}
\definecolor{PuOr-5-F}{RGB}{253,184,99}
\definecolor{PuOr-5-3}{RGB}{247,247,247}
\definecolor{PuOr-5-H}{RGB}{247,247,247}
\definecolor{PuOr-5-4}{RGB}{178,171,210}
\definecolor{PuOr-5-J}{RGB}{178,171,210}
\definecolor{PuOr-5-5}{RGB}{94,60,153}
\definecolor{PuOr-5-M}{RGB}{94,60,153}
\definecolor{PuOr-6-1}{RGB}{179,88,6}
\definecolor{PuOr-6-B}{RGB}{179,88,6}
\definecolor{PuOr-6-2}{RGB}{241,163,64}
\definecolor{PuOr-6-E}{RGB}{241,163,64}
\definecolor{PuOr-6-3}{RGB}{254,224,182}
\definecolor{PuOr-6-G}{RGB}{254,224,182}
\definecolor{PuOr-6-4}{RGB}{216,218,235}
\definecolor{PuOr-6-I}{RGB}{216,218,235}
\definecolor{PuOr-6-5}{RGB}{153,142,195}
\definecolor{PuOr-6-K}{RGB}{153,142,195}
\definecolor{PuOr-6-6}{RGB}{84,39,136}
\definecolor{PuOr-6-N}{RGB}{84,39,136}
\definecolor{PuOr-7-1}{RGB}{179,88,6}
\definecolor{PuOr-7-B}{RGB}{179,88,6}
\definecolor{PuOr-7-2}{RGB}{241,163,64}
\definecolor{PuOr-7-E}{RGB}{241,163,64}
\definecolor{PuOr-7-3}{RGB}{254,224,182}
\definecolor{PuOr-7-G}{RGB}{254,224,182}
\definecolor{PuOr-7-4}{RGB}{247,247,247}
\definecolor{PuOr-7-H}{RGB}{247,247,247}
\definecolor{PuOr-7-5}{RGB}{216,218,235}
\definecolor{PuOr-7-I}{RGB}{216,218,235}
\definecolor{PuOr-7-6}{RGB}{153,142,195}
\definecolor{PuOr-7-K}{RGB}{153,142,195}
\definecolor{PuOr-7-7}{RGB}{84,39,136}
\definecolor{PuOr-7-N}{RGB}{84,39,136}
\definecolor{PuOr-8-1}{RGB}{179,88,6}
\definecolor{PuOr-8-B}{RGB}{179,88,6}
\definecolor{PuOr-8-2}{RGB}{224,130,20}
\definecolor{PuOr-8-D}{RGB}{224,130,20}
\definecolor{PuOr-8-3}{RGB}{253,184,99}
\definecolor{PuOr-8-F}{RGB}{253,184,99}
\definecolor{PuOr-8-4}{RGB}{254,224,182}
\definecolor{PuOr-8-G}{RGB}{254,224,182}
\definecolor{PuOr-8-5}{RGB}{216,218,235}
\definecolor{PuOr-8-I}{RGB}{216,218,235}
\definecolor{PuOr-8-6}{RGB}{178,171,210}
\definecolor{PuOr-8-J}{RGB}{178,171,210}
\definecolor{PuOr-8-7}{RGB}{128,115,172}
\definecolor{PuOr-8-L}{RGB}{128,115,172}
\definecolor{PuOr-8-8}{RGB}{84,39,136}
\definecolor{PuOr-8-N}{RGB}{84,39,136}
\definecolor{PuOr-9-1}{RGB}{179,88,6}
\definecolor{PuOr-9-B}{RGB}{179,88,6}
\definecolor{PuOr-9-2}{RGB}{224,130,20}
\definecolor{PuOr-9-D}{RGB}{224,130,20}
\definecolor{PuOr-9-3}{RGB}{253,184,99}
\definecolor{PuOr-9-F}{RGB}{253,184,99}
\definecolor{PuOr-9-4}{RGB}{254,224,182}
\definecolor{PuOr-9-G}{RGB}{254,224,182}
\definecolor{PuOr-9-5}{RGB}{247,247,247}
\definecolor{PuOr-9-H}{RGB}{247,247,247}
\definecolor{PuOr-9-6}{RGB}{216,218,235}
\definecolor{PuOr-9-I}{RGB}{216,218,235}
\definecolor{PuOr-9-7}{RGB}{178,171,210}
\definecolor{PuOr-9-J}{RGB}{178,171,210}
\definecolor{PuOr-9-8}{RGB}{128,115,172}
\definecolor{PuOr-9-L}{RGB}{128,115,172}
\definecolor{PuOr-9-9}{RGB}{84,39,136}
\definecolor{PuOr-9-N}{RGB}{84,39,136}
\definecolor{PuOr-10-1}{RGB}{127,59,8}
\definecolor{PuOr-10-A}{RGB}{127,59,8}
\definecolor{PuOr-10-2}{RGB}{179,88,6}
\definecolor{PuOr-10-B}{RGB}{179,88,6}
\definecolor{PuOr-10-3}{RGB}{224,130,20}
\definecolor{PuOr-10-D}{RGB}{224,130,20}
\definecolor{PuOr-10-4}{RGB}{253,184,99}
\definecolor{PuOr-10-F}{RGB}{253,184,99}
\definecolor{PuOr-10-5}{RGB}{254,224,182}
\definecolor{PuOr-10-G}{RGB}{254,224,182}
\definecolor{PuOr-10-6}{RGB}{216,218,235}
\definecolor{PuOr-10-I}{RGB}{216,218,235}
\definecolor{PuOr-10-7}{RGB}{178,171,210}
\definecolor{PuOr-10-J}{RGB}{178,171,210}
\definecolor{PuOr-10-8}{RGB}{128,115,172}
\definecolor{PuOr-10-L}{RGB}{128,115,172}
\definecolor{PuOr-10-9}{RGB}{84,39,136}
\definecolor{PuOr-10-N}{RGB}{84,39,136}
\definecolor{PuOr-10-10}{RGB}{45,0,75}
\definecolor{PuOr-10-O}{RGB}{45,0,75}
\definecolor{PuOr-11-1}{RGB}{127,59,8}
\definecolor{PuOr-11-A}{RGB}{127,59,8}
\definecolor{PuOr-11-2}{RGB}{179,88,6}
\definecolor{PuOr-11-B}{RGB}{179,88,6}
\definecolor{PuOr-11-3}{RGB}{224,130,20}
\definecolor{PuOr-11-D}{RGB}{224,130,20}
\definecolor{PuOr-11-4}{RGB}{253,184,99}
\definecolor{PuOr-11-F}{RGB}{253,184,99}
\definecolor{PuOr-11-5}{RGB}{254,224,182}
\definecolor{PuOr-11-G}{RGB}{254,224,182}
\definecolor{PuOr-11-6}{RGB}{247,247,247}
\definecolor{PuOr-11-H}{RGB}{247,247,247}
\definecolor{PuOr-11-7}{RGB}{216,218,235}
\definecolor{PuOr-11-I}{RGB}{216,218,235}
\definecolor{PuOr-11-8}{RGB}{178,171,210}
\definecolor{PuOr-11-J}{RGB}{178,171,210}
\definecolor{PuOr-11-9}{RGB}{128,115,172}
\definecolor{PuOr-11-L}{RGB}{128,115,172}
\definecolor{PuOr-11-10}{RGB}{84,39,136}
\definecolor{PuOr-11-N}{RGB}{84,39,136}
\definecolor{PuOr-11-11}{RGB}{45,0,75}
\definecolor{PuOr-11-O}{RGB}{45,0,75}
\definecolor{BrBG-3-1}{RGB}{216,179,101}
\definecolor{BrBG-3-E}{RGB}{216,179,101}
\definecolor{BrBG-3-2}{RGB}{245,245,245}
\definecolor{BrBG-3-H}{RGB}{245,245,245}
\definecolor{BrBG-3-3}{RGB}{90,180,172}
\definecolor{BrBG-3-K}{RGB}{90,180,172}
\definecolor{BrBG-4-1}{RGB}{166,97,26}
\definecolor{BrBG-4-C}{RGB}{166,97,26}
\definecolor{BrBG-4-2}{RGB}{223,194,125}
\definecolor{BrBG-4-F}{RGB}{223,194,125}
\definecolor{BrBG-4-3}{RGB}{128,205,193}
\definecolor{BrBG-4-J}{RGB}{128,205,193}
\definecolor{BrBG-4-4}{RGB}{1,133,113}
\definecolor{BrBG-4-M}{RGB}{1,133,113}
\definecolor{BrBG-5-1}{RGB}{166,97,26}
\definecolor{BrBG-5-C}{RGB}{166,97,26}
\definecolor{BrBG-5-2}{RGB}{223,194,125}
\definecolor{BrBG-5-F}{RGB}{223,194,125}
\definecolor{BrBG-5-3}{RGB}{245,245,245}
\definecolor{BrBG-5-H}{RGB}{245,245,245}
\definecolor{BrBG-5-4}{RGB}{128,205,193}
\definecolor{BrBG-5-J}{RGB}{128,205,193}
\definecolor{BrBG-5-5}{RGB}{1,133,113}
\definecolor{BrBG-5-M}{RGB}{1,133,113}
\definecolor{BrBG-6-1}{RGB}{140,81,10}
\definecolor{BrBG-6-B}{RGB}{140,81,10}
\definecolor{BrBG-6-2}{RGB}{216,179,101}
\definecolor{BrBG-6-E}{RGB}{216,179,101}
\definecolor{BrBG-6-3}{RGB}{246,232,195}
\definecolor{BrBG-6-G}{RGB}{246,232,195}
\definecolor{BrBG-6-4}{RGB}{199,234,229}
\definecolor{BrBG-6-I}{RGB}{199,234,229}
\definecolor{BrBG-6-5}{RGB}{90,180,172}
\definecolor{BrBG-6-K}{RGB}{90,180,172}
\definecolor{BrBG-6-6}{RGB}{1,102,94}
\definecolor{BrBG-6-N}{RGB}{1,102,94}
\definecolor{BrBG-7-1}{RGB}{140,81,10}
\definecolor{BrBG-7-B}{RGB}{140,81,10}
\definecolor{BrBG-7-2}{RGB}{216,179,101}
\definecolor{BrBG-7-E}{RGB}{216,179,101}
\definecolor{BrBG-7-3}{RGB}{246,232,195}
\definecolor{BrBG-7-G}{RGB}{246,232,195}
\definecolor{BrBG-7-4}{RGB}{245,245,245}
\definecolor{BrBG-7-H}{RGB}{245,245,245}
\definecolor{BrBG-7-5}{RGB}{199,234,229}
\definecolor{BrBG-7-I}{RGB}{199,234,229}
\definecolor{BrBG-7-6}{RGB}{90,180,172}
\definecolor{BrBG-7-K}{RGB}{90,180,172}
\definecolor{BrBG-7-7}{RGB}{1,102,94}
\definecolor{BrBG-7-N}{RGB}{1,102,94}
\definecolor{BrBG-8-1}{RGB}{140,81,10}
\definecolor{BrBG-8-B}{RGB}{140,81,10}
\definecolor{BrBG-8-2}{RGB}{191,129,45}
\definecolor{BrBG-8-D}{RGB}{191,129,45}
\definecolor{BrBG-8-3}{RGB}{223,194,125}
\definecolor{BrBG-8-F}{RGB}{223,194,125}
\definecolor{BrBG-8-4}{RGB}{246,232,195}
\definecolor{BrBG-8-G}{RGB}{246,232,195}
\definecolor{BrBG-8-5}{RGB}{199,234,229}
\definecolor{BrBG-8-I}{RGB}{199,234,229}
\definecolor{BrBG-8-6}{RGB}{128,205,193}
\definecolor{BrBG-8-J}{RGB}{128,205,193}
\definecolor{BrBG-8-7}{RGB}{53,151,143}
\definecolor{BrBG-8-L}{RGB}{53,151,143}
\definecolor{BrBG-8-8}{RGB}{1,102,94}
\definecolor{BrBG-8-N}{RGB}{1,102,94}
\definecolor{BrBG-9-1}{RGB}{140,81,10}
\definecolor{BrBG-9-B}{RGB}{140,81,10}
\definecolor{BrBG-9-2}{RGB}{191,129,45}
\definecolor{BrBG-9-D}{RGB}{191,129,45}
\definecolor{BrBG-9-3}{RGB}{223,194,125}
\definecolor{BrBG-9-F}{RGB}{223,194,125}
\definecolor{BrBG-9-4}{RGB}{246,232,195}
\definecolor{BrBG-9-G}{RGB}{246,232,195}
\definecolor{BrBG-9-5}{RGB}{245,245,245}
\definecolor{BrBG-9-H}{RGB}{245,245,245}
\definecolor{BrBG-9-6}{RGB}{199,234,229}
\definecolor{BrBG-9-I}{RGB}{199,234,229}
\definecolor{BrBG-9-7}{RGB}{128,205,193}
\definecolor{BrBG-9-J}{RGB}{128,205,193}
\definecolor{BrBG-9-8}{RGB}{53,151,143}
\definecolor{BrBG-9-L}{RGB}{53,151,143}
\definecolor{BrBG-9-9}{RGB}{1,102,94}
\definecolor{BrBG-9-N}{RGB}{1,102,94}
\definecolor{BrBG-10-1}{RGB}{84,48,5}
\definecolor{BrBG-10-A}{RGB}{84,48,5}
\definecolor{BrBG-10-2}{RGB}{140,81,10}
\definecolor{BrBG-10-B}{RGB}{140,81,10}
\definecolor{BrBG-10-3}{RGB}{191,129,45}
\definecolor{BrBG-10-D}{RGB}{191,129,45}
\definecolor{BrBG-10-4}{RGB}{223,194,125}
\definecolor{BrBG-10-F}{RGB}{223,194,125}
\definecolor{BrBG-10-5}{RGB}{246,232,195}
\definecolor{BrBG-10-G}{RGB}{246,232,195}
\definecolor{BrBG-10-6}{RGB}{199,234,229}
\definecolor{BrBG-10-I}{RGB}{199,234,229}
\definecolor{BrBG-10-7}{RGB}{128,205,193}
\definecolor{BrBG-10-J}{RGB}{128,205,193}
\definecolor{BrBG-10-8}{RGB}{53,151,143}
\definecolor{BrBG-10-L}{RGB}{53,151,143}
\definecolor{BrBG-10-9}{RGB}{1,102,94}
\definecolor{BrBG-10-N}{RGB}{1,102,94}
\definecolor{BrBG-10-10}{RGB}{0,60,48}
\definecolor{BrBG-10-O}{RGB}{0,60,48}
\definecolor{BrBG-11-1}{RGB}{84,48,5}
\definecolor{BrBG-11-A}{RGB}{84,48,5}
\definecolor{BrBG-11-2}{RGB}{140,81,10}
\definecolor{BrBG-11-B}{RGB}{140,81,10}
\definecolor{BrBG-11-3}{RGB}{191,129,45}
\definecolor{BrBG-11-D}{RGB}{191,129,45}
\definecolor{BrBG-11-4}{RGB}{223,194,125}
\definecolor{BrBG-11-F}{RGB}{223,194,125}
\definecolor{BrBG-11-5}{RGB}{246,232,195}
\definecolor{BrBG-11-G}{RGB}{246,232,195}
\definecolor{BrBG-11-6}{RGB}{245,245,245}
\definecolor{BrBG-11-H}{RGB}{245,245,245}
\definecolor{BrBG-11-7}{RGB}{199,234,229}
\definecolor{BrBG-11-I}{RGB}{199,234,229}
\definecolor{BrBG-11-8}{RGB}{128,205,193}
\definecolor{BrBG-11-J}{RGB}{128,205,193}
\definecolor{BrBG-11-9}{RGB}{53,151,143}
\definecolor{BrBG-11-L}{RGB}{53,151,143}
\definecolor{BrBG-11-10}{RGB}{1,102,94}
\definecolor{BrBG-11-N}{RGB}{1,102,94}
\definecolor{BrBG-11-11}{RGB}{0,60,48}
\definecolor{BrBG-11-O}{RGB}{0,60,48}
\definecolor{PRGn-3-1}{RGB}{175,141,195}
\definecolor{PRGn-3-E}{RGB}{175,141,195}
\definecolor{PRGn-3-2}{RGB}{247,247,247}
\definecolor{PRGn-3-H}{RGB}{247,247,247}
\definecolor{PRGn-3-3}{RGB}{127,191,123}
\definecolor{PRGn-3-K}{RGB}{127,191,123}
\definecolor{PRGn-4-1}{RGB}{123,50,148}
\definecolor{PRGn-4-C}{RGB}{123,50,148}
\definecolor{PRGn-4-2}{RGB}{194,165,207}
\definecolor{PRGn-4-F}{RGB}{194,165,207}
\definecolor{PRGn-4-3}{RGB}{166,219,160}
\definecolor{PRGn-4-J}{RGB}{166,219,160}
\definecolor{PRGn-4-4}{RGB}{0,136,55}
\definecolor{PRGn-4-M}{RGB}{0,136,55}
\definecolor{PRGn-5-1}{RGB}{123,50,148}
\definecolor{PRGn-5-C}{RGB}{123,50,148}
\definecolor{PRGn-5-2}{RGB}{194,165,207}
\definecolor{PRGn-5-F}{RGB}{194,165,207}
\definecolor{PRGn-5-3}{RGB}{247,247,247}
\definecolor{PRGn-5-H}{RGB}{247,247,247}
\definecolor{PRGn-5-4}{RGB}{166,219,160}
\definecolor{PRGn-5-J}{RGB}{166,219,160}
\definecolor{PRGn-5-5}{RGB}{0,136,55}
\definecolor{PRGn-5-M}{RGB}{0,136,55}
\definecolor{PRGn-6-1}{RGB}{118,42,131}
\definecolor{PRGn-6-B}{RGB}{118,42,131}
\definecolor{PRGn-6-2}{RGB}{175,141,195}
\definecolor{PRGn-6-E}{RGB}{175,141,195}
\definecolor{PRGn-6-3}{RGB}{231,212,232}
\definecolor{PRGn-6-G}{RGB}{231,212,232}
\definecolor{PRGn-6-4}{RGB}{217,240,211}
\definecolor{PRGn-6-I}{RGB}{217,240,211}
\definecolor{PRGn-6-5}{RGB}{127,191,123}
\definecolor{PRGn-6-K}{RGB}{127,191,123}
\definecolor{PRGn-6-6}{RGB}{27,120,55}
\definecolor{PRGn-6-N}{RGB}{27,120,55}
\definecolor{PRGn-7-1}{RGB}{118,42,131}
\definecolor{PRGn-7-B}{RGB}{118,42,131}
\definecolor{PRGn-7-2}{RGB}{175,141,195}
\definecolor{PRGn-7-E}{RGB}{175,141,195}
\definecolor{PRGn-7-3}{RGB}{231,212,232}
\definecolor{PRGn-7-G}{RGB}{231,212,232}
\definecolor{PRGn-7-4}{RGB}{247,247,247}
\definecolor{PRGn-7-H}{RGB}{247,247,247}
\definecolor{PRGn-7-5}{RGB}{217,240,211}
\definecolor{PRGn-7-I}{RGB}{217,240,211}
\definecolor{PRGn-7-6}{RGB}{127,191,123}
\definecolor{PRGn-7-K}{RGB}{127,191,123}
\definecolor{PRGn-7-7}{RGB}{27,120,55}
\definecolor{PRGn-7-N}{RGB}{27,120,55}
\definecolor{PRGn-8-1}{RGB}{118,42,131}
\definecolor{PRGn-8-B}{RGB}{118,42,131}
\definecolor{PRGn-8-2}{RGB}{153,112,171}
\definecolor{PRGn-8-D}{RGB}{153,112,171}
\definecolor{PRGn-8-3}{RGB}{194,165,207}
\definecolor{PRGn-8-F}{RGB}{194,165,207}
\definecolor{PRGn-8-4}{RGB}{231,212,232}
\definecolor{PRGn-8-G}{RGB}{231,212,232}
\definecolor{PRGn-8-5}{RGB}{217,240,211}
\definecolor{PRGn-8-I}{RGB}{217,240,211}
\definecolor{PRGn-8-6}{RGB}{166,219,160}
\definecolor{PRGn-8-J}{RGB}{166,219,160}
\definecolor{PRGn-8-7}{RGB}{90,174,97}
\definecolor{PRGn-8-L}{RGB}{90,174,97}
\definecolor{PRGn-8-8}{RGB}{27,120,55}
\definecolor{PRGn-8-N}{RGB}{27,120,55}
\definecolor{PRGn-9-1}{RGB}{118,42,131}
\definecolor{PRGn-9-B}{RGB}{118,42,131}
\definecolor{PRGn-9-2}{RGB}{153,112,171}
\definecolor{PRGn-9-D}{RGB}{153,112,171}
\definecolor{PRGn-9-3}{RGB}{194,165,207}
\definecolor{PRGn-9-F}{RGB}{194,165,207}
\definecolor{PRGn-9-4}{RGB}{231,212,232}
\definecolor{PRGn-9-G}{RGB}{231,212,232}
\definecolor{PRGn-9-5}{RGB}{247,247,247}
\definecolor{PRGn-9-H}{RGB}{247,247,247}
\definecolor{PRGn-9-6}{RGB}{217,240,211}
\definecolor{PRGn-9-I}{RGB}{217,240,211}
\definecolor{PRGn-9-7}{RGB}{166,219,160}
\definecolor{PRGn-9-J}{RGB}{166,219,160}
\definecolor{PRGn-9-8}{RGB}{90,174,97}
\definecolor{PRGn-9-L}{RGB}{90,174,97}
\definecolor{PRGn-9-9}{RGB}{27,120,55}
\definecolor{PRGn-9-N}{RGB}{27,120,55}
\definecolor{PRGn-10-1}{RGB}{64,0,75}
\definecolor{PRGn-10-A}{RGB}{64,0,75}
\definecolor{PRGn-10-2}{RGB}{118,42,131}
\definecolor{PRGn-10-B}{RGB}{118,42,131}
\definecolor{PRGn-10-3}{RGB}{153,112,171}
\definecolor{PRGn-10-D}{RGB}{153,112,171}
\definecolor{PRGn-10-4}{RGB}{194,165,207}
\definecolor{PRGn-10-F}{RGB}{194,165,207}
\definecolor{PRGn-10-5}{RGB}{231,212,232}
\definecolor{PRGn-10-G}{RGB}{231,212,232}
\definecolor{PRGn-10-6}{RGB}{217,240,211}
\definecolor{PRGn-10-I}{RGB}{217,240,211}
\definecolor{PRGn-10-7}{RGB}{166,219,160}
\definecolor{PRGn-10-J}{RGB}{166,219,160}
\definecolor{PRGn-10-8}{RGB}{90,174,97}
\definecolor{PRGn-10-L}{RGB}{90,174,97}
\definecolor{PRGn-10-9}{RGB}{27,120,55}
\definecolor{PRGn-10-N}{RGB}{27,120,55}
\definecolor{PRGn-10-10}{RGB}{0,68,27}
\definecolor{PRGn-10-O}{RGB}{0,68,27}
\definecolor{PRGn-11-1}{RGB}{64,0,75}
\definecolor{PRGn-11-A}{RGB}{64,0,75}
\definecolor{PRGn-11-2}{RGB}{118,42,131}
\definecolor{PRGn-11-B}{RGB}{118,42,131}
\definecolor{PRGn-11-3}{RGB}{153,112,171}
\definecolor{PRGn-11-D}{RGB}{153,112,171}
\definecolor{PRGn-11-4}{RGB}{194,165,207}
\definecolor{PRGn-11-F}{RGB}{194,165,207}
\definecolor{PRGn-11-5}{RGB}{231,212,232}
\definecolor{PRGn-11-G}{RGB}{231,212,232}
\definecolor{PRGn-11-6}{RGB}{247,247,247}
\definecolor{PRGn-11-H}{RGB}{247,247,247}
\definecolor{PRGn-11-7}{RGB}{217,240,211}
\definecolor{PRGn-11-I}{RGB}{217,240,211}
\definecolor{PRGn-11-8}{RGB}{166,219,160}
\definecolor{PRGn-11-J}{RGB}{166,219,160}
\definecolor{PRGn-11-9}{RGB}{90,174,97}
\definecolor{PRGn-11-L}{RGB}{90,174,97}
\definecolor{PRGn-11-10}{RGB}{27,120,55}
\definecolor{PRGn-11-N}{RGB}{27,120,55}
\definecolor{PRGn-11-11}{RGB}{0,68,27}
\definecolor{PRGn-11-O}{RGB}{0,68,27}
\definecolor{PiYG-3-1}{RGB}{233,163,201}
\definecolor{PiYG-3-E}{RGB}{233,163,201}
\definecolor{PiYG-3-2}{RGB}{247,247,247}
\definecolor{PiYG-3-H}{RGB}{247,247,247}
\definecolor{PiYG-3-3}{RGB}{161,215,106}
\definecolor{PiYG-3-K}{RGB}{161,215,106}
\definecolor{PiYG-4-1}{RGB}{208,28,139}
\definecolor{PiYG-4-C}{RGB}{208,28,139}
\definecolor{PiYG-4-2}{RGB}{241,182,218}
\definecolor{PiYG-4-F}{RGB}{241,182,218}
\definecolor{PiYG-4-3}{RGB}{184,225,134}
\definecolor{PiYG-4-J}{RGB}{184,225,134}
\definecolor{PiYG-4-4}{RGB}{77,172,38}
\definecolor{PiYG-4-M}{RGB}{77,172,38}
\definecolor{PiYG-5-1}{RGB}{208,28,139}
\definecolor{PiYG-5-C}{RGB}{208,28,139}
\definecolor{PiYG-5-2}{RGB}{241,182,218}
\definecolor{PiYG-5-F}{RGB}{241,182,218}
\definecolor{PiYG-5-3}{RGB}{247,247,247}
\definecolor{PiYG-5-H}{RGB}{247,247,247}
\definecolor{PiYG-5-4}{RGB}{184,225,134}
\definecolor{PiYG-5-J}{RGB}{184,225,134}
\definecolor{PiYG-5-5}{RGB}{77,172,38}
\definecolor{PiYG-5-M}{RGB}{77,172,38}
\definecolor{PiYG-6-1}{RGB}{197,27,125}
\definecolor{PiYG-6-B}{RGB}{197,27,125}
\definecolor{PiYG-6-2}{RGB}{233,163,201}
\definecolor{PiYG-6-E}{RGB}{233,163,201}
\definecolor{PiYG-6-3}{RGB}{253,224,239}
\definecolor{PiYG-6-G}{RGB}{253,224,239}
\definecolor{PiYG-6-4}{RGB}{230,245,208}
\definecolor{PiYG-6-I}{RGB}{230,245,208}
\definecolor{PiYG-6-5}{RGB}{161,215,106}
\definecolor{PiYG-6-K}{RGB}{161,215,106}
\definecolor{PiYG-6-6}{RGB}{77,146,33}
\definecolor{PiYG-6-N}{RGB}{77,146,33}
\definecolor{PiYG-7-1}{RGB}{197,27,125}
\definecolor{PiYG-7-B}{RGB}{197,27,125}
\definecolor{PiYG-7-2}{RGB}{233,163,201}
\definecolor{PiYG-7-E}{RGB}{233,163,201}
\definecolor{PiYG-7-3}{RGB}{253,224,239}
\definecolor{PiYG-7-G}{RGB}{253,224,239}
\definecolor{PiYG-7-4}{RGB}{247,247,247}
\definecolor{PiYG-7-H}{RGB}{247,247,247}
\definecolor{PiYG-7-5}{RGB}{230,245,208}
\definecolor{PiYG-7-I}{RGB}{230,245,208}
\definecolor{PiYG-7-6}{RGB}{161,215,106}
\definecolor{PiYG-7-K}{RGB}{161,215,106}
\definecolor{PiYG-7-7}{RGB}{77,146,33}
\definecolor{PiYG-7-N}{RGB}{77,146,33}
\definecolor{PiYG-8-1}{RGB}{197,27,125}
\definecolor{PiYG-8-B}{RGB}{197,27,125}
\definecolor{PiYG-8-2}{RGB}{222,119,174}
\definecolor{PiYG-8-D}{RGB}{222,119,174}
\definecolor{PiYG-8-3}{RGB}{241,182,218}
\definecolor{PiYG-8-F}{RGB}{241,182,218}
\definecolor{PiYG-8-4}{RGB}{253,224,239}
\definecolor{PiYG-8-G}{RGB}{253,224,239}
\definecolor{PiYG-8-5}{RGB}{230,245,208}
\definecolor{PiYG-8-I}{RGB}{230,245,208}
\definecolor{PiYG-8-6}{RGB}{184,225,134}
\definecolor{PiYG-8-J}{RGB}{184,225,134}
\definecolor{PiYG-8-7}{RGB}{127,188,65}
\definecolor{PiYG-8-L}{RGB}{127,188,65}
\definecolor{PiYG-8-8}{RGB}{77,146,33}
\definecolor{PiYG-8-N}{RGB}{77,146,33}
\definecolor{PiYG-9-1}{RGB}{197,27,125}
\definecolor{PiYG-9-B}{RGB}{197,27,125}
\definecolor{PiYG-9-2}{RGB}{222,119,174}
\definecolor{PiYG-9-D}{RGB}{222,119,174}
\definecolor{PiYG-9-3}{RGB}{241,182,218}
\definecolor{PiYG-9-F}{RGB}{241,182,218}
\definecolor{PiYG-9-4}{RGB}{253,224,239}
\definecolor{PiYG-9-G}{RGB}{253,224,239}
\definecolor{PiYG-9-5}{RGB}{247,247,247}
\definecolor{PiYG-9-H}{RGB}{247,247,247}
\definecolor{PiYG-9-6}{RGB}{230,245,208}
\definecolor{PiYG-9-I}{RGB}{230,245,208}
\definecolor{PiYG-9-7}{RGB}{184,225,134}
\definecolor{PiYG-9-J}{RGB}{184,225,134}
\definecolor{PiYG-9-8}{RGB}{127,188,65}
\definecolor{PiYG-9-L}{RGB}{127,188,65}
\definecolor{PiYG-9-9}{RGB}{77,146,33}
\definecolor{PiYG-9-N}{RGB}{77,146,33}
\definecolor{PiYG-10-1}{RGB}{142,1,82}
\definecolor{PiYG-10-A}{RGB}{142,1,82}
\definecolor{PiYG-10-2}{RGB}{197,27,125}
\definecolor{PiYG-10-B}{RGB}{197,27,125}
\definecolor{PiYG-10-3}{RGB}{222,119,174}
\definecolor{PiYG-10-D}{RGB}{222,119,174}
\definecolor{PiYG-10-4}{RGB}{241,182,218}
\definecolor{PiYG-10-F}{RGB}{241,182,218}
\definecolor{PiYG-10-5}{RGB}{253,224,239}
\definecolor{PiYG-10-G}{RGB}{253,224,239}
\definecolor{PiYG-10-6}{RGB}{230,245,208}
\definecolor{PiYG-10-I}{RGB}{230,245,208}
\definecolor{PiYG-10-7}{RGB}{184,225,134}
\definecolor{PiYG-10-J}{RGB}{184,225,134}
\definecolor{PiYG-10-8}{RGB}{127,188,65}
\definecolor{PiYG-10-L}{RGB}{127,188,65}
\definecolor{PiYG-10-9}{RGB}{77,146,33}
\definecolor{PiYG-10-N}{RGB}{77,146,33}
\definecolor{PiYG-10-10}{RGB}{39,100,25}
\definecolor{PiYG-10-O}{RGB}{39,100,25}
\definecolor{PiYG-11-1}{RGB}{142,1,82}
\definecolor{PiYG-11-A}{RGB}{142,1,82}
\definecolor{PiYG-11-2}{RGB}{197,27,125}
\definecolor{PiYG-11-B}{RGB}{197,27,125}
\definecolor{PiYG-11-3}{RGB}{222,119,174}
\definecolor{PiYG-11-D}{RGB}{222,119,174}
\definecolor{PiYG-11-4}{RGB}{241,182,218}
\definecolor{PiYG-11-F}{RGB}{241,182,218}
\definecolor{PiYG-11-5}{RGB}{253,224,239}
\definecolor{PiYG-11-G}{RGB}{253,224,239}
\definecolor{PiYG-11-6}{RGB}{247,247,247}
\definecolor{PiYG-11-H}{RGB}{247,247,247}
\definecolor{PiYG-11-7}{RGB}{230,245,208}
\definecolor{PiYG-11-I}{RGB}{230,245,208}
\definecolor{PiYG-11-8}{RGB}{184,225,134}
\definecolor{PiYG-11-J}{RGB}{184,225,134}
\definecolor{PiYG-11-9}{RGB}{127,188,65}
\definecolor{PiYG-11-L}{RGB}{127,188,65}
\definecolor{PiYG-11-10}{RGB}{77,146,33}
\definecolor{PiYG-11-N}{RGB}{77,146,33}
\definecolor{PiYG-11-11}{RGB}{39,100,25}
\definecolor{PiYG-11-O}{RGB}{39,100,25}
\definecolor{RdBu-3-1}{RGB}{239,138,98}
\definecolor{RdBu-3-E}{RGB}{239,138,98}
\definecolor{RdBu-3-2}{RGB}{247,247,247}
\definecolor{RdBu-3-H}{RGB}{247,247,247}
\definecolor{RdBu-3-3}{RGB}{103,169,207}
\definecolor{RdBu-3-K}{RGB}{103,169,207}
\definecolor{RdBu-4-1}{RGB}{202,0,32}
\definecolor{RdBu-4-C}{RGB}{202,0,32}
\definecolor{RdBu-4-2}{RGB}{244,165,130}
\definecolor{RdBu-4-F}{RGB}{244,165,130}
\definecolor{RdBu-4-3}{RGB}{146,197,222}
\definecolor{RdBu-4-J}{RGB}{146,197,222}
\definecolor{RdBu-4-4}{RGB}{5,113,176}
\definecolor{RdBu-4-M}{RGB}{5,113,176}
\definecolor{RdBu-5-1}{RGB}{202,0,32}
\definecolor{RdBu-5-C}{RGB}{202,0,32}
\definecolor{RdBu-5-2}{RGB}{244,165,130}
\definecolor{RdBu-5-F}{RGB}{244,165,130}
\definecolor{RdBu-5-3}{RGB}{247,247,247}
\definecolor{RdBu-5-H}{RGB}{247,247,247}
\definecolor{RdBu-5-4}{RGB}{146,197,222}
\definecolor{RdBu-5-J}{RGB}{146,197,222}
\definecolor{RdBu-5-5}{RGB}{5,113,176}
\definecolor{RdBu-5-M}{RGB}{5,113,176}
\definecolor{RdBu-6-1}{RGB}{178,24,43}
\definecolor{RdBu-6-B}{RGB}{178,24,43}
\definecolor{RdBu-6-2}{RGB}{239,138,98}
\definecolor{RdBu-6-E}{RGB}{239,138,98}
\definecolor{RdBu-6-3}{RGB}{253,219,199}
\definecolor{RdBu-6-G}{RGB}{253,219,199}
\definecolor{RdBu-6-4}{RGB}{209,229,240}
\definecolor{RdBu-6-I}{RGB}{209,229,240}
\definecolor{RdBu-6-5}{RGB}{103,169,207}
\definecolor{RdBu-6-K}{RGB}{103,169,207}
\definecolor{RdBu-6-6}{RGB}{33,102,172}
\definecolor{RdBu-6-N}{RGB}{33,102,172}
\definecolor{RdBu-7-1}{RGB}{178,24,43}
\definecolor{RdBu-7-B}{RGB}{178,24,43}
\definecolor{RdBu-7-2}{RGB}{239,138,98}
\definecolor{RdBu-7-E}{RGB}{239,138,98}
\definecolor{RdBu-7-3}{RGB}{253,219,199}
\definecolor{RdBu-7-G}{RGB}{253,219,199}
\definecolor{RdBu-7-4}{RGB}{247,247,247}
\definecolor{RdBu-7-H}{RGB}{247,247,247}
\definecolor{RdBu-7-5}{RGB}{209,229,240}
\definecolor{RdBu-7-I}{RGB}{209,229,240}
\definecolor{RdBu-7-6}{RGB}{103,169,207}
\definecolor{RdBu-7-K}{RGB}{103,169,207}
\definecolor{RdBu-7-7}{RGB}{33,102,172}
\definecolor{RdBu-7-N}{RGB}{33,102,172}
\definecolor{RdBu-8-1}{RGB}{178,24,43}
\definecolor{RdBu-8-B}{RGB}{178,24,43}
\definecolor{RdBu-8-2}{RGB}{214,96,77}
\definecolor{RdBu-8-D}{RGB}{214,96,77}
\definecolor{RdBu-8-3}{RGB}{244,165,130}
\definecolor{RdBu-8-F}{RGB}{244,165,130}
\definecolor{RdBu-8-4}{RGB}{253,219,199}
\definecolor{RdBu-8-G}{RGB}{253,219,199}
\definecolor{RdBu-8-5}{RGB}{209,229,240}
\definecolor{RdBu-8-I}{RGB}{209,229,240}
\definecolor{RdBu-8-6}{RGB}{146,197,222}
\definecolor{RdBu-8-J}{RGB}{146,197,222}
\definecolor{RdBu-8-7}{RGB}{67,147,195}
\definecolor{RdBu-8-L}{RGB}{67,147,195}
\definecolor{RdBu-8-8}{RGB}{33,102,172}
\definecolor{RdBu-8-N}{RGB}{33,102,172}
\definecolor{RdBu-9-1}{RGB}{178,24,43}
\definecolor{RdBu-9-B}{RGB}{178,24,43}
\definecolor{RdBu-9-2}{RGB}{214,96,77}
\definecolor{RdBu-9-D}{RGB}{214,96,77}
\definecolor{RdBu-9-3}{RGB}{244,165,130}
\definecolor{RdBu-9-F}{RGB}{244,165,130}
\definecolor{RdBu-9-4}{RGB}{253,219,199}
\definecolor{RdBu-9-G}{RGB}{253,219,199}
\definecolor{RdBu-9-5}{RGB}{247,247,247}
\definecolor{RdBu-9-H}{RGB}{247,247,247}
\definecolor{RdBu-9-6}{RGB}{209,229,240}
\definecolor{RdBu-9-I}{RGB}{209,229,240}
\definecolor{RdBu-9-7}{RGB}{146,197,222}
\definecolor{RdBu-9-J}{RGB}{146,197,222}
\definecolor{RdBu-9-8}{RGB}{67,147,195}
\definecolor{RdBu-9-L}{RGB}{67,147,195}
\definecolor{RdBu-9-9}{RGB}{33,102,172}
\definecolor{RdBu-9-N}{RGB}{33,102,172}
\definecolor{RdBu-10-1}{RGB}{103,0,31}
\definecolor{RdBu-10-A}{RGB}{103,0,31}
\definecolor{RdBu-10-2}{RGB}{178,24,43}
\definecolor{RdBu-10-B}{RGB}{178,24,43}
\definecolor{RdBu-10-3}{RGB}{214,96,77}
\definecolor{RdBu-10-D}{RGB}{214,96,77}
\definecolor{RdBu-10-4}{RGB}{244,165,130}
\definecolor{RdBu-10-F}{RGB}{244,165,130}
\definecolor{RdBu-10-5}{RGB}{253,219,199}
\definecolor{RdBu-10-G}{RGB}{253,219,199}
\definecolor{RdBu-10-6}{RGB}{209,229,240}
\definecolor{RdBu-10-I}{RGB}{209,229,240}
\definecolor{RdBu-10-7}{RGB}{146,197,222}
\definecolor{RdBu-10-J}{RGB}{146,197,222}
\definecolor{RdBu-10-8}{RGB}{67,147,195}
\definecolor{RdBu-10-L}{RGB}{67,147,195}
\definecolor{RdBu-10-9}{RGB}{33,102,172}
\definecolor{RdBu-10-N}{RGB}{33,102,172}
\definecolor{RdBu-10-10}{RGB}{5,48,97}
\definecolor{RdBu-10-O}{RGB}{5,48,97}
\definecolor{RdBu-11-1}{RGB}{103,0,31}
\definecolor{RdBu-11-A}{RGB}{103,0,31}
\definecolor{RdBu-11-2}{RGB}{178,24,43}
\definecolor{RdBu-11-B}{RGB}{178,24,43}
\definecolor{RdBu-11-3}{RGB}{214,96,77}
\definecolor{RdBu-11-D}{RGB}{214,96,77}
\definecolor{RdBu-11-4}{RGB}{244,165,130}
\definecolor{RdBu-11-F}{RGB}{244,165,130}
\definecolor{RdBu-11-5}{RGB}{253,219,199}
\definecolor{RdBu-11-G}{RGB}{253,219,199}
\definecolor{RdBu-11-6}{RGB}{247,247,247}
\definecolor{RdBu-11-H}{RGB}{247,247,247}
\definecolor{RdBu-11-7}{RGB}{209,229,240}
\definecolor{RdBu-11-I}{RGB}{209,229,240}
\definecolor{RdBu-11-8}{RGB}{146,197,222}
\definecolor{RdBu-11-J}{RGB}{146,197,222}
\definecolor{RdBu-11-9}{RGB}{67,147,195}
\definecolor{RdBu-11-L}{RGB}{67,147,195}
\definecolor{RdBu-11-10}{RGB}{33,102,172}
\definecolor{RdBu-11-N}{RGB}{33,102,172}
\definecolor{RdBu-11-11}{RGB}{5,48,97}
\definecolor{RdBu-11-O}{RGB}{5,48,97}
\definecolor{RdGy-3-1}{RGB}{239,138,98}
\definecolor{RdGy-3-E}{RGB}{239,138,98}
\definecolor{RdGy-3-2}{RGB}{255,255,255}
\definecolor{RdGy-3-H}{RGB}{255,255,255}
\definecolor{RdGy-3-3}{RGB}{153,153,153}
\definecolor{RdGy-3-K}{RGB}{153,153,153}
\definecolor{RdGy-4-1}{RGB}{202,0,32}
\definecolor{RdGy-4-C}{RGB}{202,0,32}
\definecolor{RdGy-4-2}{RGB}{244,165,130}
\definecolor{RdGy-4-F}{RGB}{244,165,130}
\definecolor{RdGy-4-3}{RGB}{186,186,186}
\definecolor{RdGy-4-J}{RGB}{186,186,186}
\definecolor{RdGy-4-4}{RGB}{64,64,64}
\definecolor{RdGy-4-M}{RGB}{64,64,64}
\definecolor{RdGy-5-1}{RGB}{202,0,32}
\definecolor{RdGy-5-C}{RGB}{202,0,32}
\definecolor{RdGy-5-2}{RGB}{244,165,130}
\definecolor{RdGy-5-F}{RGB}{244,165,130}
\definecolor{RdGy-5-3}{RGB}{255,255,255}
\definecolor{RdGy-5-H}{RGB}{255,255,255}
\definecolor{RdGy-5-4}{RGB}{186,186,186}
\definecolor{RdGy-5-J}{RGB}{186,186,186}
\definecolor{RdGy-5-5}{RGB}{64,64,64}
\definecolor{RdGy-5-M}{RGB}{64,64,64}
\definecolor{RdGy-6-1}{RGB}{178,24,43}
\definecolor{RdGy-6-B}{RGB}{178,24,43}
\definecolor{RdGy-6-2}{RGB}{239,138,98}
\definecolor{RdGy-6-E}{RGB}{239,138,98}
\definecolor{RdGy-6-3}{RGB}{253,219,199}
\definecolor{RdGy-6-G}{RGB}{253,219,199}
\definecolor{RdGy-6-4}{RGB}{224,224,224}
\definecolor{RdGy-6-I}{RGB}{224,224,224}
\definecolor{RdGy-6-5}{RGB}{153,153,153}
\definecolor{RdGy-6-K}{RGB}{153,153,153}
\definecolor{RdGy-6-6}{RGB}{77,77,77}
\definecolor{RdGy-6-N}{RGB}{77,77,77}
\definecolor{RdGy-7-1}{RGB}{178,24,43}
\definecolor{RdGy-7-B}{RGB}{178,24,43}
\definecolor{RdGy-7-2}{RGB}{239,138,98}
\definecolor{RdGy-7-E}{RGB}{239,138,98}
\definecolor{RdGy-7-3}{RGB}{253,219,199}
\definecolor{RdGy-7-G}{RGB}{253,219,199}
\definecolor{RdGy-7-4}{RGB}{255,255,255}
\definecolor{RdGy-7-H}{RGB}{255,255,255}
\definecolor{RdGy-7-5}{RGB}{224,224,224}
\definecolor{RdGy-7-I}{RGB}{224,224,224}
\definecolor{RdGy-7-6}{RGB}{153,153,153}
\definecolor{RdGy-7-K}{RGB}{153,153,153}
\definecolor{RdGy-7-7}{RGB}{77,77,77}
\definecolor{RdGy-7-N}{RGB}{77,77,77}
\definecolor{RdGy-8-1}{RGB}{178,24,43}
\definecolor{RdGy-8-B}{RGB}{178,24,43}
\definecolor{RdGy-8-2}{RGB}{214,96,77}
\definecolor{RdGy-8-D}{RGB}{214,96,77}
\definecolor{RdGy-8-3}{RGB}{244,165,130}
\definecolor{RdGy-8-F}{RGB}{244,165,130}
\definecolor{RdGy-8-4}{RGB}{253,219,199}
\definecolor{RdGy-8-G}{RGB}{253,219,199}
\definecolor{RdGy-8-5}{RGB}{224,224,224}
\definecolor{RdGy-8-I}{RGB}{224,224,224}
\definecolor{RdGy-8-6}{RGB}{186,186,186}
\definecolor{RdGy-8-J}{RGB}{186,186,186}
\definecolor{RdGy-8-7}{RGB}{135,135,135}
\definecolor{RdGy-8-L}{RGB}{135,135,135}
\definecolor{RdGy-8-8}{RGB}{77,77,77}
\definecolor{RdGy-8-N}{RGB}{77,77,77}
\definecolor{RdGy-9-1}{RGB}{178,24,43}
\definecolor{RdGy-9-B}{RGB}{178,24,43}
\definecolor{RdGy-9-2}{RGB}{214,96,77}
\definecolor{RdGy-9-D}{RGB}{214,96,77}
\definecolor{RdGy-9-3}{RGB}{244,165,130}
\definecolor{RdGy-9-F}{RGB}{244,165,130}
\definecolor{RdGy-9-4}{RGB}{253,219,199}
\definecolor{RdGy-9-G}{RGB}{253,219,199}
\definecolor{RdGy-9-5}{RGB}{255,255,255}
\definecolor{RdGy-9-H}{RGB}{255,255,255}
\definecolor{RdGy-9-6}{RGB}{224,224,224}
\definecolor{RdGy-9-I}{RGB}{224,224,224}
\definecolor{RdGy-9-7}{RGB}{186,186,186}
\definecolor{RdGy-9-J}{RGB}{186,186,186}
\definecolor{RdGy-9-8}{RGB}{135,135,135}
\definecolor{RdGy-9-L}{RGB}{135,135,135}
\definecolor{RdGy-9-9}{RGB}{77,77,77}
\definecolor{RdGy-9-N}{RGB}{77,77,77}
\definecolor{RdGy-10-1}{RGB}{103,0,31}
\definecolor{RdGy-10-A}{RGB}{103,0,31}
\definecolor{RdGy-10-2}{RGB}{178,24,43}
\definecolor{RdGy-10-B}{RGB}{178,24,43}
\definecolor{RdGy-10-3}{RGB}{214,96,77}
\definecolor{RdGy-10-D}{RGB}{214,96,77}
\definecolor{RdGy-10-4}{RGB}{244,165,130}
\definecolor{RdGy-10-F}{RGB}{244,165,130}
\definecolor{RdGy-10-5}{RGB}{253,219,199}
\definecolor{RdGy-10-G}{RGB}{253,219,199}
\definecolor{RdGy-10-6}{RGB}{224,224,224}
\definecolor{RdGy-10-I}{RGB}{224,224,224}
\definecolor{RdGy-10-7}{RGB}{186,186,186}
\definecolor{RdGy-10-J}{RGB}{186,186,186}
\definecolor{RdGy-10-8}{RGB}{135,135,135}
\definecolor{RdGy-10-L}{RGB}{135,135,135}
\definecolor{RdGy-10-9}{RGB}{77,77,77}
\definecolor{RdGy-10-N}{RGB}{77,77,77}
\definecolor{RdGy-10-10}{RGB}{26,26,26}
\definecolor{RdGy-10-O}{RGB}{26,26,26}
\definecolor{RdGy-11-1}{RGB}{103,0,31}
\definecolor{RdGy-11-A}{RGB}{103,0,31}
\definecolor{RdGy-11-2}{RGB}{178,24,43}
\definecolor{RdGy-11-B}{RGB}{178,24,43}
\definecolor{RdGy-11-3}{RGB}{214,96,77}
\definecolor{RdGy-11-D}{RGB}{214,96,77}
\definecolor{RdGy-11-4}{RGB}{244,165,130}
\definecolor{RdGy-11-F}{RGB}{244,165,130}
\definecolor{RdGy-11-5}{RGB}{253,219,199}
\definecolor{RdGy-11-G}{RGB}{253,219,199}
\definecolor{RdGy-11-6}{RGB}{255,255,255}
\definecolor{RdGy-11-H}{RGB}{255,255,255}
\definecolor{RdGy-11-7}{RGB}{224,224,224}
\definecolor{RdGy-11-I}{RGB}{224,224,224}
\definecolor{RdGy-11-8}{RGB}{186,186,186}
\definecolor{RdGy-11-J}{RGB}{186,186,186}
\definecolor{RdGy-11-9}{RGB}{135,135,135}
\definecolor{RdGy-11-L}{RGB}{135,135,135}
\definecolor{RdGy-11-10}{RGB}{77,77,77}
\definecolor{RdGy-11-N}{RGB}{77,77,77}
\definecolor{RdGy-11-11}{RGB}{26,26,26}
\definecolor{RdGy-11-O}{RGB}{26,26,26}
\definecolor{RdYlBu-3-1}{RGB}{252,141,89}
\definecolor{RdYlBu-3-E}{RGB}{252,141,89}
\definecolor{RdYlBu-3-2}{RGB}{255,255,191}
\definecolor{RdYlBu-3-H}{RGB}{255,255,191}
\definecolor{RdYlBu-3-3}{RGB}{145,191,219}
\definecolor{RdYlBu-3-K}{RGB}{145,191,219}
\definecolor{RdYlBu-4-1}{RGB}{215,25,28}
\definecolor{RdYlBu-4-C}{RGB}{215,25,28}
\definecolor{RdYlBu-4-2}{RGB}{253,174,97}
\definecolor{RdYlBu-4-F}{RGB}{253,174,97}
\definecolor{RdYlBu-4-3}{RGB}{171,217,233}
\definecolor{RdYlBu-4-J}{RGB}{171,217,233}
\definecolor{RdYlBu-4-4}{RGB}{44,123,182}
\definecolor{RdYlBu-4-M}{RGB}{44,123,182}
\definecolor{RdYlBu-5-1}{RGB}{215,25,28}
\definecolor{RdYlBu-5-C}{RGB}{215,25,28}
\definecolor{RdYlBu-5-2}{RGB}{253,174,97}
\definecolor{RdYlBu-5-F}{RGB}{253,174,97}
\definecolor{RdYlBu-5-3}{RGB}{255,255,191}
\definecolor{RdYlBu-5-H}{RGB}{255,255,191}
\definecolor{RdYlBu-5-4}{RGB}{171,217,233}
\definecolor{RdYlBu-5-J}{RGB}{171,217,233}
\definecolor{RdYlBu-5-5}{RGB}{44,123,182}
\definecolor{RdYlBu-5-M}{RGB}{44,123,182}
\definecolor{RdYlBu-6-1}{RGB}{215,48,39}
\definecolor{RdYlBu-6-B}{RGB}{215,48,39}
\definecolor{RdYlBu-6-2}{RGB}{252,141,89}
\definecolor{RdYlBu-6-E}{RGB}{252,141,89}
\definecolor{RdYlBu-6-3}{RGB}{254,224,144}
\definecolor{RdYlBu-6-G}{RGB}{254,224,144}
\definecolor{RdYlBu-6-4}{RGB}{224,243,248}
\definecolor{RdYlBu-6-I}{RGB}{224,243,248}
\definecolor{RdYlBu-6-5}{RGB}{145,191,219}
\definecolor{RdYlBu-6-K}{RGB}{145,191,219}
\definecolor{RdYlBu-6-6}{RGB}{69,117,180}
\definecolor{RdYlBu-6-N}{RGB}{69,117,180}
\definecolor{RdYlBu-7-1}{RGB}{215,48,39}
\definecolor{RdYlBu-7-B}{RGB}{215,48,39}
\definecolor{RdYlBu-7-2}{RGB}{252,141,89}
\definecolor{RdYlBu-7-E}{RGB}{252,141,89}
\definecolor{RdYlBu-7-3}{RGB}{254,224,144}
\definecolor{RdYlBu-7-G}{RGB}{254,224,144}
\definecolor{RdYlBu-7-4}{RGB}{255,255,191}
\definecolor{RdYlBu-7-H}{RGB}{255,255,191}
\definecolor{RdYlBu-7-5}{RGB}{224,243,248}
\definecolor{RdYlBu-7-I}{RGB}{224,243,248}
\definecolor{RdYlBu-7-6}{RGB}{145,191,219}
\definecolor{RdYlBu-7-K}{RGB}{145,191,219}
\definecolor{RdYlBu-7-7}{RGB}{69,117,180}
\definecolor{RdYlBu-7-N}{RGB}{69,117,180}
\definecolor{RdYlBu-8-1}{RGB}{215,48,39}
\definecolor{RdYlBu-8-B}{RGB}{215,48,39}
\definecolor{RdYlBu-8-2}{RGB}{244,109,67}
\definecolor{RdYlBu-8-D}{RGB}{244,109,67}
\definecolor{RdYlBu-8-3}{RGB}{253,174,97}
\definecolor{RdYlBu-8-F}{RGB}{253,174,97}
\definecolor{RdYlBu-8-4}{RGB}{254,224,144}
\definecolor{RdYlBu-8-G}{RGB}{254,224,144}
\definecolor{RdYlBu-8-5}{RGB}{224,243,248}
\definecolor{RdYlBu-8-I}{RGB}{224,243,248}
\definecolor{RdYlBu-8-6}{RGB}{171,217,233}
\definecolor{RdYlBu-8-J}{RGB}{171,217,233}
\definecolor{RdYlBu-8-7}{RGB}{116,173,209}
\definecolor{RdYlBu-8-L}{RGB}{116,173,209}
\definecolor{RdYlBu-8-8}{RGB}{69,117,180}
\definecolor{RdYlBu-8-N}{RGB}{69,117,180}
\definecolor{RdYlBu-9-1}{RGB}{215,48,39}
\definecolor{RdYlBu-9-B}{RGB}{215,48,39}
\definecolor{RdYlBu-9-2}{RGB}{244,109,67}
\definecolor{RdYlBu-9-D}{RGB}{244,109,67}
\definecolor{RdYlBu-9-3}{RGB}{253,174,97}
\definecolor{RdYlBu-9-F}{RGB}{253,174,97}
\definecolor{RdYlBu-9-4}{RGB}{254,224,144}
\definecolor{RdYlBu-9-G}{RGB}{254,224,144}
\definecolor{RdYlBu-9-5}{RGB}{255,255,191}
\definecolor{RdYlBu-9-H}{RGB}{255,255,191}
\definecolor{RdYlBu-9-6}{RGB}{224,243,248}
\definecolor{RdYlBu-9-I}{RGB}{224,243,248}
\definecolor{RdYlBu-9-7}{RGB}{171,217,233}
\definecolor{RdYlBu-9-J}{RGB}{171,217,233}
\definecolor{RdYlBu-9-8}{RGB}{116,173,209}
\definecolor{RdYlBu-9-L}{RGB}{116,173,209}
\definecolor{RdYlBu-9-9}{RGB}{69,117,180}
\definecolor{RdYlBu-9-N}{RGB}{69,117,180}
\definecolor{RdYlBu-10-1}{RGB}{165,0,38}
\definecolor{RdYlBu-10-A}{RGB}{165,0,38}
\definecolor{RdYlBu-10-2}{RGB}{215,48,39}
\definecolor{RdYlBu-10-B}{RGB}{215,48,39}
\definecolor{RdYlBu-10-3}{RGB}{244,109,67}
\definecolor{RdYlBu-10-D}{RGB}{244,109,67}
\definecolor{RdYlBu-10-4}{RGB}{253,174,97}
\definecolor{RdYlBu-10-F}{RGB}{253,174,97}
\definecolor{RdYlBu-10-5}{RGB}{254,224,144}
\definecolor{RdYlBu-10-G}{RGB}{254,224,144}
\definecolor{RdYlBu-10-6}{RGB}{224,243,248}
\definecolor{RdYlBu-10-I}{RGB}{224,243,248}
\definecolor{RdYlBu-10-7}{RGB}{171,217,233}
\definecolor{RdYlBu-10-J}{RGB}{171,217,233}
\definecolor{RdYlBu-10-8}{RGB}{116,173,209}
\definecolor{RdYlBu-10-L}{RGB}{116,173,209}
\definecolor{RdYlBu-10-9}{RGB}{69,117,180}
\definecolor{RdYlBu-10-N}{RGB}{69,117,180}
\definecolor{RdYlBu-10-10}{RGB}{49,54,149}
\definecolor{RdYlBu-10-O}{RGB}{49,54,149}
\definecolor{RdYlBu-11-1}{RGB}{165,0,38}
\definecolor{RdYlBu-11-A}{RGB}{165,0,38}
\definecolor{RdYlBu-11-2}{RGB}{215,48,39}
\definecolor{RdYlBu-11-B}{RGB}{215,48,39}
\definecolor{RdYlBu-11-3}{RGB}{244,109,67}
\definecolor{RdYlBu-11-D}{RGB}{244,109,67}
\definecolor{RdYlBu-11-4}{RGB}{253,174,97}
\definecolor{RdYlBu-11-F}{RGB}{253,174,97}
\definecolor{RdYlBu-11-5}{RGB}{254,224,144}
\definecolor{RdYlBu-11-G}{RGB}{254,224,144}
\definecolor{RdYlBu-11-6}{RGB}{255,255,191}
\definecolor{RdYlBu-11-H}{RGB}{255,255,191}
\definecolor{RdYlBu-11-7}{RGB}{224,243,248}
\definecolor{RdYlBu-11-I}{RGB}{224,243,248}
\definecolor{RdYlBu-11-8}{RGB}{171,217,233}
\definecolor{RdYlBu-11-J}{RGB}{171,217,233}
\definecolor{RdYlBu-11-9}{RGB}{116,173,209}
\definecolor{RdYlBu-11-L}{RGB}{116,173,209}
\definecolor{RdYlBu-11-10}{RGB}{69,117,180}
\definecolor{RdYlBu-11-N}{RGB}{69,117,180}
\definecolor{RdYlBu-11-11}{RGB}{49,54,149}
\definecolor{RdYlBu-11-O}{RGB}{49,54,149}
\definecolor{Spectral-3-1}{RGB}{252,141,89}
\definecolor{Spectral-3-E}{RGB}{252,141,89}
\definecolor{Spectral-3-2}{RGB}{255,255,191}
\definecolor{Spectral-3-H}{RGB}{255,255,191}
\definecolor{Spectral-3-3}{RGB}{153,213,148}
\definecolor{Spectral-3-K}{RGB}{153,213,148}
\definecolor{Spectral-4-1}{RGB}{215,25,28}
\definecolor{Spectral-4-C}{RGB}{215,25,28}
\definecolor{Spectral-4-2}{RGB}{253,174,97}
\definecolor{Spectral-4-F}{RGB}{253,174,97}
\definecolor{Spectral-4-3}{RGB}{171,221,164}
\definecolor{Spectral-4-J}{RGB}{171,221,164}
\definecolor{Spectral-4-4}{RGB}{43,131,186}
\definecolor{Spectral-4-M}{RGB}{43,131,186}
\definecolor{Spectral-5-1}{RGB}{215,25,28}
\definecolor{Spectral-5-C}{RGB}{215,25,28}
\definecolor{Spectral-5-2}{RGB}{253,174,97}
\definecolor{Spectral-5-F}{RGB}{253,174,97}
\definecolor{Spectral-5-3}{RGB}{255,255,191}
\definecolor{Spectral-5-H}{RGB}{255,255,191}
\definecolor{Spectral-5-4}{RGB}{171,221,164}
\definecolor{Spectral-5-J}{RGB}{171,221,164}
\definecolor{Spectral-5-5}{RGB}{43,131,186}
\definecolor{Spectral-5-M}{RGB}{43,131,186}
\definecolor{Spectral-6-1}{RGB}{213,62,79}
\definecolor{Spectral-6-B}{RGB}{213,62,79}
\definecolor{Spectral-6-2}{RGB}{252,141,89}
\definecolor{Spectral-6-E}{RGB}{252,141,89}
\definecolor{Spectral-6-3}{RGB}{254,224,139}
\definecolor{Spectral-6-G}{RGB}{254,224,139}
\definecolor{Spectral-6-4}{RGB}{230,245,152}
\definecolor{Spectral-6-I}{RGB}{230,245,152}
\definecolor{Spectral-6-5}{RGB}{153,213,148}
\definecolor{Spectral-6-K}{RGB}{153,213,148}
\definecolor{Spectral-6-6}{RGB}{50,136,189}
\definecolor{Spectral-6-N}{RGB}{50,136,189}
\definecolor{Spectral-7-1}{RGB}{213,62,79}
\definecolor{Spectral-7-B}{RGB}{213,62,79}
\definecolor{Spectral-7-2}{RGB}{252,141,89}
\definecolor{Spectral-7-E}{RGB}{252,141,89}
\definecolor{Spectral-7-3}{RGB}{254,224,139}
\definecolor{Spectral-7-G}{RGB}{254,224,139}
\definecolor{Spectral-7-4}{RGB}{255,255,191}
\definecolor{Spectral-7-H}{RGB}{255,255,191}
\definecolor{Spectral-7-5}{RGB}{230,245,152}
\definecolor{Spectral-7-I}{RGB}{230,245,152}
\definecolor{Spectral-7-6}{RGB}{153,213,148}
\definecolor{Spectral-7-K}{RGB}{153,213,148}
\definecolor{Spectral-7-7}{RGB}{50,136,189}
\definecolor{Spectral-7-N}{RGB}{50,136,189}
\definecolor{Spectral-8-1}{RGB}{213,62,79}
\definecolor{Spectral-8-B}{RGB}{213,62,79}
\definecolor{Spectral-8-2}{RGB}{244,109,67}
\definecolor{Spectral-8-D}{RGB}{244,109,67}
\definecolor{Spectral-8-3}{RGB}{253,174,97}
\definecolor{Spectral-8-F}{RGB}{253,174,97}
\definecolor{Spectral-8-4}{RGB}{254,224,139}
\definecolor{Spectral-8-G}{RGB}{254,224,139}
\definecolor{Spectral-8-5}{RGB}{230,245,152}
\definecolor{Spectral-8-I}{RGB}{230,245,152}
\definecolor{Spectral-8-6}{RGB}{171,221,164}
\definecolor{Spectral-8-J}{RGB}{171,221,164}
\definecolor{Spectral-8-7}{RGB}{102,194,165}
\definecolor{Spectral-8-L}{RGB}{102,194,165}
\definecolor{Spectral-8-8}{RGB}{50,136,189}
\definecolor{Spectral-8-N}{RGB}{50,136,189}
\definecolor{Spectral-9-1}{RGB}{213,62,79}
\definecolor{Spectral-9-B}{RGB}{213,62,79}
\definecolor{Spectral-9-2}{RGB}{244,109,67}
\definecolor{Spectral-9-D}{RGB}{244,109,67}
\definecolor{Spectral-9-3}{RGB}{253,174,97}
\definecolor{Spectral-9-F}{RGB}{253,174,97}
\definecolor{Spectral-9-4}{RGB}{254,224,139}
\definecolor{Spectral-9-G}{RGB}{254,224,139}
\definecolor{Spectral-9-5}{RGB}{255,255,191}
\definecolor{Spectral-9-H}{RGB}{255,255,191}
\definecolor{Spectral-9-6}{RGB}{230,245,152}
\definecolor{Spectral-9-I}{RGB}{230,245,152}
\definecolor{Spectral-9-7}{RGB}{171,221,164}
\definecolor{Spectral-9-J}{RGB}{171,221,164}
\definecolor{Spectral-9-8}{RGB}{102,194,165}
\definecolor{Spectral-9-L}{RGB}{102,194,165}
\definecolor{Spectral-9-9}{RGB}{50,136,189}
\definecolor{Spectral-9-N}{RGB}{50,136,189}
\definecolor{Spectral-10-1}{RGB}{158,1,66}
\definecolor{Spectral-10-A}{RGB}{158,1,66}
\definecolor{Spectral-10-2}{RGB}{213,62,79}
\definecolor{Spectral-10-B}{RGB}{213,62,79}
\definecolor{Spectral-10-3}{RGB}{244,109,67}
\definecolor{Spectral-10-D}{RGB}{244,109,67}
\definecolor{Spectral-10-4}{RGB}{253,174,97}
\definecolor{Spectral-10-F}{RGB}{253,174,97}
\definecolor{Spectral-10-5}{RGB}{254,224,139}
\definecolor{Spectral-10-G}{RGB}{254,224,139}
\definecolor{Spectral-10-6}{RGB}{230,245,152}
\definecolor{Spectral-10-I}{RGB}{230,245,152}
\definecolor{Spectral-10-7}{RGB}{171,221,164}
\definecolor{Spectral-10-J}{RGB}{171,221,164}
\definecolor{Spectral-10-8}{RGB}{102,194,165}
\definecolor{Spectral-10-L}{RGB}{102,194,165}
\definecolor{Spectral-10-9}{RGB}{50,136,189}
\definecolor{Spectral-10-N}{RGB}{50,136,189}
\definecolor{Spectral-10-10}{RGB}{94,79,162}
\definecolor{Spectral-10-O}{RGB}{94,79,162}
\definecolor{Spectral-11-1}{RGB}{158,1,66}
\definecolor{Spectral-11-A}{RGB}{158,1,66}
\definecolor{Spectral-11-2}{RGB}{213,62,79}
\definecolor{Spectral-11-B}{RGB}{213,62,79}
\definecolor{Spectral-11-3}{RGB}{244,109,67}
\definecolor{Spectral-11-D}{RGB}{244,109,67}
\definecolor{Spectral-11-4}{RGB}{253,174,97}
\definecolor{Spectral-11-F}{RGB}{253,174,97}
\definecolor{Spectral-11-5}{RGB}{254,224,139}
\definecolor{Spectral-11-G}{RGB}{254,224,139}
\definecolor{Spectral-11-6}{RGB}{255,255,191}
\definecolor{Spectral-11-H}{RGB}{255,255,191}
\definecolor{Spectral-11-7}{RGB}{230,245,152}
\definecolor{Spectral-11-I}{RGB}{230,245,152}
\definecolor{Spectral-11-8}{RGB}{171,221,164}
\definecolor{Spectral-11-J}{RGB}{171,221,164}
\definecolor{Spectral-11-9}{RGB}{102,194,165}
\definecolor{Spectral-11-L}{RGB}{102,194,165}
\definecolor{Spectral-11-10}{RGB}{50,136,189}
\definecolor{Spectral-11-N}{RGB}{50,136,189}
\definecolor{Spectral-11-11}{RGB}{94,79,162}
\definecolor{Spectral-11-O}{RGB}{94,79,162}
\definecolor{RdYlGn-3-1}{RGB}{252,141,89}
\definecolor{RdYlGn-3-E}{RGB}{252,141,89}
\definecolor{RdYlGn-3-2}{RGB}{255,255,191}
\definecolor{RdYlGn-3-H}{RGB}{255,255,191}
\definecolor{RdYlGn-3-3}{RGB}{145,207,96}
\definecolor{RdYlGn-3-K}{RGB}{145,207,96}
\definecolor{RdYlGn-4-1}{RGB}{215,25,28}
\definecolor{RdYlGn-4-C}{RGB}{215,25,28}
\definecolor{RdYlGn-4-2}{RGB}{253,174,97}
\definecolor{RdYlGn-4-F}{RGB}{253,174,97}
\definecolor{RdYlGn-4-3}{RGB}{166,217,106}
\definecolor{RdYlGn-4-J}{RGB}{166,217,106}
\definecolor{RdYlGn-4-4}{RGB}{26,150,65}
\definecolor{RdYlGn-4-M}{RGB}{26,150,65}
\definecolor{RdYlGn-5-1}{RGB}{215,25,28}
\definecolor{RdYlGn-5-C}{RGB}{215,25,28}
\definecolor{RdYlGn-5-2}{RGB}{253,174,97}
\definecolor{RdYlGn-5-F}{RGB}{253,174,97}
\definecolor{RdYlGn-5-3}{RGB}{255,255,191}
\definecolor{RdYlGn-5-H}{RGB}{255,255,191}
\definecolor{RdYlGn-5-4}{RGB}{166,217,106}
\definecolor{RdYlGn-5-J}{RGB}{166,217,106}
\definecolor{RdYlGn-5-5}{RGB}{26,150,65}
\definecolor{RdYlGn-5-M}{RGB}{26,150,65}
\definecolor{RdYlGn-6-1}{RGB}{215,48,39}
\definecolor{RdYlGn-6-B}{RGB}{215,48,39}
\definecolor{RdYlGn-6-2}{RGB}{252,141,89}
\definecolor{RdYlGn-6-E}{RGB}{252,141,89}
\definecolor{RdYlGn-6-3}{RGB}{254,224,139}
\definecolor{RdYlGn-6-G}{RGB}{254,224,139}
\definecolor{RdYlGn-6-4}{RGB}{217,239,139}
\definecolor{RdYlGn-6-I}{RGB}{217,239,139}
\definecolor{RdYlGn-6-5}{RGB}{145,207,96}
\definecolor{RdYlGn-6-K}{RGB}{145,207,96}
\definecolor{RdYlGn-6-6}{RGB}{26,152,80}
\definecolor{RdYlGn-6-N}{RGB}{26,152,80}
\definecolor{RdYlGn-7-1}{RGB}{215,48,39}
\definecolor{RdYlGn-7-B}{RGB}{215,48,39}
\definecolor{RdYlGn-7-2}{RGB}{252,141,89}
\definecolor{RdYlGn-7-E}{RGB}{252,141,89}
\definecolor{RdYlGn-7-3}{RGB}{254,224,139}
\definecolor{RdYlGn-7-G}{RGB}{254,224,139}
\definecolor{RdYlGn-7-4}{RGB}{255,255,191}
\definecolor{RdYlGn-7-H}{RGB}{255,255,191}
\definecolor{RdYlGn-7-5}{RGB}{217,239,139}
\definecolor{RdYlGn-7-I}{RGB}{217,239,139}
\definecolor{RdYlGn-7-6}{RGB}{145,207,96}
\definecolor{RdYlGn-7-K}{RGB}{145,207,96}
\definecolor{RdYlGn-7-7}{RGB}{26,152,80}
\definecolor{RdYlGn-7-N}{RGB}{26,152,80}
\definecolor{RdYlGn-8-1}{RGB}{215,48,39}
\definecolor{RdYlGn-8-B}{RGB}{215,48,39}
\definecolor{RdYlGn-8-2}{RGB}{244,109,67}
\definecolor{RdYlGn-8-D}{RGB}{244,109,67}
\definecolor{RdYlGn-8-3}{RGB}{253,174,97}
\definecolor{RdYlGn-8-F}{RGB}{253,174,97}
\definecolor{RdYlGn-8-4}{RGB}{254,224,139}
\definecolor{RdYlGn-8-G}{RGB}{254,224,139}
\definecolor{RdYlGn-8-5}{RGB}{217,239,139}
\definecolor{RdYlGn-8-I}{RGB}{217,239,139}
\definecolor{RdYlGn-8-6}{RGB}{166,217,106}
\definecolor{RdYlGn-8-J}{RGB}{166,217,106}
\definecolor{RdYlGn-8-7}{RGB}{102,189,99}
\definecolor{RdYlGn-8-L}{RGB}{102,189,99}
\definecolor{RdYlGn-8-8}{RGB}{26,152,80}
\definecolor{RdYlGn-8-N}{RGB}{26,152,80}
\definecolor{RdYlGn-9-1}{RGB}{215,48,39}
\definecolor{RdYlGn-9-B}{RGB}{215,48,39}
\definecolor{RdYlGn-9-2}{RGB}{244,109,67}
\definecolor{RdYlGn-9-D}{RGB}{244,109,67}
\definecolor{RdYlGn-9-3}{RGB}{253,174,97}
\definecolor{RdYlGn-9-F}{RGB}{253,174,97}
\definecolor{RdYlGn-9-4}{RGB}{254,224,139}
\definecolor{RdYlGn-9-G}{RGB}{254,224,139}
\definecolor{RdYlGn-9-5}{RGB}{255,255,191}
\definecolor{RdYlGn-9-H}{RGB}{255,255,191}
\definecolor{RdYlGn-9-6}{RGB}{217,239,139}
\definecolor{RdYlGn-9-I}{RGB}{217,239,139}
\definecolor{RdYlGn-9-7}{RGB}{166,217,106}
\definecolor{RdYlGn-9-J}{RGB}{166,217,106}
\definecolor{RdYlGn-9-8}{RGB}{102,189,99}
\definecolor{RdYlGn-9-L}{RGB}{102,189,99}
\definecolor{RdYlGn-9-9}{RGB}{26,152,80}
\definecolor{RdYlGn-9-N}{RGB}{26,152,80}
\definecolor{RdYlGn-10-1}{RGB}{165,0,38}
\definecolor{RdYlGn-10-A}{RGB}{165,0,38}
\definecolor{RdYlGn-10-2}{RGB}{215,48,39}
\definecolor{RdYlGn-10-B}{RGB}{215,48,39}
\definecolor{RdYlGn-10-3}{RGB}{244,109,67}
\definecolor{RdYlGn-10-D}{RGB}{244,109,67}
\definecolor{RdYlGn-10-4}{RGB}{253,174,97}
\definecolor{RdYlGn-10-F}{RGB}{253,174,97}
\definecolor{RdYlGn-10-5}{RGB}{254,224,139}
\definecolor{RdYlGn-10-G}{RGB}{254,224,139}
\definecolor{RdYlGn-10-6}{RGB}{217,239,139}
\definecolor{RdYlGn-10-I}{RGB}{217,239,139}
\definecolor{RdYlGn-10-7}{RGB}{166,217,106}
\definecolor{RdYlGn-10-J}{RGB}{166,217,106}
\definecolor{RdYlGn-10-8}{RGB}{102,189,99}
\definecolor{RdYlGn-10-L}{RGB}{102,189,99}
\definecolor{RdYlGn-10-9}{RGB}{26,152,80}
\definecolor{RdYlGn-10-N}{RGB}{26,152,80}
\definecolor{RdYlGn-10-10}{RGB}{0,104,55}
\definecolor{RdYlGn-10-O}{RGB}{0,104,55}
\definecolor{RdYlGn-11-1}{RGB}{165,0,38}
\definecolor{RdYlGn-11-A}{RGB}{165,0,38}
\definecolor{RdYlGn-11-2}{RGB}{215,48,39}
\definecolor{RdYlGn-11-B}{RGB}{215,48,39}
\definecolor{RdYlGn-11-3}{RGB}{244,109,67}
\definecolor{RdYlGn-11-D}{RGB}{244,109,67}
\definecolor{RdYlGn-11-4}{RGB}{253,174,97}
\definecolor{RdYlGn-11-F}{RGB}{253,174,97}
\definecolor{RdYlGn-11-5}{RGB}{254,224,139}
\definecolor{RdYlGn-11-G}{RGB}{254,224,139}
\definecolor{RdYlGn-11-6}{RGB}{255,255,191}
\definecolor{RdYlGn-11-H}{RGB}{255,255,191}
\definecolor{RdYlGn-11-7}{RGB}{217,239,139}
\definecolor{RdYlGn-11-I}{RGB}{217,239,139}
\definecolor{RdYlGn-11-8}{RGB}{166,217,106}
\definecolor{RdYlGn-11-J}{RGB}{166,217,106}
\definecolor{RdYlGn-11-9}{RGB}{102,189,99}
\definecolor{RdYlGn-11-L}{RGB}{102,189,99}
\definecolor{RdYlGn-11-10}{RGB}{26,152,80}
\definecolor{RdYlGn-11-N}{RGB}{26,152,80}
\definecolor{RdYlGn-11-11}{RGB}{0,104,55}
\definecolor{RdYlGn-11-O}{RGB}{0,104,55}
\definecolor{Set3-3-1}{RGB}{141,211,199}
\definecolor{Set3-3-A}{RGB}{141,211,199}
\definecolor{Set3-3-2}{RGB}{255,255,179}
\definecolor{Set3-3-B}{RGB}{255,255,179}
\definecolor{Set3-3-3}{RGB}{190,186,218}
\definecolor{Set3-3-C}{RGB}{190,186,218}
\definecolor{Set3-4-1}{RGB}{141,211,199}
\definecolor{Set3-4-A}{RGB}{141,211,199}
\definecolor{Set3-4-2}{RGB}{255,255,179}
\definecolor{Set3-4-B}{RGB}{255,255,179}
\definecolor{Set3-4-3}{RGB}{190,186,218}
\definecolor{Set3-4-C}{RGB}{190,186,218}
\definecolor{Set3-4-4}{RGB}{251,128,114}
\definecolor{Set3-4-D}{RGB}{251,128,114}
\definecolor{Set3-5-1}{RGB}{141,211,199}
\definecolor{Set3-5-A}{RGB}{141,211,199}
\definecolor{Set3-5-2}{RGB}{255,255,179}
\definecolor{Set3-5-B}{RGB}{255,255,179}
\definecolor{Set3-5-3}{RGB}{190,186,218}
\definecolor{Set3-5-C}{RGB}{190,186,218}
\definecolor{Set3-5-4}{RGB}{251,128,114}
\definecolor{Set3-5-D}{RGB}{251,128,114}
\definecolor{Set3-5-5}{RGB}{128,177,211}
\definecolor{Set3-5-E}{RGB}{128,177,211}
\definecolor{Set3-6-1}{RGB}{141,211,199}
\definecolor{Set3-6-A}{RGB}{141,211,199}
\definecolor{Set3-6-2}{RGB}{255,255,179}
\definecolor{Set3-6-B}{RGB}{255,255,179}
\definecolor{Set3-6-3}{RGB}{190,186,218}
\definecolor{Set3-6-C}{RGB}{190,186,218}
\definecolor{Set3-6-4}{RGB}{251,128,114}
\definecolor{Set3-6-D}{RGB}{251,128,114}
\definecolor{Set3-6-5}{RGB}{128,177,211}
\definecolor{Set3-6-E}{RGB}{128,177,211}
\definecolor{Set3-6-6}{RGB}{253,180,98}
\definecolor{Set3-6-F}{RGB}{253,180,98}
\definecolor{Set3-7-1}{RGB}{141,211,199}
\definecolor{Set3-7-A}{RGB}{141,211,199}
\definecolor{Set3-7-2}{RGB}{255,255,179}
\definecolor{Set3-7-B}{RGB}{255,255,179}
\definecolor{Set3-7-3}{RGB}{190,186,218}
\definecolor{Set3-7-C}{RGB}{190,186,218}
\definecolor{Set3-7-4}{RGB}{251,128,114}
\definecolor{Set3-7-D}{RGB}{251,128,114}
\definecolor{Set3-7-5}{RGB}{128,177,211}
\definecolor{Set3-7-E}{RGB}{128,177,211}
\definecolor{Set3-7-6}{RGB}{253,180,98}
\definecolor{Set3-7-F}{RGB}{253,180,98}
\definecolor{Set3-7-7}{RGB}{179,222,105}
\definecolor{Set3-7-G}{RGB}{179,222,105}
\definecolor{Set3-8-1}{RGB}{141,211,199}
\definecolor{Set3-8-A}{RGB}{141,211,199}
\definecolor{Set3-8-2}{RGB}{255,255,179}
\definecolor{Set3-8-B}{RGB}{255,255,179}
\definecolor{Set3-8-3}{RGB}{190,186,218}
\definecolor{Set3-8-C}{RGB}{190,186,218}
\definecolor{Set3-8-4}{RGB}{251,128,114}
\definecolor{Set3-8-D}{RGB}{251,128,114}
\definecolor{Set3-8-5}{RGB}{128,177,211}
\definecolor{Set3-8-E}{RGB}{128,177,211}
\definecolor{Set3-8-6}{RGB}{253,180,98}
\definecolor{Set3-8-F}{RGB}{253,180,98}
\definecolor{Set3-8-7}{RGB}{179,222,105}
\definecolor{Set3-8-G}{RGB}{179,222,105}
\definecolor{Set3-8-8}{RGB}{252,205,229}
\definecolor{Set3-8-H}{RGB}{252,205,229}
\definecolor{Set3-9-1}{RGB}{141,211,199}
\definecolor{Set3-9-A}{RGB}{141,211,199}
\definecolor{Set3-9-2}{RGB}{255,255,179}
\definecolor{Set3-9-B}{RGB}{255,255,179}
\definecolor{Set3-9-3}{RGB}{190,186,218}
\definecolor{Set3-9-C}{RGB}{190,186,218}
\definecolor{Set3-9-4}{RGB}{251,128,114}
\definecolor{Set3-9-D}{RGB}{251,128,114}
\definecolor{Set3-9-5}{RGB}{128,177,211}
\definecolor{Set3-9-E}{RGB}{128,177,211}
\definecolor{Set3-9-6}{RGB}{253,180,98}
\definecolor{Set3-9-F}{RGB}{253,180,98}
\definecolor{Set3-9-7}{RGB}{179,222,105}
\definecolor{Set3-9-G}{RGB}{179,222,105}
\definecolor{Set3-9-8}{RGB}{252,205,229}
\definecolor{Set3-9-H}{RGB}{252,205,229}
\definecolor{Set3-9-9}{RGB}{217,217,217}
\definecolor{Set3-9-I}{RGB}{217,217,217}
\definecolor{Set3-10-1}{RGB}{141,211,199}
\definecolor{Set3-10-A}{RGB}{141,211,199}
\definecolor{Set3-10-2}{RGB}{255,255,179}
\definecolor{Set3-10-B}{RGB}{255,255,179}
\definecolor{Set3-10-3}{RGB}{190,186,218}
\definecolor{Set3-10-C}{RGB}{190,186,218}
\definecolor{Set3-10-4}{RGB}{251,128,114}
\definecolor{Set3-10-D}{RGB}{251,128,114}
\definecolor{Set3-10-5}{RGB}{128,177,211}
\definecolor{Set3-10-E}{RGB}{128,177,211}
\definecolor{Set3-10-6}{RGB}{253,180,98}
\definecolor{Set3-10-F}{RGB}{253,180,98}
\definecolor{Set3-10-7}{RGB}{179,222,105}
\definecolor{Set3-10-G}{RGB}{179,222,105}
\definecolor{Set3-10-8}{RGB}{252,205,229}
\definecolor{Set3-10-H}{RGB}{252,205,229}
\definecolor{Set3-10-9}{RGB}{217,217,217}
\definecolor{Set3-10-I}{RGB}{217,217,217}
\definecolor{Set3-10-10}{RGB}{188,128,189}
\definecolor{Set3-10-J}{RGB}{188,128,189}
\definecolor{Set3-11-1}{RGB}{141,211,199}
\definecolor{Set3-11-A}{RGB}{141,211,199}
\definecolor{Set3-11-2}{RGB}{255,255,179}
\definecolor{Set3-11-B}{RGB}{255,255,179}
\definecolor{Set3-11-3}{RGB}{190,186,218}
\definecolor{Set3-11-C}{RGB}{190,186,218}
\definecolor{Set3-11-4}{RGB}{251,128,114}
\definecolor{Set3-11-D}{RGB}{251,128,114}
\definecolor{Set3-11-5}{RGB}{128,177,211}
\definecolor{Set3-11-E}{RGB}{128,177,211}
\definecolor{Set3-11-6}{RGB}{253,180,98}
\definecolor{Set3-11-F}{RGB}{253,180,98}
\definecolor{Set3-11-7}{RGB}{179,222,105}
\definecolor{Set3-11-G}{RGB}{179,222,105}
\definecolor{Set3-11-8}{RGB}{252,205,229}
\definecolor{Set3-11-H}{RGB}{252,205,229}
\definecolor{Set3-11-9}{RGB}{217,217,217}
\definecolor{Set3-11-I}{RGB}{217,217,217}
\definecolor{Set3-11-10}{RGB}{188,128,189}
\definecolor{Set3-11-J}{RGB}{188,128,189}
\definecolor{Set3-11-11}{RGB}{204,235,197}
\definecolor{Set3-11-K}{RGB}{204,235,197}
\definecolor{Set3-12-1}{RGB}{141,211,199}
\definecolor{Set3-12-A}{RGB}{141,211,199}
\definecolor{Set3-12-2}{RGB}{255,255,179}
\definecolor{Set3-12-B}{RGB}{255,255,179}
\definecolor{Set3-12-3}{RGB}{190,186,218}
\definecolor{Set3-12-C}{RGB}{190,186,218}
\definecolor{Set3-12-4}{RGB}{251,128,114}
\definecolor{Set3-12-D}{RGB}{251,128,114}
\definecolor{Set3-12-5}{RGB}{128,177,211}
\definecolor{Set3-12-E}{RGB}{128,177,211}
\definecolor{Set3-12-6}{RGB}{253,180,98}
\definecolor{Set3-12-F}{RGB}{253,180,98}
\definecolor{Set3-12-7}{RGB}{179,222,105}
\definecolor{Set3-12-G}{RGB}{179,222,105}
\definecolor{Set3-12-8}{RGB}{252,205,229}
\definecolor{Set3-12-H}{RGB}{252,205,229}
\definecolor{Set3-12-9}{RGB}{217,217,217}
\definecolor{Set3-12-I}{RGB}{217,217,217}
\definecolor{Set3-12-10}{RGB}{188,128,189}
\definecolor{Set3-12-J}{RGB}{188,128,189}
\definecolor{Set3-12-11}{RGB}{204,235,197}
\definecolor{Set3-12-K}{RGB}{204,235,197}
\definecolor{Set3-12-12}{RGB}{255,237,111}
\definecolor{Set3-12-L}{RGB}{255,237,111}
\definecolor{Pastel1-3-1}{RGB}{251,180,174}
\definecolor{Pastel1-3-A}{RGB}{251,180,174}
\definecolor{Pastel1-3-2}{RGB}{179,205,227}
\definecolor{Pastel1-3-B}{RGB}{179,205,227}
\definecolor{Pastel1-3-3}{RGB}{204,235,197}
\definecolor{Pastel1-3-C}{RGB}{204,235,197}
\definecolor{Pastel1-4-1}{RGB}{251,180,174}
\definecolor{Pastel1-4-A}{RGB}{251,180,174}
\definecolor{Pastel1-4-2}{RGB}{179,205,227}
\definecolor{Pastel1-4-B}{RGB}{179,205,227}
\definecolor{Pastel1-4-3}{RGB}{204,235,197}
\definecolor{Pastel1-4-C}{RGB}{204,235,197}
\definecolor{Pastel1-4-4}{RGB}{222,203,228}
\definecolor{Pastel1-4-D}{RGB}{222,203,228}
\definecolor{Pastel1-5-1}{RGB}{251,180,174}
\definecolor{Pastel1-5-A}{RGB}{251,180,174}
\definecolor{Pastel1-5-2}{RGB}{179,205,227}
\definecolor{Pastel1-5-B}{RGB}{179,205,227}
\definecolor{Pastel1-5-3}{RGB}{204,235,197}
\definecolor{Pastel1-5-C}{RGB}{204,235,197}
\definecolor{Pastel1-5-4}{RGB}{222,203,228}
\definecolor{Pastel1-5-D}{RGB}{222,203,228}
\definecolor{Pastel1-5-5}{RGB}{254,217,166}
\definecolor{Pastel1-5-E}{RGB}{254,217,166}
\definecolor{Pastel1-6-1}{RGB}{251,180,174}
\definecolor{Pastel1-6-A}{RGB}{251,180,174}
\definecolor{Pastel1-6-2}{RGB}{179,205,227}
\definecolor{Pastel1-6-B}{RGB}{179,205,227}
\definecolor{Pastel1-6-3}{RGB}{204,235,197}
\definecolor{Pastel1-6-C}{RGB}{204,235,197}
\definecolor{Pastel1-6-4}{RGB}{222,203,228}
\definecolor{Pastel1-6-D}{RGB}{222,203,228}
\definecolor{Pastel1-6-5}{RGB}{254,217,166}
\definecolor{Pastel1-6-E}{RGB}{254,217,166}
\definecolor{Pastel1-6-6}{RGB}{255,255,204}
\definecolor{Pastel1-6-F}{RGB}{255,255,204}
\definecolor{Pastel1-7-1}{RGB}{251,180,174}
\definecolor{Pastel1-7-A}{RGB}{251,180,174}
\definecolor{Pastel1-7-2}{RGB}{179,205,227}
\definecolor{Pastel1-7-B}{RGB}{179,205,227}
\definecolor{Pastel1-7-3}{RGB}{204,235,197}
\definecolor{Pastel1-7-C}{RGB}{204,235,197}
\definecolor{Pastel1-7-4}{RGB}{222,203,228}
\definecolor{Pastel1-7-D}{RGB}{222,203,228}
\definecolor{Pastel1-7-5}{RGB}{254,217,166}
\definecolor{Pastel1-7-E}{RGB}{254,217,166}
\definecolor{Pastel1-7-6}{RGB}{255,255,204}
\definecolor{Pastel1-7-F}{RGB}{255,255,204}
\definecolor{Pastel1-7-7}{RGB}{229,216,189}
\definecolor{Pastel1-7-G}{RGB}{229,216,189}
\definecolor{Pastel1-8-1}{RGB}{251,180,174}
\definecolor{Pastel1-8-A}{RGB}{251,180,174}
\definecolor{Pastel1-8-2}{RGB}{179,205,227}
\definecolor{Pastel1-8-B}{RGB}{179,205,227}
\definecolor{Pastel1-8-3}{RGB}{204,235,197}
\definecolor{Pastel1-8-C}{RGB}{204,235,197}
\definecolor{Pastel1-8-4}{RGB}{222,203,228}
\definecolor{Pastel1-8-D}{RGB}{222,203,228}
\definecolor{Pastel1-8-5}{RGB}{254,217,166}
\definecolor{Pastel1-8-E}{RGB}{254,217,166}
\definecolor{Pastel1-8-6}{RGB}{255,255,204}
\definecolor{Pastel1-8-F}{RGB}{255,255,204}
\definecolor{Pastel1-8-7}{RGB}{229,216,189}
\definecolor{Pastel1-8-G}{RGB}{229,216,189}
\definecolor{Pastel1-8-8}{RGB}{253,218,236}
\definecolor{Pastel1-8-H}{RGB}{253,218,236}
\definecolor{Pastel1-9-1}{RGB}{251,180,174}
\definecolor{Pastel1-9-A}{RGB}{251,180,174}
\definecolor{Pastel1-9-2}{RGB}{179,205,227}
\definecolor{Pastel1-9-B}{RGB}{179,205,227}
\definecolor{Pastel1-9-3}{RGB}{204,235,197}
\definecolor{Pastel1-9-C}{RGB}{204,235,197}
\definecolor{Pastel1-9-4}{RGB}{222,203,228}
\definecolor{Pastel1-9-D}{RGB}{222,203,228}
\definecolor{Pastel1-9-5}{RGB}{254,217,166}
\definecolor{Pastel1-9-E}{RGB}{254,217,166}
\definecolor{Pastel1-9-6}{RGB}{255,255,204}
\definecolor{Pastel1-9-F}{RGB}{255,255,204}
\definecolor{Pastel1-9-7}{RGB}{229,216,189}
\definecolor{Pastel1-9-G}{RGB}{229,216,189}
\definecolor{Pastel1-9-8}{RGB}{253,218,236}
\definecolor{Pastel1-9-H}{RGB}{253,218,236}
\definecolor{Pastel1-9-9}{RGB}{242,242,242}
\definecolor{Pastel1-9-I}{RGB}{242,242,242}
\definecolor{Set1-3-1}{RGB}{228,26,28}
\definecolor{Set1-3-A}{RGB}{228,26,28}
\definecolor{Set1-3-2}{RGB}{55,126,184}
\definecolor{Set1-3-B}{RGB}{55,126,184}
\definecolor{Set1-3-3}{RGB}{77,175,74}
\definecolor{Set1-3-C}{RGB}{77,175,74}
\definecolor{Set1-4-1}{RGB}{228,26,28}
\definecolor{Set1-4-A}{RGB}{228,26,28}
\definecolor{Set1-4-2}{RGB}{55,126,184}
\definecolor{Set1-4-B}{RGB}{55,126,184}
\definecolor{Set1-4-3}{RGB}{77,175,74}
\definecolor{Set1-4-C}{RGB}{77,175,74}
\definecolor{Set1-4-4}{RGB}{152,78,163}
\definecolor{Set1-4-D}{RGB}{152,78,163}
\definecolor{Set1-5-1}{RGB}{228,26,28}
\definecolor{Set1-5-A}{RGB}{228,26,28}
\definecolor{Set1-5-2}{RGB}{55,126,184}
\definecolor{Set1-5-B}{RGB}{55,126,184}
\definecolor{Set1-5-3}{RGB}{77,175,74}
\definecolor{Set1-5-C}{RGB}{77,175,74}
\definecolor{Set1-5-4}{RGB}{152,78,163}
\definecolor{Set1-5-D}{RGB}{152,78,163}
\definecolor{Set1-5-5}{RGB}{255,127,0}
\definecolor{Set1-5-E}{RGB}{255,127,0}
\definecolor{Set1-6-1}{RGB}{228,26,28}
\definecolor{Set1-6-A}{RGB}{228,26,28}
\definecolor{Set1-6-2}{RGB}{55,126,184}
\definecolor{Set1-6-B}{RGB}{55,126,184}
\definecolor{Set1-6-3}{RGB}{77,175,74}
\definecolor{Set1-6-C}{RGB}{77,175,74}
\definecolor{Set1-6-4}{RGB}{152,78,163}
\definecolor{Set1-6-D}{RGB}{152,78,163}
\definecolor{Set1-6-5}{RGB}{255,127,0}
\definecolor{Set1-6-E}{RGB}{255,127,0}
\definecolor{Set1-6-6}{RGB}{255,255,51}
\definecolor{Set1-6-F}{RGB}{255,255,51}
\definecolor{Set1-7-1}{RGB}{228,26,28}
\definecolor{Set1-7-A}{RGB}{228,26,28}
\definecolor{Set1-7-2}{RGB}{55,126,184}
\definecolor{Set1-7-B}{RGB}{55,126,184}
\definecolor{Set1-7-3}{RGB}{77,175,74}
\definecolor{Set1-7-C}{RGB}{77,175,74}
\definecolor{Set1-7-4}{RGB}{152,78,163}
\definecolor{Set1-7-D}{RGB}{152,78,163}
\definecolor{Set1-7-5}{RGB}{255,127,0}
\definecolor{Set1-7-E}{RGB}{255,127,0}
\definecolor{Set1-7-6}{RGB}{255,255,51}
\definecolor{Set1-7-F}{RGB}{255,255,51}
\definecolor{Set1-7-7}{RGB}{166,86,40}
\definecolor{Set1-7-G}{RGB}{166,86,40}
\definecolor{Set1-8-1}{RGB}{228,26,28}
\definecolor{Set1-8-A}{RGB}{228,26,28}
\definecolor{Set1-8-2}{RGB}{55,126,184}
\definecolor{Set1-8-B}{RGB}{55,126,184}
\definecolor{Set1-8-3}{RGB}{77,175,74}
\definecolor{Set1-8-C}{RGB}{77,175,74}
\definecolor{Set1-8-4}{RGB}{152,78,163}
\definecolor{Set1-8-D}{RGB}{152,78,163}
\definecolor{Set1-8-5}{RGB}{255,127,0}
\definecolor{Set1-8-E}{RGB}{255,127,0}
\definecolor{Set1-8-6}{RGB}{255,255,51}
\definecolor{Set1-8-F}{RGB}{255,255,51}
\definecolor{Set1-8-7}{RGB}{166,86,40}
\definecolor{Set1-8-G}{RGB}{166,86,40}
\definecolor{Set1-8-8}{RGB}{247,129,191}
\definecolor{Set1-8-H}{RGB}{247,129,191}
\definecolor{Set1-9-1}{RGB}{228,26,28}
\definecolor{Set1-9-A}{RGB}{228,26,28}
\definecolor{Set1-9-2}{RGB}{55,126,184}
\definecolor{Set1-9-B}{RGB}{55,126,184}
\definecolor{Set1-9-3}{RGB}{77,175,74}
\definecolor{Set1-9-C}{RGB}{77,175,74}
\definecolor{Set1-9-4}{RGB}{152,78,163}
\definecolor{Set1-9-D}{RGB}{152,78,163}
\definecolor{Set1-9-5}{RGB}{255,127,0}
\definecolor{Set1-9-E}{RGB}{255,127,0}
\definecolor{Set1-9-6}{RGB}{255,255,51}
\definecolor{Set1-9-F}{RGB}{255,255,51}
\definecolor{Set1-9-7}{RGB}{166,86,40}
\definecolor{Set1-9-G}{RGB}{166,86,40}
\definecolor{Set1-9-8}{RGB}{247,129,191}
\definecolor{Set1-9-H}{RGB}{247,129,191}
\definecolor{Set1-9-9}{RGB}{153,153,153}
\definecolor{Set1-9-I}{RGB}{153,153,153}
\definecolor{Pastel2-3-1}{RGB}{179,226,205}
\definecolor{Pastel2-3-A}{RGB}{179,226,205}
\definecolor{Pastel2-3-2}{RGB}{253,205,172}
\definecolor{Pastel2-3-B}{RGB}{253,205,172}
\definecolor{Pastel2-3-3}{RGB}{203,213,232}
\definecolor{Pastel2-3-C}{RGB}{203,213,232}
\definecolor{Pastel2-4-1}{RGB}{179,226,205}
\definecolor{Pastel2-4-A}{RGB}{179,226,205}
\definecolor{Pastel2-4-2}{RGB}{253,205,172}
\definecolor{Pastel2-4-B}{RGB}{253,205,172}
\definecolor{Pastel2-4-3}{RGB}{203,213,232}
\definecolor{Pastel2-4-C}{RGB}{203,213,232}
\definecolor{Pastel2-4-4}{RGB}{244,202,228}
\definecolor{Pastel2-4-D}{RGB}{244,202,228}
\definecolor{Pastel2-5-1}{RGB}{179,226,205}
\definecolor{Pastel2-5-A}{RGB}{179,226,205}
\definecolor{Pastel2-5-2}{RGB}{253,205,172}
\definecolor{Pastel2-5-B}{RGB}{253,205,172}
\definecolor{Pastel2-5-3}{RGB}{203,213,232}
\definecolor{Pastel2-5-C}{RGB}{203,213,232}
\definecolor{Pastel2-5-4}{RGB}{244,202,228}
\definecolor{Pastel2-5-D}{RGB}{244,202,228}
\definecolor{Pastel2-5-5}{RGB}{230,245,201}
\definecolor{Pastel2-5-E}{RGB}{230,245,201}
\definecolor{Pastel2-6-1}{RGB}{179,226,205}
\definecolor{Pastel2-6-A}{RGB}{179,226,205}
\definecolor{Pastel2-6-2}{RGB}{253,205,172}
\definecolor{Pastel2-6-B}{RGB}{253,205,172}
\definecolor{Pastel2-6-3}{RGB}{203,213,232}
\definecolor{Pastel2-6-C}{RGB}{203,213,232}
\definecolor{Pastel2-6-4}{RGB}{244,202,228}
\definecolor{Pastel2-6-D}{RGB}{244,202,228}
\definecolor{Pastel2-6-5}{RGB}{230,245,201}
\definecolor{Pastel2-6-E}{RGB}{230,245,201}
\definecolor{Pastel2-6-6}{RGB}{255,242,174}
\definecolor{Pastel2-6-F}{RGB}{255,242,174}
\definecolor{Pastel2-7-1}{RGB}{179,226,205}
\definecolor{Pastel2-7-A}{RGB}{179,226,205}
\definecolor{Pastel2-7-2}{RGB}{253,205,172}
\definecolor{Pastel2-7-B}{RGB}{253,205,172}
\definecolor{Pastel2-7-3}{RGB}{203,213,232}
\definecolor{Pastel2-7-C}{RGB}{203,213,232}
\definecolor{Pastel2-7-4}{RGB}{244,202,228}
\definecolor{Pastel2-7-D}{RGB}{244,202,228}
\definecolor{Pastel2-7-5}{RGB}{230,245,201}
\definecolor{Pastel2-7-E}{RGB}{230,245,201}
\definecolor{Pastel2-7-6}{RGB}{255,242,174}
\definecolor{Pastel2-7-F}{RGB}{255,242,174}
\definecolor{Pastel2-7-7}{RGB}{241,226,204}
\definecolor{Pastel2-7-G}{RGB}{241,226,204}
\definecolor{Pastel2-8-1}{RGB}{179,226,205}
\definecolor{Pastel2-8-A}{RGB}{179,226,205}
\definecolor{Pastel2-8-2}{RGB}{253,205,172}
\definecolor{Pastel2-8-B}{RGB}{253,205,172}
\definecolor{Pastel2-8-3}{RGB}{203,213,232}
\definecolor{Pastel2-8-C}{RGB}{203,213,232}
\definecolor{Pastel2-8-4}{RGB}{244,202,228}
\definecolor{Pastel2-8-D}{RGB}{244,202,228}
\definecolor{Pastel2-8-5}{RGB}{230,245,201}
\definecolor{Pastel2-8-E}{RGB}{230,245,201}
\definecolor{Pastel2-8-6}{RGB}{255,242,174}
\definecolor{Pastel2-8-F}{RGB}{255,242,174}
\definecolor{Pastel2-8-7}{RGB}{241,226,204}
\definecolor{Pastel2-8-G}{RGB}{241,226,204}
\definecolor{Pastel2-8-8}{RGB}{204,204,204}
\definecolor{Pastel2-8-H}{RGB}{204,204,204}
\definecolor{Set2-3-1}{RGB}{102,194,165}
\definecolor{Set2-3-A}{RGB}{102,194,165}
\definecolor{Set2-3-2}{RGB}{252,141,98}
\definecolor{Set2-3-B}{RGB}{252,141,98}
\definecolor{Set2-3-3}{RGB}{141,160,203}
\definecolor{Set2-3-C}{RGB}{141,160,203}
\definecolor{Set2-4-1}{RGB}{102,194,165}
\definecolor{Set2-4-A}{RGB}{102,194,165}
\definecolor{Set2-4-2}{RGB}{252,141,98}
\definecolor{Set2-4-B}{RGB}{252,141,98}
\definecolor{Set2-4-3}{RGB}{141,160,203}
\definecolor{Set2-4-C}{RGB}{141,160,203}
\definecolor{Set2-4-4}{RGB}{231,138,195}
\definecolor{Set2-4-D}{RGB}{231,138,195}
\definecolor{Set2-5-1}{RGB}{102,194,165}
\definecolor{Set2-5-A}{RGB}{102,194,165}
\definecolor{Set2-5-2}{RGB}{252,141,98}
\definecolor{Set2-5-B}{RGB}{252,141,98}
\definecolor{Set2-5-3}{RGB}{141,160,203}
\definecolor{Set2-5-C}{RGB}{141,160,203}
\definecolor{Set2-5-4}{RGB}{231,138,195}
\definecolor{Set2-5-D}{RGB}{231,138,195}
\definecolor{Set2-5-5}{RGB}{166,216,84}
\definecolor{Set2-5-E}{RGB}{166,216,84}
\definecolor{Set2-6-1}{RGB}{102,194,165}
\definecolor{Set2-6-A}{RGB}{102,194,165}
\definecolor{Set2-6-2}{RGB}{252,141,98}
\definecolor{Set2-6-B}{RGB}{252,141,98}
\definecolor{Set2-6-3}{RGB}{141,160,203}
\definecolor{Set2-6-C}{RGB}{141,160,203}
\definecolor{Set2-6-4}{RGB}{231,138,195}
\definecolor{Set2-6-D}{RGB}{231,138,195}
\definecolor{Set2-6-5}{RGB}{166,216,84}
\definecolor{Set2-6-E}{RGB}{166,216,84}
\definecolor{Set2-6-6}{RGB}{255,217,47}
\definecolor{Set2-6-F}{RGB}{255,217,47}
\definecolor{Set2-7-1}{RGB}{102,194,165}
\definecolor{Set2-7-A}{RGB}{102,194,165}
\definecolor{Set2-7-2}{RGB}{252,141,98}
\definecolor{Set2-7-B}{RGB}{252,141,98}
\definecolor{Set2-7-3}{RGB}{141,160,203}
\definecolor{Set2-7-C}{RGB}{141,160,203}
\definecolor{Set2-7-4}{RGB}{231,138,195}
\definecolor{Set2-7-D}{RGB}{231,138,195}
\definecolor{Set2-7-5}{RGB}{166,216,84}
\definecolor{Set2-7-E}{RGB}{166,216,84}
\definecolor{Set2-7-6}{RGB}{255,217,47}
\definecolor{Set2-7-F}{RGB}{255,217,47}
\definecolor{Set2-7-7}{RGB}{229,196,148}
\definecolor{Set2-7-G}{RGB}{229,196,148}
\definecolor{Set2-8-1}{RGB}{102,194,165}
\definecolor{Set2-8-A}{RGB}{102,194,165}
\definecolor{Set2-8-2}{RGB}{252,141,98}
\definecolor{Set2-8-B}{RGB}{252,141,98}
\definecolor{Set2-8-3}{RGB}{141,160,203}
\definecolor{Set2-8-C}{RGB}{141,160,203}
\definecolor{Set2-8-4}{RGB}{231,138,195}
\definecolor{Set2-8-D}{RGB}{231,138,195}
\definecolor{Set2-8-5}{RGB}{166,216,84}
\definecolor{Set2-8-E}{RGB}{166,216,84}
\definecolor{Set2-8-6}{RGB}{255,217,47}
\definecolor{Set2-8-F}{RGB}{255,217,47}
\definecolor{Set2-8-7}{RGB}{229,196,148}
\definecolor{Set2-8-G}{RGB}{229,196,148}
\definecolor{Set2-8-8}{RGB}{179,179,179}
\definecolor{Set2-8-H}{RGB}{179,179,179}
\definecolor{Dark2-3-1}{RGB}{27,158,119}
\definecolor{Dark2-3-A}{RGB}{27,158,119}
\definecolor{Dark2-3-2}{RGB}{217,95,2}
\definecolor{Dark2-3-B}{RGB}{217,95,2}
\definecolor{Dark2-3-3}{RGB}{117,112,179}
\definecolor{Dark2-3-C}{RGB}{117,112,179}
\definecolor{Dark2-4-1}{RGB}{27,158,119}
\definecolor{Dark2-4-A}{RGB}{27,158,119}
\definecolor{Dark2-4-2}{RGB}{217,95,2}
\definecolor{Dark2-4-B}{RGB}{217,95,2}
\definecolor{Dark2-4-3}{RGB}{117,112,179}
\definecolor{Dark2-4-C}{RGB}{117,112,179}
\definecolor{Dark2-4-4}{RGB}{231,41,138}
\definecolor{Dark2-4-D}{RGB}{231,41,138}
\definecolor{Dark2-5-1}{RGB}{27,158,119}
\definecolor{Dark2-5-A}{RGB}{27,158,119}
\definecolor{Dark2-5-2}{RGB}{217,95,2}
\definecolor{Dark2-5-B}{RGB}{217,95,2}
\definecolor{Dark2-5-3}{RGB}{117,112,179}
\definecolor{Dark2-5-C}{RGB}{117,112,179}
\definecolor{Dark2-5-4}{RGB}{231,41,138}
\definecolor{Dark2-5-D}{RGB}{231,41,138}
\definecolor{Dark2-5-5}{RGB}{102,166,30}
\definecolor{Dark2-5-E}{RGB}{102,166,30}
\definecolor{Dark2-6-1}{RGB}{27,158,119}
\definecolor{Dark2-6-A}{RGB}{27,158,119}
\definecolor{Dark2-6-2}{RGB}{217,95,2}
\definecolor{Dark2-6-B}{RGB}{217,95,2}
\definecolor{Dark2-6-3}{RGB}{117,112,179}
\definecolor{Dark2-6-C}{RGB}{117,112,179}
\definecolor{Dark2-6-4}{RGB}{231,41,138}
\definecolor{Dark2-6-D}{RGB}{231,41,138}
\definecolor{Dark2-6-5}{RGB}{102,166,30}
\definecolor{Dark2-6-E}{RGB}{102,166,30}
\definecolor{Dark2-6-6}{RGB}{230,171,2}
\definecolor{Dark2-6-F}{RGB}{230,171,2}
\definecolor{Dark2-7-1}{RGB}{27,158,119}
\definecolor{Dark2-7-A}{RGB}{27,158,119}
\definecolor{Dark2-7-2}{RGB}{217,95,2}
\definecolor{Dark2-7-B}{RGB}{217,95,2}
\definecolor{Dark2-7-3}{RGB}{117,112,179}
\definecolor{Dark2-7-C}{RGB}{117,112,179}
\definecolor{Dark2-7-4}{RGB}{231,41,138}
\definecolor{Dark2-7-D}{RGB}{231,41,138}
\definecolor{Dark2-7-5}{RGB}{102,166,30}
\definecolor{Dark2-7-E}{RGB}{102,166,30}
\definecolor{Dark2-7-6}{RGB}{230,171,2}
\definecolor{Dark2-7-F}{RGB}{230,171,2}
\definecolor{Dark2-7-7}{RGB}{166,118,29}
\definecolor{Dark2-7-G}{RGB}{166,118,29}
\definecolor{Dark2-8-1}{RGB}{27,158,119}
\definecolor{Dark2-8-A}{RGB}{27,158,119}
\definecolor{Dark2-8-2}{RGB}{217,95,2}
\definecolor{Dark2-8-B}{RGB}{217,95,2}
\definecolor{Dark2-8-3}{RGB}{117,112,179}
\definecolor{Dark2-8-C}{RGB}{117,112,179}
\definecolor{Dark2-8-4}{RGB}{231,41,138}
\definecolor{Dark2-8-D}{RGB}{231,41,138}
\definecolor{Dark2-8-5}{RGB}{102,166,30}
\definecolor{Dark2-8-E}{RGB}{102,166,30}
\definecolor{Dark2-8-6}{RGB}{230,171,2}
\definecolor{Dark2-8-F}{RGB}{230,171,2}
\definecolor{Dark2-8-7}{RGB}{166,118,29}
\definecolor{Dark2-8-G}{RGB}{166,118,29}
\definecolor{Dark2-8-8}{RGB}{102,102,102}
\definecolor{Dark2-8-H}{RGB}{102,102,102}
\definecolor{Paired-3-1}{RGB}{166,206,227}
\definecolor{Paired-3-A}{RGB}{166,206,227}
\definecolor{Paired-3-2}{RGB}{31,120,180}
\definecolor{Paired-3-B}{RGB}{31,120,180}
\definecolor{Paired-3-3}{RGB}{178,223,138}
\definecolor{Paired-3-C}{RGB}{178,223,138}
\definecolor{Paired-4-1}{RGB}{166,206,227}
\definecolor{Paired-4-A}{RGB}{166,206,227}
\definecolor{Paired-4-2}{RGB}{31,120,180}
\definecolor{Paired-4-B}{RGB}{31,120,180}
\definecolor{Paired-4-3}{RGB}{178,223,138}
\definecolor{Paired-4-C}{RGB}{178,223,138}
\definecolor{Paired-4-4}{RGB}{51,160,44}
\definecolor{Paired-4-D}{RGB}{51,160,44}
\definecolor{Paired-5-1}{RGB}{166,206,227}
\definecolor{Paired-5-A}{RGB}{166,206,227}
\definecolor{Paired-5-2}{RGB}{31,120,180}
\definecolor{Paired-5-B}{RGB}{31,120,180}
\definecolor{Paired-5-3}{RGB}{178,223,138}
\definecolor{Paired-5-C}{RGB}{178,223,138}
\definecolor{Paired-5-4}{RGB}{51,160,44}
\definecolor{Paired-5-D}{RGB}{51,160,44}
\definecolor{Paired-5-5}{RGB}{251,154,153}
\definecolor{Paired-5-E}{RGB}{251,154,153}
\definecolor{Paired-6-1}{RGB}{166,206,227}
\definecolor{Paired-6-A}{RGB}{166,206,227}
\definecolor{Paired-6-2}{RGB}{31,120,180}
\definecolor{Paired-6-B}{RGB}{31,120,180}
\definecolor{Paired-6-3}{RGB}{178,223,138}
\definecolor{Paired-6-C}{RGB}{178,223,138}
\definecolor{Paired-6-4}{RGB}{51,160,44}
\definecolor{Paired-6-D}{RGB}{51,160,44}
\definecolor{Paired-6-5}{RGB}{251,154,153}
\definecolor{Paired-6-E}{RGB}{251,154,153}
\definecolor{Paired-6-6}{RGB}{227,26,28}
\definecolor{Paired-6-F}{RGB}{227,26,28}
\definecolor{Paired-7-1}{RGB}{166,206,227}
\definecolor{Paired-7-A}{RGB}{166,206,227}
\definecolor{Paired-7-2}{RGB}{31,120,180}
\definecolor{Paired-7-B}{RGB}{31,120,180}
\definecolor{Paired-7-3}{RGB}{178,223,138}
\definecolor{Paired-7-C}{RGB}{178,223,138}
\definecolor{Paired-7-4}{RGB}{51,160,44}
\definecolor{Paired-7-D}{RGB}{51,160,44}
\definecolor{Paired-7-5}{RGB}{251,154,153}
\definecolor{Paired-7-E}{RGB}{251,154,153}
\definecolor{Paired-7-6}{RGB}{227,26,28}
\definecolor{Paired-7-F}{RGB}{227,26,28}
\definecolor{Paired-7-7}{RGB}{253,191,111}
\definecolor{Paired-7-G}{RGB}{253,191,111}
\definecolor{Paired-8-1}{RGB}{166,206,227}
\definecolor{Paired-8-A}{RGB}{166,206,227}
\definecolor{Paired-8-2}{RGB}{31,120,180}
\definecolor{Paired-8-B}{RGB}{31,120,180}
\definecolor{Paired-8-3}{RGB}{178,223,138}
\definecolor{Paired-8-C}{RGB}{178,223,138}
\definecolor{Paired-8-4}{RGB}{51,160,44}
\definecolor{Paired-8-D}{RGB}{51,160,44}
\definecolor{Paired-8-5}{RGB}{251,154,153}
\definecolor{Paired-8-E}{RGB}{251,154,153}
\definecolor{Paired-8-6}{RGB}{227,26,28}
\definecolor{Paired-8-F}{RGB}{227,26,28}
\definecolor{Paired-8-7}{RGB}{253,191,111}
\definecolor{Paired-8-G}{RGB}{253,191,111}
\definecolor{Paired-8-8}{RGB}{255,127,0}
\definecolor{Paired-8-H}{RGB}{255,127,0}
\definecolor{Paired-9-1}{RGB}{166,206,227}
\definecolor{Paired-9-A}{RGB}{166,206,227}
\definecolor{Paired-9-2}{RGB}{31,120,180}
\definecolor{Paired-9-B}{RGB}{31,120,180}
\definecolor{Paired-9-3}{RGB}{178,223,138}
\definecolor{Paired-9-C}{RGB}{178,223,138}
\definecolor{Paired-9-4}{RGB}{51,160,44}
\definecolor{Paired-9-D}{RGB}{51,160,44}
\definecolor{Paired-9-5}{RGB}{251,154,153}
\definecolor{Paired-9-E}{RGB}{251,154,153}
\definecolor{Paired-9-6}{RGB}{227,26,28}
\definecolor{Paired-9-F}{RGB}{227,26,28}
\definecolor{Paired-9-7}{RGB}{253,191,111}
\definecolor{Paired-9-G}{RGB}{253,191,111}
\definecolor{Paired-9-8}{RGB}{255,127,0}
\definecolor{Paired-9-H}{RGB}{255,127,0}
\definecolor{Paired-9-9}{RGB}{202,178,214}
\definecolor{Paired-9-I}{RGB}{202,178,214}
\definecolor{Paired-10-1}{RGB}{166,206,227}
\definecolor{Paired-10-A}{RGB}{166,206,227}
\definecolor{Paired-10-2}{RGB}{31,120,180}
\definecolor{Paired-10-B}{RGB}{31,120,180}
\definecolor{Paired-10-3}{RGB}{178,223,138}
\definecolor{Paired-10-C}{RGB}{178,223,138}
\definecolor{Paired-10-4}{RGB}{51,160,44}
\definecolor{Paired-10-D}{RGB}{51,160,44}
\definecolor{Paired-10-5}{RGB}{251,154,153}
\definecolor{Paired-10-E}{RGB}{251,154,153}
\definecolor{Paired-10-6}{RGB}{227,26,28}
\definecolor{Paired-10-F}{RGB}{227,26,28}
\definecolor{Paired-10-7}{RGB}{253,191,111}
\definecolor{Paired-10-G}{RGB}{253,191,111}
\definecolor{Paired-10-8}{RGB}{255,127,0}
\definecolor{Paired-10-H}{RGB}{255,127,0}
\definecolor{Paired-10-9}{RGB}{202,178,214}
\definecolor{Paired-10-I}{RGB}{202,178,214}
\definecolor{Paired-10-10}{RGB}{106,61,154}
\definecolor{Paired-10-J}{RGB}{106,61,154}
\definecolor{Paired-11-1}{RGB}{166,206,227}
\definecolor{Paired-11-A}{RGB}{166,206,227}
\definecolor{Paired-11-2}{RGB}{31,120,180}
\definecolor{Paired-11-B}{RGB}{31,120,180}
\definecolor{Paired-11-3}{RGB}{178,223,138}
\definecolor{Paired-11-C}{RGB}{178,223,138}
\definecolor{Paired-11-4}{RGB}{51,160,44}
\definecolor{Paired-11-D}{RGB}{51,160,44}
\definecolor{Paired-11-5}{RGB}{251,154,153}
\definecolor{Paired-11-E}{RGB}{251,154,153}
\definecolor{Paired-11-6}{RGB}{227,26,28}
\definecolor{Paired-11-F}{RGB}{227,26,28}
\definecolor{Paired-11-7}{RGB}{253,191,111}
\definecolor{Paired-11-G}{RGB}{253,191,111}
\definecolor{Paired-11-8}{RGB}{255,127,0}
\definecolor{Paired-11-H}{RGB}{255,127,0}
\definecolor{Paired-11-9}{RGB}{202,178,214}
\definecolor{Paired-11-I}{RGB}{202,178,214}
\definecolor{Paired-11-10}{RGB}{106,61,154}
\definecolor{Paired-11-J}{RGB}{106,61,154}
\definecolor{Paired-11-11}{RGB}{255,255,153}
\definecolor{Paired-11-K}{RGB}{255,255,153}
\definecolor{Paired-12-1}{RGB}{166,206,227}
\definecolor{Paired-12-A}{RGB}{166,206,227}
\definecolor{Paired-12-2}{RGB}{31,120,180}
\definecolor{Paired-12-B}{RGB}{31,120,180}
\definecolor{Paired-12-3}{RGB}{178,223,138}
\definecolor{Paired-12-C}{RGB}{178,223,138}
\definecolor{Paired-12-4}{RGB}{51,160,44}
\definecolor{Paired-12-D}{RGB}{51,160,44}
\definecolor{Paired-12-5}{RGB}{251,154,153}
\definecolor{Paired-12-E}{RGB}{251,154,153}
\definecolor{Paired-12-6}{RGB}{227,26,28}
\definecolor{Paired-12-F}{RGB}{227,26,28}
\definecolor{Paired-12-7}{RGB}{253,191,111}
\definecolor{Paired-12-G}{RGB}{253,191,111}
\definecolor{Paired-12-8}{RGB}{255,127,0}
\definecolor{Paired-12-H}{RGB}{255,127,0}
\definecolor{Paired-12-9}{RGB}{202,178,214}
\definecolor{Paired-12-I}{RGB}{202,178,214}
\definecolor{Paired-12-10}{RGB}{106,61,154}
\definecolor{Paired-12-J}{RGB}{106,61,154}
\definecolor{Paired-12-11}{RGB}{255,255,153}
\definecolor{Paired-12-K}{RGB}{255,255,153}
\definecolor{Paired-12-12}{RGB}{177,89,40}
\definecolor{Paired-12-L}{RGB}{177,89,40}
\definecolor{Accent-3-1}{RGB}{127,201,127}
\definecolor{Accent-3-A}{RGB}{127,201,127}
\definecolor{Accent-3-2}{RGB}{190,174,212}
\definecolor{Accent-3-B}{RGB}{190,174,212}
\definecolor{Accent-3-3}{RGB}{253,192,134}
\definecolor{Accent-3-C}{RGB}{253,192,134}
\definecolor{Accent-4-1}{RGB}{127,201,127}
\definecolor{Accent-4-A}{RGB}{127,201,127}
\definecolor{Accent-4-2}{RGB}{190,174,212}
\definecolor{Accent-4-B}{RGB}{190,174,212}
\definecolor{Accent-4-3}{RGB}{253,192,134}
\definecolor{Accent-4-C}{RGB}{253,192,134}
\definecolor{Accent-4-4}{RGB}{255,255,153}
\definecolor{Accent-4-D}{RGB}{255,255,153}
\definecolor{Accent-5-1}{RGB}{127,201,127}
\definecolor{Accent-5-A}{RGB}{127,201,127}
\definecolor{Accent-5-2}{RGB}{190,174,212}
\definecolor{Accent-5-B}{RGB}{190,174,212}
\definecolor{Accent-5-3}{RGB}{253,192,134}
\definecolor{Accent-5-C}{RGB}{253,192,134}
\definecolor{Accent-5-4}{RGB}{255,255,153}
\definecolor{Accent-5-D}{RGB}{255,255,153}
\definecolor{Accent-5-5}{RGB}{56,108,176}
\definecolor{Accent-5-E}{RGB}{56,108,176}
\definecolor{Accent-6-1}{RGB}{127,201,127}
\definecolor{Accent-6-A}{RGB}{127,201,127}
\definecolor{Accent-6-2}{RGB}{190,174,212}
\definecolor{Accent-6-B}{RGB}{190,174,212}
\definecolor{Accent-6-3}{RGB}{253,192,134}
\definecolor{Accent-6-C}{RGB}{253,192,134}
\definecolor{Accent-6-4}{RGB}{255,255,153}
\definecolor{Accent-6-D}{RGB}{255,255,153}
\definecolor{Accent-6-5}{RGB}{56,108,176}
\definecolor{Accent-6-E}{RGB}{56,108,176}
\definecolor{Accent-6-6}{RGB}{240,2,127}
\definecolor{Accent-6-F}{RGB}{240,2,127}
\definecolor{Accent-7-1}{RGB}{127,201,127}
\definecolor{Accent-7-A}{RGB}{127,201,127}
\definecolor{Accent-7-2}{RGB}{190,174,212}
\definecolor{Accent-7-B}{RGB}{190,174,212}
\definecolor{Accent-7-3}{RGB}{253,192,134}
\definecolor{Accent-7-C}{RGB}{253,192,134}
\definecolor{Accent-7-4}{RGB}{255,255,153}
\definecolor{Accent-7-D}{RGB}{255,255,153}
\definecolor{Accent-7-5}{RGB}{56,108,176}
\definecolor{Accent-7-E}{RGB}{56,108,176}
\definecolor{Accent-7-6}{RGB}{240,2,127}
\definecolor{Accent-7-F}{RGB}{240,2,127}
\definecolor{Accent-7-7}{RGB}{191,91,23}
\definecolor{Accent-7-G}{RGB}{191,91,23}
\definecolor{Accent-8-1}{RGB}{127,201,127}
\definecolor{Accent-8-A}{RGB}{127,201,127}
\definecolor{Accent-8-2}{RGB}{190,174,212}
\definecolor{Accent-8-B}{RGB}{190,174,212}
\definecolor{Accent-8-3}{RGB}{253,192,134}
\definecolor{Accent-8-C}{RGB}{253,192,134}
\definecolor{Accent-8-4}{RGB}{255,255,153}
\definecolor{Accent-8-D}{RGB}{255,255,153}
\definecolor{Accent-8-5}{RGB}{56,108,176}
\definecolor{Accent-8-E}{RGB}{56,108,176}
\definecolor{Accent-8-6}{RGB}{240,2,127}
\definecolor{Accent-8-F}{RGB}{240,2,127}
\definecolor{Accent-8-7}{RGB}{191,91,23}
\definecolor{Accent-8-G}{RGB}{191,91,23}
\definecolor{Accent-8-8}{RGB}{102,102,102}
\definecolor{Accent-8-H}{RGB}{102,102,102}

